VecCity: A Taxonomy-guided Library for Map Entity Representation Learning

Electronic maps consist of diverse entities, such as points of interest (POIs), road networks, and land parcels, playing a vital role in applications like ITS and LBS. Map entity representation learning (MapRL) generates versatile and reusable data representations, providing essential tools for efficiently managing and utilizing map entity data. Despite the progress in MapRL, two key challenges constrain further development. First, existing research is fragmented, with models classified by the type of map entity, limiting the reusability of techniques across different tasks. Second, the lack of unified benchmarks makes systematic evaluation and comparison of models difficult. To address these challenges, we propose a novel taxonomy for MapRL that organizes models based on functional module-such as encoders, pre-training tasks, and downstream tasks-rather than by entity type. Building on this taxonomy, we present a taxonomy-driven library, VecCity, which offers easy-to-use interfaces for encoding, pre-training, fine-tuning, and evaluation. The library integrates datasets from nine cities and reproduces 21 mainstream MapRL models, establishing the first standardized benchmarks for the field. VecCity also allows users to modify and extend models through modular components, facilitating seamless experimentation. Our comprehensive experiments cover multiple types of map entities and evaluate 21 VecCity pre-built models across various downstream tasks. Experimental results demonstrate the effectiveness of VecCity in streamlining model development and provide insights into the impact of various components on performance. By promoting modular design and reusability, VecCity offers a unified framework to advance research and innovation in MapRL. The code is available at https://github.com/Bigscity-VecCity/VecCity.

==> 0-TODO.tex <==
% 现在的版本存在几个问题：
% 1. embedding 层按道理来说不应该加requires_grad，但是我记得这一项没关系。

==> 0-response-backup.tex <==
% \newtcolorbox{cmt}[1][]{%
%   colframe = black!60!white,    % 边框颜色
%   colback = black!5!white,      % 背景颜色
%   coltext = black,              % 文本颜色
%   fonttitle = \bfseries,        % 标题字体
%   title={#1},                   % 自定义标题
%   enhanced,                     % 增强模式
% }


\newtcolorbox{cmt}[1][]{%
  colframe = black!60!white,    % Border color
  colback = black!5!white,      % Background color
  coltext = black,              % Text color
  fonttitle = \bfseries,        % Title font
  title={#1},                   % Custom title
  enhanced,                     % Enhanced mode
  breakable,                    % Allows box splitting
}


\newcommand{\commenttitle}[2]{%
  \underline{\textbf{\textcolor{blue}{#1:}}}\\[8pt]
}


\newcommand{\responseletterstyle}{
    % 自定义章节编号为字母
    \renewcommand{\thesection}{\Alph{section}}
    % % 一级标题加粗并不缩进
    % \renewcommand{\cftsecfont}{\bfseries}
    % \renewcommand{\cftsecindent}{0em}
    % % 二级标题缩进
    % \renewcommand{\cftsubsecfont}{}
    % \renewcommand{\cftsubsecindent}{2em}
    % % 一级标题与页码之间的行间距
    % \renewcommand{\cftsecafterpnum}{\vskip0.5em}
    % 自定义目录标题
    \renewcommand{\contentsname}{}
    % 调整目录标题与内容的间距
}
% \renewcommand{\contentsname}{Response Letter Contents}
\titlecontents{section}
  [0em] % 左缩进
  {\addvspace{1.5em}\bfseries\color{blue}} % 格式化条目
  {\textcolor{blue}{\thecontentslabel}\quad} % 标签格式
  {}
  {\hfill\textcolor{blue}{\contentspage}} % 页码位置

\titlecontents{subsection}
  [1em]
  {\addvspace{0.5em}\color{blue}}
  {\textcolor{blue}{\thecontentslabel}\quad}
  {}
  {\hfill\textcolor{blue}{\contentspage}}

\responseletterstyle % 启用 Response Letter 样式


\section*{\centering \huge Cover Letter}
\vspace{10pt}
\pagestyle{plain} % 恢复默认页眉页脚样式
\noindent\textbf{Manuscript Title:} VecCity: A Taxonomy-guided Library for Map Entity Representation Learning.

\noindent\textbf{Manuscript ID:} \#1016

\noindent\textbf{Track Name:} Experiment, Analysis \& Benchmark

\noindent\textbf{Authors:} Wentao Zhang, Jingyuan Wang, Yifan Yang, and Leong Hou U.
\vspace{10pt}

\noindent
Dear Meta Reviewer and Reviewers:
\vspace{0.2cm}

Attached is the revised manuscript entitled “VecCity: A Taxonomy-guided Library for Map Entity Representation Learning” (Paper ID: 1016), which was categorized as "Revision" after review.

We sincerely thank the reviewers for their thorough evaluation and constructive feedback. In this revised version, we have carefully addressed all comments from the reviewers and meta-reviewer, which have greatly improved the quality of our work. A detailed point-by-point response to each comment is provided, with significant changes in the manuscript highlighted in \textcolor{blue}{blue}. Each comment is restated, followed by our response and the corresponding manuscript revisions.

We hope that the revised submission meets the reviewers’ expectations and adheres to the high standards of the VLDB conference. Once again, we sincerely thank you for your thoughtful consideration of our work.


\vspace{0.2cm}
\noindent
Sincerely,

%\vspace{0.2cm}
\noindent
Wentao Zhang, Jingyuan Wang, Yifan Yang, and Leong Hou U.


\newpage
\section{Response to the Meta Reviewer}
 
\commenttitle{Meta Review}

The reviewers found the paper overall well-executed and with a timely topic. There are some specific requests raised towards a revision that are discussed below. Crucially, please ensure the link to the artifacts is working.
\begin{enumerate}[leftmargin=*]
    \item discuss results in terms of time performance of downstream tasks, where scalability may be a concern.
    \item expand on (i) scalability issues and (ii) model size VS inference time tradeoff.
    \item consider adding more models to ensure a broader representation of the field.
    \item align table 1 with the proposed taxonomy.
    \item discuss the distinctions between vector and raster data models and their implications on the benchmarking process, ensuring clarity and relevance to MapRL tasks.
    \item  $[$artifact availability is required$]$ ensure URL to the benchmark works.
    \item  $[$optional$]$ use an established standard data format instead of introducing a new one to enhance compatibility, reduce complexity, and encourage adoption.
\end{enumerate}

\vspace{0.1cm}
\noindent
\commenttitle{Response}

We would like to thank the meta-reviewer for giving us the opportunity to revise the manuscript! For the major comments, we have made the following modifications.

\textbf{\textcolor{red}{For (1) and (2):}} We have expanded our discussion on scalability, particularly addressing performance scalability (Section \ref{sec:431}), efficiency scalability (Section \ref{sec:432}), and the trade-offs between model size and inference time (Section \ref{sec:433}). Specifically, we analyze how model performance scales with increasing fine-tuning dataset size, how efficiency is impacted by the number of entities, and the trade-offs between model complexity and inference efficiency. Additional results and discussions are provided in \updateo{\hyperref[com:32]{Response for Reviewer \#3 Comment 3.2}} and Section \ref{sec:43}. 

\textbf{\textcolor{red}{For (3):}} In \updateo{\hyperref[com:11]{Response to Reviewer \#1 Comment 1.1}}, we have clearly defined the boundaries of our taxonomy and expanded it by adding new relevant models. Additionally, we provide explanations for some related models that were not included. These updates expand the taxonomy’s coverage and enhance its comprehensiveness.

\textbf{\textcolor{red}{For (4):}} We have carefully discussed the necessity of the original Table 1 in \updateo{\hyperref[com:12]{Response to Reviewer \#1 Comment 1.2}} and have made a thoughtful revision. Specifically, we have added a new column to introduce the categorization of methods, ensuring better alignment with the proposed taxonomy. This enhancement improves clarity and helps readers more easily understand the relationships between different approaches.

\textbf{\textcolor{red}{For (5):}} We have added a discussion in \updateo{\hyperref[com:14]{Response to Reviewer \#1 Comment 1.4}} to clarify the distinctions between vector and raster data models and their relevance to MapRL tasks. Specifically, we explain how vector and raster data differ in data features, benchmarking, and model design. We also outline our plans to integrate raster data into VecCity.

\textbf{\textcolor{red}{For (6):}} We have carefully verified the URL and ensured that all artifacts are accessible. Additionally, we have provided an alternative access URL on \updateo{\href{https://drive.google.com/file/d/1JqnGsprG2zpJ4tisf0o3liOLy3GR7t0i/view?usp=drive_link}{Google Drive}} to guarantee the availability of the artifacts.

\textbf{\textcolor{red}{For (7):}} In \updateo{\hyperref[com:13]{Response to Reviewer \#1 Comment 1.3}}, we provide a detailed discussion on the importance of atomic files in our benchmark. We also recognize the role of standard data formats in reducing complexity and enhancing interpretability. Therefore, while retaining atomic files, we offer users an interface that accepts input files in standard formats such as SHP, to simplify the use of the tool. However, to ensure the tool's simplicity, we have imposed certain limitations on the input files. For more details, please refer to \updateo{\hyperref[com:13]{Response to Reviewer \#1 Comment 1.3}}.

In the following sections, we have responded point by point to all comments of the reviewers and revised the manuscript according to the reviewer’s suggestion. The major modifications are summarized as the following:
\begin{itemize} [leftmargin=*]
    \item We have aligned Table 1 with the proposed taxonomy and added more relevant models. 
    \item We have expanded the discussion to analyze scalability issues in MapRL models. 
    \item We introduced the impact of randomness on model performance in the main experiments and provided explanations and analyses for the observed instability. 
    \item We have explored the performance of heterogeneous pretraining task combinations, providing valuable insights for MapRL design based on both performance and time efficiency. For more details, please refer to \updateo{\hyperref[com:21]{Response to Reviewer \#2 Comment 2.1}} and \updateo{Section \ref{sec:pretraintask}}.
\end{itemize}


\newpage
\addtocontents{toc}{\protect\setcounter{tocdepth}{-1}}
\section*{Contents}
\tableofcontents
\addtocontents{toc}{\protect\setcounter{tocdepth}{2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 1
\newpage
\section{Response to Reviewer \#1 (Week Reject)} 
\vspace{1pt}

% 感谢评委所花费的时间，他专业的视角为我们的论文提供了很多有建设意义的评论。我们认真并仔细的对这些意见进行了讨论和思考，并尽我们可能的给出合适的回答，对文章进行修改提升，希望能够解决之前给您造成的疑惑。下面我将分条分点回答您给出的comments。
We sincerely thank you for taking the time to review our manuscript and for providing insightful feedback. Your expertise has been invaluable in helping us improve the quality of our work. We have carefully addressed each of your comments, making corresponding revisions to the manuscript to resolve the concerns you raised. In the following, we provide detailed point-by-point responses to your comments.
\vspace{-1pt}
%%%%%%%%%%%%% Comment 1.1
\subsection{Comment 1.1 and Response 1.1} \label{com:11}
\commenttitle{Comment 1.1 (W1 \& R1)}

{\em (W1).} Limited Model Coverage: Table 1 lists only a subset of MapRL models, leaving out many important ones without clear justification for their exclusion. This undermines the comprehensiveness of the proposed taxonomy.
\vspace{4pt}

\noindent
{\em (R1).} Expand the Model Coverage: Compile a more comprehensive list of existing models to ensure inclusivity and provide a broader representation of the field. 

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your constructive feedback. In this response, we will clarify the scope of our work, introduce the newly added models, explain the reasons for excluding certain related models, and outline the modifications made to the paper. These steps aim to clearly define the boundaries of our study and enhance the clarity of its presentation.

\paratitle{Scope of Our Work.} Our work aims to provide a novel and comprehensive taxonomy and a standardized benchmark for Map Entity Representation Learning (MapRL). Therefore, models included in our review must meet the following criteria.
\begin{enumerate}[leftmargin=*]
    \item The model or algorithm should focus on learning versatile and reusable representations for map entities, such as Points of Interest (POI, represented as points), road segments (represented as polylines), or land parcels (represented as polygons).
    \item The data required for training the model should be commonly available in most geographic scenarios and frequently used in relevant tasks. Examples include intrinsic attributes of map entities, trajectory data, origin-destination (OD) data, and check-in data. This ensures that the models can be widely applied, thereby enhancing the general applicability of our review.
\end{enumerate}
These two criteria serve as the basis for selecting the models included in our review.

\paratitle{Included More Related Models.} To enhance the comprehensiveness of our work, we conducted a thorough review of the related literature, and the details of the newly added models are summarized in \tab\ref{tab:newmodel}.

% Table generated by Excel2LaTeX from sheet 'add'
\begin{table}[htbp]
\centering
\vspace{-2mm}
\caption{Newly Added Models in VecCity.}% TODO add citation
\vspace{-2mm}
\resizebox{0.8\textwidth}{!}{
\setlength{\tabcolsep}{0.5mm}
    \begin{tabular}{c|r|ccc|ccc|cccc|ccc|ccc|ccc|cc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{Encoders} & \multicolumn{10}{c|}{Pretraining Tasks}                                       & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
    \cmidrule{3-23}    \multicolumn{2}{c|}{} & Token & Graph & \multicolumn{1}{c|}{Seq} & TokRI & TRCL  & AToCL & NFI   & \multicolumn{1}{c}{GAu} & \multicolumn{1}{c}{NCL} & AGCL  & \multicolumn{1}{c}{TrajP} & \multicolumn{1}{c}{MTR} & ATrCL & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & \multicolumn{1}{c|}{Temp} & Traj  & Rel \\
    \midrule
    \multirow{4}{*}{POI} & Place2Vec\citeNew{Place2Vec} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} &       &       & GR \\
              & Semantic\citeNew{semantic} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} &       &       & GR \\
          & MT-POI\citeNew{MT-POI} & \checkmark     &       &       &   \checkmark  & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} &  \checkmark     &       & GR \\
    & CatEM\citeNew{CatEM} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     & \checkmark     &       & CIT   &  \\
    \midrule
    \multirow{1}{*}{Segment} & R2Vec\citeNew{R2Vec} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{} & \checkmark     &       &       & GR \\
    \midrule
    Parcel & HGI\citeNew{HGI}   & \checkmark     & \checkmark     &       &       & \checkmark     & \checkmark     &       &       &      &       &       &       &       & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     &       &       & GR \\
    \bottomrule
    \end{tabular}%
}
\label{tab:newmodel}%
\end{table}%
Although these models were not included in the initial draft, they can still be classified using the same taxonomy.

Place2Vec\citeNew{Place2Vec}, Semantic\citeNew{semantic}, MT-POI\citeNew{MT-POI}, and CatEM\citeNew{CatEM} focus on POI category representation learning. Place2Vec applies a random walk algorithm on a geospatial network constructed from POI spatial relationships, and sampling trajectories to capture POI co-occurrence patterns. Semantic and MT-POI extend Place2Vec by incorporating POI category semantic similarities, leveraging Token Relation Contrastive Learning  (TRCL) to enhance representations. For instance, 'supermarkets' and 'shopping malls' belong to the same high-level 'shopping' category and should have similar embeddings. In contrast, CatEM utilizes check-in trajectories to learn POI category representations. While these methods differ from conventional POI-based MapRL, which learns unique representations for POI entities rather than categories, their techniques provide valuable insights.

R2Vec\citeNew{R2Vec} focuses on road intersection representation learning, employing random walks on road networks and using TRCL to model co-occurrence relationships among intersections. Although R2Vec differs from road segment-based MapRL, it offers transferable techniques.

HGI\citeNew{HGI} targets land parcel representation learning by constructing a hierarchical entity network spanning four levels: POI category → POI → land parcel → city. It first pretrains POI category embeddings using Semantic\citeNew{semantic}, then aggregates lower-level representations into higher-level ones via attention and Graph Neural Network (GNN)-based methods. Finally, it applies TRCL, ensuring embeddings of related entities remain similar across different hierarchical levels.

Additionally, we have integrated several open-source models into VecCity, including CAPE \citeNew{CAPE} and CatEM \citeNew{CatEM} for POI, TrajRNE \citeNew{TrajRNE}, JGRM \citeNew{JGRM}, and R2Vec \citeNew{R2Vec} for road segment, and ReDCL \citeNew{RegionDCL}, HAFus \citeNew{HAFusion}, and HGI \citeNew{HGI} for land parcel.

\paratitle{Related but Excluded Models.} Several MapRL models are not included in our taxonomy because they rely on specific types of auxiliary data, such as images and text, which limits their practicality in real-world applications. These dependencies introduce additional complexity and reduce their applicability in cases where such data is expensive to collect, inconsistent across regions, or unavailable in standard map data pipelines. Below, we summarize the main reasons for their exclusion:
\begin{itemize}[leftmargin=*] 
    \item {\em Reliance on Image Data:} Reliance on Image Data: Models such as Garner \citeNew{Garner}, USPM \citeNew{USPM}, Tile2Vec \citeNew{Tile2Vec}, RegionEncoder \citeNew{RegionEncoder}, Urban2Vec \citeNew{urban2Vec}, M3G \citeNew{M3G}, UrbanCLIP \citeNew{UrbanCLIP}, and UrbanVLP \citeNew{UrbanVLP} integrate image data into their pretraining process to improve entity representations. While this can be effective, the reliance on geospatial imagery complicates deployment in regions without high-quality image coverage or where privacy concerns limit access to such data.
    \item {\em Reliance on Text Data:} Models like SpaBERT \citeNew{SpaBERT}, MGeo \citeNew{MGeo}, and ERNIE-GeoL \citeNew{ERNIEGeoL} enhance map representations using text-based information, including user reviews, entity descriptions, and search queries. However, obtaining such data is non-trivial, may require private data access, or is inconsistent across platforms, making these models difficult to generalize in many practical applications.
\end{itemize}
Given these constraints, models that depend heavily on image or text data were excluded from our taxonomy to ensure a more broadly applicable categorization of MapRL methods.

\paratitle{Revsion Made.} Based on the above discussion, we have incorporated the additional models into Table 1 and the relevant sections of the paper. The modifications are as follows:
\begin{table*}[htbp]
  \centering
  \vspace{-0.3cm}
  \caption{\updateo{Revision of Table 1 by adding new MapRL models.}}
  \vspace{-0.3cm}
  \resizebox{\textwidth}{!}{

    \begin{tabular}{c|r|c|ccc|ccc|cccc|ccc|ccc|rcr|cc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}[4]{*}{Method}} & Taxnomy & \multicolumn{3}{c|}{Encoders} & \multicolumn{10}{c|}{Pretraining Tasks}                                       & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
\cline{4-24}    \multicolumn{2}{c|}{} & Type  & Token & Graph & Seq   & TokRI & TRCL  & AToCL & NFI   & GAu   & NCL   & AGCL  & TrajP & MTR   & ATrCL & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & \multicolumn{1}{c|}{Temp} & Traj  & Rel \\
    \midrule
    \multirow{13}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Point of Interest}}} 
    & CWAP~\citeNew{CWAP}  & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & CAPE~\citeNew{CAPE}  & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{r}{} &       & CIT   &  \\
    & MT-POI~\citeNew{MT-POI} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       &       & GR \\

    & \textcolor{blue}{Place2V}~\citeNew{Place2Vec} & \textcolor{blue}{Token-based} & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \multicolumn{1}{l}{\textcolor{blue}{\checkmark}} &  &  & \textcolor{blue}{GR} \\
    & \textcolor{blue}{Semant}~\citeNew{semantic} & \textcolor{blue}{Token-based} & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \multicolumn{1}{l}{\textcolor{blue}{\checkmark}} &  &  & \textcolor{blue}{GR} \\
    & \textcolor{blue}{CatEM}~\citeNew{CatEM} & \textcolor{blue}{Token-based} & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \multicolumn{1}{l}{\textcolor{blue}{\checkmark}} &  & \textcolor{blue}{CIT}   &  \\
    
    & SkipG*~\citeNew{Word2Vec} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} &       & CIT   &  \\
    & Tale*~\citeNew{TALE} & Token-based & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & Teaser*~\citeNew{Teaser} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   & GR \\
    & Hier*~\citeNew{Hier1} & Seq-based & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       &       &       & \checkmark     &       & CIT   & GR \\
    & P2Vec*~\citeNew{POI2VEC} & Token-based & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \checkmark     &       & CIT   & GR \\
    & CACSR*~\citeNew{CACSR} & Seq.-based & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       &       &       & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & CTLE*~\citeNew{CTLE} & Seq.-based & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    \midrule
    \multirow{11}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Road Segment}}} 
    & DyToast~\citeNew{DyToast} & Graph-based & \checkmark     & \checkmark     &       &       & \checkmark     &       & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{l}{\checkmark} &       & CDT   & GR \\
    
    & \textcolor{blue}{R2Vec}~\citeNew{R2Vec} & \textcolor{blue}{Token-based} & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  &  & \textcolor{blue}{\checkmark} &  &  & \textcolor{blue}{GR} \\
    & \textcolor{blue}{TrajRNE}~\citeNew{TrajRNE} & \textcolor{blue}{Graph-based} & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \multicolumn{1}{r}{} &  & \textcolor{blue}{CDT}   & \textcolor{blue}{GR/SR} \\
    & \textcolor{blue}{JGRM}~\citeNew{JGRM} & \textcolor{blue}{Seq.-based} & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  & \textcolor{blue}{\checkmark} &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \textcolor{blue}{\checkmark} & \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}} & \textcolor{blue}{CDT}   & \textcolor{blue}{GR} \\

    
    & RN2Vec*~\citeNew{RN2Vec} & Token-based & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & HRNR*~\citeNew{HRNR} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & SARN*~\citeNew{SARN} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & Toast*~\citeNew{Toast} & Seq.-based & \checkmark     &       & \checkmark     &       & \checkmark     &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & HRoad*~\citeNew{HyperRoad} & Graph-based & \checkmark     & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & START*~\citeNew{START} & Seq.-based & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & JCLRNT*~\citeNew{JCLRNT} & Seq.-based & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    \midrule
    \multirow{15}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Land Parcel}}} 
    & CGAL~\citeNew{CGAL}  & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & DLCL~\citeNew{DLCL}  & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & HUGAT~\citeNew{HUGAT} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    & Re2Vec~\citeNew{Region2Vec} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & ReCP~\citeNew{ReCP}  & Token-based & \checkmark     &       &       &  \checkmark & \checkmark     & \checkmark  &      &       &       &       &       &       &   & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & SR \\

    & \textcolor{blue}{HGI}~\citeNew{HGI}  & \textcolor{blue}{Graph-based} & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  &  & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  & \textcolor{blue}{\checkmark} & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \textcolor{blue}{\checkmark} &  &  & \textcolor{blue}{GR} \\
    & \textcolor{black}{ReDCL}~\citeNew{RegionDCL} & \textcolor{black}{Token-based} & \textcolor{black}{\checkmark} &  &  & \textcolor{black}{\checkmark} & \textcolor{black}{\checkmark} & \textcolor{black}{\checkmark} &  &  &  &  &  &  &  & \textcolor{black}{\checkmark} &  & \textcolor{black}{\checkmark} & \multicolumn{1}{c}{\textcolor{black}{\checkmark}} & \textcolor{black}{\checkmark} &  &  & \textcolor{black}{GR} \\
    & \textcolor{black}{HAFus}~\citeNew{HAFusion} & \textcolor{black}{Graph-based} & \textcolor{black}{\checkmark} & \textcolor{black}{\checkmark} &  &  &  &  &  & \textcolor{black}{\checkmark} &  &  &  &  &  & \textcolor{black}{\checkmark} &  & \textcolor{black}{\checkmark} & \multicolumn{1}{c}{\textcolor{black}{\checkmark}} & \textcolor{black}{\checkmark} &  &  & \textcolor{black}{GR/SR} \\


    
    & ZEMob*~\citeNew{ZEMob} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} &       & SR \\
    & GMEL*~\citeNew{GMEL} & Graph-based & \checkmark     & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    & MGFN*~\citeNew{MGFN} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     &       &       & SR \\
    & HDGE*~\citeNew{HDGE} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    & MVURE*~\citeNew{MVURE} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & SR \\
    & ReMVC*~\citeNew{REMVC} & Token-based & \checkmark     &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & SR \\
    & HREP*~\citeNew{HREP} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    \bottomrule
    \end{tabular}%
        }
  \label{tab:models}%
    \vspace{-0.4cm}
\end{table*}%

 Based on the updated taxonomy, we can make the following assurances:
\begin{enumerate}[leftmargin=*]
    \item Our taxonomy can encompass all models that meet the two criteria outlined in the "Scope of Our Work."
    \item For all models included in our review with open-source implementations, VecCity has incorporated them.
\end{enumerate}
We hope this expanded set of models and clearer scope address the concerns regarding comprehensiveness and demonstrate the extensibility of our taxonomy.
% 需要列出我们补充的所有新的模型，以及新增的实验。


\vspace{0.3cm}

\newpage

\subsection{Comment 1.2 and Response 1.2} \label{com:12}
%%%%%%%%%%%%% Comment 1.2
\commenttitle{Comment 1.2 (W2 \& R3)}

{\em (W2).} Inconsistencies in Taxonomy Claims: The classification in Table 1 appears inconsistent with the stated taxonomy based on points, graphs, and sequences, creating ambiguity in how the models are categorized.
\vspace{4pt}

\noindent
{\em (R3).} Align Table 1 with the proposed taxonomy.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your insightful comment. We apologize for any confusion caused by the presentation of our work. We address your comment by discussing {\em the necessity of Table 1} and the {\em revisions made} to resolve the issue.

\paratitle{The Necessity of Table 1.} In our work, MapRL models are categorized into token-based, graph-based, and sequence-based models according to the proposed method-based taxonomy. This taxonomy provides a unified way to classify models across different map entity types, enabling a deeper understanding of the design insights behind MapRL models.

However, the classification in Table 1, which organizes models based on the type of map entities they target, may have confused. The reason for this entity-based organization is to maintain consistency with the VecCity Library and experiment analysis sections later in the paper. While the design insights underlying MapRL methods are shared across different entity types, there are significant differences in terms of data requirements and evaluation approaches.

\begin{itemize}[leftmargin=*]
    \item {\em Data Differences:} Different types of MapRL models require distinct datasets. For instance, datasets like NY can be used for POI-focused MapRL but lack the critical data needed for road segment-focused models.
    \item {\em Evaluation Differences:} Each category of map entities has its own unique downstream tasks and evaluation processes.
\end{itemize}
Given these differences, organizing Table 1 by map entity type provides a consistent perspective for readers, making it easier to understand our work and reducing the cognitive load required to navigate our results.

\paratitle{The Possibility of Separating Table.} To address this concern, we explored the possibility of fully separating the models into distinct tables according to their taxonomy.  For reference, we have included the split tables (\tab\ref{tab:newtoken}: Token-based Models, \tab\ref{tab:newgraph}: Graph-based Models, \tab\ref{tab:newsequence}: Sequence-based Models) 
as supplementary material in this letter. However, after careful consideration, we found that completely separating the models significantly increased the paper’s length and fragmented the information, making cross-comparisons between models more difficult. Given the structure of the VecCity library and our experimental setup, we decided to adopt a more balanced approach.

% Table generated by Excel2LaTeX from sheet 'Table1_token'
\begin{table}[htbp]
  \centering
  \small
  \caption{Summary of token-based MapRL models.}
  \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{r|c|ccc|ccc|ccc|cp{1.645em}c|cc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{Entity} & \multicolumn{3}{c|}{Encoders} & \multicolumn{3}{c|}{Pretraining Tasks} & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
\cline{3-16}          &       & Token & Graph & Seq   & TokRI & TRCL  & AToCL & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & Temp  & Traj  & Rel \\
    \midrule
    CWAP  & \multirow{10}{*}{POI} & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    CAPE  &       & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       &       & \checkmark     & \multicolumn{1}{c}{} &       & CIT   &  \\
    MT-POI &       & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} &       &       & GR \\
    Place2V* &       & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} &       &       & GR \\
    Semantic* &       & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} &       &       & GR \\
    CatEM* &       & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} &       & CIT   &  \\
    SkipG* &       & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &       & CIT   &  \\
    Tale* &       & \checkmark     &       &       & \checkmark     &       &       & \checkmark     &       &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    Teaser* &       & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{c}{} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   & GR \\
    P2Vec* &       & \checkmark     &       &       & \checkmark     &       &       & \checkmark     &       &       & \multicolumn{1}{c}{} & \checkmark     &       & CIT   & GR \\
    \midrule
    R2Vec* & \multirow{2}{*}{Segment} & \checkmark     &       &       &       & \checkmark     &       &       & \checkmark     &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\checkmark} &       &       & GR \\
    RN2Vec* &       & \checkmark     &       &       & \checkmark     &       &       &       & \checkmark     &       & \checkmark     & \checkmark     &       &       & GR \\
    \midrule
    ReCP  & \multirow{5}{*}{Parcel} & \checkmark     &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     &       &       & SR \\
    ReDCL* &       & \checkmark     &       &       & \checkmark     & \checkmark     & \checkmark     & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     &       &       & GR \\
    ZEMob* &       & \checkmark     &       &       &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} &       & SR \\
    HDGE* &       & \checkmark     &       &       &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c}{} & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    ReMVC* &       & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     &       &       & SR \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:newtoken}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Table1_token'
\begin{table}[htbp]
  \centering
  \small
  \caption{Summary of graph-based MapRL models.}
  % \setlength{\tabcolsep}{0.5mm}
  \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{r|c|ccc|cccc|ccc|rcr|cc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{Entity} & \multicolumn{3}{c|}{Encoders} & \multicolumn{4}{c|}{Pretrain Tasks} & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
\cline{3-17}          &       & Token & Graph & Seq   & NFI   & GAu   & NCL   & AGCL  & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & \multicolumn{1}{c|}{Temp} & Traj  & Rel \\
    \midrule
    DyToast & \multirow{5}{*}{Segment} & \checkmark     & \checkmark     &       & \checkmark     &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{l}{\checkmark} &       & CDT   & GR \\
    TrajRNE* &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{r}{} &       & CDT   & GR/SR \\
    HRNR* &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    SARN* &       & \checkmark     & \checkmark     &       &       &       &       & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    HRoad* &       & \checkmark     & \checkmark     &       & \checkmark     & \checkmark     &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    \midrule
    CGAL  & \multirow{10}{*}{Parcel} & \checkmark     & \checkmark     &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    DLCL  &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    HUGAT &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    Re2Vec &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    HGI*  &       & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    HAFus* &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    GMEL* &       & \checkmark     & \checkmark     &       & \checkmark     & \checkmark     &       &       &       &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    MGFN* &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       &       &       & \checkmark     &       & \checkmark     &       &       & SR \\
    MVURE* &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & SR \\
    HREP* &       & \checkmark     & \checkmark     &       &       & \checkmark     & \checkmark     &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:newgraph}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Table1_token'
\begin{table}[htbp]
  \centering
  \small
  \caption{Summary of sequence-based MapRL models.}
  % \setlength{\tabcolsep}{0.5mm}
  \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{r|c|ccc|ccc|ccc|ccc|cc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[4]{*}{Method}} & \multirow{2}[4]{*}{Entity} & \multicolumn{3}{c|}{Encoders} & \multicolumn{3}{c|}{Pretraining Tasks} & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
\cmidrule{3-16}          &       & Token & Graph & Seq   & TrajP & MTR   & ATrCL & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & \multicolumn{1}{c|}{Temp} & Traj  & Rel \\
    \midrule
    Hier* & \multirow{3}{*}{POI} & \checkmark     &       & \checkmark     & \checkmark     &       &       & \checkmark     &       &       & \multicolumn{1}{c}{} & \checkmark     & \multicolumn{1}{c|}{} & CIT   & GR \\
    CACSR* &       & \checkmark     &       & \checkmark     &       &       & \checkmark     & \checkmark     &       &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \checkmark     & CIT   &  \\
    CTLE* &       & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{c}{} & \checkmark     & \checkmark     & CIT   &  \\
    \midrule
    JGRM* & \multirow{4}{*}{Segment} & \checkmark     & \checkmark     & \checkmark     &       & \checkmark     & \checkmark     &       & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     & CDT   & GR \\
    Toast* &       & \checkmark     &       & \checkmark     &       & \checkmark     & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{} & \multicolumn{1}{r}{} & \checkmark     & CDT   & GR \\
    START* &       & \checkmark     & \checkmark     & \checkmark     &       & \checkmark     & \checkmark     &       & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     & CDT   & GR \\
    JCLRNT* &       & \checkmark     & \checkmark     & \checkmark     &       &       & \checkmark     &       & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     & CDT   & GR \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:newsequence}%
\end{table}%


\paratitle{Revisions made to Table 1.} Finally, We retain the original Table 1 structure but add a new column "Taxonomy Type", explicitly indicating whether a model belongs to the Token-based, Graph-based, or Sequence-based model.

We hope these revisions fully address your concern and clarify the logic behind our model classification. Thank you again for your valuable feedback.
\begin{table*}[ht]
  \centering
  \vspace{-0.3cm}
  \caption{\updateo{Revision of Table 1 by adding "Taxonomy Category"}}
  \vspace{-0.3cm}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|r|c|ccc|ccc|cccc|ccc|ccc|rcr|cc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}[4]{*}{Method}} & \updateo{Taxonomy} & \multicolumn{3}{c|}{Encoders} & \multicolumn{10}{c|}{Pretraining Tasks}                                       & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
\cline{4-24}    \multicolumn{2}{c|}{} & \updateo{Category}  & Token & Graph & Seq   & TokRI & TRCL  & AToCL & NFI   & GAu   & NCL   & AGCL  & TrajP & MTR   & ATrCL & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & \multicolumn{1}{c|}{Temp} & Traj  & Rel \\
    \midrule
    \multirow{13}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Point of Interest}}} 
    & CWAP~\citeNew{CWAP}  & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & CAPE~\citeNew{CAPE}  & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{r}{} &       & CIT   &  \\
    & MT-POI~\citeNew{MT-POI} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       &       & GR \\
    & Place2V~\citeNew{Place2Vec} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       &       & GR \\
    & Semant~\citeNew{semantic} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       &       & GR \\
    & CatEM~\citeNew{CatEM} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       & CIT   &  \\
    & SkipG*~\citeNew{Word2Vec} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} &       & CIT   &  \\
    & Tale*~\citeNew{TALE} & \textcolor{blue}{Token-based} & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & Teaser*~\citeNew{Teaser} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   & GR \\
    & Hier*~\citeNew{Hier1} & \textcolor{blue}{Seq.-based} & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       &       &       & \checkmark     &       & CIT   & GR \\
    & P2Vec*~\citeNew{POI2VEC} & \textcolor{blue}{Token-based} & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \checkmark     &       & CIT   & GR \\
    & CACSR*~\citeNew{CACSR} & \textcolor{blue}{Seq.-based} & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       &       &       & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & CTLE*~\citeNew{CTLE} & \textcolor{blue}{Seq.-based} & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    \midrule
    \multirow{11}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Road Segment}}} 
    & DyToast~\citeNew{DyToast} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       & \checkmark     &       & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{l}{\checkmark} &       & CDT   & GR \\
    & R2Vec~\citeNew{R2Vec} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       &       & GR \\
    & TrajRNE~\citeNew{TrajRNE} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{r}{} &       & CDT   & GR/SR \\
    & JGRM~\citeNew{JGRM} & \textcolor{blue}{Seq.-based} & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & RN2Vec*~\citeNew{RN2Vec} & \textcolor{blue}{Token-based} & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & HRNR*~\citeNew{HRNR} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & SARN*~\citeNew{SARN} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & Toast*~\citeNew{Toast} & \textcolor{blue}{Seq.-based} & \checkmark     &       & \checkmark     &       & \checkmark     &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & HRoad*~\citeNew{HyperRoad} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & START*~\citeNew{START} & \textcolor{blue}{Seq.-based} & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & JCLRNT*~\citeNew{JCLRNT} & \textcolor{blue}{Seq.-based} & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    \midrule
    \multirow{15}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Land Parcel}}} 
    & CGAL~\citeNew{CGAL}  & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & DLCL~\citeNew{DLCL}  & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & HUGAT~\citeNew{HUGAT} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    & Re2Vec~\citeNew{Region2Vec} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & ReCP~\citeNew{ReCP}  & \textcolor{blue}{Token-based} & \checkmark     &       &       &  \checkmark & \checkmark     & \checkmark  &      &       &       &       &       &       &   & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & SR \\
    & HGI~\citeNew{HGI}  & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & ReDCL~\citeNew{RegionDCL} & \textcolor{blue}{Token-based} & \checkmark     &       &       & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & HAFus~\citeNew{HAFusion} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & ZEMob*~\citeNew{ZEMob} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} &       & SR \\
    & GMEL*~\citeNew{GMEL} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    & MGFN*~\citeNew{MGFN} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     &       &       & SR \\
    & HDGE*~\citeNew{HDGE} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    & MVURE*~\citeNew{MVURE} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & SR \\
    & ReMVC*~\citeNew{REMVC} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & SR \\
    & HREP*~\citeNew{HREP} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    \bottomrule
    \end{tabular}%
        }
  \label{tab:models}%
    \vspace{-0.4cm}
\end{table*}%


\newpage


\vspace{0.3cm}

%%%%%%%%%%%%% Comment 1.3
\subsection{Comment 1.3 and Response 1.3} \label{com:13}
\commenttitle{Comment 1.3 (W3 \& R2)}

{\em (W3).} Introduction of a New Data Format: The paper proposes a new atomic data format, which adds yet another standard to the field instead of leveraging an existing one, potentially complicating interoperability and adoption.
\vspace{4pt}

\noindent
{\em (R2)} Adopt Standard Data Formats: Use an established standard data format instead of introducing a new one to enhance compatibility, reduce complexity, and encourage adoption.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your valuable feedback. We understand the importance of standard formats in ensuring interoperability and adoption. Below, we clarify the motivation for introducing the atomic data format, compare it with existing formats, and describe improvements made to enhance usability and compatibility.

\paratitle{Motivation for Proposing a New Atomic Data Format.} MapRL models rely on diverse data types, including map entity attributes, entity relation networks, and auxiliary data (e.g., trajectories and OD flows). However, these data are often collected from different platforms and stored in heterogeneous formats, increasing preprocessing complexity. For example, in the New York (NY) dataset:
\begin{itemize}
    \item {\em POIs:} Foursquare dataset (.txt)
    \item {\em Road Segments:} OpenStreetMap (.shp)
    \item {\em Land Parcels:} NYC.gov (.shp)
    \item {\em Check-in Trajectories:} Foursquare (.txt)
    \item {\em OD Data:} NYC.gov (.parquet or .csv)
\end{itemize}
Instead of requiring users to manually process these diverse inputs, we propose an atomic data format that:
\begin{itemize}
    \item Provides a {\em consistent, structured format} across different data sources.
    \item {\em Automates spatial alignment} by handling Coordinate Reference System (CRS) inconsistencies.
    \item {\em Handles missing data} through filtering and completion.
    \item {\em Optimizes computational efficiency} by reducing file parsing overhead.
\end{itemize}
By unifying datasets into atomic files, VecCity simplifies the data-loading process and significantly reduces user burden.

\paratitle{Comparison with Existing Standard Formats.} We acknowledge the importance of standard data formats in ensuring interoperability. However, existing standard formats pose several challenges that hinder seamless dataset integration:
\begin{itemize}
    \item {\em Inconsistent CRS:} Different datasets may adopt different CRS settings, requiring additional preprocessing steps for alignment. This inconsistency complicates the direct integration of multiple datasets.
    \item {\em Non-unified Data Structures:} Due to the complexity of map data, standard formats often lack a consistent data structure across datasets. This increases the learning curve for users and complicates data utilization.
\end{itemize}
These issues introduce significant challenges for MapRL, necessitating a standardized and unified data processing framework.
% This diversity in data sources and file formats is not unique to the NY dataset—each city dataset comes with its own unique data sources and formats. If we use raw data as input, it would introduce significant complexity into library implementation and take down the reusable of VecCity. To address this issue, we propose a new atomic data format. By converting all raw data into a unified atomic data format, VecCity ensures a consistent data format and streamlined data loading process. This not only reduces the complexity for users but also enhances code modularity, improves processing efficiency, and lowers the barrier for understanding and using the library.

% In addition to the challenges associated with file formats, preprocessing operations serve as another key motivation for adopting the atomic data format. Each map entity has its own geometric, such as point, ployline and polygon, which is contrust by GPS points. However, GPS points are often derived from different Coordinate Reference System (CRS) settings. As a result, identical geographic locations may not align across datasets without proper CRS standardization. This discrepancy introduces an additional cost of complexity, particularly for users unfamiliar with geospatial data processing. Moreover, handling missing data—such as filling in gaps or filtering out incomplete entries—is a crucial preprocessing step. The atomic data addresses these issues upfront by performing CRS alignment, data filtering, and completion operations automatically, ensuring consistency and usability while significantly reducing the time and effort required for data preprocessing.

\paratitle{Modifications to Enhance Compatibility.} 
To address the reviewer's concern, we have made the following improvements to enhance compatibility with standard formats:
\begin{itemize}
    \item Provided Python conversion scripts for transforming Shapefiles, GeoJSON, and CSV data into atomic files.
    \item Users can input datasets in standard formats, provided that:
        \begin{itemize}
            \item {\em Consistent CRS:} All input files must share the same Coordinate Reference System (CRS).
            \item {\em No Missing Values:} Attribute fields should be complete, ensuring data integrity.
            \item {\em Unified Data Schema:} A standardized schema is required to maintain the name of feature alignment and enable cross-file indexing.
        \end{itemize}
\end{itemize}
These improvements ensure that VecCity remains flexible and interoperable, allowing users to integrate it into their existing workflows without being restricted to the atomic format. And you can find all the changes in the GitHub repository.


% Based on the advantages described above, we retained the atomic file format as the primary input format for VecCity. To address your concern, we have made the following modifications to the VecCity Library:
% \begin{enumerate}[leftmargin=*]
%     \item Released Python scripts for converting shapefiles and other raw files into atomic files.
%     \item Provided detailed documentation with step-by-step instructions for the conversion process.
% \end{enumerate}
% To further promote interoperability, we plan to introduce direct support for loading and processing:
% \begin{itemize}
%     \item GeoJSON and Shapefiles as alternative inputs.
%     \item OSM XML for road network processing.
%     \item CSV for structured storage of trajectory data.
% \end{itemize}
% This will allow users to choose between the optimized atomic format and standard formats based on their specific needs.

% You can access the VecCity Library documentation at the following link: [Insert Link Here]. 


% We hope this response fully addresses your concerns. Thank you again for your valuable feedback, which has helped us improve the usability and clarity of the VecCity Library.

\vspace{0.3cm}

\subsection{Comment 1.4 and Response 1.4} \label{com:14}
\commenttitle{Comment 1.4 (R4)}

{\em (R4).} Discuss the distinctions between vector and raster data models and their implications on the benchmarking process, ensuring clarity and relevance to MapRL tasks.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for the insightful feedback. In geographic information systems (GIS), map data is generally represented in two primary formats: vector and raster data. While existing map entity representation learning (MapRL) methods mainly focus on vector-based representations (such as POI embeddings), recent advancements suggest that incorporating raster data (e.g., satellite imagery, and environmental grids) can notably enhance representation learning for map entities. In this section, we highlight the key differences between raster and vector data, their modeling approaches, and their impact on benchmarking, ultimately suggesting ways to integrate both into VecCity.

\paratitle{Difference Between Raster and Vector Data.}
In Geographic Information Systems (GIS), vector and raster data serve distinct roles:
\begin{itemize}[leftmargin=*]
    \item Vector Data: Represent geographical features using {\em points, polylines, and polygons, preserving precise geometry within a specific Coordinate Reference System (CRS)}. They are commonly used to model discrete map entities such as POIs, road segments, and land parcels.
    \item Raster Data: Represent maps as {\em grids of equally sized cells, with each cell holding a value corresponding to spatial properties (e.g., elevation, temperature).} Raster data are widely used for continuous spatial information, such as satellite imagery, and environmental modeling.
\end{itemize}
The fundamental difference between raster and vector data lies in their spatial structure and intended use cases:
\begin{table}[h]
\centering
\caption{Comparison Between Raster and Vector Data}
    \begin{tabular}{l|c|c}
        \toprule
        \textbf{Attribute} & \textbf{Raster Data} & \textbf{Vector Data} \\
        \midrule
        \textbf{Spatial Structure} & Regular grid, fixed-size cells & Polygons with irregular boundaries \\
        \textbf{Data Representation} & Pixel values or numerical fields & Points, lines, and polygons \\
        \textbf{Storage Formats} & GeoTIFF, HDF5 & Shapefile, GeoJSON \\
        \textbf{Common Applications} & Remote sensing, environmental monitoring & Land-use mapping, city planning \\
        \bottomrule
    \end{tabular}
\end{table}

\paratitle{Modeling Approaches for Raster and Vector Data.} The distinction in spatial structure leads to differences in modeling approaches:
\begin{itemize}[leftmargin=*]
    \item Vector Data: Relationships are modeled using \textbf{graph structures}, where entities are interconnected via edges. Graph Neural Networks (GNNs) effectively capture these structured relationships.
    \item Raster Data: Spatial relationships are inferred through \textbf{grid-cell proximity}, similar to image processing. Convolutional Neural Networks (CNNs) are commonly used to extract features from raster data.
\end{itemize}
% \paratitle{Applications.} Vector and raster data models exhibit distinct strengths and are applied to different types of tasks based on their characteristics.
% \begin{itemize}[leftmargin=*]
%     \item Vector Data: Widely applied in tasks such as navigation and recommendation systems, which focus on pathfinding, proximity queries, and user location-based services. These tasks benefit from the fine-grained, object-level information that vector data provide.
%     \item Commonly used in applications like land-use classification, population density estimation, and environmental monitoring, which leverage raster data's dense and continuous spatial coverage.
% \end{itemize}

\paratitle{Impact on Benchmarking.} Differences in data structure and representation influence the design of benchmarking practices:
\begin{itemize}[leftmargin=*]
    \item Datasets: Vector data often use datasets like Foursquare, trajectory datasets, and road network datasets; Raster data typically rely on datasets such as remote sensing imagery, weather datasets, and terrain datasets.
    \item Baseline Models: Raster-based and vector-based MapRL adopt different baseline models due to their distinct data structures. Raster data models commonly utilize CNNs to encode spatial relationships. For example, BFLG~\citeNew{BFLG} encodes raster data using CNN-based networks. Vector data models rely on GNNs for encoding spatial relationships, such as the START model introduced in our paper.
\end{itemize}

\begin{table}[h]
    \centering
    \caption{Comparison of Task Types between Vector and Raster Data}
    \begin{tabular}{l|l|l}
        \toprule
        \textbf{Task Type} & \textbf{Raster-based Examples}  & \textbf{Vector-based Examples} \\
        \midrule
        \textbf{Classification} & Satellite image classification for land cover mapping & Land-use classification using POI distributions  \\
        \textbf{Regression} & Forecasting air pollution and temperature changes & Predicting POI visit counts and ETA estimations  \\
        \textbf{Prediction} & Predicting future population density or weather variations & Predicting user trajectories or next POI visits  \\
        \bottomrule
    \end{tabular}
    \label{tab:vector_raster_tasks}
\end{table}
Even though raster and vector data have differences in datasets and models, their benchmarking tasks share fundamental similarities: All tasks involve entity embeddings, but the primary distinction lies in \emph{how labels are assigned}:
\begin{itemize}[leftmargin=*]
    \item Vector data labels describe discrete objects (e.g., POI type, road connectivity).
    \item Raster data labels describe grid cell values (e.g., pixel classification, environmental variables).
\end{itemize}

\paratitle{Integrating Raster Data in MapRL.}
Although VecCity currently focuses on vector-based models, recent studies have demonstrated the potential of raster data in MapRL:
\begin{itemize}[leftmargin=*]% 需要检查
    \item \textbf{Urban2Vec~\citeNew{urban2Vec}}: Integrates raster-based features to enhance the land pracel representation learning.
    \item \textbf{RoadTagger~\citeNew{roadtagger}}: An end-to-end architecture that combines both satellite imagery and the spatial correlation of road segments to learn road segment representations.
\end{itemize}
To further explore the role of raster data in MapRL, we plan to extend VecCity by: (1) incorporating MapRL methods with raster data or hyper data and (2) expanding the VecCity library to include raster-based MapRL models for multi-modal representation learning.

% \paratitle{Revisions Made.}
% \begin{cmt}
% [TODO] Adding a new subsection in Related Work to introduce the evolution of MapRL methods.
% \end{cmt}




\vspace{0.3cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 2
\newpage
\section{Response to Reviewer \#2 (Accept)} 

%%%%%%%%%%%% Comment 2.1'
\subsection{Comment 2.1 and Response 2.1} \label{com:21}
\commenttitle{Comment 2.1 (W1 \& D1)}

{\em (W1).} The experimental insights could be deeper.
\vspace{4pt}

\noindent
{\em (D1).} The final experimental insights, while certainly good, seem a bit too intuitive to me. It feels natural that diverse pre-training tasks, suitable pre-training tasks, and well-crafted encoders should boost the performance. While it is certainly important to valide seemingly intuitive ideas (as we all know, intuitions can often be misguided), I can't help wonder if deeper insights can be made from the experiments. For instance, concerning the diversity of the pre-training tasks, can we summarize what SPECIFIC combinations of heterogeneous pre-training tasks can yield the best gains on what SPECIFIC types of datasets and in what SPECIFIC downstream tasks? Surely, it is impossible for any one method to emcompass all the possible pre-training tasks, and future researchers can certainly benefict a lot from a general guideline on what pre-training tasks to prioritize when the maximum number of pre-training tasks are limited. And I don't think the answer of this Comment is very far away, as the authors already observed that there are certain pre-training tasks that are more suitable to certain tasks. The answer to this qustion would simply be an extension to the authors' existing observation.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your valuable comments. Your feedback provides meaningful insights and offers important direction for improving our work. However, conducting a comprehensive exploration of the optimal combinations of pretraining tasks across different datasets and downstream tasks through experiments is highly complex and computationally intensive.

Taking the POI MapRL as an example, there are 3 categories of methods for token-based pretraining tasks, 4 for graph-based pretraining tasks, and 3 for sequence-based pretraining tasks (disregarding variations within each category due to different implementations). Moreover, our paper demonstrates the performance of the relevant model across 5 datasets and 3 downstream tasks. Therefore, fully exploring all possible combinations would require $5 \times 3 \times 3 \times 4 \times 3 = 640$ experiments. Additionally, if similar experiments were conducted for each entity, this number would need to be tripled.

We believe that exploring all possible combinations to find an optimal solution represents an impractical and unattainable workload. Therefore, introducing principles or theoretical frameworks to guide the selection of promising combinations and conducting targeted experiments would be a more feasible and effective approach. However, research in this area remains an open problem and represents an important direction for future exploration.

For the above reasons, VecCity presents a simplified version of the experiment in Section 4.4 and \tab~6, \tab~7, and \tab~8. We conducted extension and ablation experiments based on the best-performing models (CTLE for POI, JCLRNT for road segment, and HREP for land parcel), aiming to summarize the insights. However, we recognize that the results of these experiments did not fully convince reviewers. Therefore, we further extended the experiments from Section 4.4 by incorporating more choice spaces and combinations, as well as expanding the experiments from a single dataset to all datasets, to more comprehensively explore the optimal combinations for various datasets and downstream tasks. 

\paratitle{Experimental Space.} In this experiment, we aim to identify the best pretraining task combinations for MapRL. The candidate combination set is constructed by combining different categories of pretraining tasks. For POI entities, we consider token-based pretraining tasks (TokRI, TRCL) and sequence-based pretraining tasks (TrajP, MTR, ATrCL), forming combinations such as TokRI+TrajP and TRCL+MTR. Similarly, for road segment and land parcel entities, candidate sets are formed by combining token-based, graph-based, and sequence-based pretraining tasks (if applicable), as shown in Table~\ref{tab:com_pretraining_tasks}.

\begin{table}[ht]
    \vspace{-2mm}
    \caption{Overview of Pretraining Tasks, Datasets, and Seeds by Entity Types.}
    \centering
    % \renewcommand{\arraystretch}{1.5} % Adjust row height
    \resizebox{0.8\textwidth}{!}{
        \setlength{\tabcolsep}{8pt}       % Adjust column spacing
        \begin{tabular}{c|c|c|c|c|c}
            \toprule
            \textbf{Entity Type} & \textbf{Token-based Task} & \textbf{Graph-based Task} & \textbf{Seq-based Task} & \textbf{Datasets} & \textbf{Seeds} \\ 
            \midrule
            POI & TokRI, TRCL & -- & TrajP, MTR, ATrCL & NY, TYO, CHI, SIN, SF & 1, 13, 31, 42, 131 \\ 
            \hline
            Road Segment & TokRI, TRCL & NFI, GAu, AGCL & TrajP, MTR, ATrCL & BJ, CD, XA, PRT, SF & 1, 13, 31, 42, 131 \\ 
            \hline
            Land Parcel & TokRI, TRCL, AToCL & NFI, GAu, NCL & -- & BJ, CD, XA, PRT, SF & 1, 13, 31, 42, 131 \\ 
            \bottomrule
        \end{tabular}
    } 
    \label{tab:com_pretraining_tasks}
\end{table}

\noindent The experimental space is constructed based on three rules: (1) selecting pretraining tasks implemented and validated by existing models; (2) using available datasets for testing; and (3) repeating all experiments five times with different random seeds.

For rule (1), only pretraining tasks already implemented and validated by existing models are included, avoiding invalid task selections. For example, the complete experimental space for token-based pretraining tasks in POI MapRL includes Token Relation Inference (TokRI), Token Relation Contrastive Learning  (TRCL), and Augmented Token Contrastive Learning (AToCL). However, since existing POI MapRL models do not use AToCL, the actual experimental space includes only TokRI and TRCL for token-based pretraining tasks. To ensure experimental feasibility, we further narrow the experimental scope by selecting only one pretraining task from each category for candidate combinations. The experimental spaces for other entity types follow the same principle.

\paratitle{Model Architecture.} To eliminate the influence of model architecture on the final results, we use the same encoder within each type of MapRL model and include only the necessary encoding components. Specifically:
\begin{itemize}[leftmargin=*]
    \item {\em Token Encoder:} A simple, learnable embedding layer is used to convert entity IDs into token representations. Specifically, the token encoder for POI incorporates spatial features by transforming coordinates (latitude and longitude) into a vector using an MLP, while the land parcel encoder integrates POI feature information in a similar way.
    \item {\em Graph Encoder:} Graph Convolution Network (GCN) is employed to encode auxiliary data associated with the graph-based task. For land parcels, the relation network considers POI similarity, spatial distance, and mobility as edge weights, following the approach in HREP~\citeNew{HREP}.
    \item {\em Sequence Encoder:} A Transformer layer is utilized to encode data corresponding to the sequence pretraining task.
\end{itemize}

The model parameters are configured as follows:
\begin{table*}[ht]
\centering
    \caption{Model parameter configuration.}
    \renewcommand{\arraystretch}{1} % Adjust row height for better readability
    \begin{tabular}{l|c||l|c}
    \hline
    \textbf{Parameter}               & \textbf{Value} & \textbf{Parameter}            & \textbf{Value} \\ \hline
    Learning Rate                    & 1e-3           & Embedding Dimension           & 128            \\ \hline
    Hidden Dimension                 & 256            & Max Check-in Trajectory Length       & 32             \\ \hline
    Max Coordinates Trajectory Length      & 128            & Train-Test Ratio              & 6:4            \\ \hline
    Number of Training Steps         & 50,000         &                               &                \\ \hline
    \end{tabular}
    
    \label{tab:model_parameters_dual_column}
\end{table*}

As discussed in Section~\ref{sec:taxonomy_pretraining}, the model organizes the different types of encoders in the commonly used order: Token → Graph → Sequence.

\paratitle{Static Information of the City Dataset.}
For clarity, we provide a detailed overview of the datasets in \tab\ref{tab:newdataset}. In addition to the original information, we incorporate visit frequency (Freq), average speed (Speed), and average travel time (Time). Visit frequency represents the number of records associated with each map entity, speed is measured in km/h and reflects the average velocity of trajectories, while travel time indicates the total duration of trajectories.

% Table generated by Excel2LaTeX from sheet 'data'
\begin{table}[htbp]
  \centering
  \caption{Pre-prepared datasets for \fullname.}
  \setlength{\tabcolsep}{0.8mm}
  \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{l|rrr|rrr|rrrrr|r}
    \toprule
    \multirow{2}{*}{City} & \multicolumn{1}{c}{\multirow{2}{*}{\#POI}} & \multicolumn{1}{c}{\multirow{2}{*}{\#Segment}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Parcel}} & \multicolumn{3}{c|}{Check-in Traj} & \multicolumn{5}{c|}{Coor. Traj}       & \multicolumn{1}{c}{\multirow{2}{*}{\#OD}} \\
\cline{5-12}          &       &       &       & \multicolumn{1}{c}{\#Traj} & \multicolumn{1}{c}{\#User} & \multicolumn{1}{c|}{Freq} & \multicolumn{1}{c}{\#Traj} & \multicolumn{1}{c}{\#User} & \multicolumn{1}{c}{Speed} & \multicolumn{1}{c}{Time(s)} & \multicolumn{1}{c|}{Freq} &  \\
    \midrule
    NY    & 79,627 & 90,781 & 262   & 823,853 & 2,758 & 30.1  & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c|}{-}     & 28,189 \\
    CHI   & 28,141 & 47,701 & 77    & 279,183 & 921   & 56.5 & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c|}{-}     & 4,631 \\
    TYO   & 61,858 & 407,905 & 64    & 573,703 & 2,227 & 29.3 & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c|}{-}     & \multicolumn{1}{c}{-} \\
    SIN   & 75,329 & 35,084 & 332   & 827,828 & 3,489 & 48.6 & 226,782 & \multicolumn{1}{c}{-}  & 32.9 & 1,198 & 35    & \multicolumn{1}{c}{-} \\
    PRT   & 4,521 & 11,095 & 382   & 19,402 & 126   & 9.2  & 695,085 & 435   & 12.7 & 481   & 2,430 & 324 \\
    SF    & 15,674 & 27,274 & 194   & 171,873 & 361   & 23.1 & 500,516 & 405   & 9.5  & 1,044 & 771   & 24,716 \\
    BJ    & 81,181 & 40,306 & 11,208 & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c|}{-}     & 1,018,312 & 1,677 & 10.2 & 1,115 & 856   & 687,890 \\
    CD    & 17,301 & 6,195  & 1,306  & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c|}{-}     & 559,729 & 48,295 & 20.5 & 397   & 1,551 & 64,482 \\
    XA & 19,108 & 5,269  & 1,056  & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     & \multicolumn{1}{c|}{-}     & 384,618 & 26,787 & 19.1 & 486   & 1,359 & 54,365 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:newdataset}%
\end{table}%

\paratitle{Performance Analysis.} 
The complete experimental results are presented in \tab\ref{tab:poi_comb}, \tab\ref{tab:road_segment_comb}, and \tab\ref{tab:land_parcel_comb}. To facilitate comparison, we also highlight the Top 3 task combinations based on the average ranking across tasks and datasets in \fig\ref{fig:comb}, where each subfigure corresponds to a specific downstream task or dataset. The horizontal axis shows the ranking (lower is better), and the vertical axis lists the top three combinations, with lighter colors indicating lower ranks. In \fig~\ref{fig:comb}(a) for POI entities, the first three subfigures show each model’s average ranking in a specific downstream task (POIC, NPP, or TUL) across multiple datasets. We refer to these as {\em task-oriented rankings}. In contrast, the last five subfigures show each model’s average ranking across all tasks within a specific dataset (NY, TYO, CHI, SIN, or SF), which we refer to as {\em dataset-oriented rankings}. The same ranking logic applies to \fig~\ref{fig:comb}(b) for road segments and \fig~\ref{fig:comb}(c) for land parcels. Based on the results, we have several key findings:

1) {\em Optimal Combinations for POI:}
According to both task-oriented and dataset-oriented rankings, TokRI + MTR consistently achieves the best performance across POI tasks. HHowever, in SF, where data sparsity is a concern due to the smallest number of check-in trajectories, TokRI + TrajP emerges as the better choice.

2) {\em Optimal Combinations for Road Segment:}
For road segments, no single combination dominates across all tasks. Combinations containing TRCL + AGCL emerge as the most effective for ASI and TTE, while TokRI + GAu + MTR stands out in STS. From a dataset-oriented perspective, combinations containing AGCL + MTR perform best on CD and PRT, benefiting from high visit frequencies (CD: 1551, PRT: 2430). In contrast, combinations containing AGCL + TrajP achieve better results on BJ and SF, where lower visit frequencies (BJ: 856, SF: 771) make this combination more effective.

3) {\em Optimal Combinations for Land Parcel:}
For land parcels, the best pretraining task combination also varies by task. Combinations containing NFI consistently excel in Flow Inference (FI) and Mobility Inference (MI), while NCL is widely used among top-performing models in land parcel classification (LPC), highlighting its effectiveness in classification. From a dataset-oriented perspective, combinations containing TokRI perform better on BJ, XA, and PRT, whereas AToCL emerges as the best choice for CD and SF.



% We first examine the performance of pretraining task combinations on each downstream task and observe the following patterns:
% \begin{itemize}[leftmargin=*]
%     \item For POI task, \textbf{Token Relation Inference (TokRI) + Masked Trajectory Recovery (MTR)} combination consistently achieves the best performance across all tasks.
%     \item For segment task, no single combination dominates across all tasks. \textbf{TRCL + AGCL + ATrCL} and \textbf{TRCL + AGCL + TrajP} exhibit slight performance advantages, suggesting that \textbf{TRCL + AGCL} serves as the most effective core combination in Traffic Speed Inference (TSI) and Travel Time Eastimation (TTE) downstream task. However, in the \textbf{Similarity Trajectory Search (STS) task}, the \textbf{TokRI + GAu + MTR} combination outperforms others by a significant margin.
%     \item For the parcel task, the best pretraining combination varies by task. However, two trends stand out: (1) \textbf{NFI} consistently excels in \textbf{FI} and \textbf{MI}, making it well-suited for \textbf{flow estimation}; (2) the top 3 models in \textbf{LPC} all use \textbf{NCL}, highlighting its strength in \textbf{parcel classification}.
% \end{itemize}

% \paratitle{Comparition cross Different Datasets.} Next, we analyze how dataset characteristics influence the effectiveness of pretraining task combinations:
% \begin{itemize}[leftmargin=*]
%     \item For POI task, the \textbf{TokRI + MTR} combination performs best across all datasets, except for \textbf{SF}, where data sparsity makes \textbf{TokRI + TrajP} a more effective alternative.
%     \item For segment task, \textbf{AGCL + TrajP} achieves the best performance on \textbf{BJ, XA, and SF}, while \textbf{NCL + MTR} performs better on \textbf{CD and PRT}. The \textbf{BJ and SF datasets}, characterized by a \textbf{high number of road segments, long trajectory paths, and fewer visits per entity}, favor \textbf{AGCL + TrajP}.In contrast, the \textbf{CD and PRT datasets}, with \textbf{fewer road segments but higher visit frequencies per entity}, favor \textbf{AGCL + MTR}.
%     \item For parcel task, the best pretraining task combination varies across datasets. But, \textbf{TokRI-based combinations} perform better in \textbf{BJ, XA, PRT, and SF}, while \textbf{AToCL} is more effective in \textbf{CD}.
% \end{itemize}


\begin{table*}[t]
  \centering
  \vspace{-0.3cm}
  \caption{Performance comparison of pretraining task combinations for POI across various datasets. The bold/underlined font means the best/the second-best result. "↑" means bigger is better, and "↓" means smaller is better.}
    \vspace{-0.3cm}
      \resizebox{\textwidth}{!}{
      \setlength{\tabcolsep}{0.5mm}
       \setlength{\extrarowheight}{-1pt}
        \begin{tabular}{ccc|cccccc|cccccc|cccccc|cccccc|cccccc|cc}
            \toprule
            \multicolumn{3}{c|}{Dataset} & \multicolumn{6}{c|}{New York}                 & \multicolumn{6}{c|}{Tokyo}                    & \multicolumn{6}{c|}{Chicago}                  & \multicolumn{6}{c|}{Singapore}                & \multicolumn{6}{c|}{San Francisco}             & \multicolumn{2}{c}{Overall} \\
            \midrule
            \multicolumn{1}{c}{\multirow{2}{*}{Token}} & \multirow{2}{*}{Graph} & \multirow{2}{*}{Seq} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c}{NPP} & \multicolumn{2}{c|}{TUL} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c}{NPP} & \multicolumn{2}{c|}{TUL} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c}{NPP} & \multicolumn{2}{c|}{TUL} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c}{NPP} & \multicolumn{2}{c|}{TUL} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c}{NPP} & \multicolumn{2}{c|}{TUL} &\multirow{2}{*}{\makecell{Per Ave\\Rank}} & \multirow{2}{*}{\makecell{Per\\Rank}} \\
                  &       &       & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   &       &  \\
            \midrule
            TokRI & \multicolumn{1}{c}{-}    & TrajP & \textbf{0.072} & \underline{0.005} & \underline{0.172} & \underline{0.363} & \underline{0.695} & \underline{0.419} & \underline{0.326} & \underline{0.011} & \underline{0.187} & \underline{0.394} & \underline{0.501} & \underline{0.281} & 0.233 & 0.068 & \underline{0.181} & \underline{0.375} & \underline{0.734} & \underline{0.543} & 0.126 & 0.003 & \underline{0.113} & \textbf{0.254} & \underline{0.454} & \underline{0.215} & \textbf{0.050} & \textbf{0.012} & 0.147 & \textbf{0.410} & \textbf{0.777} & \underline{0.466} & \underline{2.217} & 2 \\
            TokRI & \multicolumn{1}{c}{-}    & MTR   & \underline{0.072} & 0.003 & \textbf{0.183} & \textbf{0.392} & \textbf{0.700} & \textbf{0.434} & \textbf{0.334} & \textbf{0.012} & \textbf{0.197} & \textbf{0.407} & \textbf{0.527} & \textbf{0.307} & 0.242 & 0.076 & \textbf{0.209} & \textbf{0.412} & \textbf{0.771} & \textbf{0.611} & \textbf{0.140} & \textbf{0.004} & \textbf{0.114} & \underline{0.235} & \textbf{0.455} & \textbf{0.215} & 0.041 & 0.011 & \textbf{0.161} & \underline{0.370} & \underline{0.760} & \textbf{0.525} & \textbf{1.600} & 1 \\
            TokRI & \multicolumn{1}{c}{-}    & ATrCL & 0.062 & 0.004 & 0.023 & 0.050 & 0.087 & 0.008 & 0.326 & 0.009 & 0.059 & 0.129 & 0.040 & 0.006 & 0.218 & 0.068 & 0.031 & 0.086 & 0.170 & 0.013 & 0.126 & 0.003 & 0.011 & 0.036 & 0.016 & 0.000 & 0.036 & 0.007 & \underline{0.153} & 0.314 & 0.641 & 0.397 & 5.050 & 6 \\
            \midrule
            TRCL  & \multicolumn{1}{c}{-}    & TrajP & 0.055 & \textbf{0.006} & 0.130 & 0.275 & 0.531 & 0.259 & 0.315 & 0.008 & 0.045 & 0.126 & 0.050 & 0.010 & \textbf{0.280} & \textbf{0.094} & 0.063 & 0.178 & 0.262 & 0.055 & \underline{0.132} & 0.004 & 0.035 & 0.092 & 0.217 & 0.075 & \underline{0.045} & \underline{0.012} & 0.119 & 0.291 & 0.571 & 0.314 & 3.700 & 4 \\
            TRCL  & \multicolumn{1}{c}{-}    & MTR   & 0.059 & 0.004 & 0.069 & 0.164 & 0.409 & 0.144 & 0.312 & 0.009 & 0.060 & 0.145 & 0.155 & 0.049 & 0.251 & \underline{0.080} & 0.122 & 0.290 & 0.588 & 0.346 & 0.131 & \underline{0.004} & 0.046 & 0.111 & 0.264 & 0.099 & 0.041 & 0.007 & 0.144 & 0.339 & 0.624 & 0.332 & 3.433 & 3 \\
            TRCL  & \multicolumn{1}{c}{-}    & ATrCL & 0.057 & 0.004 & 0.024 & 0.060 & 0.242 & 0.070 & 0.318 & 0.009 & 0.037 & 0.123 & 0.032 & 0.004 & \underline{0.251} & 0.071 & 0.045 & 0.094 & 0.262 & 0.049 & 0.129 & 0.003 & 0.020 & 0.061 & 0.107 & 0.011 & 0.041 & 0.010 & 0.042 & 0.116 & 0.212 & 0.013 & 5.000 & 5 \\
            \bottomrule
        \end{tabular}%
    }
  \label{tab:poi_comb}
\end{table*}

\begin{table*}[t]
  \centering
  \vspace{-0.3cm}
  \caption{Performance comparison of pretraining task combinations for segment across various datasets.}
    \vspace{-0.3cm}
      \resizebox{\textwidth}{!}{
      \setlength{\tabcolsep}{0.5mm}
     \setlength{\extrarowheight}{-1pt}
        \begin{tabular}{ccc|cccccc|cccccc|cccccc|cccccc|cccccc|cc}
        \toprule
        \multicolumn{3}{c|}{Dataset} & \multicolumn{6}{c|}{Beijing}                  & \multicolumn{6}{c|}{Chendu}                   & \multicolumn{6}{c|}{Xi'an}                    & \multicolumn{6}{c|}{Porto}                    & \multicolumn{6}{c|}{San Fransico}             & \multicolumn{2}{c}{Overall} \\
        \midrule
        \multicolumn{1}{c}{\multirow{2}[2]{*}{Token}} & \multirow{2}[2]{*}{Graph} & \multirow{2}[2]{*}{Seq} & \multicolumn{2}{c}{TSI} & \multicolumn{2}{c}{TTE} & \multicolumn{2}{c|}{STS} & \multicolumn{2}{c}{TSI} & \multicolumn{2}{c}{TTE} & \multicolumn{2}{c|}{STS} & \multicolumn{2}{c}{TSI} & \multicolumn{2}{c}{TTE} & \multicolumn{2}{c|}{STS} & \multicolumn{2}{c}{TSI} & \multicolumn{2}{c}{TTE} & \multicolumn{2}{c|}{STS} & \multicolumn{2}{c}{TSI} & \multicolumn{2}{c}{TTE} & \multicolumn{2}{c|}{STS} & \multirow{2}{*}{\makecell{Per Ave\\Rank}} & \multirow{2}{*}{\makecell{Per\\Rank}} \\
              &       &       & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@3↑ & MR↓   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@3↑ & MR↓   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@3↑ & MR↓   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@3↑ & MR↓   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@3↑ & MR↓   &       &  \\
    \midrule
    TokRI & NFI   & TrajP & 2.809 & 30.06 & 609.1 & 2592  & 0.961 & 3.06  & 6.304 & 185.4 & 91.70 & 143.1 & 0.735 & 7.40  & 5.616 & 121.9 & \textbf{117.1} & 186.1 & 0.776 & 4.19  & 4.307 & 61.70 & 86.76 & 133.1 & 0.961 & 1.67  & 2.498 & 28.81 & 806.7 & 7638  & 0.683 & 7.000 & 10.19 & 12 \\
    TokRI & NFI   & MTR   & 2.787 & 29.82 & 636.2 & 2660  & 0.944 & 1.50  & 6.215 & 183.1 & \textbf{88.05} & \textbf{141.1} & 0.643 & 6.68  & 5.576 & 121.5 & 119.6 & 189.3 & 0.714 & 5.17  & 4.307 & 61.67 & 87.97 & 133.9 & 0.913 & 3.00  & 2.491 & 28.77 & 671.7 & 7618  & 0.813 & 5.500 & 9.90  & 11 \\
    TokRI & NFI   & ATrCL & 2.831 & 30.13 & 644.5 & 2597  & 0.531 & 24.33 & 6.152 & 183.0 & 116.14 & 168.7 & 0.315 & 27.58 & 5.546 & 122.1 & 202.7 & 267.4 & 0.349 & 26.73 & 4.287 & 61.42 & 90.44 & 135.1 & 0.846 & 4.55  & \textbf{2.066} & \textbf{23.94} & \textbf{589.4} & \textbf{6372} & 0.703 & 7.367 & 13.03 & 18 \\
    \midrule
    TokRI & GAu   & TrajP & 2.819 & 30.16 & 634.8 & 2646  & 0.269 & 26.27 & 6.049 & 180.8 & 91.50 & 144.6 & 0.231 & 59.72 & 5.463 & 119.9 & 119.5 & 188.0 & \underline{0.879} & \textbf{2.40} & 4.276 & 61.32 & 87.68 & 134.6 & 0.943 & 2.36  & 2.477 & 28.73 & 761.1 & 7592  & 0.743 & 6.200 & 10.52 & 14 \\
    TokRI & GAu   & MTR   & 2.816 & 30.09 & 598.1 & 2587  & 0.356 & 14.98 & 6.041 & 180.7 & 92.78 & 147.0 & 0.654 & 3.75  & 5.405 & 119.6 & 189.8 & 263.4 & 0.657 & 3.99  & 4.288 & 61.39 & 88.19 & 133.4 & \textbf{0.968} & 1.97  & 2.477 & 28.72 & \underline{610.4} & 7617  & 0.867 & 5.400 & 9.45  & 8 \\
    TokRI & GAu   & ATrCL & 2.816 & 30.09 & 608.6 & 2615  & 0.783 & 6.54  & \underline{5.999} & 179.5 & 115.41 & 168.4 & 0.743 & 3.26  & 5.404 & 119.6 & 128.1 & 192.4 & 0.590 & 6.33  & 4.310 & 61.55 & 87.05 & 133.2 & 0.323 & 17.11 & 2.486 & 28.78 & 702.5 & 7607  & 0.720 & 6.600 & 10.61 & 16 \\
    \midrule
    TokRI & AGCL  & TrajP & 2.823 & 30.11 & 577.9 & 2493  & 0.912 & 8.42  & 6.087 & 181.9 & \underline{88.73} & \underline{141.6} & \textbf{0.903} & 2.62  & 5.410 & 119.2 & \underline{118.7} & \underline{186.1} & \textbf{0.909} & 3.41  & 4.266 & 61.18 & 91.95 & 136.2 & 0.961 & 1.66  & 2.474 & \underline{28.66} & 645.3 & 7614  & \textbf{0.887} & \textbf{3.900} & \textbf{6.13} & \textbf{1} \\
    TokRI & AGCL  & MTR   & 2.816 & 30.09 & \textbf{511.4} & 2390  & 0.361 & 15.93 & \textbf{5.964} & \textbf{178.9} & 91.98 & 143.2 & 0.668 & 6.94  & 5.434 & 119.4 & 118.9 & 188.7 & 0.759 & 4.49  & 4.263 & 60.99 & 86.78 & 132.7 & 0.956 & 1.83  & 2.476 & 28.70 & 724.9 & 7656  & 0.777 & 6.367 & 8.06  & 4 \\
    TokRI & AGCL  & ATrCL & 2.817 & 30.13 & 578.2 & 2518  & 0.808 & 5.42  & 6.009 & 179.8 & 93.62 & 146.1 & 0.570 & 6.77  & \textbf{5.374} & \textbf{118.3} & 139.6 & 208.6 & 0.513 & 8.78  & 4.269 & 61.16 & 87.23 & 133.6 & 0.927 & 2.10  & \underline{2.473} & 28.68 & 742.9 & 7648  & 0.690 & 6.067 & 9.71  & 9 \\
    \midrule
    TRCL  & NFI   & TrajP & 2.803 & 29.97 & 692.7 & 2668  & 0.949 & 5.71  & 6.283 & 182.6 & 89.73 & 143.6 & 0.717 & 6.07  & 5.652 & 121.2 & 119.7 & 187.4 & 0.876 & 5.31  & 4.332 & 61.71 & 86.46 & 133.4 & 0.928 & 2.06  & 2.494 & 28.85 & 762.0 & \underline{7592} & 0.777 & 6.900 & 10.39 & 13 \\
    TRCL  & NFI   & MTR   & 2.791 & 29.86 & 776.7 & 2722  & 0.977 & \textbf{1.18} & 6.222 & 181.5 & 88.91 & 141.7 & 0.677 & 6.53  & 5.587 & 120.8 & 120.7 & 188.5 & 0.782 & 3.78  & 4.320 & 61.71 & 104.44 & 156.7 & 0.571 & 13.53 & 2.494 & 28.84 & 699.0 & 7619  & 0.857 & 5.967 & 10.58 & 15 \\
    TRCL  & NFI   & ATrCL & \textbf{2.089} & \textbf{22.38} & 542.6 & \textbf{2025} & 0.793 & 7.28  & 6.207 & 183.0 & 148.14 & 196.5 & 0.719 & 4.21  & 5.639 & 122.2 & 184.0 & 250.5 & 0.294 & 30.13 & 4.302 & 61.51 & 96.14 & 144.5 & 0.833 & 4.26  & 2.494 & 28.83 & 635.9 & 7647  & 0.740 & 8.167 & 12.19 & 17 \\
    \midrule
    TRCL  & GAu   & TrajP & 2.809 & 30.11 & 575.1 & 2591  & 0.957 & 5.27  & 6.092 & 181.6 & 89.75 & 142.0 & 0.730 & 7.33  & 5.379 & 119.1 & 123.2 & 192.2 & 0.795 & \underline{2.53} & 4.294 & 61.38 & 97.00 & 140.1 & 0.953 & 2.97  & 2.477 & 28.71 & 795.7 & 7668  & 0.683 & 7.200 & 9.81  & 10 \\
    TRCL  & GAu   & MTR   & 2.811 & 30.09 & 613.8 & 2553  & \textbf{0.980} & \underline{1.34} & 6.060 & 181.3 & 92.09 & 145.0 & 0.751 & 5.07  & 5.468 & 121.1 & 123.4 & 191.2 & 0.689 & 8.47  & 4.285 & 61.29 & 91.96 & 136.3 & \underline{0.965} & \textbf{1.57} & 2.476 & 28.70 & 816.9 & 7665  & 0.697 & 5.833 & 9.23  & 7 \\
    TRCL  & GAu   & ATrCL & 2.810 & 30.10 & 594.4 & 2572  & 0.702 & 9.87  & 6.001 & \underline{179.5} & 90.93 & 144.8 & 0.872 & \textbf{1.98} & \underline{5.378} & 118.9 & 127.4 & 197.3 & 0.313 & 27.37 & 4.276 & 61.21 & 86.92 & 132.5 & 0.962 & 1.74  & 2.475 & 28.70 & 848.5 & 7662  & 0.807 & 5.933 & 8.32  & 5 \\
    \midrule
    TRCL  & AGCL  & TrajP & \underline{2.310} & \underline{24.84} & \underline{514.0} & \underline{2214} & 0.915 & 6.10  & 6.193 & 181.9 & 90.13 & 142.0 & 0.707 & 5.87  & 5.411 & 120.0 & 119.1 & \textbf{185.7} & 0.839 & 2.87  & 4.284 & 61.32 & 87.85 & 132.3 & 0.959 & \underline{1.62} & 2.478 & 28.70 & 627.4 & 7625  & 0.767 & 6.233 & \underline{7.00} & \underline{2} \\
    TRCL  & AGCL  & MTR   & 2.771 & 29.81 & 616.8 & 2657  & \underline{0.978} & 1.50  & 6.121 & 179.9 & 90.27 & 143.5 & 0.679 & 5.59  & 5.438 & 118.9 & 118.8 & 188.3 & 0.673 & 10.08 & \underline{3.922} & \underline{56.14} & \textbf{80.67} & \underline{122.1} & 0.951 & 1.75  & 2.478 & 28.71 & 706.3 & 7647  & 0.810 & 5.833 & 7.35  & 3 \\
    TRCL  & AGCL  & ATrCL & 2.790 & 29.96 & 595.9 & 2624  & 0.821 & 5.12  & 6.019 & 180.2 & 99.14 & 149.2 & \underline{0.873} & \underline{2.04} & 5.410 & \underline{118.8} & 146.7 & 215.4 & 0.640 & 8.10  & \textbf{3.578} & \textbf{51.15} & \underline{80.84} & \textbf{116.8} & 0.778 & 4.08  & 2.478 & 28.71 & 785.2 & 7669  & \underline{0.880} & \underline{4.933} & 8.42  & 6 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:road_segment_comb}
\end{table*}

\begin{table*}[t]
  \centering
  \vspace{-0.3cm}
  \caption{Performance comparison of pretraining task combinations for land parcel across various datasets.}
    \vspace{-0.3cm}
      \resizebox{\textwidth}{!}{
      \setlength{\tabcolsep}{0.3mm}
    \begin{tabular}{ccc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
    \toprule
    \multicolumn{3}{c|}{Dataset} & \multicolumn{6}{c|}{Beijing}                  & \multicolumn{6}{c|}{Chendu}                   & \multicolumn{6}{c|}{Xi'an}                    & \multicolumn{6}{c|}{Porto}                    & \multicolumn{6}{c|}{San Francisco}            & \multicolumn{2}{c}{Overall} \\
    \midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Token}} & \multirow{2}[2]{*}{Graph} & \multirow{2}[2]{*}{Seq~} & \multicolumn{2}{c|}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c|}{MFI} & \multicolumn{2}{c|}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c|}{MFI} & \multicolumn{2}{c|}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c|}{MFI} & \multicolumn{2}{c|}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c|}{MFI} & \multicolumn{2}{c|}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c|}{MFI} & \multirow{2}{*}{\makecell{Per Ave\\Rank}} & \multirow{2}{*}{\makecell{Per\\Rank}} \\
          &       &       & ACC@1↑ & F1↑   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@1↑ & F1↑   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@1↑ & F1↑   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@1↑ & F1↑   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & ACC@1↑ & F1↑   & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ &       &  \\
    \midrule
    TokRI & NFI   & --   & \underline{0.528} & \underline{0.382} & \textbf{12.33} & \textbf{40.17} & \underline{0.272} & \underline{0.669} & 0.563 & 0.487 & \textbf{147.8} & \textbf{406.4} & 5.9   & \textbf{29} & 0.625 & 0.476 & 177.0 & 964   & 3.4   & 18    & 0.357 & 0.339 & 223.4 & 283.7 & 22.64 & 38.44 & \textbf{0.827} & \textbf{0.504} & 462.0 & 902   & 7.015 & 22.30 & \textbf{3.677} & \textbf{1} \\
    TokRI & GAu   & --   & 0.430 & 0.350 & 18.58 & 63.73 & 0.340 & 0.977 & 0.552 & 0.445 & 164.2 & 690.0 & 24.7  & 175   & 0.638 & 0.531 & 184.6 & 941   & 494.7 & 2067  & 0.339 & 0.332 & \textbf{194.1} & \textbf{257.5} & \textbf{19.91} & \underline{30.15} & \underline{0.826} & 0.479 & \underline{394.3} & \underline{802} & \textbf{6.679} & \underline{22.00} & 4.452 & 4 \\
    TokRI & NCL   & --   & 0.376 & 0.143 & 24.43 & \underline{49.95} & 0.292 & 0.697 & 0.394 & 0.298 & 156.1 & 443.5 & 4.2   & \underline{30} & 0.476 & 0.278 & \textbf{133.9} & \textbf{327} & \underline{2.8} & \underline{18} & 0.257 & 0.234 & 516.8 & 589.8 & 44.82 & 72.23 & 0.819 & 0.450 & 466.0 & 872   & 12.050 & 28.07 & 5.935 & 9 \\
    \midrule
    TRCL  & NFI   & --   & \textbf{0.538} & \textbf{0.386} & 16.70 & 78.81 & 0.394 & 1.266 & 0.531 & 0.417 & 171.9 & 566.9 & 27.4  & 768   & 0.585 & 0.427 & 190.1 & 1311  & 3.9   & 22    & \textbf{0.374} & \textbf{0.365} & 245.2 & 327.5 & 21.98 & 38.44 & 0.816 & 0.454 & 424.4 & 819   & 6.913 & 22.15 & 5.161 & 5 \\
    TRCL  & GAu   & --   & 0.480 & 0.340 & 19.32 & 66.27 & 0.290 & 0.798 & \textbf{0.616} & \textbf{0.552} & 174.3 & 596.8 & 307.3 & 2096  & \underline{0.664} & \textbf{0.601} & 303.7 & 1730  & 525.6 & 3456  & 0.357 & 0.352 & 248.4 & 377.9 & 20.97 & 31.56 & 0.818 & 0.450 & 450.0 & 910   & 6.989 & 22.17 & 5.355 & 6 \\
    TRCL  & NCL   & --   & 0.370 & 0.140 & 28.96 & 53.82 & \textbf{0.257} & 0.727 & 0.423 & 0.272 & \underline{155.0} & 442.5 & \underline{3.6} & 30    & 0.504 & 0.293 & \underline{133.9} & \underline{327} & 2.9   & \textbf{18} & 0.292 & 0.279 & 515.9 & 588.5 & 44.78 & 72.19 & 0.820 & 0.452 & 526.4 & 1233  & 7.141 & 22.59 & 5.871 & 8 \\
    \midrule
    AToCL & NFI   & --   & 0.464 & 0.290 & \underline{13.71} & 67.49 & 0.279 & \textbf{0.665} & \underline{0.614} & \underline{0.548} & 164.7 & 469.7 & 6.2   & 30    & 0.603 & 0.461 & 241.8 & 2169  & 3.9   & 22    & 0.357 & 0.342 & \underline{215.2} & \underline{273.9} & 22.33 & 39.79 & 0.822 & 0.479 & \textbf{382.2} & \textbf{764} & \underline{6.714} & \textbf{21.86} & 4.097 & 3 \\
    AToCL & GAu   & --   & 0.360 & 0.270 & 16.51 & 66.88 & 0.284 & 0.731 & 0.567 & 0.499 & 158.4 & \underline{414.9} & 83.0  & 198   & \textbf{0.674} & \underline{0.565} & 148.6 & 697   & 22.2  & 106   & \underline{0.363} & \underline{0.353} & 217.5 & 305.0 & \underline{20.82} & \textbf{29.92} & 0.823 & \underline{0.504} & 425.3 & 817   & 6.840 & 22.05 & \underline{3.968} & \underline{2} \\
    AToCL & NCL   & --   & 0.366 & 0.260 & 25.18 & 50.45 & \textbf{0.355} & 0.753 & 0.418 & 0.274 & 155.4 & 443.1 & \textbf{3.6} & 30    & 0.512 & 0.306 & 134.3 & 327   & \textbf{2.7} & 18    & 0.298 & 0.295 & 517.3 & 590.4 & 44.79 & 72.19 & 0.825 & 0.502 & 471.5 & 880   & 7.061 & 22.53 & 5.548 & 7 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:land_parcel_comb}
\end{table*}

\begin{figure}
    \centering
    \subfigure[Top 3 combinations for POI map entity.]{\includegraphics[width=0.33\columnwidth]{figures/rebuttal/top5_rank_poi.pdf}}
    \subfigure[Top 3 combinations for segment map entity.]{\includegraphics[width=0.33\columnwidth]{figures/rebuttal/top5_rank_road.pdf}}
    \subfigure[Top 3 combinations for parcel map entity.]{\includegraphics[width=0.33\columnwidth]{figures/rebuttal/top5_rank_region.pdf}}
    \vspace{-4mm}
    \caption{Top 3 pretraining task combinations' preformance.}
    \vspace{-4mm}
    \label{fig:comb}
\end{figure}

\paratitle{Time Efficiency.}
In addition, we evaluate the training time efficiency of each pretraining task, with the results presented in \tab\ref{tab:compttime}. All time measurements are collected under the same computing environment as the performance experiments to ensure consistency. The convergence criterion is defined as the point where the loss approaches its minimum value and remains stable for at least 10 consecutive epochs. This criterion is applied uniformly across all pretraining tasks to ensure a fair comparison.

From the results, we observe that AToCL, NCL, and ATrCL are the most computationally efficient pretraining tasks for token-based, graph-based, and sequence-based pre-training tasks, respectively. AToCL achieves the shortest convergence time among token-based pre-training tasks, making it the most efficient choice. For graph-based pretraining tasks, NCL converges the fastest, requiring fewer steps than NFI, which remains efficient but slightly slower. In contrast, GAu and AGCL demand significantly more time, making them less favorable. Among sequence-based pretraining tasks, ATrCL is the most time-efficient, converging much faster than TrajP and MTR, with MTR being the slowest.

\paratitle{Conclusion.} 
Based on the comprehensive analysis of performance and time efficiency, we provide the following recommendations for MapRL model design:

1) {\em Advice for POI MapRL:} The TokRI + MTR combination consistently delivers the best performance. However, MTR is computationally expensive, making it less suitable for time-constrained scenarios. In such cases, TokRI + TrajP offers a strong alternative, balancing performance and efficiency.

2) {\em Advice for Road Segment MapRL:} AGCL + TrajP performs better on datasets with sparse auxiliary data (small visit frequency), while AGCL + MTR excels in dense auxiliary data (large visit frequency). However, both are inefficient. NFI and ATrCL are more computationally efficient alternatives.

3) {\em Advice for Land Parcel MapRL:} The optimal choice varies by task. NCL is well-suited for classification tasks, as all top-performing LPC models incorporate it, while NFI is preferable for flow estimation, respectively. In terms of time efficiency, AToCL + NCL is the most efficient combination, maintaining strong performance while significantly reducing computational costs, making it a practical choice for large-scale applications.

% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[t]
  \centering
  \small
  \caption{Time Efficiency Comparison for Pretraining Tasks. "Conver." is short for "Convergence" .}
  \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{r|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[6]{*}{\makecell{Pretrining\\Task}} & \multicolumn{3}{c|}{POI} & \multicolumn{3}{c|}{Road Segment} & \multicolumn{3}{c|}{Land Parcel} & \multicolumn{1}{c}{\multirow{2}[6]{*}{\makecell{Relative\\Rank}}} \\
\cline{2-10}          & \multicolumn{1}{c}{\makecell{Step\\Time (ms)}} & \multicolumn{1}{c}{\makecell{Conver.\\Step}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time (min)}} & \multicolumn{1}{c}{\makecell{Step\\Time (ms)}} & \multicolumn{1}{c}{\makecell{Conver.\\Step}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time (min)}}& \multicolumn{1}{c}{\makecell{Step\\Time (ms)}} & \multicolumn{1}{c}{\makecell{Conver.\\Step}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time (min)}}&  \\
    \midrule
    TokRI & 6.62 & 7367  & 1.0   & 197   & 31037 & 102   & 38    & 23840 & 15    & 2 \\
    TRCL  & 6.69 & 19100 & 2.2   & 307   & 28086 & 144   & 54    & 22387 & 20    & 3 \\
    AToCL & -     & -     & -     & -     & -     & -     & 4     & 23134 & 2     & 1 \\
    \midrule
    NFI   & -     & -     & -     & 223   & 29526 & 110   & 45    & 21192 & 16    & 2 \\
    NCL   & -     & -     & -     & -     & -     & -     & 45    & 20138 & 15    & 1 \\
    GAu   & -     & -     & -     & 264   & 32033 & 133   & 54    & 23943 & 22    & 3 \\
    AGCL  & -     & -     & -     & 289   & 28367 & 137   & -     & -     & -     & 4 \\
    \midrule
    TrajP & 18.81 & 15600 & 5.4   & 554   & 34152 & 315   & -     & -     & -     & 2 \\
    MTR   & 22.66 & 17050 & 7.2   & 1436  & 27483 & 658   & -     & -     & -     & 3 \\
    ATrCL & 25.14 & 6750  & 2.7   & 524   & 25800 & 225   & -     & -     & -     & 1 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:compttime}%
\end{table}%

\paratitle{Revisions Made.} Based on the results presented in \tab~\ref{tab:poi_comb}-\ref{tab:land_parcel_comb} and Figure.\ref{fig:comb}, we revised Section.\ref{sec:pretraintask} by replacing the original experiments on modified models with experiments focusing on the optimal combination of pretraining tasks.
\begin{cmt}
In our experimental analysis in Section \ref{sec:experiment}, we conclude that utilizing multiple pretraining tasks can enhance the performance of MapRL models. Moreover, greater task heterogeneity—incorporating token-based, graph-based, and sequence-based pretraining tasks—can further improve model capability. To fully inveterate the influence of task heterogeneity on performance, we conduct deep dive experiments to figure out what specific combinations of heterogeneous pretraining tasks can yield the best gains on MapRL.

\paratitle{Experimental Space.} In this section, we aim to identify the best pretraining task combinations for MapRL. The candidate combination set is constructed by combining different categories of pretraining tasks. For POI entities, we consider token-based pretraining tasks (TokRI, TRCL) and sequence-based pretraining tasks (TrajP, MTR, ATrCL), forming combinations such as TokRI+TrajP and TRCL+MTR. Similarly, for road segments and land parcels, candidate sets are formed by combining token-, graph-, and sequence-based pretraining tasks (if applicable), as shown in Table~\ref{tab:pretraining_tasks}.

% \begin{table}[t]
%     \vspace{-2mm}
%     \caption{Available Pretraining Tasks by Entity Types.}
%     \centering
%     % \renewcommand{\arraystretch}{1.5} % Adjust row height
%     \resizebox{\linewidth}{!}{
%         \setlength{\tabcolsep}{8pt}       % Adjust column spacing
%         \begin{tabular}{r|ccc}
%         \toprule
%         Task Type & POI   & Road Segment & Land Parcel \\
%         \midrule
%         Token-based & TokRI, TRCL & TokRI, TRCL & TokRI, TRCL, AToCL \\
%         Graph-based & --     & NFI, GAu,AGCL   & NFI, GAu,NCL \\
%         Seq-based & TrajP, MTR, ATrCL & TrajP, MTR, ATrCL & -- \\
%         \bottomrule
%         \end{tabular}%
%     } 
%     \label{tab:pretraining_tasks}
% \end{table}

\noindent The experimental space is constructed based on three rules: (1) selecting pretraining tasks implemented and validated by existing models; (2) using available datasets for testing; and (3) repeating all experiments five times with different random seeds.

For rule (1), only pretraining tasks already implemented and validated by existing models are included, avoiding invalid task selections. For example, the complete experimental space for token-based pretraining tasks in POI MapRL includes Token Relation Inference (TokRI), Token Relation Contrastive Learning (TRCL), and Augmented Token Contrastive Learning (AToCL). However, since existing POI MapRL models do not use AToCL, the actual experimental space includes only TokRI and TRCL for token-based pretraining tasks. To ensure experimental feasibility, we further narrow the experimental scope by selecting only one pretraining task from each category for candidate combinations. The experimental spaces for other entity types follow the same principle.

\paratitle{Model Architecture.} To eliminate the influence of model architecture on the final results, we use the same encoder within each type of MapRL model and include only the necessary encoding components. Specifically:
\begin{itemize}[leftmargin=*]
    \item {\em Token Encoder:} A simple, learnable embedding layer is used to convert entity IDs into token representations. Specifically, the token encoder for POI incorporates spatial features by transforming coordinates (latitude and longitude) into a vector using an MLP, while the land parcel encoder integrates POI feature information in a similar way.
    \item {\em Graph Encoder:} Graph Convolution Network (GCN) is employed to encode auxiliary data associated with the graph-based task. For land parcels, the relation network considers POI similarity, spatial distance, and mobility as edge weights, following the approach in HREP~\citeNew{HREP}.
    \item {\em Sequence Encoder:} A Transformer layer is utilized to encode data corresponding to the sequence pretraining task.
\end{itemize}
The model is configured with a learning rate of 1e-3, embedding dimension of 128, hidden dimension of 256, and maximum sequence lengths of 32 for POI inputs and 128 for segments. Training follows a 6:2:2 train-validation-test split, with a maximum of 50,000 training steps and early stopping enabled. Encoders are arranged in the order: Token → Graph → Sequence.

\paratitle{Experimental Result.} 
Due to space constraints, we focus on the top three pretraining task combinations for each map entity type (POI, road segments, and land parcels), determined by their average rankings across tasks and datasets. The results are presented in \fig~\ref{fig:pretraintask} where each subfigure corresponds to a specific downstream task or dataset. The horizontal axis shows the ranking (higher is better), and the vertical axis lists the top three combinations, with lighter colors indicating lower ranks. In \fig~\ref{fig:pretraintask}(a) for POI entities, the first three subfigures show each model’s average ranking in a specific downstream task (POIC, NPP, or TUL) across multiple datasets. We refer to these as {\em task-oriented rankings}. In contrast, the last five subfigures show each model’s average ranking across all tasks within a specific dataset (NY, TYO, CHI, SIN, or SF), which we refer to as {\em dataset-oriented rankings}. The same ranking logic applies to \fig~\ref{fig:pretraintask}(b) for road segments and \fig~\ref{fig:pretraintask}(c) for land parcels. Based on the results, we have several key findings:

1) {\em Optimal Combinations for POI:}
According to both task-oriented and dataset-oriented rankings, TokRI + MTR consistently achieves the best performance across POI tasks. However, in SF, where data sparsity is a concern, TokRI + TrajP proves to be a better choice.

2) {\em Optimal Combinations for Road Segment:}
For road segments, no single combination dominates across all tasks. Combinations containing TRCL + AGCL emerge as the most effective for ASI and TTE, while TokRI + GAu + MTR stands out in STS. From a dataset-oriented perspective, combinations containing AGCL + MTR perform best on CD and PRT, benefiting from high visit frequencies (CD: 1551, PRT: 2430). In contrast, combinations containing AGCL + TrajP achieve better results on BJ and SF, where lower visit frequencies (BJ: 856, SF: 771) make this combination more effective.

3) {\em Optimal Combinations for Land Parcel:}
For land parcels, the best pretraining task combination varies by task. Combinations containing NFI consistently excel in Flow Inference (FI) and Mobility Inference (MI), while NCL is widely used among top-performing models in Land Parcel Classification (LPC), highlighting its effectiveness in parcel classification. From a dataset perspective, combinations containing TokRI perform better on BJ, XA, and PRT, whereas AToCL emerges as the best choice for CD and SF.



% % Table generated by Excel2LaTeX from sheet 'Sheet4'
% \begin{table}[t]
%   \centering
%   \small
%   \caption{\updatetw{Time Efficiency Comparison for Pretraining Tasks. "Conver." stands for "Convergence." The unit for "Step Time" is milliseconds, while "Conver. Time" is measured in minutes.}}
%   \resizebox{\linewidth}{!}{
%     \begin{tabular}{r|cc|cc|cc|c}
%     \toprule
%     \multirow{2}[4]{*}{Method} & \multicolumn{2}{c|}{POI} & \multicolumn{2}{c|}{Road Segment} & \multicolumn{2}{c|}{Land Parcel} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\makecell{Relativ\\Rank}}} \\
% \cmidrule{2-7}          &\multicolumn{1}{c}{\makecell{Step\\Time}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time}} & \multicolumn{1}{c}{\makecell{Step\\Time}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time}} & \multicolumn{1}{c}{\makecell{Step\\Time}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time}} &  \\
%     \midrule
%     TokRI & 6.6 & 1.0   & 197   & 102   & 38    & 15    & 2 \\
%     TRCL  & 6.7 & 2.2   & 307   & 144   & 54    & 20    & 3 \\
%     AToCL & --     & --     & --     & --     & 4     & 2     & 1 \\
%     \midrule
%     NFI   & --     & --     & 223   & 110   & 45    & 16    & 2 \\
%     NCL   & --     & --     & --     & --     & 45    & 15    & 1 \\
%     GAu   & --     & --     & 264   & 133   & 54    & 22    & 3 \\
%     AGCL  & --     & --     & 289   & 137   & --     & --     & 4 \\
%     \midrule
%     TrajP & 18.8 & 5.4   & 554   & 315   & --     & --     & 2 \\
%     MTR   & 22.6 & 7.2   & 1436  & 658   & --     & --     & 3 \\
%     ATrCL & 25.1 & 2.7   & 524   & 225   & --     & --     & 1 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:pttime}%
% \end{table}%
\paratitle{Time Efficiency.}
In addition, we evaluate the training time efficiency of each pretraining task, with the results presented in \tab\ref{tab:pttime}. All time measurements are collected under the same computing environment as the performance experiments to ensure consistency. The convergence criterion is defined as the point where the loss approaches its minimum value and remains stable for at least 10 consecutive epochs. This criterion is applied uniformly across all pretraining tasks to ensure a fair comparison.

From the results, we observe that AToCL, NCL, and ATrCL are the most computationally efficient pretraining tasks for token-based, graph-based, and sequence-based pre-training tasks, respectively. AToCL achieves the shortest convergence time among token-based pre-training tasks, making it the most efficient choice. For graph-based pretraining tasks, NCL converges the fastest, requiring fewer steps than NFI, which remains efficient but slightly slower. In contrast, GAu and AGCL demand significantly more time, making them less favorable. Among sequence-based pretraining tasks, ATrCL is the most time-efficient, converging much faster than TrajP and MTR, with MTR being the slowest.

\paratitle{Conclusion.} 
Based on the comprehensive analysis of performance and time efficiency, we provide the following recommendations for MapRL model design:

1) {\em Advice for POI MapRL:} The TokRI + MTR combination consistently delivers the best performance. However, MTR is computationally expensive, making it less suitable for time-constrained scenarios. In such cases, TokRI + TrajP offers a strong alternative, balancing performance and efficiency.

2) {\em Advice for Road Segment MapRL:} AGCL + TrajP performs better on datasets with sparse auxiliary data (small visit frequency), while AGCL + MTR excels in dense auxiliary data (large visit frequency). However, both are inefficient. NFI and ATrCL are more computationally efficient alternatives.

3) {\em Advice for Land Parcel MapRL:} The optimal choice varies by task. NCL is well-suited for classification tasks, as all top-performing LPC models incorporate it, while NFI is preferable for flow estimation, respectively. In terms of time efficiency, AToCL + NCL is the most efficient combination, maintaining strong performance while significantly reducing computational costs, making it a practical choice for large-scale applications.
    
\end{cmt}


\vspace{0.3cm}


%%%%%%%%%%%%% Comment 2.2
\subsection{Comment 2.2 and Response 2.2} \label{com:22}

\commenttitle{Comment 1.2 (W2 \& R3)}

{\em (W2).} Could address the randomness in the experiments.
\vspace{4pt}

\noindent
{\em (D2).} In the experiments, it would appear that the randomness in dataset separation and model initializations is not explicitly addressed. It would be interesting to see the effect of this. In particular, which types of methods are more robust or sensitive against such randomness? This would be an interesting Comment to answer.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

We sincerely appreciate your valuable comments on the potential impact of randomness in our experiments. To systematically evaluate this, we conducted experiments using multiple random seeds {1, 13, 31, 42, 131}. These seeds were carefully selected to ensure diverse initialization conditions and dataset splits, allowing us to assess the stability and robustness of different MapRL models.

In this section, we specifically analyze the effects of randomness by examining performance variations across different runs. Our goal is to identify which models and tasks are most sensitive to dataset partitioning and initialization variability, providing insights into their stability.

%\rotatebox{90}{
%\underline  \underline
% ±

\begin{table*}[htbp]
  \centering
  \vspace{-0.3cm}
  \caption{Revison for Table 3 by addressing the randomness.}
\vspace{-0.3cm}
    % \setlength{\tabcolsep}{0.5mm}
    \renewcommand{\arraystretch}{0.8}
    \small
    \setlength{\extrarowheight}{-1pt}
  \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{ccc|ccccccc}
        \toprule
        \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{Task} & Metric & SkipG & Teaser & Tale  & Hier  & P2Vec & CACSR & CTLE \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{New York}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & \underline{0.073±0.001} & 0.071±0.005 & 0.063±0.006 & 0.073±0.014 & \textbf{0.082±0.007} & 0.055±0.016 & 0.055±0.005 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.006±0.004 & \underline{0.006±0.005} & 0.016±0.006 & 0.006±0.002 & \textbf{0.022±0.006} & 0.013±0.001 & 0.014±0.002 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.099±0.017 & \underline{0.097±0.021} & 0.143±0.008 & 0.115±0.003 & 0.126±0.006 & 0.141±0.049 & \textbf{0.152±0.009} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.252±0.035 & 0.254±0.046 & 0.326±0.004 & 0.293±0.005 & 0.161±0.004 & \underline{0.327±0.038} & \textbf{0.329±0.010} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.569±0.034 & \underline{0.572±0.024} & 0.674±0.003 & 0.576±0.034 & 0.635±0.007 & 0.638±0.026 & \textbf{0.694±0.004} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.260±0.033 & \underline{0.266±0.029} & 0.438±0.007 & 0.282±0.039 & 0.328±0.004 & 0.391±0.068 & \textbf{0.453±0.007} \\ 
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Tokyo}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & \underline{0.347±0.008} & 0.382±0.016 & \textbf{0.220±0.004} & 0.338±0.035 & 0.318±0.003 & 0.303±0.041 & 0.302±0.039 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.020±0.013 & \textbf{0.024±0.014} & 0.047±0.006 & 0.008±0.012 & \underline{0.042±0.003} & 0.018±0.001 & 0.017±0.003 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.161±0.004 & 0.156±0.011 & 0.156±0.007 & \textbf{0.164±0.001} & \underline{0.162±0.005} & 0.156±0.060 & 0.162±0.004 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.324±0.006 & 0.303±0.036 & 0.303±0.004 & \textbf{0.335±0.002} & \underline{0.329±0.007} & 0.326±0.015 & 0.327±0.007 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.430±0.013 & 0.436±0.017 & 0.401±0.006 & 0.440±0.031 & 0.454±0.003 & \underline{0.459±0.098} & \textbf{0.504±0.002} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.227±0.009 & 0.232±0.014 & 0.228±0.008 & 0.235±0.010 & 0.249±0.004 & \underline{0.277±0.099} & \textbf{0.289±0.004} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Chicago}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & 0.075±0.004 & 0.071±0.011 & 0.102±0.004 & 0.082±0.004 & \textbf{0.117±0.005} & \underline{0.104±0.012} & 0.102±0.017 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.006±0.001 & 0.004±0.001 & 0.017±0.005 & 0.006±0.003 & \textbf{0.024±0.008} & 0.017±0.006 & \underline{0.018±0.006} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.083±0.021 & 0.055±0.030 & 0.102±0.005 & 0.095±0.034 & 0.150±0.005 & \underline{0.154±0.053} & \textbf{0.177±0.010} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.237±0.046 & 0.179±0.078 & 0.238±0.005 & 0.263±0.060 & 0.364±0.007 & \textbf{0.399±0.036} & \underline{0.378±0.014} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.457±0.084 & 0.434±0.071 & 0.620±0.007 & 0.552±0.020 & 0.656±0.005 & \underline{0.668±0.069} & \textbf{0.764±0.011} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.198±0.068 & 0.186±0.010 & 0.366±0.005 & 0.300±0.008 & 0.423±0.007 & \underline{0.439±0.058} & \textbf{0.603±0.028} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Singapore}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & 0.094±0.039 & 0.061±0.003 & 0.037±0.006 & \underline{0.116±0.043} & 0.072±0.004 & 0.105±0.043 & \textbf{0.126±0.025} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.004±0.000 & \underline{0.009±0.005} & 0.014±0.006 & 0.002±0.002 & \textbf{0.026±0.009} & 0.007±0.002 & 0.003±0.003 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.025±0.004 & 0.028±0.003 & 0.049±0.007 & 0.050±0.017 & 0.081±0.006 & \textbf{0.108±0.044} & \underline{0.104±0.025} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.062±0.007 & 0.069±0.005 & 0.104±0.002 & 0.114±0.028 & \underline{0.177±0.006} & \textbf{0.184±0.051} & 0.136±0.051 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.257±0.057 & 0.269±0.056 & 0.309±0.006 & 0.274±0.080 & 0.396±0.008 & \underline{0.397±0.052} & \textbf{0.442±0.026} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.111±0.037 & 0.139±0.009 & 0.169±0.005 & 0.157±0.009 & 0.178±0.006 & \underline{0.181±0.066} & \textbf{0.246±0.003} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Sanfransico}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & 0.055±0.026 & 0.061±0.014 & \underline{0.012±0.003} & \textbf{0.065±0.016} & 0.038±0.005 & 0.057±0.023 & 0.059±0.014 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.002±0.000 & 0.004±0.004 & 0.010±0.007 & 0.003±0.002 & \textbf{0.023±0.008} & \underline{0.012±0.005} & 0.003±0.002 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.019±0.007 & 0.019±0.003 & 0.012±0.003 & \underline{0.036±0.015} & 0.026±0.006 & 0.027±0.029 & \textbf{0.060±0.004} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.057±0.011 & 0.056±0.010 & 0.056±0.007 & \underline{0.099±0.007} & 0.058±0.008 & 0.064±0.055 & \textbf{0.123±0.009} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.252±0.079 & 0.302±0.153 & 0.335±0.005 & 0.354±0.117 & 0.521±0.005 & \underline{0.533±0.061} & \textbf{0.612±0.011} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.130±0.013 & 0.099±0.055 & 0.155±0.003 & 0.150±0.054 & 0.263±0.006 & \underline{0.291±0.018} & \textbf{0.324±0.006} \\
        \midrule
        \multicolumn{3}{c|}{Per. Avg. Rank} & 5.8   & 4.5   & 5.7   & 4.2   & 3.0   & \underline{2.9} & \textbf{2.4} \\
        \bottomrule
    \end{tabular}%
    }
  \label{tab:compoi}%
\end{table*}%

\paratitle{Randomness Sensitivity in POI MapRL Models.}
POI representation learning is particularly affected by randomness due to variations in data partitioning and the selection of positive and negative samples in the pretraining task. As shown in \tab\ref{tab:compoi}, we summarize key observations below:

\begin{itemize}[leftmargin=*]
    \item SkipG, Teaser, and CACSR demonstrate significant instability across different runs. These models depend on contrastive learning techniques, making their performance highly susceptible to variations in dataset partitioning and the selection of negative samples. 
    
    \item P2Vec and Tale demonstrate greater stability across various random seeds, likely due to their utilization of Token Relation Inference, a supervised pretraining task that enhances robustness. This approach involves predicting relationships between map entities based on their representation vectors, providing a structured learning framework that contributes to consistent performance.  

    \item The TUL task exhibits heightened sensitivity to randomness, particularly within the Chicago (CHI) and San Francisco (SF) datasets. This increased sensitivity is primarily attributed to the limited number of user records in these cities (CHI: 921, SF: 361), leading to imbalanced training distributions. Consequently, a small subset of POIs disproportionately influences the learning process, resulting in significant variance across different random splits.

\end{itemize}




% Table generated by Excel2LaTeX from sheet 'Road3'
\begin{table*}[t]
    \centering
    \caption{Revision of Table 4 by addressing randomness.}
    % \setlength{\tabcolsep}{0.5mm}
    \renewcommand{\arraystretch}{0.8}
    \small
    \setlength{\extrarowheight}{-1pt}
    \resizebox{0.8\textwidth}{!}{ % 让表格自动缩放
    \begin{tabular}{ccc|ccccccc}
        \toprule
        \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{Task} & Metric & RN2Vec & HRNR  & SARN  & Toast & HRoad & START & JCLRNT \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Beijing}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 3.582±0.005 & 3.162±0.004 & 2.805±0.004 & 2.737±0.012 & \textbf{2.711±0.009} & 2.717±0.008 & \underline{2.803±0.019} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 5.734±0.001 & 5.589±0.001 & 5.481±0.001 & 5.512±0.009 & 5.407±0.003 & \textbf{5.390±0.004} & \underline{5.480±0.010} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 661.3±33.98 & 631.0±29.387 & 596.5±20.78 & \underline{533.0±52.97} & 584.8±16.34 & \textbf{512.3±19.87} & 514.3±38.30 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 2978±98.23 & 2968±101.9 & 2581±14.11 & 2576±79.44 & 2554±35.22 & \underline{2502±37.89} & \textbf{2464±36.07} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.764±0.032 & 0.816±0.030 & 0.843±0.029 & 0.787±0.099 & 0.867±0.007 & \textbf{0.901±0.025} & \underline{0.900±0.045} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 12.38±1.543 & \underline{11.48±1.937} & 13.297±1.168 & 12.76±4.812 & 14.00±3.421 & 11.87±3.982 & \textbf{11.45±4.148} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Chendu}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 6.565±0.064 & 6.424±0.044 & 5.988±0.021 & 6.357±0.026 & \textbf{5.931±0.023} & 6.046±0.011 & \underline{6.354±0.079} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 14.01±0.074 & 13.74±0.072 & 13.33±0.043 & 13.34±0.163 & \textbf{13.22±0.002} & \underline{13.46±0.007} & 13.46±0.132 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 106.1±0.057 & \underline{100.3±0.040} & \textbf{88.27±4.267} & 94.95±2.435 & 88.51±5.478 & 95.78±3.119 & 97.01±4.077 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 154.9±0.065 & 149.9±0.054 & 156.7±6.695 & 150.1±2.747 & \textbf{136.8±5.665} & \underline{151.0±3.841} & 147.7±3.790 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.687±0.037 & \underline{0.728±0.062} & 0.683±0.127 & 0.688±0.024 & 0.675±0.054 & \textbf{0.761±0.034} & 0.723±0.001 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 48.11±1.667 & 42.95±3.373 & 36.62±2.138 & 22.41±3.660 & 24.37±5.014 & \underline{19.22±2.722} & \textbf{18.73±2.534} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Xi'an}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 6.327±0.029 & \underline{5.794±0.121} & \textbf{5.359±0.026} & 5.633±0.014 & 5.411±0.073 & 5.384±0.068 & 5.670±0.023 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 13.08±0.368 & \underline{11.21±0.104} & \textbf{10.58±0.011} & 10.84±0.117 & 10.73±0.048 & 10.82±0.071 & 10.93±0.063 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 137±6.669 & 134.3±5.089 & \underline{109.7±4.258} & 122.2±4.519 & 110.3±3.678 & 115.3±15.44 & \textbf{107.7±6.816} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & \underline{198.7±8.232} & 203.0±11.88 & \textbf{169.0±5.630} & 190.9±3.617 & 171.9±8.943 & 169.9±13.92 & 177.8±8.341 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.709±0.014 & 0.745±0.036 & 0.717±0.075 & \textbf{0.795±0.032} & 0.735±0.006 & 0.752±0.038 & \underline{0.773±0.016} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 12.91±1.706 & \underline{12.1±3.479} & 12.53±3.624 & 16.47±6.278 & 18.96±6.951 & \textbf{10.81±4.540} & 11.95±5.148 \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Porto}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 4.390±0.001 & 4.397±0.001 & 4.287±0.000 & 4.362±0.009 & \textbf{4.196±0.010} & 4.205±0.003 & \underline{4.347±0.047} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 7.901±0.002 & \textbf{7.581±0.001} & 7.777±0.001 & \underline{7.931±0.047} & 7.705±0.007 & 7.793±0.040 & 7.792±0.054 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 99.46±1.781 & 101.3±1.981 & \underline{97.15±1.384} & 98.40±1.812 & 98.54±2.826 & 97.50±6.916 & \textbf{96.84±1.296} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 149.5±3.597 & 147.2±2.598 & \underline{142.7±1.798} & 146.7±2.479 & \textbf{140.5±2.224} & 157.7±7.044 & 144.8±1.031 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.803±0.098 & 0.822±0.109 & 0.832±0.030 & \textbf{0.901±0.064} & 0.835±0.035 & \underline{0.881±0.020} & 0.871±0.039 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 14.33±4.907 & \underline{11.98±1.809} & 17.86±5.396 & 12.06±4.026 & 18.20±4.804 & 13.68±4.440 & \textbf{11.40±6.376} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Sanfransico}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 2.981±0.003 & 2.511±0.001 & 2.489±0.008 & 2.555±0.002 & 2.485±0.005 & \underline{2.454±0.003} & \textbf{2.424±0.009} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 5.802±0.004 & 5.379±0.005 & \underline{5.289±0.014} & 5.295±0.002 & \textbf{5.246±0.003} & 5.332±0.001 & 5.367±0.001 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 289.0±0.022 & 287.8±0.006 & 278.7±0.212 & 273.6±19.04 & \underline{270.4±12.64} & \textbf{267.6±15.17} & 275.2±13.29 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 1479±4.301 & 1449±4.426 & 1499±3.618 & \textbf{1372±58.16} & 1501±56.35 & 1597±78.46 & \underline{1446±61.11} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.837±0.039 & 0.911±0.004 & 0.860±0.069 & \textbf{0.943±0.035} & \underline{0.923±0.014} & 0.896±0.073 & 0.872±0.053 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 7.195±3.190 & 7.003±0.015 & 8.478±3.050 & 9.224±7.285 & \underline{6.551±1.222} & 6.711±4.013 & \textbf{6.490±3.633} \\
        \midrule
        \multicolumn{3}{c|}{Per Avg Rank} & 6.333 & 4.900 & 3.900 & 3.867 & 3.200 & \underline{2.933} & \textbf{2.867} \\
        \bottomrule
    \end{tabular}%
}
\label{tab:comroad}
\end{table*}

\paratitle{Randomness Sensitivity in Road Segment MapRL Models}
Road segment representation learning is significantly affected by data partitioning and the data generation process for Similarity Trajectory Search (STS), where the labels are assigned through a random detour process based on original coordinate trajectories. As shown in \tab\ref{tab:comroad}, our results confirm this conclusion: among the various downstream tasks, STS is the most affected, while ASI (Average Speed Inference) is relatively robust. Additional findings are summarized as follows:

\begin{itemize}[leftmargin=*]
    \item Toast, START, and JCLRNT exhibit higher instability compared to other models, as they rely on contrastive learning techniques, such as Token Relation Contrastive Learning  (TRCL) used by Toast and Augmented Trajectory Contrastive Learning (ATrCL) using by START and JCLRNT. These methods are highly susceptible to variations introduced by dataset partitioning and negative sampling, leading to performance fluctuations across different runs.
    
    \item RN2Vec is the most robust model, consistently demonstrating low variance across different datasets. Its stability is likely attributed to its Token Relation Inference (TokRI) pretraining task, thereby mitigating sensitivity to randomness.
    
    \item TTE and STS tasks show significant sensitivity to randomness, as they rely on graph-based and sequence-based representation learning, making them particularly prone to dataset partitioning effects. In contrast, TSI tasks remain largely unaffected due to their structured numerical relationships, which exhibit greater stability across different random seeds.
    
    \item Downstream tasks in Beijing (BJ) and San Francisco (SF) display higher variance than in other cities. This can be attributed to their large number of road segments (BJ: 40,306, SF: 27,274), which increases trajectory diversity, thereby amplifying the impact of dataset partitioning on model performance.
\end{itemize}

\begin{table*}[t]
  \centering
  \vspace{-0.3cm}
  \caption{Revision of Table 5 by addressing randomness.}
  \vspace{-0.3cm}
    \renewcommand{\arraystretch}{0.8}
    \small
    \setlength{\extrarowheight}{-1pt}
    \resizebox{0.8\textwidth}{!}{ % 让表格自动缩放
    \begin{tabular}{ccc|ccccccc}
        \toprule
        \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{Task} & Metric & ZEMob & GMEL  & HDGE  & MVURE & MGFN  & ReMVC & HREP \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Beijing}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.427±0.028 & 0.456±0.030 & 0.406±0.002 & 0.482±0.002 & \underline{0.595±0.016} & \textbf{0.750±0.018} & 0.499±0.015 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.113±0.002 & 0.612±0.025 & 0.221±0.005 & 0.277±0.008 & \underline{0.650±0.045} & \textbf{0.714±0.018} & 0.381±0.014 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 30.94±0.026 & 27.70±0.013 & \underline{20.76±4.905} & 29.57±0.829 & 30.12±0.024 & 27.83±0.016 & \textbf{20.60±1.334} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 55.26±0.039 & 58.96±0.039 & \underline{44.79±5.787} & 53.72±1.360 & 54.47±0.020 & 52.72±0.037 & \textbf{42.62±1.863} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 0.429±0.029 & 0.464±0.028 & 0.345±0.025 & \textbf{0.269±0.011} & 0.304±0.032 & \underline{0.300±0.015} & 0.319±0.002 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 0.795±0.024 & 0.743±0.023 & 0.700±0.034 & 0.712±0.016 & 0.760±0.038 & \underline{0.695±0.023} & \textbf{0.664±0.008} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Chengdu}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.360±0.013 & 0.383±0.040 & 0.422±0.034 & 0.481±0.004 & 0.482±0.079 & \textbf{0.664±0.032} & \underline{0.536±0.005} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.174±0.034 & 0.162±0.032 & 0.266±0.064 & 0.274±0.015 & 0.348±0.123 & \textbf{0.586±0.026} & \underline{0.456±0.009} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 154.9±0.025 & \underline{154.8±0.019} & 159.1±2.020 & 156.2±3.099 & 157.5±5.687 & \textbf{147.7±0.016} & 156.5±18.80 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 441.2±0.022 & 441.1±0.041 & 403.3±1.125 & 442.8±4.280 & \textbf{337.4±64.38} & 431.0±0.029 & \underline{395.7±49.70} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & \textbf{3.640±0.032} & 4.622±0.036 & 5.171±0.013 & \underline{3.968±0.711} & 5.142±0.020 & 5.292±0.037 & 5.471±0.121 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 29.70±0.024 & 29.71±0.030 & \underline{28.73±0.154} & 29.58±0.125 & 29.32±1.139 & 29.05±0.061 & \textbf{28.30±0.071} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Xi'an}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.360±0.031 & 0.365±0.028 & 0.444±0.017 & 0.531±0.009 & 0.478±0.085 & \underline{0.574±0.004} & \textbf{0.589±0.013} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.188±0.036 & 0.418±0.034 & 0.254±0.009 & 0.264±0.017 & 0.284±0.072 & \textbf{0.460±0.034} & \underline{0.453±0.024} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 133.8±0.028 & 133.1±0.018 & \underline{124.1±5.867} & 127.1±3.846 & \textbf{119.2±9.305} & 131.6±0.038 & 128.6±0.798 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 326.2±0.020 & 324.5±0.034 & \underline{289.0±26.30} & 317.8±4.766 & \textbf{241.2±28.38} & 324.6±0.033 & 296.9±9.101 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 3.828±0.034 & 3.710±0.035 & 3.916±0.031 & \textbf{3.333±0.351} & \underline{3.696±0.112} & 3.911±0.052 & 4.019±0.042 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 17.68±0.034 & 17.65±0.026 & \textbf{16.62±0.139} & 17.41±0.004 & 16.79±1.321 & 16.81±0.050 & \underline{16.71±0.201} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Porto}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.343±0.035 & 0.330±0.037 & \underline{0.424±0.047} & 0.297±0.014 & 0.303±0.005 & \textbf{0.444±0.032} & 0.358±0.022 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.211±0.006 & 0.384±0.029 & \underline{0.407±0.074} & 0.272±0.017 & 0.200±0.027 & \textbf{0.414±0.038} & 0.319±0.029 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 527.5±0.027 & 525.1±0.009 & 501.0±18.03 & \underline{401.6±71.84} & 476.7±97.28 & 527.3±0.015 & \textbf{288.6±121.6} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 595.2±0.022 & 592.0±0.035 & 581.9±14.39 & 472.0±71.13 & \underline{443.2±96.75} & 594.9±0.031 & \textbf{355.4±126.9} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 44.88±0.021 & 41.12±0.026 & 30.79±4.571 & 37.76±0.648 & \underline{29.80±7.256} & 39.39±0.047 & \textbf{28.26±5.297} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 72.32±0.019 & 56.23±0.037 & 45.70±4.910 & 54.11±4.679 & \underline{45.45±9.793} & 56.68±0.029 & \textbf{42.17±8.930} \\
        \midrule
        \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Sanfransico}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & \underline{0.845±0.016} & 0.638±0.011 & 0.825±0.006 & 0.845±0.021 & 0.831±0.012 & \textbf{0.858±0.033} & 0.838±0.006 \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.529±0.030 & \underline{0.565±0.010} & 0.497±0.030 & 0.516±0.053 & 0.440±0.096 & 0.473±0.036 & \textbf{0.570±0.028} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 509.2±0.036 & 514.0±0.015 & 387.2±73.13 & \underline{349.3±73.67} & 356.2±125.5 & 444.7±0.010 & \textbf{324.5±65.78} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 910.5±0.043 & 916.7±0.021 & \underline{693.0±135.10} & 700.3±123.6 & 748.3±130.3 & 852.4±0.024 & \textbf{624.4±101.4} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & \textbf{5.877±0.027} & 7.402±0.019 & 6.514±0.510 & 6.461±0.424 & 6.396±0.838 & 6.870±0.037 & \underline{5.895±0.496} \\
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 23.49±0.009 & 22.31±0.015 & 21.46±0.281 & 20.63±1.212 & \underline{20.16±2.343} & 22.66±0.031 & \textbf{19.10±1.506} \\
        \midrule
        \multicolumn{3}{c|}{Per Avg Rank} & 5.667  & 5.100  & 4.000  & 3.733  & 3.533  & \underline{3.500} & \textbf{2.433} \\
        \bottomrule
    \end{tabular}%
    }
  \label{tab:letterregion}%
  \vspace{-0.3cm}
\end{table*}%

\paratitle{Randomness Sensitivity in Land Parcel MapRL Models}
Land parcel representation learning exhibits different levels of sensitivity across tasks. Classification tasks (LPC) are generally stable, while Flow Inference (FI) and Mobility Inference (MI) tasks show higher sensitivity. Other findings are summarized as follows:

\begin{itemize}[leftmargin=*]
    \item ZEMob, GMEL, and ReMVC are among the most stable models across all datasets. Despite employing contrastive learning as pretraining tasks—which tends to be sensitive in other MapRL models—their stability may be attributed to the smaller number of parcel entities. For instance, San Francisco contains 194 parcel entities compared to 27,274 road segment entities. This smaller number of parcel entities likely results in more stable negative sampling.

    \item MGFN is notably sensitive across datasets, as it utilizes clustering techniques to construct the base graph structure for representation learning, introducing sensitivity to randomness.

    \item FI and MI tasks exhibit greater sensitivity to randomness than LPC classification tasks. This is expected because these two tasks involve graph-based regression, which is sensitive to data partitioning.
\end{itemize}

\paratitle{Cross-Task Observations on Randomness Sensitivity}
Finally, we identify broader trends that affect MapRL models across all types of representations:

\begin{itemize}[leftmargin=*] 
    \item Models utilizing contrastive learning pretraining tasks, such as Token Relation Contrastive Learning (TRCL), Augmented Token Contrastive Learning (AToCL), and Augmented Trajectory Contrastive Learning, exhibit increased sensitivity to randomness. However, this sensitivity may diminish when dealing with smaller datasets.
    
    \item Downstream tasks that rely on graph-based representation learning, including Travel Time Estimation (TTE), Similar Trajectory Search (STS), Flow Inference (FI), and Mobility Inference (MI), may experience significant structural variations across different training runs due to their dependence on graph structures.
    
    \item Datasets with greater diversity can amplify the impact of randomness, leading to increased variability in model performance.
\end{itemize}
These observations underscore the necessity of evaluating model robustness across multiple random seeds and carefully considering dataset characteristics when selecting pretraining task combinations.

\paratitle{Revision Made:} We have incorporated our findings on the impact of randomness in Section 4 and provided the corresponding experimental analysis as follows:

\begin{cmt}[Section 4.2.1 Experimental Results for POI MapRL.]
4) {\em Instability Introduced by Contrastive Learning.} SkipG, Teaser, and CACSR show significant instability due to their reliance on contrastive learning, which is sensitive to dataset partitioning and negative sample selection. In contrast, P2Vec and Tale are more stable, likely because they use token relation inference, a supervised pretraining task that enhances robustness by predicting relationships between map entities.
\end{cmt}

\begin{cmt}[Section 4.2.2 Experimental Results for Road Segment MapRL.]
3) {\em Fluctuating Results for SARN, Toast, START, and JCLRNT:}
These models experience higher performance variability compared to other models, largely due to their dependence on contrastive pretraining techniques such as Token Relation Contrastive Learning (TRCL), Augmented Graph Contrastive Learning (AGCL), and Augmented Trajectory Contrastive Learning (ATrCL). These methods are particularly vulnerable to shifts in training data splits and the inherent randomness in negative sample selection, leading to inconsistent results across multiple runs.
\end{cmt}

\begin{cmt}[Section 4.2.3 Experimental Results for Land Parcel MapRL.]
3) {\em Fluctuating Results for MGFN}: 
Although MGFN ranks third overall (with an average rank of 3.53), its performance varies considerably under different random seeds, indicating a degree of instability. This instability arises because MGFN relies on clustering techniques to build the base relation network for representation learning, making it more sensitive to randomness across datasets.

4) {\em Small Datasets Mitigate Instability in Negative Sampling}: ZEMob, GMEL, and ReMVC are among the most stable models across all datasets. Despite employing contrastive learning as pretraining tasks—which tends to be sensitive in other MapRL models—their stability may be attributed to the smaller number of parcel entities. For instance, San Francisco contains 194 parcel entities compared to 27,274 road segment entities. This smaller number of parcel entities likely results in more stable negative sampling.
\end{cmt}

\begin{cmt}[Section 4.2.4 Summary for Overall Experiments.]
4) {Instable Introduced by Contrastive Learning}: Models utilizing contrastive learning pretraining tasks exhibit increased sensitivity to randomness. However, this sensitivity may diminish when dealing with smaller datasets.
\end{cmt}






\vspace{0.3cm}


%%%%%%%%%%%%% Comment 2.3
\subsection{Comment 2.3 and Response 2.3} \label{com:23}

\commenttitle{Comment 1.2 (W3 \& D3)}

{\em (W3).} Could discuss potential domain-specific niche MapRL tasks and methods.
\vspace{4pt}

\noindent
{\em (D3).} While this work is mainly intended for an over-arching taxonomy and experimental review of existing MapRL methods, I believe there is room to discuss niche tasks, data and methods found in specific applications, if indeed there are existing works on this front.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your valuable feedback. A clear discussion of domain-specific MapRL methods not only provides a direct demonstration of how MapRL techniques apply to specific tasks but also elucidates the motivations behind their design.

Our study introduces nine downstream tasks spanning various applications, including POI Classification (POIC), Next POI Prediction (NPP), Trajectory User Link (TUL), Average Speed Inference (ASI), Travel Time Estimation (TTE), Trajectory Similarity Search (STS), Land Parcel Classification (LPC), Flow Inference (FI), and Mobility Inference (MI). These tasks are widely studied in location-based services, traffic prediction, and spatiotemporal data mining, making them representative of domain-specific MapRL applications.

Among these, POIC, ASI, and LPC do not yet have specifically designed models. Below, we elaborate on the task definitions, datasets, and existing models for the remaining tasks, illustrating how MapRL techniques are applied in various domains.

\paratitle{Next POI Prediction:} The Next POI Prediction (NPP) task aims to recommend the most relevant points of interest (POIs) to users based on their historical behavior, interests, and current location. Common datasets for this task include those from social platforms like Foursquare \citeNew{fours1}, Instagram \citeNew{CAPE}, and Yelp\citeNew{yelp}. The Foursquare dataset, which includes global user check-in trajectory data, is the most widely used, while Instagram and Yelp offer smaller datasets but include valuable user review text that has recently been leveraged to enhance model accuracy. Traditional models often rely on Recurrent Neural Networks (RNNs) or Transformers to model sequential user behavior. DeepMove \citeNew{deepmove}, for instance, employs a GRU \citeNew{GRU} with an attention mechanism \citeNew{attention} to predict the next POI a user might visit. Recent advancements integrate temporal and contextual factors (e.g., weather, time of day) to further improve recommendation accuracy.

\paratitle{Trajectory User Link:} The Trajectory User Link task aims to match anonymous trajectories with the users who generated them. This task is critical for various spatial-temporal applications, including location-based services and urban anomaly detection. Traditional methods typically train models using known user trajectory data, mapping trajectories into a vector space using RNNs or Transformers, followed by Multiple-layer preception with softmax to compute the probability of matching a trajectory to a user. A notable example, DeepTUL\citeNew{deeptul}, encodes trajectory data using GRUs, leveraging user history for embedding similarity computation. A key challenge in this task is sparse trajectory data, requiring robust generalization techniques to improve matching performance.

\paratitle{Travel Time Estimation:} The Travel Time Estimation (TTE) task aims to predict the travel time between the start and end of a given trajectory. Accurate TTE helps individuals optimize travel plans, avoid congested routes, and save time, while also aiding traffic management in road planning and traffic control. Traditional TTE methods, such as using speed detectors (e.g., loop sensors), suffer from high installation costs and limited applicability. Moreover, simply summing the travel times for each road segment fails to account for intersection delays. With the rise of Didi Chuxing and other ride-hailing trajectory datasets, data-driven methods have gained popularity. Some approaches estimate travel time by averaging historical travel durations, but these often fail to handle real-time variations. DeepTTE \citeNew{deeptte} addresses these issues by using an LSTM to model temporal dependencies and incorporating external factors (e.g., weather, road conditions, driver behavior) to enhance prediction accuracy.

\paratitle{Similarity Trajectory Search:} The Similarity Trajectory Search task aims to find the most similar trajectory to a query trajectory from a trajectory database. The core of this task is to calculate the similarity between trajectories. Trajectory similarity measures can be classified into two categories: non-learned and learned measures. Non-learned measures, such as the Hausdorff distance \citeNew{hausdorff}, calculate similarity by matching points between trajectories but are computationally expensive, with a time complexity of $O(n^2)$, making them unsuitable for large datasets. In recent years, learned measures based on deep learning have gained popularity. These methods encode trajectories as vectors (trajectory embeddings) and compute the distance between embedding vectors, using methods such as RNNs and self-attention models (like Transformers). Learned measures not only improve computational efficiency but also enhance similarity measurement accuracy, especially in cases with low-quality trajectories. Methods like NEUTRAJ\citeNew{neutraj} and T3S\citeNew{T3S} learn to approximate non-learned measures, further optimizing efficiency, while t2vec\citeNew{t2vec} and TrajCL\citeNew{TrajCL} employ self-supervised learning to directly learn from unlabeled trajectories.

\paratitle{Flow Inference \& Mobility Inference :} Mobility Inference predicts the flow of people or OD flow between land parcel over specific time periods. Flow Inference is a subtask of Mobility Inference, focusing on predicting the inflow or outflow of people in a parcel. These tasks are widely used for predicting passenger demand, especially in ride-hailing platforms like Didi and Uber. Graph-based models, such as ZEMob \citeNew{ZEMob}, construct spatial graphs where nodes represent land parcels and edges denote travel demand, using graph representation learning for prediction. However, these models often overlook temporal fluctuations. ODMP \citeNew{ODMP} introduces spatiotemporal graphs, leveraging GNNs, RNNs, and Transformers to capture both spatial relationships and temporal trends for more accurate forecasting.

We sincerely appreciate this suggestion, as it strengthens the practical relevance of our study and highlights the broader impact of MapRL techniques. We will further refine our discussion in the final version to ensure clarity and completeness.

\paratitle{Revision Made:} 
\begin{cmt}[Niche Tasks for \rl.]
    In recent years, various downstream tasks in MapRL have been widely studied, including Next POI Prediction (NPP), Trajectory User Link (TUL), Travel Time Estimation (TTE), Trajectory Similarity Search (STS), and Mobility Inference (MI). These tasks are central to location-based services, traffic prediction, and spatiotemporal data mining. Many models for NPP rely on Recurrent Neural Networks (RNNs) or Transformers, with methods like DeepMove\citeNew{deepmove} using attention mechanisms to predict users’ next POI. TUL, exemplified by DeepTUL\citeNew{deeptul}, links anonymous trajectories to users, leveraging trajectory and user embeddings. TTE methods, such as DeepTTE\citeNew{deeptte}, use LSTMs to model temporal dependencies and include factors like weather and traffic conditions for more accurate travel time predictions. For similarity trajectory search, recent advancements in learned measures, including NEUTRAJ\citeNew{neutraj} and T3S\citeNew{T3S}, outperform traditional non-learned methods by encoding trajectories as vectors. Finally, Flow and Mobility Inference tasks, integral to ride-hailing platforms like Didi and Uber, use graph-based models such as ODMP\citeNew{ODMP}, which combine spatial and temporal information via GNNs, RNNs, and Transformers for accurate demand forecasting.
\end{cmt}

\vspace{0.3cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 3
\newpage

\section{Response to Reviewer \#3 (Accept)}

%%%%%%%%%%%%% Comment 3.1
\subsection{Comment 3.1 and Response 3.1} \label{com:31}

\commenttitle{Comment 3.1 (W1)}

{\em (W1).} Taxonomy does not seem to be that novel as it is based on well-known concepts. A discussion on what are the main advantages and novelty of proposing the taxonomy is welcome.

\vspace{0.1cm}
\noindent
\commenttitle{Response}
 
We appreciate your insightful feedback regarding the novelty and advantages of our proposed taxonomy in Map Entity Representation Learning (MapRL). Your comments have prompted us to clarify and elaborate on the unique contributions and practical benefits of our work.

\paratitle{Novelty and Necessity of our Taxonomy.} MapRL is an emerging research field that aims to generate versatile and reusable data representations for various map entities, including Points of Interest (POIs), road segments, and land parcels. Despite its growing importance in applications such as Intelligent Transportation Systems (ITS) and Location-Based Services (LBS), existing research in this domain remains fragmented, with methods primarily categorized by entity type. This fragmentation limits the transferability of techniques across different tasks and hinders systematic model comparisons.

While our taxonomy builds upon well-established principles in fields like Natural Language Processing (NLP) and Computer Vision (CV), it is uniquely designed to address the distinct challenges of MapRL. Unlike NLP and CV, where structured text or images serve as the primary input, MapRL involves spatial constraints, multi-scale entity relationships, and the integration of auxiliary information such as trajectories and mobility patterns. Our taxonomy categorizes models based on their functional components—encoders, pretraining tasks, and downstream tasks—rather than entity type, allowing for a more generalizable and modular perspective. This method-centric classification introduces a novel way to organize MapRL approaches, promoting knowledge transfer between different subfields and enabling researchers to systematically explore model design choices.

\paratitle{Practical Advantages of Our Taxonomy.} Our taxonomy offers several practical benefits to researchers and practitioners:
\begin{itemize}[leftmargin=*]
    \item Guidance in Model Selection: By classifying MapRL models based on their underlying methodologies and corresponding pretraining tasks, our taxonomy helps researchers identify the most effective approaches for specific map entities and downstream tasks.
    \item Identification of Research Gaps: The structured framework reveals unexplored combinations of pretraining tasks and model architectures, providing insights into potential areas for future research and innovation.
    \item Standardization of Evaluation: Integrated with the VecCity library, our taxonomy facilitates the development of standardized benchmarks and evaluation protocols, promoting consistency and comparability across studies.
\end{itemize}

\paratitle{Empirical Validation through VecCity library.} 
Building upon our taxonomy, we developed VecCity, the first benchmark specifically designed for MapRL. As a taxonomy-guided library, VecCity provides a standardized framework for MapRL, enabling systematic evaluation of various models and pretraining tasks within our proposed classification. Through extensive experiments across diverse datasets and tasks, VecCity reveals distinct performance patterns among different taxonomy branches. Notably, our findings indicate that incorporating heterogeneous pretraining tasks significantly enhances model performance. These results empirically validate the relevance and effectiveness of our taxonomy in guiding model development and evaluation in MapRL.

\paratitle{Conlusion.} In summary, our taxonomy addresses a critical gap in the MapRL field by providing a structured, method-centric framework that reflects the unique challenges of MapRL. It offers practical advantages in guiding research and development, and its validity is empirically supported through the VecCity benchmark. We hope this clarifies the novelty and significance of our contribution.

Thank you once again for your thoughtful feedback. We hope this clarifies the distinct contributions and importance of our work. Thank you again for your thoughtful feedback.

\vspace{0.3cm}



%%%%%%%%%%%%% Comment 3.2
\subsection{Comment 3.2 and Response 3.2} \label{com:32}

\commenttitle{Comment 3.2 (W2)}

{\em (W2).} Scalability and efficiency of benchmarked algorithms are briefly discussed in section 4.2.1 and 4.2.2. It would be a great plus to extend the discussion in this sense.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

We sincerely appreciate your valuable feedback on the scalability analysis of MapRL models. Scalability is crucial in MapRL, as it directly influences the applicability of learned representations to large-scale, real-world scenarios. In response, we have expanded our evaluation of the benchmarked models to focus on three core dimensions: effectiveness, efficiency, and the trade-offs between them.

\paratitle{Effectiveness.}
\noindent Effectiveness scalability assesses whether a model’s performance continues to improve as more data becomes available. In Section 4.4, we specifically investigate how reducing the fine-tuning dataset to 10\%, 20\%, 30\%, 40\%, and 50\% of its full-size impacts:
\begin{itemize}[leftmargin=*]
    \item Model Robustness Under Limited Data: By reducing the fine-tuning dataset size, we can identify which models remain reliable and maintain performance when data are scarce.
    \item Performance Growth with Additional Data: Starting from 10\% of the fine-tuning dataset and scaling up to 50\% (a fivefold increase), we can evaluate which MapRL models most effectively leverage additional data to significantly boost performance.
\end{itemize}

In the initial draft, we presented findings on Model Robustness Under Limited Data, concluding that:

1) {\em Stability in Attribute Inference Tasks}: \rl models show stable performance across varying training data sizes in attribute inference tasks, such as POI Classification (POIC) in \fig~\ref{fig:dive}~(a), Average Speed Inference (ASI) in \fig~\ref{fig:dive}~(d), and Land Parcel Classification (LPC) in \fig~\ref{fig:dive}~(g). This stability arises because these tasks focus on inferring entity attributes, which are effectively captured during pre-training. As a result, the fine-tuning phase requires only a small amount of labeled data to maintain good performance.

2) {\em Fluctuations in Trajectory-Related and Graph-Related Tasks}: Models exhibit notable performance fluctuations in trajectory-related tasks (e.g., NPP, TUL, TTE) and graph-related tasks (e.g., FI, MI). Trajectory-related tasks require sequence-level predictions, whereas most encoders and pre-training tasks generate single-entity embeddings, making these tasks especially sensitive to smaller fine-tuning datasets. By contrast, Similarity Trajectory Search (STS) relies on similarity comparisons rather than prediction, making it less effective. Additionally, Flow Inference (FI) and Mobility Inference (MI), although not strictly trajectory-based, capture human mobility flows that vary greatly over time. This temporal heterogeneity demands more labeled data to accurately model these patterns, leading to further performance variability when data are limited.

However, our initial analysis lacked insights into performance scalability, i.e., how model performance improves as more labeled data becomes available. To address this, we have added a discussion on performance scalability in Section 4.3.
\begin{cmt} [4.3.1 Effectiveness.]
1) {\em Performance Scalability.} Token-based MapRL models (represented by dashed lines) exhibit weaker performance scalability, showing limited improvement as the fine-tuning dataset size increases from 10\% to 50\%, with performance gains plateauing around the 30\% mark. In contrast, graph-based and sequence-based models maintain steady gains up to 50\%, demonstrating stronger scalability. Notably, methods incorporating contrastive learning techniques—such as CACSR, START, JCLRNT, and HREP—show particularly strong improvements, suggesting that contrastive learning further enhances performance as more data becomes available. However, due to the inherent instability of contrastive learning, increasing the number of negative samples may be necessary to ensure more stable results.
\end{cmt}

\begin{cmt} [4.3.1 Effectiveness.]
Overall, token-based models show weaker performance scalability, with diminishing returns as dataset size increases, particularly beyond 30\%. In contrast, graph-based and sequence-based models, especially those employing contrastive learning methods (e.g., CACSR, START, JCLRNT, HREP), exhibit more significant performance improvements as the amount of labeled data increases, demonstrating stronger scalability in data-intensive scenarios. Moreover, existing \rl models exhibit varying sensitivity to the size of labeled data across different tasks. For tasks less influenced by temporal information, such as attribute inference (ASI, POIC, LPC) and Similarity Trajectory Search (STS), models maintain stable performance even with limited training data. However, for tasks with time-dependent labels, such as trajectory-related tasks (NPP, TUL, TTE) and Flow/Mobility Inference tasks (FI, MI), larger amounts of labeled data are necessary to effectively capture temporal dynamics.
\end{cmt}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/rebuttal/efficient.pdf}
    \caption{Model efficiency on parameter size, training time, and inference time.}
    \label{fig:efficient}
\end{figure}

\paratitle{Efficiency.}
\noindent We evaluate the efficiency of MapRL models across the following three aspects: (1) parameter count which represent the space complexity of MapRL models; (2) training time per epoch, which identifies the time cost of training the models. We collect the time cost for 100 training epochs and take the mean of 100 epochs as the training time per epoch; And (3) inference time, which identifies the time cost for the evaluation of the downstream task. These measurements are collected across all five datasets used in the main experiments. These datasets, which have different entity counts, help us investigate the scalability of model efficiency.

1)\emph{Paramter Count.} We measure the parameter count of all models, as shown in Figure 1 (a), (d), and (g). Figure 1 (a) presents the parameter count for POI-oriented models, (d) for road segment-oriented models, and (g) for land-parcel-oriented models. The horizontal axis represents the number of entities on a $10^3$ scale, while the vertical axis represents the parameter count in millions. Several key findings emerge:
\begin{itemize}[leftmargin=*]
    \item Token-based models (represented by dashed lines) generally achieve better scalability in parameter size.
    \item Sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) often exhibit higher parameter counts.
    \item Graph-based models like SARN, GMEL, MVURE, and HREP, show slow changes in parameter count with increasing entity numbers, demonstrating better scalability in scenarios with a large number of map entities.
\end{itemize}

2)\emph{Training Time.} We measure the per-epoch training time for all MapRL models, with results shown in Figure 1 (b), (e), and (h) for POI, road segment, and land-parcel-oriented models, respectively. The horizontal axis represents the number of entities (scaled to $10^3$), and the vertical axis shows the average training time per epoch (in seconds) over 100 epochs. Key findings include:
\begin{itemize}[leftmargin=*]
    \item Token-based models exhibit better scalability in POI-oriented models but perform worse in land-parcel-oriented models due to differences in entity counts: $1 \times 10^4 - 8 \times 10^4$ for POI and $2 \times 10^2 - 1 \times 10^4$ for land parcels. Therefore, token-based models may have a greater competitive advantage in large-scale datasets.
    \item Sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) tend to incur higher training times.
    \item Graph-based models using GAu (e.g., HRNR, HRoad, GMEL, MGFN) exhibit more-than-linear growth in training time, presenting challenges for large-scale datasets. HREP, which also uses GAu, does not show significant growth in training time, likely due to its lower space complexity.
\end{itemize}

3)\emph{Inference Time.} We measure the inference time for all MapRL models, with results shown in Figure 1 (c), (f), and (i) for POI, road segment, and land-parcel-oriented models, respectively. The horizontal axis represents the number of entities on a $10^3$ scale, and the vertical axis shows inference time (in seconds). Key findings include:
\begin{itemize}[leftmargin=*]
    \item All MapRL models exhibit the same increasing trend. However, the rise in inference time is more pronounced for POI and land-parcel-oriented models compared to road segment-oriented models. This suggests that inference time is more strongly influenced by the number of entities in the downstream tasks for POI and parcel models.
    \item Sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) tend to incur higher inference times.
    \item HRNR exhibits much higher inference times than other road segment-oriented models, largely due to the dynamic graph construction during inference.
\end{itemize}



% \paratitle{Trade-offs between model size and inference time.} Beyond the individual aspects of effectiveness and efficiency, we further analyze the trade-offs between model size and inference time through Figure \ref{fig:comtradeoff}, which visualizes the relationship between parameter count and inference time across all benchmarked models. To present the inference time for all models in one figure, we report the inference time per sample rather than the total inference time. As shown in Figure \ref{fig:comtradeoff}, the horizontal axis represents parameter count in millions, and the vertical axis represents single-sample inference time in milliseconds. Key observations include:
\begin{itemize}[leftmargin=*]
    \item land-parcel-oriented models maintain relatively stable inference times despite an increase in parameter size, possibly due to lower downstream task complexity. POI and road segment-oriented models show a more linear or sometimes steeper increase.
    \item Models using sequence encoders (e.g., Hier, CACSR, CTLE, JCLRNT, START, Toast) generally increase inference times due to the integration of multiple encoders and heterogeneous pretraining tasks. 
    \item Attention mechanisms (e.g., Transformers in Toast, JCLRNT, START, and GAT-based MGFN) increase both parameter counts and inference times.
    \item Graph encoder-based models  (e.g., HyperRoad, SARN, GMEL, MGFN, HDGE, HREP) do not necessarily incur high inference times, except for HRNR, which uses multiple GNN layers during inference.
\end{itemize}
\noindent These results underscore the trade-offs between model size and inference time, providing insights into how to balance computational costs with performance requirements.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/rebuttal/time_tradeoff.pdf}
    \caption{Trade-offs between model size and inference time.}
    \label{fig:comtradeoff}
\end{figure}

\paratitle{Conclusion}
\noindent We thank the reviewer for emphasizing the importance of scalability analysis. Our revised manuscript now provides a more structured discussion, encompassing effectiveness, efficiency, and their inherent trade-offs. We believe these findings will benefit both researchers and practitioners, helping to inform model selection based on computational constraints and performance needs.

\paratitle{Revision Made:} Based on the above analysis, we revision our paper by adding new findings in Section 4.3.
\begin{cmt} [4.3.2 Efficiency.]
To fully investigate the efficiency scalability of MapRL models, we evaluate them across three key aspects: (1) Parameter count, representing the space complexity of the models; (2) Training time per epoch, indicating the time cost of training; and (3) Inference time, reflecting the time required for downstream task evaluation. These measurements are collected from all five datasets used in the main experiments, each with different entity counts. Figure.~\ref{fig:efficiency} presents the evaluation results: \fig~\ref{fig:efficiency} (a) to (c) show results for POI-oriented models, \fig~\ref{fig:efficiency} (d) to (f) display results for road segment-oriented models, and \fig~\ref{fig:efficiency} (g) to (i) provide results for land parcel-oriented models. The horizontal axis of all figures represents the number of entities on a $10^3$ scale, while the vertical axis represents the parameter count in millions, training time per epoch in seconds, and total inference time in seconds, respectively. Based on these figures, we have several key findings:

 1) {\em Model Size:} Token-based models (dashed lines) generally achieve better scalability in parameter size, while sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) often have higher parameter counts. In contrast, graph-based models such as SARN, GMEL, MVURE, and HREP show relatively stable parameter counts as the number of entities increases, demonstrating better scalability in scenarios with large numbers of map entities.

2) {\em Training Time:} Token-based models (dashed lines) demonstrate better training time scalability in POI-oriented models but perform less efficiently in land parcel-oriented models. This difference is influenced by entity count variations, with POI datasets containing between $1 \times 10^4$ and $8 \times 10^4$ entities, while land parcel datasets range from $2 \times 10^2$ to $1 \times 10^4$ entities. The results suggest that token-based models may have a greater competitive advantage in large-scale datasets. Sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) generally incur longer training times. Graph-based models employing GAu pretraining tasks (HRNR, HRoad, GMEL, MGFN) show more-than-linear growth in training time, posing scalability challenges for large datasets, whereas HREP, despite using GAu pretraining, maintains relatively stable training time due to its lower space complexity.

3) {\em Inference Time:} All models show an increasing trend in inference time. However, the rise is more pronounced in POI- and land parcel-oriented models compared to road segment-oriented models, indicating that inference time is more heavily influenced by the number of entities in downstream tasks for POIs and parcels. Sequence-based models (e.g., CTLE, Toast, START, JCLRNT) generally require longer inference times, while HRNR stands out among road segment-oriented models with significantly higher inference times due to its dynamic graph construction during inference.
\end{cmt}

\begin{cmt} [4.3.3 Trade-offs between model size and inference time.]
In Section \ref{sec:experiment}, we conclude that more complex models often achieve higher accuracy. However, increased model complexity can lead to efficiency challenges, particularly in inference time, which may limit their practicality in real-world applications. The efficiency analysis in the previous section does not provide a direct view of the relationship between model complexity and inference time. To explore this trade-off, we conducted an experiment evaluating the relationship between parameter count and inference time. This experiment uses the same dataset as in Section 4.3.1 on effectiveness: POI-oriented models are evaluated on the Tokyo dataset, while road segment- and land parcel-oriented models are tested on the Xi’an dataset. To enable a unified comparison across the three entity types, the horizontal axis represents the parameter count (in millions), and the vertical axis represents the single-sample inference time (in milliseconds).

Figure.\ref{fig:tradeoff} presents the results, showing that land-parcel-oriented models maintain relatively stable inference times despite increases in parameter size, likely due to lower downstream task complexity. In contrast, POI and road segment-oriented models exhibit a more linear or steeper increase in inference time as model complexity grows. Sequence-based models (e.g., Hier, CACSR, CTLE, JCLRNT, START, Toast) generally show higher inference times due to the integration of multiple encoders. Attention mechanisms, such as those employed by Transformers (Toast, JCLRNT, START) and the GAT(MGFN), contribute to increased parameter counts and inference times. Meanwhile, graph-based models (e.g., HyperRoad, SARN, GMEL, MGFN, HDGE, HREP) tend to maintain lower inference times, with the exception of HRNR, which uses dynamic graph construct during inference, leading to significantly higher inference times.
\end{cmt}


\vspace{0.3cm}


%%%%%%%%%%%%% Comment 3.3
\subsection{Comment 3.3 and Response 3.3} \label{com:33}

\commenttitle{Comment 3.3 (W3)}

{\em (W3).} The link to download data is not working in the Github repo.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

We apologize for the inconvenience caused by the non-functional data download link in our GitHub repository. This issue may be due to restrictions associated with Beihang University's hosting services. To ensure more reliable access, we have provided an alternative download link via \updateo{\href{https://drive.google.com/file/d/1JqnGsprG2zpJ4tisf0o3liOLy3GR7t0i/view?usp=drive_link}{Google Drive}}.

We are committed to maintaining the availability and functionality of our tools and resources. If you encounter any further issues or have additional questions, please do not hesitate to contact us.
\vspace{0.3cm}

\bibliographystyleNew{ieeetr}
\bibliographyNew{sample1}


==> 0-response.tex <==
% \newtcolorbox{cmt}[1][]{%
%   colframe = black!60!white,    % 边框颜色
%   colback = black!5!white,      % 背景颜色
%   coltext = black,              % 文本颜色
%   fonttitle = \bfseries,        % 标题字体
%   title={#1},                   % 自定义标题
%   enhanced,                     % 增强模式
% }


\newtcolorbox{cmt}[1][]{%
  colframe = black!60!white,    % Border color
  colback = black!5!white,      % Background color
  coltext = black,              % Text color
  fonttitle = \bfseries,        % Title font
  title={#1},                   % Custom title
  enhanced,                     % Enhanced mode
  breakable,                    % Allows box splitting
}


\newcommand{\commenttitle}[2]{%
  \underline{\textbf{\textcolor{blue}{#1:}}}\\[8pt]
}
\newcommand{\updatec}[1]{{\color{blue} #1}}

\newcommand{\responseletterstyle}{
    % 自定义章节编号为字母
    \renewcommand{\thesection}{\Alph{section}}
    % % 一级标题加粗并不缩进
    % \renewcommand{\cftsecfont}{\bfseries}
    % \renewcommand{\cftsecindent}{0em}
    % % 二级标题缩进
    % \renewcommand{\cftsubsecfont}{}
    % \renewcommand{\cftsubsecindent}{2em}
    % % 一级标题与页码之间的行间距
    % \renewcommand{\cftsecafterpnum}{\vskip0.5em}
    % 自定义目录标题
    \renewcommand{\contentsname}{}
    % 调整目录标题与内容的间距
}
% \renewcommand{\contentsname}{Response Letter Contents}
\titlecontents{section}
  [0em] % 左缩进
  {\addvspace{1.5em}\bfseries\color{blue}} % 格式化条目
  {\textcolor{blue}{\thecontentslabel}\quad} % 标签格式
  {}
  {\hfill\textcolor{blue}{\contentspage}} % 页码位置

\titlecontents{subsection}
  [1em]
  {\addvspace{0.5em}\color{blue}}
  {\textcolor{blue}{\thecontentslabel}\quad}
  {}
  {\hfill\textcolor{blue}{\contentspage}}

\responseletterstyle % 启用 Response Letter 样式


\section*{\centering \huge Response Letter}
\vspace{10pt}
\pagestyle{plain} % 恢复默认页眉页脚样式
\noindent\textbf{Paper Title:} VecCity: A Taxonomy-guided Library for Map Entity Representation Learning.

\noindent\textbf{Paper ID:} 1995 (Revision of 1016)

\noindent\textbf{Track Name:} Experiment, Analysis \& Benchmark

\noindent\textbf{Authors:} Wentao Zhang, Jingyuan Wang, Yifan Yang, and Leong Hou U.
\vspace{10pt}

\noindent
Dear Meta Reviewer and Reviewers:
\vspace{0.2cm}

Attached is a revised manuscript entitled “VecCity: A Taxonomy-guided Library for Map Entity Representation Learning” (Paper ID: 1995, Revision of 1016), in "Experiment, Analysis \& Benchmark" track.

We would like to thank all the reviewers for reading through our submission and providing constructive feedbacks. In this revised version, we have carefully addressed all comments from the reviewers and meta-reviewer, which have greatly improved the quality of our work. A detailed point-by-point response to each comment is provided, with significant changes in the manuscript highlighted in \textcolor{blue}{blue}. Each comment is restated, followed by our response and the corresponding manuscript revisions.

We hope that the revised submission meets the reviewers’ expectations and adheres to the high standards of the VLDB conference. Once again, we sincerely thank you for your thoughtful consideration of our work.


\vspace{0.2cm}
\noindent
Sincerely,

%\vspace{0.2cm}
\noindent
Wentao Zhang, Jingyuan Wang, Yifan Yang, and Leong Hou U.


\newpage
\section{Response to the Meta Reviewer}
 
\commenttitle{Meta Review}

The reviewers found the paper overall well-executed and with a timely topic. There are some specific requests for a revision are raised and discussed below. Crucially, please ensure the link to the artifacts is working.
\begin{enumerate}[leftmargin=*]
    \item discuss results in terms of time performance of downstream tasks, where scalability may be a concern.
    \item expand on (i) scalability issues and (ii) model size VS inference time tradeoff.
    \item consider adding more models to ensure a broader representation of the field.
    \item align table 1 with the proposed taxonomy.
    \item discuss the distinctions between vector and raster data models and their implications on the benchmarking process, ensuring clarity and relevance to MapRL tasks.
    \item  $[$artifact availability is required$]$ ensure URL to the benchmark works.
    \item  $[$optional$]$ use an established standard data format instead of introducing a new one to enhance compatibility, reduce complexity, and encourage adoption.
\end{enumerate}

\vspace{0.1cm}
\noindent
\commenttitle{Response}

We would like to thank the meta-reviewer for giving us the opportunity to revise the manuscript! For the major comments, we have made the following modifications.

\textbf{\textcolor{red}{For (1) and (2):}} We have expanded our discussion on scalability, particularly addressing performance scalability (\underline{\updateo{Section \ref{sec:431}}}), efficiency scalability (\underline{\updateo{Section \ref{sec:432}}}), and the trade-offs between model size and inference time (\underline{\updateo{Section \ref{sec:433}}}). Specifically, we analyze how model performance scales with increasing fine-tuning dataset size, how efficiency is impacted by the number of entities, and the trade-offs between model complexity and inference efficiency. %Additional results and discussions are provided in \updateo{\hyperref[com:32]{Response for Reviewer \#3 Comment 3.2}} and Section \ref{sec:43}. 

\textbf{\textcolor{red}{For (3):}} We included more related MapRL models in our taxonomy (\underline{\updateo{\hyperref[sec:t221]{Section 2}}}). Additionally, in \underline{\updateo{\hyperref[com:11]{Response to Reviewer \#1 Comment 1.1}}}, we have clearly defined the boundaries of our taxonomy and provided explanations for some related models that were not included. These updates expand the taxonomy’s coverage and enhance its comprehensiveness.

\textbf{\textcolor{red}{For (4):}} We have made a revision for \underline{\updateo{Table~\ref{tab:models}}} by adding a new column that introduces the categorization of methods, ensuring better alignment with the proposed taxonomy.

\textbf{\textcolor{red}{For (5):}} We have added a discussion in the paper’s \underline{\updateo{Section \ref{sec:relatedwork}}} to illustrate the distinctions between vector and raster data models and clarify their relevance to MapRL. 

\textbf{\textcolor{red}{For (6):}} We have carefully verified the URL and ensured that all artifacts are accessible. Additionally, we have provided an alternative access URL on \underline{\updateo{\href{https://drive.google.com/file/d/1JqnGsprG2zpJ4tisf0o3liOLy3GR7t0i/view?usp=drive_link}{Google Drive}}} to guarantee the availability of the artifacts.

\textbf{\textcolor{red}{For (7):}} We offer users an interface that accepts input files in standard formats to simplify the use of the tool. Meanwhile, we retain atomic files for their crucial role in streamlining data processing.
%In \underline{\updateo{\hyperref[com:13]{Response to Reviewer \#1 Comment 1.3}}}, we provide a detailed discussion on the importance of atomic files in our benchmark and provide a detailed illustration of the solutions for incorporating standard format input files into VecCity.

In the following sections, we respond to all reviewer comments point by point and outline the corresponding revisions. The major modifications are summarized as follows:
\begin{itemize} [leftmargin=*]
    \item {\em Taxonomy}: 1) We have aligned \underline{\updateo{Table~\ref{tab:models}}} with the proposed taxonomy and included additional relevant models. 2) We have clarified the distinctions between raster data and vector data in \underline{\updateo{Section~\ref{sec:relatedwork}}}.
    \item {\em The Library}: We have implemented a new interface to incorporate input files in standard formats.
    \item {\em Experiments}: 1) Address Randomness: We analyzed the impact of randomness on model performance in \underline{\updateo{\hyperref[sec:t42]{Section 4.2}}} and provided explanations for observed instability. 2) We have expanded the discussion on scalability issues in \underline{\updateo{\hyperref[sec:t43]{Section 4.3}}}, covering effectiveness, efficiency, and the trade-offs between model size and inference time.
    3) Exploring Pretraining Tasks: We systematically explored various combinations of pretraining tasks, uncovering key insights that guide the design of the MapRL model. Further details are available in \underline{\updateo{Section \ref{sec:pretraintask}}} and \underline{\updateo{\hyperref[com:21]{Response to Reviewer \#2 Comment 2.1}}}.
\end{itemize}


\newpage
\addtocontents{toc}{\protect\setcounter{tocdepth}{-1}}
\section*{Contents}
\tableofcontents
\addtocontents{toc}{\protect\setcounter{tocdepth}{2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 1
\newpage
\section{Response to Reviewer \#1} 
\vspace{1pt}

\vspace{-1pt}
%%%%%%%%%%%%% Comment 1.1
\subsection{Comment 1.1 and Response 1.1} \label{com:11}
\commenttitle{Comment 1.1 (W1 \& R1)}

{\em (W1).} Limited Model Coverage: Table 1 lists only a subset of MapRL models, leaving out many important ones without clear justification for their exclusion. This undermines the comprehensiveness of the proposed taxonomy.
\vspace{4pt}

\noindent
{\em (R1).} Expand the Model Coverage: Compile a more comprehensive list of existing models to ensure inclusivity and provide a broader representation of the field. 

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thanks for your constructive feedback. In response, we have expanded the model coverage by including additional related models, clarified the scope of our work, and explained the reasons for excluding certain models. The revisions for Table 1 are as follows:

\begin{table*}[htbp]
  \centering
  \caption{\updateo{Revision of Table 1 by adding new MapRL models.}}
  \resizebox{\textwidth}{!}{

    \begin{tabular}{c|r|c|ccc|ccc|cccc|ccc|ccc|rcr|cc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}[4]{*}{Method}} & Taxnomy & \multicolumn{3}{c|}{Encoders} & \multicolumn{10}{c|}{Pretraining Tasks}                                       & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
\cline{4-24}    \multicolumn{2}{c|}{} & Type  & Token & Graph & Seq   & TokRI & TRCL  & AToCL & NFI   & GAu   & NCL   & AGCL  & TrajP & MTR   & ATrCL & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & \multicolumn{1}{c|}{Temp} & Traj  & Rel \\
    \midrule
    \multirow{13}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Point of Interest}}} 
    & CWAP~\citeNew{CWAP}  & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & CAPE~\citeNew{CAPE}  & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{r}{} &       & CIT   &  \\
    & MT-POI~\citeNew{MT-POI} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       &       & GR \\

    & \textcolor{blue}{Place2V}~\citeNew{Place2Vec} & \textcolor{blue}{Token-based} & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \multicolumn{1}{l}{\textcolor{blue}{\checkmark}} &  &  & \textcolor{blue}{GR} \\
    & \textcolor{blue}{Semant}~\citeNew{semantic} & \textcolor{blue}{Token-based} & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \multicolumn{1}{l}{\textcolor{blue}{\checkmark}} &  &  & \textcolor{blue}{GR} \\
    & \textcolor{blue}{CatEM}~\citeNew{CatEM} & \textcolor{blue}{Token-based} & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \multicolumn{1}{l}{\textcolor{blue}{\checkmark}} &  & \textcolor{blue}{CIT}   &  \\
    
    & SkipG*~\citeNew{Word2Vec} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} &       & CIT   &  \\
    & Tale*~\citeNew{TALE} & Token-based & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & Teaser*~\citeNew{Teaser} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   & GR \\
    & Hier*~\citeNew{Hier1} & Seq-based & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       &       &       & \checkmark     &       & CIT   & GR \\
    & P2Vec*~\citeNew{POI2VEC} & Token-based & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \checkmark     &       & CIT   & GR \\
    & CACSR*~\citeNew{CACSR} & Seq.-based & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       &       &       & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & CTLE*~\citeNew{CTLE} & Seq.-based & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    \midrule
    \multirow{11}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Road Segment}}} 
    & DyToast~\citeNew{DyToast} & Graph-based & \checkmark     & \checkmark     &       &       & \checkmark     &       & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{l}{\checkmark} &       & CDT   & GR \\
    
    & \textcolor{blue}{R2Vec}~\citeNew{R2Vec} & \textcolor{blue}{Token-based} & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  &  & \textcolor{blue}{\checkmark} &  &  & \textcolor{blue}{GR} \\
    & \textcolor{blue}{TrajRNE}~\citeNew{TrajRNE} & \textcolor{blue}{Graph-based} & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  & \textcolor{blue}{\checkmark} &  &  &  & \textcolor{blue}{\checkmark} &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \multicolumn{1}{r}{} &  & \textcolor{blue}{CDT}   & \textcolor{blue}{GR/SR} \\
    & \textcolor{blue}{JGRM}~\citeNew{JGRM} & \textcolor{blue}{Seq.-based} & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  & \textcolor{blue}{\checkmark} &  & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \textcolor{blue}{\checkmark} & \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}} & \textcolor{blue}{CDT}   & \textcolor{blue}{GR} \\

    
    & RN2Vec*~\citeNew{RN2Vec} & Token-based & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & HRNR*~\citeNew{HRNR} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & SARN*~\citeNew{SARN} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & Toast*~\citeNew{Toast} & Seq.-based & \checkmark     &       & \checkmark     &       & \checkmark     &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & HRoad*~\citeNew{HyperRoad} & Graph-based & \checkmark     & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & START*~\citeNew{START} & Seq.-based & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & JCLRNT*~\citeNew{JCLRNT} & Seq.-based & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    \midrule
    \multirow{15}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Land Parcel}}} 
    & CGAL~\citeNew{CGAL}  & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & DLCL~\citeNew{DLCL}  & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & HUGAT~\citeNew{HUGAT} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    & Re2Vec~\citeNew{Region2Vec} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & ReCP~\citeNew{ReCP}  & Token-based & \checkmark     &       &       &  \checkmark & \checkmark     & \checkmark  &      &       &       &       &       &       &   & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & SR \\

    & \textcolor{blue}{HGI}~\citeNew{HGI}  & \textcolor{blue}{Graph-based} & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  &  & \textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} &  &  &  &  &  &  &  & \textcolor{blue}{\checkmark} &  & \textcolor{blue}{\checkmark} & \multicolumn{1}{c}{\textcolor{blue}{\checkmark}} & \textcolor{blue}{\checkmark} &  &  & \textcolor{blue}{GR} \\
    & \textcolor{black}{ReDCL}~\citeNew{RegionDCL} & \textcolor{black}{Token-based} & \textcolor{black}{\checkmark} &  &  & \textcolor{black}{\checkmark} & \textcolor{black}{\checkmark} & \textcolor{black}{\checkmark} &  &  &  &  &  &  &  & \textcolor{black}{\checkmark} &  & \textcolor{black}{\checkmark} & \multicolumn{1}{c}{\textcolor{black}{\checkmark}} & \textcolor{black}{\checkmark} &  &  & \textcolor{black}{GR} \\
    & \textcolor{black}{HAFus}~\citeNew{HAFusion} & \textcolor{black}{Graph-based} & \textcolor{black}{\checkmark} & \textcolor{black}{\checkmark} &  &  &  &  &  & \textcolor{black}{\checkmark} &  &  &  &  &  & \textcolor{black}{\checkmark} &  & \textcolor{black}{\checkmark} & \multicolumn{1}{c}{\textcolor{black}{\checkmark}} & \textcolor{black}{\checkmark} &  &  & \textcolor{black}{GR/SR} \\


    
    & ZEMob*~\citeNew{ZEMob} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} &       & SR \\
    & GMEL*~\citeNew{GMEL} & Graph-based & \checkmark     & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    & MGFN*~\citeNew{MGFN} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     &       &       & SR \\
    & HDGE*~\citeNew{HDGE} & Token-based & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    & MVURE*~\citeNew{MVURE} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & SR \\
    & ReMVC*~\citeNew{REMVC} & Token-based & \checkmark     &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & SR \\
    & HREP*~\citeNew{HREP} & Graph-based & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    \bottomrule
    \end{tabular}%
        }
  \label{tab:commodels2}%
\end{table*}%

Besides, we have added descriptions of the newly included models in \underline{\updateo{\hyperref[sec:t221]{Section 2}}}, as follows:
\begin{cmt}[Revision of "Include new model to our taxonomy" in our paper's Section 2.2.1]
For TokRI and TRCL tasks, the primary innovation in existing models lies in how they construct token relations. These methods can be categorized into three classes: $i$) {\em Distance-Based Relations}: This approach establishes token relations based on spatial proximity. In TokRI tasks, RN2Vec~\cite{RN2Vec} defines a relationship between entities if their geographical distance falls below a predefined threshold. In TRCL tasks, Teaser~\cite{Teaser} selects the $K$ nearest entities as positive samples for contrastive learning. $ii$) {\em Semantic-Based Relations}: MT-POI~\cite{MT-POI}, Place2V~\cite{Place2Vec}, and Senmant~\cite{semantic} select entities that have the same or similar semantic features as positive samples for contrastive learning. $iii$) {\em Auxiliary Data-Based Relations}: This method leverages additional data, such as trajectories, to define relations. In TokRI tasks, P2Vec~\cite{POI2VEC} and Tale~\cite{TALE} treat a trajectory as a sentence and the entities within it as words, using the Continuous Bag of Words (CBOW) model~\cite{Word2Vec} to learn representations for ``words'' (map entities). In TRCL tasks, Teaser~\cite{Teaser}, R2Vec~\cite{r2vec}, and CatEM~\cite{CatEM} employ the SkipGram model~\cite{Word2Vec} with negative sampling to capture contextual relations along trajectories. When trajectory data is unavailable, ``virtual trajectories'' can be generated via random walks on relation networks~\cite{HDGE}. Beyond trajectories, ZEMob~\cite{ZEMob} leverages OD flows between entities to identify relationships.
\end{cmt}

\begin{cmt} [Revision of "Include new model to our taxonomy" in our paper's Section 2.2.2]
Recent advancements also investigate relationships across different types of map entities. For example, HGI~\cite{hgi} and HRoad~\cite{HyperRoad} utilize hypergraphs to capture these inter-entity relationships.
\end{cmt}

\textbf{More Details:} In the following section, we detail the selection process for models included or excluded in our taxonomy. We begin by defining the scope of our study, followed by an introduction to the newly incorporated models, and conclude with an explanation for the exclusion of certain related models.

\paratitle{Scope of Our Work.} Our work aims to provide a novel and comprehensive taxonomy and a standardized benchmark for Map Entity Representation Learning (MapRL). Therefore, models included in our review must meet the following criteria.
\begin{enumerate}[leftmargin=*]
    \item The model or algorithm should focus on learning versatile and reusable representations for map entities, such as Points of Interest (POI, represented as points), road segments (represented as polylines), or land parcels (represented as polygons).
    \item The data required for training the model should be commonly available in most geographic scenarios and frequently used in relevant tasks. Examples include intrinsic attributes of map entities, trajectory data, origin-destination (OD) data, and check-in data. This ensures that the models can be widely applied, thereby enhancing the general applicability of our review.
\end{enumerate}
These two criteria serve as the basis for selecting the models included in our review.

\paratitle{Included More Related Models.} To enhance the comprehensiveness of our work, we conducted a thorough review of the related literature, and the details of the newly added models are summarized in \tab\ref{tab:newmodel}.

% Table generated by Excel2LaTeX from sheet 'add'
\begin{table}[htbp]
\centering
\caption{Newly added models in VecCity.}% TODO add citation
\resizebox{0.8\textwidth}{!}{
\setlength{\tabcolsep}{0.5mm}
    \begin{tabular}{c|r|ccc|ccc|cccc|ccc|ccc|ccc|cc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{Encoders} & \multicolumn{10}{c|}{Pretraining Tasks}                                       & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
    \cmidrule{3-23}    \multicolumn{2}{c|}{} & Token & Graph & \multicolumn{1}{c|}{Seq} & TokRI & TRCL  & AToCL & NFI   & \multicolumn{1}{c}{GAu} & \multicolumn{1}{c}{NCL} & AGCL  & \multicolumn{1}{c}{TrajP} & \multicolumn{1}{c}{MTR} & ATrCL & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & \multicolumn{1}{c|}{Temp} & Traj  & Rel \\
    \midrule
    \multirow{4}{*}{POI} & Place2Vec\citeNew{Place2Vec} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} &       &       & GR \\
              & Semantic\citeNew{semantic} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} &       &       & GR \\
          & MT-POI\citeNew{MT-POI} & \checkmark     &       &       &   \checkmark  & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} &  \checkmark     &       & GR \\
    & CatEM\citeNew{CatEM} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     & \checkmark     &       & CIT   &  \\
    \midrule
    \multirow{1}{*}{Segment} & R2Vec\citeNew{R2Vec} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{} & \checkmark     &       &       & GR \\
    \midrule
    Parcel & HGI\citeNew{HGI}   & \checkmark     & \checkmark     &       &       & \checkmark     & \checkmark     &       &       &      &       &       &       &       & \checkmark     &       & \checkmark     & \checkmark     & \checkmark     &       &       & GR \\
    \bottomrule
    \end{tabular}%
}
\label{tab:newmodel}%
\end{table}%
The initial exclusion of these models was due to a mismatch in representation targets: Place2Vec, Semantic, MT-POI, and CatEM focus on POI category representation learning, whereas our work targets POI entity representation learning. Likewise, R2Vec specializes in road intersection representation learning, while we focus on road segment representation learning. Despite these differences, their techniques offer valuable insights, leading to their inclusion in our revision. Additionally, HGI was unintentionally overlooked in the initial draft.

Place2Vec\citeNew{Place2Vec}, Semantic\citeNew{semantic}, MT-POI\citeNew{MT-POI}, and CatEM\citeNew{CatEM} focus on POI category representation learning. Place2Vec utilizes a random walk algorithm to generate trajectory samples from a relation network based on POI spatial relationships, effectively capturing POI co-occurrence patterns along these trajectories. Semantic and MT-POI extend Place2Vec by incorporating POI category semantic similarities, leveraging Token Relation Contrastive Learning  (TRCL) to enhance representations. For instance, since both "supermarkets" and "shopping malls" fall under the broader "shopping" category, their embeddings are deliberately aligned to reflect this shared semantic relationship. CatEM utilizes check-in trajectories to learn POI category representations. 

R2Vec~\citeNew{R2Vec} focuses on road intersection representation learning, employing random walks on road networks and using TRCL to model co-occurrence relationships among intersections. 

HGI~\citeNew{HGI} targets land parcel representation learning by constructing a hierarchical entity network spanning four levels: POI category → POI → land parcel → city. It first pretrains POI category embeddings using Semantic\citeNew{semantic}, then aggregates lower-level representations into higher-level ones via attention and Graph Neural Network (GNN)-based methods. Finally, it applies TRCL, ensuring that embeddings of related entities remain similar across different hierarchical levels.

\paratitle{Related but Excluded Models.} Several MapRL models are not included in our taxonomy because they rely on specific types of auxiliary data, such as images and text, which limits their practicality in real-world applications. These dependencies introduce additional complexity and reduce their applicability in cases where such data is expensive to collect, inconsistent across regions, or unavailable in standard map data pipelines. Below, we summarize the main reasons for their exclusion:
\begin{itemize}[leftmargin=*] 
    \item {\em Reliance on Image Data:} Models such as Garner \citeNew{Garner}, USPM \citeNew{USPM}, Tile2Vec \citeNew{Tile2Vec}, RegionEncoder \citeNew{RegionEncoder}, Urban2Vec \citeNew{urban2Vec}, M3G \citeNew{M3G}, UrbanCLIP \citeNew{UrbanCLIP}, and UrbanVLP \citeNew{UrbanVLP} integrate image data into their pretraining process to improve entity representations. While this can be effective, the reliance on geospatial imagery complicates deployment in regions without high-quality image coverage or where privacy concerns limit access to such data.
    \item {\em Reliance on Text Data:} Models like SpaBERT \citeNew{SpaBERT}, MGeo \citeNew{MGeo}, and ERNIE-GeoL \citeNew{ERNIEGeoL} enhance map representations using text-based information, including user reviews, entity descriptions, and search queries. However, obtaining such data is non-trivial, may require private data access, or is inconsistent across platforms, making these models difficult to generalize in many practical applications.
\end{itemize}
Given these constraints, models that depend heavily on image or text data were excluded from our taxonomy to ensure a more broadly applicable categorization of MapRL methods.



\vspace{0.3cm}

\subsection{Comment 1.2 and Response 1.2} \label{com:12}
%%%%%%%%%%%%% Comment 1.2
\commenttitle{Comment 1.2 (W2 \& R3)}

{\em (W2).} Inconsistencies in Taxonomy Claims: The classification in Table 1 appears inconsistent with the stated taxonomy based on points, graphs, and sequences, creating ambiguity in how the models are categorized.
\vspace{4pt}

\noindent
{\em (R3).} Align Table 1 with the proposed taxonomy.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your insightful comment. We apologize for the confusion caused by the presentation of our work. In response, we have added a new column, "Taxonomy Category," to indicate the category each model belongs to. The specific revision is as follows:

\begin{table*}[ht]
  \centering
  \vspace{-0.3cm}
  \caption{\updateo{Revision of Table 1 by adding "Taxonomy Category"}}
  \vspace{-0.3cm}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|r|c|ccc|ccc|cccc|ccc|ccc|rcr|cc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}[4]{*}{Method}} & \updateo{Taxonomy} & \multicolumn{3}{c|}{Encoders} & \multicolumn{10}{c|}{Pretraining Tasks}                                       & \multicolumn{3}{c|}{Map Entity} & \multicolumn{3}{c|}{Features} & \multicolumn{2}{c}{Aux. Data} \\
\cline{4-24}    \multicolumn{2}{c|}{} & \updateo{Category}  & Token & Graph & Seq   & TokRI & TRCL  & AToCL & NFI   & GAu   & NCL   & AGCL  & TrajP & MTR   & ATrCL & POI   & RS    & LP    & \multicolumn{1}{c}{Sem} & \multicolumn{1}{c}{Spa} & \multicolumn{1}{c|}{Temp} & Traj  & Rel \\
    \midrule
    \multirow{13}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Point of Interest}}} 
    & CWAP~\citeNew{CWAP}  & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & CAPE~\citeNew{CAPE}  & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{r}{} &       & CIT   &  \\
    & MT-POI~\citeNew{MT-POI} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       &       & GR \\
    & Place2V~\citeNew{Place2Vec} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       &       & GR \\
    & Semant~\citeNew{semantic} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       &       & GR \\
    & CatEM~\citeNew{CatEM} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{l}{\checkmark} &       & CIT   &  \\
    & SkipG*~\citeNew{Word2Vec} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} &       & CIT   &  \\
    & Tale*~\citeNew{TALE} & \textcolor{blue}{Token-based} & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & Teaser*~\citeNew{Teaser} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   & GR \\
    & Hier*~\citeNew{Hier1} & \textcolor{blue}{Seq.-based} & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       &       &       & \checkmark     &       & CIT   & GR \\
    & P2Vec*~\citeNew{POI2VEC} & \textcolor{blue}{Token-based} & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       &       & \checkmark     &       & CIT   & GR \\
    & CACSR*~\citeNew{CACSR} & \textcolor{blue}{Seq.-based} & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       &       &       & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    & CTLE*~\citeNew{CTLE} & \textcolor{blue}{Seq.-based} & \checkmark     &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CIT   &  \\
    \midrule
    \multirow{11}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Road Segment}}} 
    & DyToast~\citeNew{DyToast} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       & \checkmark     &       & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{l}{\checkmark} &       & CDT   & GR \\
    & R2Vec~\citeNew{R2Vec} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       &       & GR \\
    & TrajRNE~\citeNew{TrajRNE} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{r}{} &       & CDT   & GR/SR \\
    & JGRM~\citeNew{JGRM} & \textcolor{blue}{Seq.-based} & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & RN2Vec*~\citeNew{RN2Vec} & \textcolor{blue}{Token-based} & \checkmark     &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & HRNR*~\citeNew{HRNR} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & SARN*~\citeNew{SARN} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & Toast*~\citeNew{Toast} & \textcolor{blue}{Seq.-based} & \checkmark     &       & \checkmark     &       & \checkmark     &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & HRoad*~\citeNew{HyperRoad} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & START*~\citeNew{START} & \textcolor{blue}{Seq.-based} & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       &       &       & \checkmark     & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    & JCLRNT*~\citeNew{JCLRNT} & \textcolor{blue}{Seq.-based} & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       & \checkmark     &       &       & \checkmark     &       & \checkmark     &       & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} & CDT   & GR \\
    \midrule
    \multirow{15}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Land Parcel}}} 
    & CGAL~\citeNew{CGAL}  & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & DLCL~\citeNew{DLCL}  & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & HUGAT~\citeNew{HUGAT} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    & Re2Vec~\citeNew{Region2Vec} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & ReCP~\citeNew{ReCP}  & \textcolor{blue}{Token-based} & \checkmark     &       &       &  \checkmark & \checkmark     & \checkmark  &      &       &       &       &       &       &   & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & SR \\
    & HGI~\citeNew{HGI}  & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & ReDCL~\citeNew{RegionDCL} & \textcolor{blue}{Token-based} & \checkmark     &       &       & \checkmark     & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR \\
    & HAFus~\citeNew{HAFusion} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & GR/SR \\
    & ZEMob*~\citeNew{ZEMob} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{\checkmark} &       & SR \\
    & GMEL*~\citeNew{GMEL} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    & MGFN*~\citeNew{MGFN} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     &       &       & SR \\
    & HDGE*~\citeNew{HDGE} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       & \checkmark     &       &       &       &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c|}{\checkmark} &       & GR/SR \\
    & MVURE*~\citeNew{MVURE} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     &       &       &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & SR \\
    & ReMVC*~\citeNew{REMVC} & \textcolor{blue}{Token-based} & \checkmark     &       &       &       &       & \checkmark     &       &       &       &       &       &       &       & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} & \checkmark     &       &       & SR \\
    & HREP*~\citeNew{HREP} & \textcolor{blue}{Graph-based} & \checkmark     & \checkmark     &       &       &       &       &       & \checkmark     & \checkmark     &       &       &       &       & \checkmark     &       & \checkmark     &       & \checkmark     &       &       & GR/SR \\
    \bottomrule
    \end{tabular}%
        }
  \label{tab:commodels}%
    \vspace{-0.4cm}
\end{table*}%


\newpage


\vspace{0.3cm}

%%%%%%%%%%%%% Comment 1.3
\subsection{Comment 1.3 and Response 1.3} \label{com:13}
\commenttitle{Comment 1.3 (W3 \& R2)}

{\em (W3).} Introduction of a New Data Format: The paper proposes a new atomic data format, which adds yet another standard to the field instead of leveraging an existing one, potentially complicating interoperability and adoption.
\vspace{4pt}

\noindent
{\em (R2)} Adopt Standard Data Formats: Use an established standard data format instead of introducing a new one to enhance compatibility, reduce complexity, and encourage adoption.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your valuable feedback. As suggested, we have enhanced VecCity by introducing a new interface that enables users to organize input data in standard formats. However, standard datasets may pose several challenges, such as missing values and inconsistent Coordinate Reference Systems (CRS), which can lead to execution errors. To ensure seamless integration with VecCity, we impose the following constraints:
\begin{itemize} [leftmargin=*]
    \item {\em Consistent CRS:} All input files must share the same CRS (e.g., "EPSG:4326"). 
    \item {\em No Missing Values:} Attribute fields should be complete to ensure data integrity. 
    \item {\em Unified Data Schema:} A standardized schema is required to ensure feature alignment and enable cross-file indexing. 
\end{itemize} 
More details about these constraints can be found in our GitHub repository.

At the same time, we have retained the atomic file format, as it provides a consistent and structured approach for integrating diverse datasets. This significantly reduces the complexity of preprocessing while optimizing computational efficiency. 

% \textbf{More details are as follows:} In the following sections, we first present the motivation for retaining the Atomic File Format, and then provide a detailed illustration of the solution for incorporating standard data formats in VecCity.

% \paratitle{Motivation for Retaining Atomic File Format.} MapRL models rely on diverse data types, including map entity attributes, entity relation networks, and auxiliary data (e.g., trajectories and OD flows). However, these data are often collected from different platforms and stored in heterogeneous formats, increasing preprocessing complexity. For example, in the New York (NY) dataset:
% \begin{itemize}[leftmargin=*]
%     \item POIs are collected from the Foursquare dataset in .txt format.
%     \item Road Segments are sourced from OpenStreetMap in .shp format.
%     \item Land Parcels are obtained from NYC.gov in .shp format.
%     \item Check-in Trajectories are from Foursquare in .txt format.
%     \item OD flow data is provided by NYC.gov in .parquet or .csv formats.
% \end{itemize}
% Instead of requiring users to manually process these diverse inputs, we propose an atomic data format that:
% \begin{itemize}[leftmargin=*]
%     \item Provides a {\em consistent, structured format} across different data sources.
%     \item {\em Automates spatial alignment} by handling Coordinate Reference System (CRS) inconsistencies.
%     \item {\em Handles missing data} through filtering and completion.
%     \item {\em Optimizes computational efficiency} by reducing file parsing overhead.
% \end{itemize}
% By unifying these datasets into atomic files, VecCity streamlines the data-loading process and significantly reduces user burden.

% \paratitle{Solutions for Incorporating Standard Data Formats.} 
% We acknowledge the importance of standard data formats in ensuring interoperability. However, existing standard formats pose several challenges that hinder seamless dataset integration:
% \begin{itemize}[leftmargin=*]
%     \item {\em Inconsistent CRS:} Different datasets may adopt different CRS settings, requiring additional preprocessing steps for alignment. This inconsistency complicates the direct integration of multiple datasets.
%     \item {\em Non-unified Data Structures:} Due to the complexity of map data, standard formats often lack a consistent data structure across datasets. This increases the learning curve for users and complicates data utilization.
% \end{itemize}
% In response to these challenges, we have made the following constrains to ensure that users can easily work with standard data formats while maintaining compatibility with VecCity: 
% \begin{itemize} [leftmargin=*]
%     \item {\em Consistent CRS:} All input files must share the same Coordinate Reference System (CRS). 
%     \item {\em No Missing Values:} Attribute fields should be complete to ensure data integrity. 
%     \item {\em Unified Data Schema:} A standardized schema is required to ensure feature alignment and enable cross-file indexing. 
% \end{itemize} 
% More details about the constraints can be found in our GitHub repository. To assist users, we also provide Python conversion scripts to transform Shapefiles, GeoJSON, and CSV data into atomic files. These changes allow VecCity to remain flexible and interoperable, ensuring that users can integrate it into their existing workflows without being limited to the atomic format. All updates are available in the GitHub repository.

\vspace{0.3cm}

\subsection{Comment 1.4 and Response 1.4} \label{com:14}
\commenttitle{Comment 1.4 (R4)}

{\em (R4).} Discuss the distinctions between vector and raster data models and their implications on the benchmarking process, ensuring clarity and relevance to MapRL tasks.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for the insightful feedback. As suggested, we clarify the relations between raster data models and MapRL tasks, which predominantly focus on vector data. We have incorporated a discussion in the Related Work section to clarify the distinction between the raster and vector data models and their respective implications for benchmarking. The specific revisions are as follows:
\begin{cmt} [Revision of "Discuss the distinctions between vector and raster data models and their implications on the benchmarking process" in paper's related work section.]
    Raster and vector data models are the two primary formats for electronic maps. The raster model structures spatial information through grids, which are commonly used in remote sensing and environmental analysis. In contrast, the vector model represents map entities as points, polylines, and polygons, leveraging graph structures to represent relations between entities. These structural differences lead to different modeling approaches: CNNs are usually used for raster-based learning, while GNNs better capture spatial relations in vector data. As a result, raster and vector models have distinct benchmarks. Due to its high precision and accuracy, the vector data model serves as the fundamental representation for electronic maps.
\end{cmt}
%Moreover, we also revised our introduction to clarify the relationship.
% \begin{cmt} [Revision of "clarify the relations between raster data models and MapRL tasks" in paper's introduction.]
%     Geospatial information systems (GIS) implement electronic maps through two foundational data models: raster and vector. While raster models excel at encoding continuous phenomena like elevation, vector maps uniquely preserve structured semantics. These explicit spatial relationships are indispensable for MapRL tasks in intelligent transportation systems (ITS), where a routing agent must reason over connectivity constraints rather than pixel proximity.
% \end{cmt}


\begin{table}[h]
\centering
\caption{Comparison between raster and vector Data}
    \begin{tabular}{l|c|c}
        \toprule
        \textbf{Attribute} & \textbf{Raster Data} & \textbf{Vector Data} \\
        \midrule
        \textbf{Spatial Structure} & Regular grid, fixed-size cells & Polygons with irregular boundaries \\
        \textbf{Data Representation} & Pixel values or numerical fields & Points, lines, and polygons \\
        \textbf{Storage Formats} & GeoTIFF, HDF5 & Shapefile, GeoJSON \\
        \textbf{Common Applications} & Remote sensing, environmental monitoring & Land-use mapping, city planning \\
        \bottomrule
    \end{tabular}
    \label{tab:rasterandvector}
\end{table}
\textbf{More Details:} Due to space constraints, we only provide a brief discussion about the distinctions between vector and raster data models. In the following section, we provide more detailed illustrations.

\paratitle{Difference Between Raster and Vector Data.}
In geographic information systems (GIS), map data is generally represented in two primary formats: vector and raster data. Here, we compare the key differences between them:
\begin{itemize}[leftmargin=*]
    \item Vector Data: Represent geographical features using {\em points, polylines, and polygons, preserving precise geometry within a specific Coordinate Reference System (CRS)}. They are commonly used to model discrete map entities such as POIs, road segments, and land parcels.
    \item Raster Data: Represent maps as {\em grids of equally sized cells, with each cell holding a value corresponding to spatial properties (e.g., elevation, temperature).} Raster data are widely used for continuous spatial information, such as satellite imagery and environmental modeling.
\end{itemize}
The fundamental difference between raster and vector data lies in their spatial structure and intended use cases, as shown in \tab~\ref{tab:rasterandvector}


\paratitle{Modeling Approaches for Raster and Vector Data.} The distinction in spatial structure leads to differences in modeling approaches:
\begin{itemize}[leftmargin=*]
    \item Vector Data: Relationships are modeled using \textbf{graph structures}, where entities are interconnected via edges. Graph Neural Networks (GNNs) effectively capture these structured relationships.
    \item Raster Data: Spatial relationships are inferred through \textbf{grid-cell proximity}, similar to image processing. Convolutional Neural Networks (CNNs) are commonly used to extract features from raster data.
\end{itemize}
When modeling, the vector data model needs to select an appropriate entity type (e.g., POIs, road segments, land parcels) to ensure meaningful representation. In contrast, raster data requires selecting an appropriate scale to balance spatial resolution and computational efficiency, as finer scales capture more details but increase storage and processing costs.
% \paratitle{Applications.} Vector and raster data models exhibit distinct strengths and are applied to different types of tasks based on their characteristics.
% \begin{itemize}[leftmargin=*]
%     \item Vector Data: Widely applied in tasks such as navigation and recommendation systems, which focus on pathfinding, proximity queries, and user location-based services. These tasks benefit from the fine-grained, object-level information that vector data provide.
%     \item Commonly used in applications like land-use classification, population density estimation, and environmental monitoring, which leverage raster data's dense and continuous spatial coverage.
% \end{itemize}

\paratitle{Impact on Benchmarking.} Differences in data structure and representation influence the design of benchmarking practices. The specific differences are as follows:
\begin{itemize}[leftmargin=*]
    \item Datasets: Vector data often use datasets like Foursquare, trajectory datasets, and road network datasets; Raster data typically rely on datasets such as remote sensing imagery, weather datasets, and terrain datasets.
    \item Baseline Models: Raster-based and vector-based models adopt different baseline models due to their distinct data structures. %Raster data models commonly utilize CNNs to encode spatial relationships. For example, BFLG~\citeNew{BFLG} encodes raster data using CNN-based networks. Vector data models rely on GNNs for encoding spatial relationships, such as the START model introduced in our paper.
\end{itemize}

\begin{table}[h]
    \centering
    \caption{Comparison of task types between vector and raster Data}
    \begin{tabular}{l|l|l}
        \toprule
        \textbf{Task Type} & \textbf{Raster-based Examples}  & \textbf{Vector-based Examples} \\
        \midrule
        \textbf{Classification} & Satellite image classification for land cover mapping & Land-use classification using POI distributions  \\
        \textbf{Regression} & Forecasting air pollution and temperature changes & Predicting POI visit counts and ETA estimations  \\
        \textbf{Prediction} & Predicting future population density or weather variations & Predicting user trajectories or next POI visits  \\
        \bottomrule
    \end{tabular}
    \label{tab:vector_raster_tasks}
\end{table}
Even though raster and vector data have differences in datasets and models, their benchmarking tasks share fundamental similarities: All tasks involve entity embeddings, but the primary distinction lies in \emph{how labels are assigned}:
\begin{itemize}[leftmargin=*]
    \item Vector data labels describe discrete objects (e.g., POI type, road connectivity).
    \item Raster data labels describe grid cell values (e.g., pixel classification, environmental variables).
\end{itemize}

% \paratitle{Integrating Vector Data with Raster Data.}
% Although VecCity currently focuses on vector data models, recent studies have demonstrated the potential of raster data in MapRL:
% \begin{itemize}[leftmargin=*]% 需要检查
%     \item \textbf{UrbanCLIP~\citeNew{urban2Vec}}: Integrates raster-based features to enhance the land pracel representation learning.
%     \item \textbf{RoadTagger~\citeNew{roadtagger}}: An end-to-end architecture that combines both satellite imagery and the spatial correlation of road segments to learn road segment representations.
% \end{itemize}
% To further explore the role of raster data in MapRL, we plan to extend VecCity by: (1) incorporating MapRL methods with raster data or hyper data and (2) expanding the VecCity library to include raster-based MapRL models for multi-modal representation learning.

% \paratitle{Revisions Made.}
% \begin{cmt}
% [TODO] Adding a new subsection in Related Work to introduce the evolution of MapRL methods.
% \end{cmt}




\vspace{0.3cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 2
\newpage
\section{Response to Reviewer \#2} 

%%%%%%%%%%%% Comment 2.1'
\subsection{Comment 2.1 and Response 2.1} \label{com:21}
\commenttitle{Comment 2.1 (W1 \& D1)}

{\em (W1).} The experimental insights could be deeper.
\vspace{4pt}

\noindent
{\em (D1).} The final experimental insights, while certainly good, seem a bit too intuitive to me. It feels natural that diverse pre-training tasks, suitable pre-training tasks, and well-crafted encoders should boost the performance. While it is certainly important to valide seemingly intuitive ideas (as we all know, intuitions can often be misguided), I can't help wonder if deeper insights can be made from the experiments. For instance, concerning the diversity of the pre-training tasks, can we summarize what SPECIFIC combinations of heterogeneous pre-training tasks can yield the best gains on what SPECIFIC types of datasets and in what SPECIFIC downstream tasks? Surely, it is impossible for any one method to emcompass all the possible pre-training tasks, and future researchers can certainly benefict a lot from a general guideline on what pre-training tasks to prioritize when the maximum number of pre-training tasks are limited. And I don't think the answer of this Comment is very far away, as the authors already observed that there are certain pre-training tasks that are more suitable to certain tasks. The answer to this qustion would simply be an extension to the authors' existing observation.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your valuable comments. Your feedback provides meaningful insights and offers important direction for improving our work. However, conducting a comprehensive exploration of the optimal combinations of pretraining tasks across different datasets and downstream tasks through experiments is highly complex and computationally intensive.

Taking the POI MapRL as an example, there are 3 categories of methods for token-based pretraining tasks, 4 for graph-based pretraining tasks, and 3 for sequence-based pretraining tasks (disregarding variations within each category due to different implementations). Moreover, our paper demonstrates the performance of the relevant model across 5 datasets and 3 downstream tasks. Therefore, fully exploring all possible combinations would require $5 \times 3 \times 3 \times 4 \times 3 = 640$ experiments. Additionally, if similar experiments were conducted for each entity, this number would need to be tripled.

We believe that exploring all possible combinations to find an optimal solution represents an impractical and unattainable workload. Therefore, introducing principles or theoretical frameworks to guide the selection of promising combinations and conducting targeted experiments would be a more feasible and effective approach. However, research in this area remains an open problem and represents an important direction for future exploration.

For these reasons, we present a simplified version of the experiments in our paper by selecting a subset of the overall possible combinations. At the same time, we comprehensively tested these combinations across five datasets, running each scenario with five different random seeds to introduce variability. The specific revisions have been presented in our paper's \underline{\updateo{\hyperref[sec:pretraintask]{Section 5}}}:
% \begin{cmt} [Revision of "Delving into Pretraining Tasks" in paper's Section 5.]
% In our experimental analysis in Section.\ref{sec:experiment}, we conclude that utilizing multiple pretraining tasks can enhance the performance of MapRL models. Moreover, greater task heterogeneity—incorporating token-based, graph-based, and sequence-based pretraining tasks—can further improve model capability. To fully inveterate the influence of task heterogeneity on performance, we conduct deep dive experiments to figure out what specific combinations of heterogeneous pretraining tasks can yield the best gains on MapRL.

% \paratitle{Experimental Space.} In this section, we aim to identify the best pretraining task combinations for MapRL. The candidate combination set is constructed by combining different categories of pretraining tasks. For POI entities, we consider token-based pretraining tasks (TokRI, TRCL) and sequence-based pretraining tasks (TrajP, MTR, ATrCL), forming combinations such as TokRI+TrajP, TRCL+MTR, \etc. Similarly, for road segments and land parcels, candidate sets are formed by combining token-, graph-, and sequence-based pretraining tasks (if applicable), as shown in Table~\ref{tab:pretraining_tasks}.

% The candidate set is constructed based on three rules: (1) selecting pretraining tasks implemented and validated by existing models; (2) using available datasets for testing; and (3) repeating all experiments five times with different random seeds. To ensure experimental feasibility, we further narrow the experimental scope by selecting only one pretraining task from each category for candidate combinations. The candidate set for other entity types follows the same principle.

% \paratitle{Model Architecture.} To eliminate the influence of model architecture on the final results, we use the same encoder within each type of MapRL model and include only the necessary encoding components. Specifically, token-based encoders map entity IDs to embeddings. Additionally, the token encoder for POI incorporates spatial features by transforming coordinates into a vector using an MLP, while the token encoder for land parcel integrates semantic features in a similar way. Graph-based encoders use GCNs to process relation networks. For land parcels, the relation network defines edges using POI similarity, spatial distance, and human mobility transitions, following HREP~\cite{HREP}. Sequence-based encoders leverage Transformer layers to encode sequential auxiliary data.

% The model is configured with a learning rate of 1e-3, embedding dimension of 128, hidden dimension of 256, and maximum sequence lengths of 32 for POI inputs and 128 for segments. Training follows a 6:2:2 train-validation-test split, with a maximum of 50,000 training steps and early stopping enabled. Encoders are arranged in the order: Token → Graph → Sequence.

% \paratitle{Experimental Result.} 
% To ensure a focused discussion, we highlight the top three pretraining task combinations for each entity type, ranked by their average performance across tasks and datasets. The results are shown in \fig~\ref{fig:pretraintask}, where each subfigure corresponds to a specific downstream task or dataset. The horizontal axis represents rankings (lower is better), while the vertical axis lists the top three combinations, with lighter colors indicating lower ranks. In \fig~\ref{fig:pretraintask}(a) for POI entities, the first three subfigures show each model’s average ranking in a specific downstream task (POIC, NPP, or TUL) across multiple datasets. We refer to these as {\em task-oriented rankings}. In contrast, the last five subfigures show each model’s average ranking across all tasks within a specific dataset (NY, TYO, CHI, SIN, or SF), which we refer to as {\em dataset-oriented rankings}. The same ranking logic applies to \fig~\ref{fig:pretraintask}(b) for road segments and \fig~\ref{fig:pretraintask}(c) for parcels. 
% Based on the results, we have several key findings:

% 1) {\em Optimal Combinations for POI:}
% TokRI + MTR consistently ranks highest, likely due to its ability to model POI categories and sequence dependencies—two key attributes for POIs. However, in SF, where data sparsity is more pronounced, TokRI + TrajP emerges as a more suitable alternative, as TrajP focuses on local sequential patterns, making it more reliable in sparse data scenarios.

% 2) {\em Optimal Combinations for Road Segment:}
% AGCL outperforms others in all scenarios, as it effectively captures important spatial dependencies in geographic relation networks, which is critical for modeling road segments. From a dataset-oriented perspective, AGCL + MTR achieves the best results in CD and PRT, where visit frequencies are higher (CD: 1551, PRT: 2430), allowing MTR to learn sequential dependencies from dense trajectory data. In contrast, AGCL + TrajP works better in BJ and SF, where visit frequencies are lower (BJ: 856, SF: 771). This suggests that MTR benefits more from dense data, while TrajP is better suited for sparse data.


% 3) {\em Optimal Combinations for Land Parcel:}
% AToCL achieves the best performance in 5/8 cases, likely because its augmentation technique enhances the model’s ability to capture key semantic features while filtering out noise. This is especially important for land parcels, where POI category distributions define functional attributes. GAu and NFI are also well-suited for land parcels, as they better model similarity-driven connectivity in social relation networks.

% By integrating these insights, we provide a general guide for selecting pretraining tasks across different entity types:

% 1) {\em Token-based}: Encoding semantic features is a key capability of token-based encoders. TokRI is well-suited for structured categorical attributes, while AToCL’s augmentation-based contrastive learning better handles high-dimensional and redundant semantic features, making it particularly effective for land parcels.

% 2) {\em Graph-based}: AGCL is well-suited for geographic relation networks, as it effectively captures key spatial dependencies. In contrast, GAu and NFI perform better in social relation networks due to their ability to model similarity-driven connectivity.

% 3) {\em Sequence-based}: MTR excels at capturing sequential dependencies, making it the best choice for sequence-based tasks, but it requires dense data to be effective. In contrast, TrajP is more reliable in sparse data scenarios.
    
% \end{cmt}

\textbf{Further Details:} Due to space constraints, our paper includes only key details of this experiment. The following section provides a comprehensive description of the model architecture and full results, extending beyond the top three combinations presented in the paper. Additionally, all detailed information will be available in our technical report on GitHub.

% \paratitle{Experimental Space.} In this experiment, we aim to identify the best pretraining task combinations for MapRL. The candidate combination set is constructed by combining different categories of pretraining tasks. For POI entities, we consider token-based pretraining tasks (TokRI, TRCL) and sequence-based pretraining tasks (TrajP, MTR, ATrCL), forming combinations such as TokRI+TrajP and TRCL+MTR. Similarly, for road segment and land parcel entities, candidate sets are formed by combining token-based, graph-based, and sequence-based pretraining tasks (if applicable), as shown in Table~\ref{tab:com_pretraining_tasks}.

% \begin{table}[ht]
%     \vspace{-2mm}
%     \caption{Overview of Pretraining Tasks, Datasets, and Seeds by Entity Types.}
%     \centering
%     % \renewcommand{\arraystretch}{1.5} % Adjust row height
%     \resizebox{0.8\textwidth}{!}{
%         \setlength{\tabcolsep}{8pt}       % Adjust column spacing
%         \begin{tabular}{c|c|c|c|c|c}
%             \toprule
%             \textbf{Entity Type} & \textbf{Token-based Task} & \textbf{Graph-based Task} & \textbf{Seq-based Task} & \textbf{Datasets} & \textbf{Seeds} \\ 
%             \midrule
%             POI & TokRI, TRCL & -- & TrajP, MTR, ATrCL & NY, TYO, CHI, SIN, SF & 1, 13, 31, 42, 131 \\ 
%             \hline
%             Road Segment & TokRI, TRCL & NFI, GAu, AGCL & TrajP, MTR, ATrCL & BJ, CD, XA, PRT, SF & 1, 13, 31, 42, 131 \\ 
%             \hline
%             Land Parcel & TokRI, TRCL, AToCL & NFI, GAu, NCL & -- & BJ, CD, XA, PRT, SF & 1, 13, 31, 42, 131 \\ 
%             \bottomrule
%         \end{tabular}
%     } 
%     \label{tab:com_pretraining_tasks}
% \end{table}

% \noindent The experimental space is constructed based on three rules: (1) selecting pretraining tasks implemented and validated by existing models; (2) using available datasets for testing; and (3) repeating all experiments five times with different random seeds.

% For rule (1), only pretraining tasks already implemented and validated by existing models are included, avoiding invalid task selections. For example, the complete experimental space for token-based pretraining tasks in POI MapRL includes Token Relation Inference (TokRI), Token Relation Contrastive Learning  (TRCL), and Augmented Token Contrastive Learning (AToCL). However, since existing POI MapRL models do not use AToCL, the actual experimental space includes only TokRI and TRCL for token-based pretraining tasks. To ensure experimental feasibility, we further narrow the experimental scope by selecting only one pretraining task from each category for candidate combinations. The experimental spaces for other entity types follow the same principle.

\paratitle{Model Architecture.} To eliminate the influence of model architecture on the final results, we use the same encoder within each type of model and include only the necessary encoding components. Specifically:
\begin{itemize}[leftmargin=*]
    \item {\em Token Encoder:} A simple, learnable embedding layer is used to convert entity IDs into token representations. Specifically, the token encoder for POI incorporates spatial features by transforming coordinates (latitude and longitude) into a vector using an MLP, while the land parcel encoder integrates POI feature information in a similar way.
    \item {\em Graph Encoder:} Graph Convolution Network (GCN) is employed to encode auxiliary data associated with the graph-based task. For land parcels, the relation network considers POI similarity, spatial distance, and mobility as edge weights, following the approach used in HREP~\citeNew{HREP}.
    \item {\em Sequence Encoder:} A Transformer layer is utilized to encode data corresponding to the sequence-based pretraining task.
\end{itemize}

The model parameters are configured as follows:
\begin{table*}[ht]
\centering
    \caption{Model settings.}
    \renewcommand{\arraystretch}{1} % Adjust row height for better readability
    \begin{tabular}{l|c||l|c}
    \hline
    \textbf{Parameter}               & \textbf{Value} & \textbf{Parameter}            & \textbf{Value} \\ \hline
    Learning Rate                    & 1e-3           & Embedding Dimension           & 128            \\ \hline
    Hidden Dimension                 & 256            & Max Check-in Trajectory Length       & 32             \\ \hline
    Max Coordinates Trajectory Length      & 128            & Train-Valid-Test Ratio              & 6:2:2            \\ \hline
    Number of Training Steps         & 50,000         &                               &                \\ \hline
    \end{tabular}
    \label{tab:model_parameters_dual_column}
\end{table*}

As discussed in Section~\ref{sec:taxonomy_pretraining}, the model organizes the different types of encoders in the commonly used order: Token → Graph → Sequence.

\paratitle{Static Information of the City Dataset.}
For clarity, we provide a detailed overview of the datasets in \tab\ref{tab:newdataset}. In addition to the original information, we incorporate visit frequency (Freq). Visit frequency represents the number of records associated with each map entity.

% Table generated by Excel2LaTeX from sheet 'data'
\begin{table}[htbp]
  \centering
  \caption{Pre-prepared datasets for \fullname.}
  \setlength{\tabcolsep}{0.8mm}
  \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{l|rrr|rrr|rrr|r}
    \toprule
    \multirow{2}{*}{City} & \multicolumn{1}{c}{\multirow{2}{*}{\#POI}} & \multicolumn{1}{c}{\multirow{2}{*}{\#Segment}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Parcel}} & \multicolumn{3}{c|}{Check-in Traj} & \multicolumn{3}{c|}{Coor. Traj} & \multicolumn{1}{c}{\multirow{2}{*}{\#OD}} \\
\cline{5-10}          &       &       &       & \multicolumn{1}{c}{\#Traj} & \multicolumn{1}{c}{\#User} & \multicolumn{1}{c|}{Freq} & \multicolumn{1}{c}{\#Traj} & \multicolumn{1}{c}{\#User} & \multicolumn{1}{c|}{Freq} &  \\
    \midrule
    NY    & 79,627 & 90,781 & 262   & 823,853 & 2,758 & 30    & \multicolumn{1}{c}{--}     & \multicolumn{1}{c}{--}     & \multicolumn{1}{c|}{--}     & 28,189 \\
    CHI   & 28,141 & 47,669 & 77    & 279,183 & 921   & 57    & \multicolumn{1}{c}{--}     & \multicolumn{1}{c}{--}     & \multicolumn{1}{c|}{--}     & 4,631 \\
    TYO   & 61,858 & 407,905 & 64    & 823,853 & 2,227 & 29    & \multicolumn{1}{c}{--}     & \multicolumn{1}{c}{--}     & \multicolumn{1}{c|}{--}     & \multicolumn{1}{c}{--} \\
    SIN   & 75,329 & 35,084 & 332   & 827,828 & 3,489 & 49    & 226,782 & None  & 35    & \multicolumn{1}{c}{--} \\
    PRT   & 4,521 & 11,095 & 382   & 19,402 & 126   & 9     & 695,085 & 435   & 2,430 & 324 \\
    SF    & 15,674 & 27,274 & 194   & 171,873 & 361   & 23    & 500,516 & 405   & 771   & 24,716 \\
    BJ    & 81,181 & 40,306 & 11,208 & \multicolumn{1}{c}{--}     & \multicolumn{1}{c}{--}     & \multicolumn{1}{c|}{--}     & 1,018,312 & 1,677 & 856   & 687,890 \\
    CD    & 17,301 & 6,195 & 1,306 & \multicolumn{1}{c}{--}     & \multicolumn{1}{c}{--}     & \multicolumn{1}{c|}{--}     & 559,729 & 48,295 & 1,551 & 64,482 \\
    XA    & 19,108 & 5,269 & 1,056 & \multicolumn{1}{c}{--}     & \multicolumn{1}{c}{--}     & \multicolumn{1}{c|}{--}     & 384,618 & 26,787 & 1,359 & 54,365 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:newdataset}%
\end{table}%

% \paratitle{Performance Analysis.} 
% The complete experimental results are presented in \tab\ref{tab:poi_comb} for POI, \tab\ref{tab:road_segment_comb} for road segment, and \tab\ref{tab:land_parcel_comb} for land parcel. To facilitate comparison, we also highlight the Top 3 task combinations based on the average ranking across tasks and datasets in \fig\ref{fig:comb}, where each subfigure corresponds to a specific downstream task or dataset. The horizontal axis shows the ranking (lower is better), and the vertical axis lists the top three combinations, with lighter colors indicating lower ranks. In \fig~\ref{fig:comb}(a) for POI entities, the first three subfigures show each model’s average ranking in a specific downstream task (POIC, NPP, or TUL) across multiple datasets. We refer to these as {\em task-oriented rankings}. In contrast, the last five subfigures show each model’s average ranking across all tasks within a specific dataset (NY, TYO, CHI, SIN, or SF), which we refer to as {\em dataset-oriented rankings}. The same ranking logic applies to \fig~\ref{fig:comb}(b) for road segments and \fig~\ref{fig:comb}(c) for land parcels. Based on the results, we have several key findings:

% 1) {\em Optimal Combinations for POI:}
% TokRI + MTR consistently ranks highest, likely due to its ability to model POI categories and sequence dependencies—two key attributes for POIs. However, in SF, where data sparsity is more pronounced, TokRI + TrajP emerges as a more suitable alternative, as TrajP focuses on local sequential patterns, making it more reliable in sparse data scenarios.

% 2) {\em Optimal Combinations for Road Segment:}
% AGCL outperforms others in all scenarios, as it effectively captures important spatial dependencies in geographic relation networks, which is critical for modeling road segments. From a dataset-oriented perspective, AGCL + MTR achieves the best results in CD and PRT, where visit frequencies are higher (CD: 1551, PRT: 2430), allowing MTR to learn sequential dependencies from dense trajectory data. In contrast, AGCL + TrajP works better in BJ and SF, where visit frequencies are lower (BJ: 856, SF: 771). This suggests that MTR benefits more from dense data, while TrajP is better suited for sparse data.

% 3) {\em Optimal Combinations for Land Parcel:}
% AToCL achieves the best performance in 5/8 cases, likely because its augmentation technique enhances the model’s ability to capture key semantic features while filtering out noise. This is especially important for land parcels, where POI category distributions define functional attributes. GAu and NFI are also well-suited for land parcels, as they better model similarity-driven connectivity in social relation networks.

\paratitle{Complete Performance Comparison of Pretraining Task Combinations.} The full results for POI are presented in \tab~\ref{tab:poi_comb}, while \tab~\ref{tab:road_segment_comb} and \tab~\ref{tab:land_parcel_comb} provide the corresponding results for road segments and land parcels, respectively.
\begin{table*}[ht]
  \centering
  \begin{minipage}{0.4\linewidth}
  \caption{Performance comparison of pretraining task combinations for POI across various datasets.}
      \resizebox{\linewidth}{!}{
      \setlength{\tabcolsep}{0.5mm}
       \setlength{\extrarowheight}{-1pt}
    \begin{tabular}{c|cc|ccc|ccc}
        \toprule
        \multicolumn{3}{c|}{Token-based} & \multicolumn{3}{c|}{TokRI} & \multicolumn{3}{c}{TRCL} \\
        \midrule
        \multicolumn{3}{c|}{Sequence-based} & TrajP & MTR   & ATrCL & TrajP & MTR   & ATrCL \\
        \midrule
        \multirow{6}[2]{*}{\rotatebox{90}{New York}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & \textbf{0.072} & \underline{0.072} & 0.062 & 0.055 & 0.059 & 0.057 \\
              & \multicolumn{1}{c}{} & F1↑   & \underline{0.005} & 0.003 & 0.004 & \textbf{0.006} & 0.004 & 0.004 \\
              & \multicolumn{1}{c}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & \underline{0.172} & \textbf{0.183} & 0.023 & 0.130 & 0.069 & 0.024 \\
              & \multicolumn{1}{c}{} & ACC@5↑ & \underline{0.363} & \textbf{0.392} & 0.050 & 0.275 & 0.164 & 0.060 \\
              & \multicolumn{1}{c}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & \underline{0.695} & \textbf{0.700} & 0.087 & 0.531 & 0.409 & 0.242 \\
              & \multicolumn{1}{c}{} & F1↑   & \underline{0.419} & \textbf{0.434} & 0.008 & 0.259 & 0.144 & 0.070 \\
        \midrule
        \multirow{6}[2]{*}{\rotatebox{90}{Tokyo}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & \underline{0.326} & \textbf{0.334} & 0.326 & 0.315 & 0.312 & 0.318 \\
              & \multicolumn{1}{c}{} & F1↑   & \underline{0.011} & \textbf{0.012} & 0.009 & 0.008 & 0.009 & 0.009 \\
              & \multicolumn{1}{c}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & \underline{0.187} & \textbf{0.197} & 0.059 & 0.045 & 0.060 & 0.037 \\
              & \multicolumn{1}{c}{} & ACC@5↑ & \underline{0.394} & \textbf{0.407} & 0.129 & 0.126 & 0.145 & 0.123 \\
              & \multicolumn{1}{c}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & \underline{0.501} & \textbf{0.527} & 0.040 & 0.050 & 0.155 & 0.032 \\
              & \multicolumn{1}{c}{} & F1↑  & \underline{0.281} & \textbf{0.307} & 0.006 & 0.010 & 0.049 & 0.004 \\
        \midrule
        \multirow{6}[2]{*}{\rotatebox{90}{Chicago}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & 0.233 & 0.242 & 0.218 & \textbf{0.280} & 0.251 & \underline{0.251} \\
              & \multicolumn{1}{c}{} & F1↑   & 0.068 & 0.076 & 0.068 & \textbf{0.094} & \underline{0.080} & 0.071 \\
              & \multicolumn{1}{c}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & \underline{0.181} & \textbf{0.209} & 0.031 & 0.063 & 0.122 & 0.045 \\
              & \multicolumn{1}{c}{} & ACC@5↑ & \underline{0.375} & \textbf{0.412} & 0.086 & 0.178 & 0.290 & 0.094 \\
              & \multicolumn{1}{c}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & \underline{0.734} & \textbf{0.771} & 0.170 & 0.262 & 0.588 & 0.262 \\
              & \multicolumn{1}{c}{} & F1↑   & \underline{0.543} & \textbf{0.611} & 0.013 & 0.055 & 0.346 & 0.049 \\
        \midrule
        \multirow{6}[2]{*}{\rotatebox{90}{Singapore}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & 0.126 & \textbf{0.140} & 0.126 & \underline{0.132} & 0.131 & 0.129 \\
              & \multicolumn{1}{c}{} & F1↑   & 0.003 & \textbf{0.004} & 0.003 & 0.004 & \underline{0.004} & 0.003 \\
              & \multicolumn{1}{c}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & \underline{0.113} & \textbf{0.114} & 0.011 & 0.035 & 0.046 & 0.020 \\
              & \multicolumn{1}{c}{} & ACC@5↑ & \textbf{0.254} & \underline{0.235} & 0.036 & 0.092 & 0.111 & 0.061 \\
              & \multicolumn{1}{c}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & \underline{0.454} & \textbf{0.455} & 0.016 & 0.217 & 0.264 & 0.107 \\
              & \multicolumn{1}{c}{} & F1↑   & \underline{0.215} & \textbf{0.215} & 0.000 & 0.075 & 0.099 & 0.011 \\
        \midrule
        \multirow{6}[2]{*}{\rotatebox{90}{San Francisco}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & \textbf{0.050} & 0.041 & 0.036 & \underline{0.045} & 0.041 & 0.041 \\
              & \multicolumn{1}{c}{} & F1↑   & \textbf{0.012} & 0.011 & 0.007 & \underline{0.012} & 0.007 & 0.010 \\
              & \multicolumn{1}{c}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.147 & \textbf{0.161} & \underline{0.153} & 0.119 & 0.144 & 0.042 \\
              & \multicolumn{1}{c}{} & ACC@5↑ & \textbf{0.410} & \underline{0.370} & 0.314 & 0.291 & 0.339 & 0.116 \\
              & \multicolumn{1}{c}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & \textbf{0.777} & \underline{0.760} & 0.641 & 0.571 & 0.624 & 0.212 \\
              & \multicolumn{1}{c}{} & F1↑   & \underline{0.466} & \textbf{0.525} & 0.397 & 0.314 & 0.332 & 0.013 \\
        \midrule
        \multirow{2}{*}{Overall} & \multicolumn{2}{c|}{Per Ave Rank} & \underline{2.217} & \textbf{1.600} & 5.050 & 3.700 & 3.433 & 5.000 \\
              & \multicolumn{2}{c|}{Per Rank} & 2     & 1     & 6     & 4     & 3     & 5 \\
        \bottomrule
    \end{tabular}%
    }
  \label{tab:poi_comb}
\end{minipage}\hspace{0.6cm}
\begin{minipage}{0.44\linewidth}
  \centering
  \caption{Performance comparison of pretraining task combinations for land parcel across various datasets.}
      \resizebox{\linewidth}{!}{
      \setlength{\tabcolsep}{0.3mm}
    \begin{tabular}{c|cc|ccc|ccc|ccc}
    \toprule
    \multicolumn{3}{c|}{Token-based} & \multicolumn{3}{c|}{TokRI} & \multicolumn{3}{c|}{TRCL} & \multicolumn{3}{c}{AToCL} \\
    \midrule
    \multicolumn{3}{c|}{Graph-based} & NFI   & GAu   & NCL   & NFI   & GAu   & NCL   & NFI   & GAu   & NCL \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{Beijing}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & \underline{0.528} & 0.430 & 0.376 & \textbf{0.538} & 0.480 & 0.370 & 0.464 & 0.360 & 0.366 \\
          & \multicolumn{1}{c|}{} & F1↑   & \underline{0.382} & 0.350 & 0.143 & \textbf{0.386} & 0.340 & 0.140 & 0.290 & 0.270 & 0.260 \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & \textbf{12.33} & 18.58 & 24.43 & 16.70 & 19.32 & 28.96 & \underline{13.71} & 16.51 & 25.18 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & \textbf{40.17} & 63.73 & \underline{49.95} & 78.81 & 66.27 & 53.82 & 67.49 & 66.88 & 50.45 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & \underline{0.272} & 0.340 & 0.292 & 0.394 & 0.290 & \textbf{0.257} & 0.279 & 0.284 & \textbf{0.355} \\
          & \multicolumn{1}{c|}{} & RMSE↓ & \underline{0.669} & 0.977 & 0.697 & 1.266 & 0.798 & 0.727 & \textbf{0.665} & 0.731 & 0.753 \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{Chendu}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.563 & 0.552 & 0.394 & 0.531 & \textbf{0.616} & 0.423 & \underline{0.614} & 0.567 & 0.418 \\
          & \multicolumn{1}{c|}{} & F1↑   & 0.487 & 0.445 & 0.298 & 0.417 & \textbf{0.552} & 0.272 & \underline{0.548} & 0.499 & 0.274 \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & \textbf{147.8} & 164.2 & 156.1 & 171.9 & 174.3 & \underline{155.0} & 164.7 & 158.4 & 155.4 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & \textbf{406.4} & 690.0 & 443.5 & 566.9 & 596.8 & 442.5 & 469.7 & \underline{414.9} & 443.1 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 5.9   & 24.7  & 4.2   & 27.4  & 307.3 & \underline{3.6} & 6.2   & 83.0  & \textbf{3.6} \\
          & \multicolumn{1}{c|}{} & RMSE↓ & \textbf{29} & 175   & \underline{30} & 768   & 2096  & 30    & 30    & 198   & 30 \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{Xi'an}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.625 & 0.638 & 0.476 & 0.585 & \underline{0.664} & 0.504 & 0.603 & \textbf{0.674} & 0.512 \\
          & \multicolumn{1}{c|}{} & F1↑   & 0.476 & 0.531 & 0.278 & 0.427 & \textbf{0.601} & 0.293 & 0.461 & \underline{0.565} & 0.306 \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 177.0 & 184.6 & \textbf{133.9} & 190.1 & 303.7 & \underline{133.9} & 241.8 & 148.6 & 134.3 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 964   & 941   & \textbf{327} & 1311  & 1730  & \underline{327} & 2169  & 697   & 327 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 3.4   & 494.7 & \underline{2.8} & 3.9   & 525.6 & 2.9   & 3.9   & 22.2  & \textbf{2.7} \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 18    & 2067  & \underline{18} & 22    & 3456  & \textbf{18} & 22    & 106   & 18 \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{Porto}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.357 & 0.339 & 0.257 & \textbf{0.374} & 0.357 & 0.292 & 0.357 & \underline{0.363} & 0.298 \\
          & \multicolumn{1}{c|}{} & F1↑   & 0.339 & 0.332 & 0.234 & \textbf{0.365} & 0.352 & 0.279 & 0.342 & \underline{0.353} & 0.295 \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 223.4 & \textbf{194.1} & 516.8 & 245.2 & 248.4 & 515.9 & \underline{215.2} & 217.5 & 517.3 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 283.7 & \textbf{257.5} & 589.8 & 327.5 & 377.9 & 588.5 & \underline{273.9} & 305.0 & 590.4 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 22.64 & \textbf{19.91} & 44.82 & 21.98 & 20.97 & 44.78 & 22.33 & \underline{20.82} & 44.79 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 38.44 & \underline{30.15} & 72.23 & 38.44 & 31.56 & 72.19 & 39.79 & \textbf{29.92} & 72.19 \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{San Francisco}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & \textbf{0.827} & \underline{0.826} & 0.819 & 0.816 & 0.818 & 0.820 & 0.822 & 0.823 & 0.825 \\
          & \multicolumn{1}{c|}{} & F1↑   & \textbf{0.504} & 0.479 & 0.450 & 0.454 & 0.450 & 0.452 & 0.479 & \underline{0.504} & 0.502 \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 462.0 & \underline{394.3} & 466.0 & 424.4 & 450.0 & 526.4 & \textbf{382.2} & 425.3 & 471.5 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 902   & \underline{802} & 872   & 819   & 910   & 1233  & \textbf{764} & 817   & 880 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 7.015 & \textbf{6.679} & 12.050 & 6.913 & 6.989 & 7.141 & \underline{6.714} & 6.840 & 7.061 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 22.30 & \underline{22.00} & 28.07 & 22.15 & 22.17 & 22.59 & \textbf{21.86} & 22.05 & 22.53 \\
    \midrule
    \multirow{2}{*}{Overall} & \multicolumn{2}{c|}{Per Ave Rank} & \textbf{3.677} & 4.452 & 5.935 & 5.161 & 5.355 & 5.871 & 4.097 & \underline{3.968} & 5.548 \\
          & \multicolumn{2}{c|}{Per Rank} & \textbf{1} & 4     & 9     & 5     & 6     & 8     & 3     & \underline{2} & 7 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:land_parcel_comb}
  \end{minipage}
\end{table*}


\begin{table*}[ht]
  \centering
  \caption{Performance comparison of pretraining task combinations for segment across various datasets.}
      \resizebox{0.85\linewidth}{!}{
      \setlength{\tabcolsep}{0.5mm}
     \setlength{\extrarowheight}{-1pt}
            \begin{tabular}{c|cc|ccc|ccc|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{3}{c|}{Token-based} & \multicolumn{9}{c|}{TokRI}                                            & \multicolumn{9}{c}{TRCL} \\
\cmidrule{1-21}    \multicolumn{3}{c|}{Graph-based} & \multicolumn{3}{c|}{NFI} & \multicolumn{3}{c|}{GAu} & \multicolumn{3}{c|}{AGCL} & \multicolumn{3}{c|}{NFI} & \multicolumn{3}{c|}{GAu} & \multicolumn{3}{c}{AGCL} \\
\cmidrule{1-21}    \multicolumn{3}{c|}{Sequence-based} & TrajP & MTR   & ATrCL & TrajP & MTR   & ATrCL & TrajP & MTR   & ATrCL & TrajP & MTR   & ATrCL & TrajP & MTR   & ATrCL & TrajP & MTR   & ATrCL \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{Beijing}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 2.809 & 2.787 & 2.831 & 2.819 & 2.816 & 2.816 & 2.823 & 2.816 & 2.817 & 2.803 & 2.791 & \textbf{2.089} & 2.809 & 2.811 & 2.810 & \underline{2.310} & 2.771 & 2.790 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 5.483 & 5.461 & 5.489 & 5.492 & 5.485 & 5.485 & 5.487 & 5.485 & 5.489 & 5.475 & 5.464 & \textbf{4.731} & 5.487 & 5.486 & 5.487 & \underline{4.984} & 5.460 & 5.474 \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 609.1 & 636.2 & 644.5 & 634.8 & 598.1 & 608.6 & 577.9 & \textbf{511.4} & 578.2 & 692.7 & 776.7 & 542.6 & 575.1 & 613.8 & 594.4 & \underline{514.0} & 616.8 & 595.9 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 2592  & 2660  & 2597  & 2646  & 2587  & 2615  & 2493  & 2390  & 2518  & 2668  & 2722  & \textbf{2025} & 2591  & 2553  & 2572  & \underline{2214} & 2657  & 2624 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.961 & 0.944 & 0.531 & 0.269 & 0.356 & 0.783 & 0.912 & 0.361 & 0.808 & 0.949 & 0.977 & 0.793 & 0.957 & \textbf{0.980} & 0.702 & 0.915 & \underline{0.978} & 0.821 \\
          & \multicolumn{1}{c|}{} & MR↓   & 7.06  & 5.50  & 28.33 & 30.27 & 18.98 & 10.54 & 12.42 & 19.93 & 9.42  & 9.71  & \textbf{5.18} & 11.28 & 9.27  & \underline{5.34} & 13.87 & 10.10 & 5.50  & 9.12 \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{Chendu}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 6.304 & 6.215 & 6.152 & 6.049 & 6.041 & \underline{5.999} & 6.087 & \textbf{5.964} & 6.009 & 6.283 & 6.222 & 6.207 & 6.092 & 6.060 & 6.001 & 6.193 & 6.121 & 6.019 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 13.62 & 13.53 & 13.53 & 13.45 & 13.44 & 13.40 & 13.49 & \textbf{13.38} & 13.41 & 13.51 & 13.47 & 13.53 & 13.48 & 13.47 & \underline{13.40} & 13.49 & 13.41 & 13.43 \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 91.70 & \textbf{88.05} & 116.14 & 91.50 & 92.78 & 115.41 & \underline{88.73} & 91.98 & 93.62 & 89.73 & 88.91 & 148.14 & 89.75 & 92.09 & 90.93 & 90.13 & 90.27 & 99.14 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 143.1 & \textbf{141.1} & 168.7 & 144.6 & 147.0 & 168.4 & \underline{141.6} & 143.2 & 146.1 & 143.6 & 141.7 & 196.5 & 142.0 & 145.0 & 144.8 & 142.0 & 143.5 & 149.2 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.735 & 0.643 & 0.315 & 0.231 & 0.654 & 0.743 & \textbf{0.903} & 0.668 & 0.570 & 0.717 & 0.677 & 0.719 & 0.730 & 0.751 & 0.872 & 0.707 & 0.679 & \underline{0.873} \\
          & \multicolumn{1}{c|}{} & MR↓   & 15.40 & 14.68 & 35.58 & 67.72 & 11.75 & 11.26 & 10.62 & 14.94 & 14.77 & 14.07 & 14.53 & 12.21 & 15.33 & 13.07 & \textbf{9.98} & 13.87 & 13.59 & \underline{10.04} \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{Xi'an}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 5.616 & 5.576 & 5.546 & 5.463 & 5.405 & 5.404 & 5.410 & 5.434 & \textbf{5.374} & 5.652 & 5.587 & 5.639 & 5.379 & 5.468 & \underline{5.378} & 5.411 & 5.438 & 5.410 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 11.04 & 11.02 & 11.05 & 10.95 & 10.94 & 10.94 & 10.92 & 10.93 & \textbf{10.87} & 11.01 & 10.99 & 11.05 & 10.91 & 11.01 & 10.90 & 10.95 & 10.90 & \underline{10.90} \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & \textbf{117.1} & 119.6 & 202.7 & 119.5 & 189.8 & 128.1 & \underline{118.7} & 118.9 & 139.6 & 119.7 & 120.7 & 184.0 & 123.2 & 123.4 & 127.4 & 119.1 & 118.8 & 146.7 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 186.1 & 189.3 & 267.4 & 188.0 & 263.4 & 192.4 & \underline{186.1} & 188.7 & 208.6 & 187.4 & 188.5 & 250.5 & 192.2 & 191.2 & 197.3 & \textbf{185.7} & 188.3 & 215.4 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.776 & 0.714 & 0.349 & \underline{0.879} & 0.657 & 0.590 & \textbf{0.909} & 0.759 & 0.513 & 0.876 & 0.782 & 0.294 & 0.795 & 0.689 & 0.313 & 0.839 & 0.673 & 0.640 \\
          & \multicolumn{1}{c|}{} & MR↓   & 8.19  & 9.17  & 30.73 & \textbf{6.40} & 7.99  & 10.33 & 7.41  & 8.49  & 12.78 & 9.31  & 7.78  & 34.13 & \underline{6.53} & 12.47 & 31.37 & 6.87  & 14.08 & 12.10 \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{Porto}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 4.307 & 4.307 & 4.287 & 4.276 & 4.288 & 4.310 & 4.266 & 4.263 & 4.269 & 4.332 & 4.320 & 4.302 & 4.294 & 4.285 & 4.276 & 4.284 & \underline{3.922} & \textbf{3.578} \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 7.855 & 7.853 & 7.837 & 7.831 & 7.835 & 7.845 & 7.822 & 7.810 & 7.820 & 7.855 & 7.855 & 7.843 & 7.834 & 7.829 & 7.824 & 7.830 & \underline{7.493} & \textbf{7.152} \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 86.76 & 87.97 & 90.44 & 87.68 & 88.19 & 87.05 & 91.95 & 86.78 & 87.23 & 86.46 & 104.44 & 96.14 & 97.00 & 91.96 & 86.92 & 87.85 & \textbf{80.67} & \underline{80.84} \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 133.1 & 133.9 & 135.1 & 134.6 & 133.4 & 133.2 & 136.2 & 132.7 & 133.6 & 133.4 & 156.7 & 144.5 & 140.1 & 136.3 & 132.5 & 132.3 & \underline{122.1} & \textbf{116.8} \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.961 & 0.913 & 0.846 & 0.943 & \textbf{0.968} & 0.323 & 0.961 & 0.956 & 0.927 & 0.928 & 0.571 & 0.833 & 0.953 & \underline{0.965} & 0.962 & 0.959 & 0.951 & 0.778 \\
          & \multicolumn{1}{c|}{} & MR↓   & 6.67  & 8.00  & 9.55  & 7.36  & 6.97  & 22.11 & 6.66  & 6.83  & 7.10  & 7.06  & 18.53 & 9.26  & 7.97  & \textbf{6.57} & 6.74  & \underline{6.62} & 6.75  & 9.08 \\
    \midrule
    \multirow{6}[2]{*}{\rotatebox{90}{San Francisco}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 2.498 & 2.491 & \textbf{2.066} & 2.477 & 2.477 & 2.486 & 2.474 & 2.476 & \underline{2.473} & 2.494 & 2.494 & 2.494 & 2.477 & 2.476 & 2.475 & 2.478 & 2.478 & 2.478 \\
          & \multicolumn{1}{c|}{} & RMSE↓ & 5.368 & 5.364 & \textbf{4.893} & 5.360 & 5.359 & 5.365 & \underline{5.353} & 5.358 & 5.356 & 5.371 & 5.370 & 5.370 & 5.358 & 5.358 & 5.357 & 5.358 & 5.358 & 5.358 \\
          & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  &  406.7 & 371.7 & \textbf{289.4} & 461.1 & \underline{310.4} & 402.5 & 345.3 & 424.9 & 442.9 & 462.0 & 399.0 & 335.9 & 495.7 & 516.9 & 448.5 & 327.4 & 406.3 & 485.2\\
          & \multicolumn{1}{c|}{} & RMSE↓ &  2638  & 2618  & \textbf{1372} & 2592  & 2617  & 2607  & 2614  & 2656  & 2648  & \underline{2592} & 2619  & 2647  & 2668  & 2665  & 2662  & 2625  & 2647  & 2669 \\
          & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.683 & 0.813 & 0.703 & 0.743 & 0.867 & 0.720 & \textbf{0.887} & 0.777 & 0.690 & 0.777 & 0.857 & 0.740 & 0.683 & 0.697 & 0.807 & 0.767 & 0.810 & \underline{0.880} \\
          & \multicolumn{1}{c|}{} & MR↓   & 9.000 & 7.500 & 9.367 & 8.200 & 7.400 & 8.600 & \textbf{5.900} & 8.367 & 8.067 & 8.900 & 7.967 & 10.167 & 9.200 & 7.833 & 7.933 & 8.233 & 7.833 & \underline{6.933} \\
    \midrule
    \multirow{2}{*}{Overall} & \multicolumn{2}{c|}{Per Ave Rank} & 10.19 & 9.90  & 13.03 & 10.52 & 9.45  & 10.61 & \textbf{6.13} & 8.06  & 9.71  & 10.39 & 10.58 & 12.19 & 9.81  & 9.23  & 8.32  & \underline{7.00} & 7.35  & 8.42 \\
          & \multicolumn{2}{c|}{Per Rank} & 12    & 11    & 18    & 14    & 8     & 16    & \textbf{1} & 4     & 9     & 13    & 15    & 17    & 10    & 7     & 5     & \underline{2} & 3     & 6 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:road_segment_comb}
\end{table*}
\FloatBarrier

% \begin{figure}
%     \centering
%     \subfigure[Top 3 combinations for POI map entity.]{\includegraphics[width=0.33\columnwidth]{figures/rebuttal/top5_rank_poi.pdf}}
%     \subfigure[Top 3 combinations for segment map entity.]{\includegraphics[width=0.33\columnwidth]{figures/rebuttal/top5_rank_road.pdf}}
%     \subfigure[Top 3 combinations for parcel map entity.]{\includegraphics[width=0.33\columnwidth]{figures/rebuttal/top5_rank_region.pdf}}
%     \vspace{-4mm}
%     \caption{Top 3 pretraining task combinations' preformance.}
%     \vspace{-4mm}
%     \label{fig:comb}
% \end{figure}

% By integrating these insights, we provide a general guide for selecting pretraining tasks across different entity types:

% 1) {\em Token-based}: Encoding semantic features is a key capability of token-based encoders. TokRI is well-suited for structured categorical attributes, while AToCL’s augmentation-based contrastive learning better handles high-dimensional and redundant semantic features, making it particularly effective for land parcels.

% 2) {\em Graph-based}: AGCL is well-suited for geographic relation networks, as it effectively captures key spatial dependencies. In contrast, GAu and NFI perform better in social relation networks due to their ability to model similarity-driven connectivity.

% 3) {\em Sequence-based}: MTR excels at capturing sequential dependencies, making it the best choice for sequence-based tasks, but it requires dense data to be effective. In contrast, TrajP is more reliable in sparse data scenarios.

\paratitle{Time Efficiency.}
In addition, we evaluate the training time efficiency of each pretraining task, with the results presented in \tab\ref{tab:compttime}. All time measurements are collected under the same computing environment as the performance experiments to ensure consistency. The convergence criterion is defined as the point where the loss approaches its minimum value and remains stable for at least 10 consecutive epochs. This criterion is applied uniformly across all pretraining tasks to ensure a fair comparison.
\begin{table}[ht]
  \centering
  \small
  \caption{Time efficiency comparison for pretraining tasks. "Conver." is short for "Convergence" .}
  \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{r|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[6]{*}{\makecell{Pretrining\\Task}} & \multicolumn{3}{c|}{POI} & \multicolumn{3}{c|}{Road Segment} & \multicolumn{3}{c|}{Land Parcel} & \multicolumn{1}{c}{\multirow{2}[6]{*}{\makecell{Relative\\Rank}}} \\
\cline{2-10}          & \multicolumn{1}{c}{\makecell{Step\\Time (ms)}} & \multicolumn{1}{c}{\makecell{Conver.\\Step}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time (min)}} & \multicolumn{1}{c}{\makecell{Step\\Time (ms)}} & \multicolumn{1}{c}{\makecell{Conver.\\Step}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time (min)}}& \multicolumn{1}{c}{\makecell{Step\\Time (ms)}} & \multicolumn{1}{c}{\makecell{Conver.\\Step}} & \multicolumn{1}{c|}{\makecell{Conver.\\Time (min)}}&  \\
    \midrule
    TokRI & 6.62 & 7367  & 1.0   & 197   & 31037 & 102   & 38    & 23840 & 15    & 2 \\
    TRCL  & 6.69 & 19100 & 2.2   & 307   & 28086 & 144   & 54    & 22387 & 20    & 3 \\
    AToCL & -     & -     & -     & -     & -     & -     & 4     & 23134 & 2     & 1 \\
    \midrule
    NFI   & -     & -     & -     & 223   & 29526 & 110   & 45    & 21192 & 16    & 2 \\
    NCL   & -     & -     & -     & -     & -     & -     & 45    & 20138 & 15    & 1 \\
    GAu   & -     & -     & -     & 264   & 32033 & 133   & 54    & 23943 & 22    & 3 \\
    AGCL  & -     & -     & -     & 289   & 28367 & 137   & -     & -     & -     & 4 \\
    \midrule
    TrajP & 18.81 & 15600 & 5.4   & 554   & 34152 & 315   & -     & -     & -     & 2 \\
    MTR   & 22.66 & 17050 & 7.2   & 1436  & 27483 & 658   & -     & -     & -     & 3 \\
    ATrCL & 25.14 & 6750  & 2.7   & 524   & 25800 & 225   & -     & -     & -     & 1 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:compttime}%
\end{table}%

From the results, we observe that AToCL, NCL, and ATrCL are the most computationally efficient pretraining tasks for token-based, graph-based, and sequence-based pre-training tasks, respectively. AToCL achieves the shortest convergence time among token-based pre-training tasks, making it the most efficient choice. For graph-based pretraining tasks, NCL converges the fastest, requiring fewer steps than NFI, which remains efficient but is slightly slower. In contrast, GAu and AGCL demand significantly more time, making them less favorable. Among sequence-based pretraining tasks, ATrCL is the most time-efficient, converging much faster than TrajP and MTR, with MTR being the slowest.





\vspace{0.3cm}


%%%%%%%%%%%%% Comment 2.2
\subsection{Comment 2.2 and Response 2.2} \label{com:22}

\commenttitle{Comment 1.2 (W2 \& R3)}

{\em (W2).} Could address the randomness in the experiments.
\vspace{4pt}

\noindent
{\em (D2).} In the experiments, it would appear that the randomness in dataset separation and model initializations is not explicitly addressed. It would be interesting to see the effect of this. In particular, which types of methods are more robust or sensitive against such randomness? This would be an interesting Comment to answer.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

We sincerely appreciate your valuable comments on the potential impact of randomness in our experiments. As suggested, we extend our experiments in paper's Section 4 by conducting experiments using multiple random seeds {1, 13, 31, 42, 131} and adding the discussion on which type of method is more robust or sensitive against the randomness. Specific revisions are presented in the paper's \underline{\updateo{\hyperref[sec:t42]{Section 4.2}}}.

% \begin{cmt}[Revision of "Address randomness for POI MapRL" in paper's Section 4.2.1.]
% 4) {\em Instability Introduced by Contrastive Learning.} SkipG, Teaser, and CACSR show significant instability due to their reliance on contrastive learning, which is sensitive to dataset partitioning and negative sample selection. In contrast, P2Vec and Tale are more stable, likely because they use token relation inference, a supervised pretraining task that enhances robustness by predicting relationships between map entities.
% \end{cmt}

% \begin{cmt}[Revision of "Address randomness for road segment MapRL" in paper's Section 4.2.2.]
% 3) {\em Fluctuating Results for SARN, Toast, START, and JCLRNT:}
% These models experience higher performance variability compared to other models, largely due to their dependence on contrastive pretraining techniques such as Token Relation Contrastive Learning (TRCL), Augmented Graph Contrastive Learning (AGCL), and Augmented Trajectory Contrastive Learning (ATrCL). These methods are particularly vulnerable to shifts in training data splits and the inherent randomness in negative sample selection, leading to inconsistent results across multiple runs.
% \end{cmt}

% \begin{cmt}[Revision of "Address randomness for land parcel MapRL" in paper's Section 4.2.3.]
% 3) {\em Fluctuating Results for MGFN}: 
% Although MGFN ranks third overall (with an average rank of 3.53), its performance varies considerably under different random seeds, indicating a degree of instability. This instability arises because MGFN relies on clustering techniques to build the base relation network for representation learning, making it more sensitive to randomness across datasets.

% 4) {\em Small Datasets Mitigate Instability in Negative Sampling}: ZEMob, GMEL, and ReMVC are among the most stable models across all datasets. Despite employing contrastive learning as pretraining tasks—which tends to be sensitive in other MapRL models—their stability may be attributed to the smaller number of parcel entities. For instance, San Francisco contains 194 parcel entities compared to 27,274 road segment entities. This smaller number of parcel entities likely results in more stable negative sampling.
% \end{cmt}

% \begin{cmt}[Revision of "Address Randomness from overall persepactive" in paper's Section 4.2.4.]
% 4) {Instable Introduced by Contrastive Learning}: Models utilizing contrastive learning pretraining tasks exhibit increased sensitivity to randomness. However, this sensitivity may diminish when dealing with smaller datasets.
% \end{cmt}


% \textbf{More Detail:} In the following section, we provide a more detail disscution for the impact of randomness. Specifically we analyze the effects of randomness by examining performance variations across different runs and identify which models and tasks are most sensitive to dataset partitioning and initialization variability, providing insights into their stability.

% %\rotatebox{90}{
% %\underline  \underline
% % ±

% \begin{table*}[htbp]
%   \centering
%   \vspace{-0.3cm}
%   \caption{Revison for Table 3 by addressing the randomness.}
% \vspace{-0.3cm}
%     % \setlength{\tabcolsep}{0.5mm}
%     \renewcommand{\arraystretch}{0.8}
%     \small
%     \setlength{\extrarowheight}{-1pt}
%   \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{ccc|ccccccc}
%         \toprule
%         \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{Task} & Metric & SkipG & Teaser & Tale  & Hier  & P2Vec & CACSR & CTLE \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{New York}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & \underline{0.073±0.001} & 0.071±0.005 & 0.063±0.006 & 0.073±0.014 & \textbf{0.082±0.007} & 0.055±0.016 & 0.055±0.005 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.006±0.004 & \underline{0.006±0.005} & 0.016±0.006 & 0.006±0.002 & \textbf{0.022±0.006} & 0.013±0.001 & 0.014±0.002 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.099±0.017 & \underline{0.097±0.021} & 0.143±0.008 & 0.115±0.003 & 0.126±0.006 & 0.141±0.049 & \textbf{0.152±0.009} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.252±0.035 & 0.254±0.046 & 0.326±0.004 & 0.293±0.005 & 0.161±0.004 & \underline{0.327±0.038} & \textbf{0.329±0.010} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.569±0.034 & \underline{0.572±0.024} & 0.674±0.003 & 0.576±0.034 & 0.635±0.007 & 0.638±0.026 & \textbf{0.694±0.004} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.260±0.033 & \underline{0.266±0.029} & 0.438±0.007 & 0.282±0.039 & 0.328±0.004 & 0.391±0.068 & \textbf{0.453±0.007} \\ 
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Tokyo}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & \underline{0.347±0.008} & 0.382±0.016 & \textbf{0.220±0.004} & 0.338±0.035 & 0.318±0.003 & 0.303±0.041 & 0.302±0.039 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.020±0.013 & \textbf{0.024±0.014} & 0.047±0.006 & 0.008±0.012 & \underline{0.042±0.003} & 0.018±0.001 & 0.017±0.003 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.161±0.004 & 0.156±0.011 & 0.156±0.007 & \textbf{0.164±0.001} & \underline{0.162±0.005} & 0.156±0.060 & 0.162±0.004 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.324±0.006 & 0.303±0.036 & 0.303±0.004 & \textbf{0.335±0.002} & \underline{0.329±0.007} & 0.326±0.015 & 0.327±0.007 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.430±0.013 & 0.436±0.017 & 0.401±0.006 & 0.440±0.031 & 0.454±0.003 & \underline{0.459±0.098} & \textbf{0.504±0.002} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.227±0.009 & 0.232±0.014 & 0.228±0.008 & 0.235±0.010 & 0.249±0.004 & \underline{0.277±0.099} & \textbf{0.289±0.004} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Chicago}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & 0.075±0.004 & 0.071±0.011 & 0.102±0.004 & 0.082±0.004 & \textbf{0.117±0.005} & \underline{0.104±0.012} & 0.102±0.017 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.006±0.001 & 0.004±0.001 & 0.017±0.005 & 0.006±0.003 & \textbf{0.024±0.008} & 0.017±0.006 & \underline{0.018±0.006} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.083±0.021 & 0.055±0.030 & 0.102±0.005 & 0.095±0.034 & 0.150±0.005 & \underline{0.154±0.053} & \textbf{0.177±0.010} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.237±0.046 & 0.179±0.078 & 0.238±0.005 & 0.263±0.060 & 0.364±0.007 & \textbf{0.399±0.036} & \underline{0.378±0.014} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.457±0.084 & 0.434±0.071 & 0.620±0.007 & 0.552±0.020 & 0.656±0.005 & \underline{0.668±0.069} & \textbf{0.764±0.011} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.198±0.068 & 0.186±0.010 & 0.366±0.005 & 0.300±0.008 & 0.423±0.007 & \underline{0.439±0.058} & \textbf{0.603±0.028} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Singapore}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & 0.094±0.039 & 0.061±0.003 & 0.037±0.006 & \underline{0.116±0.043} & 0.072±0.004 & 0.105±0.043 & \textbf{0.126±0.025} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.004±0.000 & \underline{0.009±0.005} & 0.014±0.006 & 0.002±0.002 & \textbf{0.026±0.009} & 0.007±0.002 & 0.003±0.003 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.025±0.004 & 0.028±0.003 & 0.049±0.007 & 0.050±0.017 & 0.081±0.006 & \textbf{0.108±0.044} & \underline{0.104±0.025} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.062±0.007 & 0.069±0.005 & 0.104±0.002 & 0.114±0.028 & \underline{0.177±0.006} & \textbf{0.184±0.051} & 0.136±0.051 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.257±0.057 & 0.269±0.056 & 0.309±0.006 & 0.274±0.080 & 0.396±0.008 & \underline{0.397±0.052} & \textbf{0.442±0.026} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.111±0.037 & 0.139±0.009 & 0.169±0.005 & 0.157±0.009 & 0.178±0.006 & \underline{0.181±0.066} & \textbf{0.246±0.003} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{SanFrancisco}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{POIC}} & ACC@1↑ & 0.055±0.026 & 0.061±0.014 & \underline{0.012±0.003} & \textbf{0.065±0.016} & 0.038±0.005 & 0.057±0.023 & 0.059±0.014 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.002±0.000 & 0.004±0.004 & 0.010±0.007 & 0.003±0.002 & \textbf{0.023±0.008} & \underline{0.012±0.005} & 0.003±0.002 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{NPP}} & ACC@1↑ & 0.019±0.007 & 0.019±0.003 & 0.012±0.003 & \underline{0.036±0.015} & 0.026±0.006 & 0.027±0.029 & \textbf{0.060±0.004} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ACC@5↑ & 0.057±0.011 & 0.056±0.010 & 0.056±0.007 & \underline{0.099±0.007} & 0.058±0.008 & 0.064±0.055 & \textbf{0.123±0.009} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{TUL}} & ACC@1↑ & 0.252±0.079 & 0.302±0.153 & 0.335±0.005 & 0.354±0.117 & 0.521±0.005 & \underline{0.533±0.061} & \textbf{0.612±0.011} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.130±0.013 & 0.099±0.055 & 0.155±0.003 & 0.150±0.054 & 0.263±0.006 & \underline{0.291±0.018} & \textbf{0.324±0.006} \\
%         \midrule
%         \multicolumn{3}{c|}{Per. Avg. Rank} & 5.8   & 4.5   & 5.7   & 4.2   & 3.0   & \underline{2.9} & \textbf{2.4} \\
%         \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:compoi}%
% \end{table*}%

% \paratitle{Randomness Sensitivity in POI MapRL Models.}
% POI representation learning is particularly affected by randomness due to variations in data partitioning and the selection of positive and negative samples in the pretraining task. As shown in \tab\ref{tab:compoi}, we summarize key observations below:

% \begin{itemize}[leftmargin=*]
%     \item SkipG, Teaser, and CACSR demonstrate significant instability across different runs. These models depend on contrastive learning techniques, making their performance highly susceptible to variations in dataset partitioning and the selection of negative samples. 
    
%     \item P2Vec and Tale demonstrate greater stability across various random seeds, likely due to their utilization of Token Relation Inference, a supervised pretraining task that enhances robustness. This approach involves predicting relationships between map entities based on their representation vectors, providing a structured learning framework that contributes to consistent performance.  

%     \item The TUL task exhibits heightened sensitivity to randomness, particularly within the Chicago (CHI) and San Francisco (SF) datasets. This increased sensitivity is primarily attributed to the limited number of user records in these cities (CHI: 921, SF: 361), leading to imbalanced training distributions. Consequently, a small subset of POIs disproportionately influences the learning process, resulting in significant variance across different random splits.

% \end{itemize}




% % Table generated by Excel2LaTeX from sheet 'Road3'
% \begin{table*}[ht]
%     \centering
%     \caption{Revision of Table 4 by addressing randomness.}
%     % \setlength{\tabcolsep}{0.5mm}
%     \renewcommand{\arraystretch}{0.8}
%     \small
%     \setlength{\extrarowheight}{-1pt}
%     \resizebox{0.8\textwidth}{!}{ % 让表格自动缩放
%     \begin{tabular}{ccc|ccccccc}
%         \toprule
%         \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{Task} & Metric & RN2Vec & HRNR  & SARN  & Toast & HRoad & START & JCLRNT \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Beijing}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 3.582±0.005 & 3.162±0.004 & 2.805±0.004 & 2.737±0.012 & \textbf{2.711±0.009} & 2.717±0.008 & \underline{2.803±0.019} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 5.734±0.001 & 5.589±0.001 & 5.481±0.001 & 5.512±0.009 & 5.407±0.003 & \textbf{5.390±0.004} & \underline{5.480±0.010} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 661.3±33.98 & 631.0±29.387 & 596.5±20.78 & \underline{533.0±52.97} & 584.8±16.34 & \textbf{512.3±19.87} & 514.3±38.30 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 2978±98.23 & 2968±101.9 & 2581±14.11 & 2576±79.44 & 2554±35.22 & \underline{2502±37.89} & \textbf{2464±36.07} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.764±0.032 & 0.816±0.030 & 0.843±0.029 & 0.787±0.099 & 0.867±0.007 & \textbf{0.901±0.025} & \underline{0.900±0.045} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 12.38±1.543 & \underline{11.48±1.937} & 13.297±1.168 & 12.76±4.812 & 14.00±3.421 & 11.87±3.982 & \textbf{11.45±4.148} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Chendu}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 6.565±0.064 & 6.424±0.044 & 5.988±0.021 & 6.357±0.026 & \textbf{5.931±0.023} & 6.046±0.011 & \underline{6.354±0.079} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 14.01±0.074 & 13.74±0.072 & 13.33±0.043 & 13.34±0.163 & \textbf{13.22±0.002} & \underline{13.46±0.007} & 13.46±0.132 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 106.1±0.057 & \underline{100.3±0.040} & \textbf{88.27±4.267} & 94.95±2.435 & 88.51±5.478 & 95.78±3.119 & 97.01±4.077 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 154.9±0.065 & 149.9±0.054 & 156.7±6.695 & 150.1±2.747 & \textbf{136.8±5.665} & \underline{151.0±3.841} & 147.7±3.790 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.687±0.037 & \underline{0.728±0.062} & 0.683±0.127 & 0.688±0.024 & 0.675±0.054 & \textbf{0.761±0.034} & 0.723±0.001 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 48.11±1.667 & 42.95±3.373 & 36.62±2.138 & 22.41±3.660 & 24.37±5.014 & \underline{19.22±2.722} & \textbf{18.73±2.534} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Xi'an}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 6.327±0.029 & \underline{5.794±0.121} & \textbf{5.359±0.026} & 5.633±0.014 & 5.411±0.073 & 5.384±0.068 & 5.670±0.023 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 13.08±0.368 & \underline{11.21±0.104} & \textbf{10.58±0.011} & 10.84±0.117 & 10.73±0.048 & 10.82±0.071 & 10.93±0.063 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 137±6.669 & 134.3±5.089 & \underline{109.7±4.258} & 122.2±4.519 & 110.3±3.678 & 115.3±15.44 & \textbf{107.7±6.816} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & \underline{198.7±8.232} & 203.0±11.88 & \textbf{169.0±5.630} & 190.9±3.617 & 171.9±8.943 & 169.9±13.92 & 177.8±8.341 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.709±0.014 & 0.745±0.036 & 0.717±0.075 & \textbf{0.795±0.032} & 0.735±0.006 & 0.752±0.038 & \underline{0.773±0.016} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 12.91±1.706 & \underline{12.1±3.479} & 12.53±3.624 & 16.47±6.278 & 18.96±6.951 & \textbf{10.81±4.540} & 11.95±5.148 \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Porto}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 4.390±0.001 & 4.397±0.001 & 4.287±0.000 & 4.362±0.009 & \textbf{4.196±0.010} & 4.205±0.003 & \underline{4.347±0.047} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 7.901±0.002 & \textbf{7.581±0.001} & 7.777±0.001 & \underline{7.931±0.047} & 7.705±0.007 & 7.793±0.040 & 7.792±0.054 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 99.46±1.781 & 101.3±1.981 & \underline{97.15±1.384} & 98.40±1.812 & 98.54±2.826 & 97.50±6.916 & \textbf{96.84±1.296} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 149.5±3.597 & 147.2±2.598 & \underline{142.7±1.798} & 146.7±2.479 & \textbf{140.5±2.224} & 157.7±7.044 & 144.8±1.031 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.803±0.098 & 0.822±0.109 & 0.832±0.030 & \textbf{0.901±0.064} & 0.835±0.035 & \underline{0.881±0.020} & 0.871±0.039 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 14.33±4.907 & \underline{11.98±1.809} & 17.86±5.396 & 12.06±4.026 & 18.20±4.804 & 13.68±4.440 & \textbf{11.40±6.376} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{SanFrancisco}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{ASI}} & MAE↓  & 2.981±0.003 & 2.511±0.001 & 2.489±0.008 & 2.555±0.002 & 2.485±0.005 & \underline{2.454±0.003} & \textbf{2.424±0.009} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 5.802±0.004 & 5.379±0.005 & \underline{5.289±0.014} & 5.295±0.002 & \textbf{5.246±0.003} & 5.332±0.001 & 5.367±0.001 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{TTE}} & MAE↓  & 289.0±0.022 & 287.8±0.006 & 278.7±0.212 & 273.6±19.04 & \underline{270.4±12.64} & \textbf{267.6±15.17} & 275.2±13.29 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 1479±4.301 & 1449±4.426 & 1499±3.618 & \textbf{1372±58.16} & 1501±56.35 & 1597±78.46 & \underline{1446±61.11} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & 0.837±0.039 & 0.911±0.004 & 0.860±0.069 & \textbf{0.943±0.035} & \underline{0.923±0.014} & 0.896±0.073 & 0.872±0.053 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & MR↓   & 7.195±3.190 & 7.003±0.015 & 8.478±3.050 & 9.224±7.285 & \underline{6.551±1.222} & 6.711±4.013 & \textbf{6.490±3.633} \\
%         \midrule
%         \multicolumn{3}{c|}{Per Avg Rank} & 6.333 & 4.900 & 3.900 & 3.867 & 3.200 & \underline{2.933} & \textbf{2.867} \\
%         \bottomrule
%     \end{tabular}%
% }
% \label{tab:comroad}
% \end{table*}

% \paratitle{Randomness Sensitivity in Road Segment MapRL Models}
% Road segment representation learning is significantly affected by data partitioning and the data generation process for Similarity Trajectory Search (STS), where the labels are assigned through a random detour process based on original coordinate trajectories. As shown in \tab\ref{tab:comroad}, our results confirm this conclusion: among the various downstream tasks, STS is the most affected, while ASI (Average Speed Inference) is relatively robust. Additional findings are summarized as follows:

% \begin{itemize}[leftmargin=*]
%     \item Toast, START, and JCLRNT exhibit higher instability compared to other models, as they rely on contrastive learning techniques, such as Token Relation Contrastive Learning  (TRCL) used by Toast and Augmented Trajectory Contrastive Learning (ATrCL) using by START and JCLRNT. These methods are highly susceptible to variations introduced by dataset partitioning and negative sampling, leading to performance fluctuations across different runs.
    
%     \item RN2Vec is the most robust model, consistently demonstrating low variance across different datasets. Its stability is likely attributed to its Token Relation Inference (TokRI) pretraining task, thereby mitigating sensitivity to randomness.
    
%     \item TTE and STS tasks show significant sensitivity to randomness, as they rely on graph-based and sequence-based representation learning, making them particularly prone to dataset partitioning effects. In contrast, TSI tasks remain largely unaffected due to their structured numerical relationships, which exhibit greater stability across different random seeds.
    
%     \item Downstream tasks in Beijing (BJ) and San Francisco (SF) display higher variance than in other cities. This can be attributed to their large number of road segments (BJ: 40,306, SF: 27,274), which increases trajectory diversity, thereby amplifying the impact of dataset partitioning on model performance.
% \end{itemize}

% \begin{table*}[htbp]
%   \centering
%   \vspace{-0.3cm}
%   \caption{Revision of Table 5 by addressing randomness.}
%   \vspace{-0.3cm}
%     \renewcommand{\arraystretch}{0.8}
%     \small
%     \setlength{\extrarowheight}{-1pt}
%     \resizebox{0.8\textwidth}{!}{ % 让表格自动缩放
%     \begin{tabular}{ccc|ccccccc}
%         \toprule
%         \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{Task} & Metric & ZEMob & GMEL  & HDGE  & MVURE & MGFN  & ReMVC & HREP \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Beijing}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.427±0.028 & 0.456±0.030 & 0.406±0.002 & 0.482±0.002 & \underline{0.595±0.016} & \textbf{0.750±0.018} & 0.499±0.015 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.113±0.002 & 0.612±0.025 & 0.221±0.005 & 0.277±0.008 & \underline{0.650±0.045} & \textbf{0.714±0.018} & 0.381±0.014 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 30.94±0.026 & 27.70±0.013 & \underline{20.76±4.905} & 29.57±0.829 & 30.12±0.024 & 27.83±0.016 & \textbf{20.60±1.334} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 55.26±0.039 & 58.96±0.039 & \underline{44.79±5.787} & 53.72±1.360 & 54.47±0.020 & 52.72±0.037 & \textbf{42.62±1.863} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 0.429±0.029 & 0.464±0.028 & 0.345±0.025 & \textbf{0.269±0.011} & 0.304±0.032 & \underline{0.300±0.015} & 0.319±0.002 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 0.795±0.024 & 0.743±0.023 & 0.700±0.034 & 0.712±0.016 & 0.760±0.038 & \underline{0.695±0.023} & \textbf{0.664±0.008} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Chengdu}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.360±0.013 & 0.383±0.040 & 0.422±0.034 & 0.481±0.004 & 0.482±0.079 & \textbf{0.664±0.032} & \underline{0.536±0.005} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.174±0.034 & 0.162±0.032 & 0.266±0.064 & 0.274±0.015 & 0.348±0.123 & \textbf{0.586±0.026} & \underline{0.456±0.009} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 154.9±0.025 & \underline{154.8±0.019} & 159.1±2.020 & 156.2±3.099 & 157.5±5.687 & \textbf{147.7±0.016} & 156.5±18.80 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 441.2±0.022 & 441.1±0.041 & 403.3±1.125 & 442.8±4.280 & \textbf{337.4±64.38} & 431.0±0.029 & \underline{395.7±49.70} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & \textbf{3.640±0.032} & 4.622±0.036 & 5.171±0.013 & \underline{3.968±0.711} & 5.142±0.020 & 5.292±0.037 & 5.471±0.121 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 29.70±0.024 & 29.71±0.030 & \underline{28.73±0.154} & 29.58±0.125 & 29.32±1.139 & 29.05±0.061 & \textbf{28.30±0.071} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Xi'an}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.360±0.031 & 0.365±0.028 & 0.444±0.017 & 0.531±0.009 & 0.478±0.085 & \underline{0.574±0.004} & \textbf{0.589±0.013} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.188±0.036 & 0.418±0.034 & 0.254±0.009 & 0.264±0.017 & 0.284±0.072 & \textbf{0.460±0.034} & \underline{0.453±0.024} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 133.8±0.028 & 133.1±0.018 & \underline{124.1±5.867} & 127.1±3.846 & \textbf{119.2±9.305} & 131.6±0.038 & 128.6±0.798 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 326.2±0.020 & 324.5±0.034 & \underline{289.0±26.30} & 317.8±4.766 & \textbf{241.2±28.38} & 324.6±0.033 & 296.9±9.101 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 3.828±0.034 & 3.710±0.035 & 3.916±0.031 & \textbf{3.333±0.351} & \underline{3.696±0.112} & 3.911±0.052 & 4.019±0.042 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 17.68±0.034 & 17.65±0.026 & \textbf{16.62±0.139} & 17.41±0.004 & 16.79±1.321 & 16.81±0.050 & \underline{16.71±0.201} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{Porto}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & 0.343±0.035 & 0.330±0.037 & \underline{0.424±0.047} & 0.297±0.014 & 0.303±0.005 & \textbf{0.444±0.032} & 0.358±0.022 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.211±0.006 & 0.384±0.029 & \underline{0.407±0.074} & 0.272±0.017 & 0.200±0.027 & \textbf{0.414±0.038} & 0.319±0.029 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 527.5±0.027 & 525.1±0.009 & 501.0±18.03 & \underline{401.6±71.84} & 476.7±97.28 & 527.3±0.015 & \textbf{288.6±121.6} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 595.2±0.022 & 592.0±0.035 & 581.9±14.39 & 472.0±71.13 & \underline{443.2±96.75} & 594.9±0.031 & \textbf{355.4±126.9} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & 44.88±0.021 & 41.12±0.026 & 30.79±4.571 & 37.76±0.648 & \underline{29.80±7.256} & 39.39±0.047 & \textbf{28.26±5.297} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 72.32±0.019 & 56.23±0.037 & 45.70±4.910 & 54.11±4.679 & \underline{45.45±9.793} & 56.68±0.029 & \textbf{42.17±8.930} \\
%         \midrule
%         \multicolumn{1}{c|}{\multirow{6}[3]{*}{\rotatebox{90}{SanFrancisco}}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{LPC}} & ACC@1↑ & \underline{0.845±0.016} & 0.638±0.011 & 0.825±0.006 & 0.845±0.021 & 0.831±0.012 & \textbf{0.858±0.033} & 0.838±0.006 \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1↑   & 0.529±0.030 & \underline{0.565±0.010} & 0.497±0.030 & 0.516±0.053 & 0.440±0.096 & 0.473±0.036 & \textbf{0.570±0.028} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{FI}} & MAE↓  & 509.2±0.036 & 514.0±0.015 & 387.2±73.13 & \underline{349.3±73.67} & 356.2±125.5 & 444.7±0.010 & \textbf{324.5±65.78} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 910.5±0.043 & 916.7±0.021 & \underline{693.0±135.10} & 700.3±123.6 & 748.3±130.3 & 852.4±0.024 & \textbf{624.4±101.4} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{MI}} & MAE↓  & \textbf{5.877±0.027} & 7.402±0.019 & 6.514±0.510 & 6.461±0.424 & 6.396±0.838 & 6.870±0.037 & \underline{5.895±0.496} \\
%         \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RMSE↓ & 23.49±0.009 & 22.31±0.015 & 21.46±0.281 & 20.63±1.212 & \underline{20.16±2.343} & 22.66±0.031 & \textbf{19.10±1.506} \\
%         \midrule
%         \multicolumn{3}{c|}{Per Avg Rank} & 5.667  & 5.100  & 4.000  & 3.733  & 3.533  & \underline{3.500} & \textbf{2.433} \\
%         \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:letterregion}%
%   \vspace{-0.3cm}
% \end{table*}%

% \paratitle{Randomness Sensitivity in Land Parcel MapRL Models}
% Land parcel representation learning exhibits different levels of sensitivity across tasks. Classification tasks (LPC) are generally stable, while Flow Inference (FI) and Mobility Inference (MI) tasks show higher sensitivity. Other findings are summarized as follows:

% \begin{itemize}[leftmargin=*]
%     \item ZEMob, GMEL, and ReMVC are among the most stable models across all datasets. Despite employing contrastive learning as pretraining tasks—which tends to be sensitive in other MapRL models—their stability may be attributed to the smaller number of parcel entities. For instance, San Francisco contains 194 parcel entities compared to 27,274 road segment entities. This smaller number of parcel entities likely results in more stable negative sampling.

%     \item MGFN is notably sensitive across datasets, as it utilizes clustering techniques to construct the base graph structure for representation learning, introducing sensitivity to randomness.

%     \item FI and MI tasks exhibit greater sensitivity to randomness than LPC classification tasks. This is expected because these two tasks involve graph-based regression, which is sensitive to data partitioning.
% \end{itemize}

% \paratitle{Cross-Task Observations on Randomness Sensitivity}
% Finally, we identify broader trends that affect MapRL models across all types of representations:

% \begin{itemize}[leftmargin=*] 
%     \item Models utilizing contrastive learning pretraining tasks, such as Token Relation Contrastive Learning (TRCL), Augmented Token Contrastive Learning (AToCL), and Augmented Trajectory Contrastive Learning, exhibit increased sensitivity to randomness. However, this sensitivity may diminish when dealing with smaller datasets.
    
%     \item Downstream tasks that rely on graph-based representation learning, including Travel Time Estimation (TTE), Similar Trajectory Search (STS), Flow Inference (FI), and Mobility Inference (MI), may experience significant structural variations across different training runs due to their dependence on graph structures.
    
%     \item Datasets with greater diversity can amplify the impact of randomness, leading to increased variability in model performance.
% \end{itemize}
% These observations underscore the necessity of evaluating model robustness across multiple random seeds and carefully considering dataset characteristics when selecting pretraining task combinations.








\vspace{0.3cm}


%%%%%%%%%%%%% Comment 2.3
\subsection{Comment 2.3 and Response 2.3} \label{com:23}

\commenttitle{Comment 1.2 (W3 \& D3)}

{\em (W3).} Could discuss potential domain-specific niche MapRL tasks and methods.
\vspace{4pt}

\noindent
{\em (D3).} While this work is mainly intended for an over-arching taxonomy and experimental review of existing MapRL methods, I believe there is room to discuss niche tasks, data and methods found in specific applications, if indeed there are existing works on this front.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

Thank you for your valuable feedback. A clear discussion of domain-specific MapRL methods has been provided in our paper's Section 6. Specific revisions are as follows:
\begin{cmt}[Revision of "Discuss potential niche tasks for \rl" in paper's Section 6]
    In recent years, various downstream tasks in MapRL have been widely studied, including Next POI Prediction (NPP), Trajectory User Link (TUL), Travel Time Estimation (TTE), Trajectory Similarity Search (STS), and Mobility Inference (MI). These tasks are central to location-based services, traffic prediction, and spatiotemporal data mining. Many models for NPP rely on Recurrent Neural Networks (RNNs) or Transformers, with methods like DeepMove\citeNew{deepmove} using attention mechanisms to predict users’ next POI. TUL, exemplified by DeepTUL\citeNew{deeptul}, links anonymous trajectories to users, leveraging trajectory and user embeddings. TTE methods, such as DeepTTE\citeNew{deeptte}, use LSTMs to model temporal dependencies and include factors like weather and traffic conditions for more accurate travel time predictions. For similarity trajectory search, recent advancements in learned measures, including NEUTRAJ\citeNew{neutraj} and T3S\citeNew{T3S}, outperform traditional non-learned methods by encoding trajectories as vectors. Finally, Flow and Mobility Inference tasks, integral to ride-hailing platforms like Didi and Uber, use graph-based models such as ODMP\citeNew{ODMP}, which combine spatial and temporal information via GNNs, RNNs, and Transformers for accurate demand forecasting.
\end{cmt}


\textbf{More Details:} In the following section, we provide a more detailed discussion of domain-specific niche MapRL tasks.

Our study introduces nine downstream tasks spanning various applications, including POI Classification (POIC), Next POI Prediction (NPP), Trajectory User Link (TUL), Average Speed Inference (ASI), Travel Time Estimation (TTE), Similarity Trajectory Search (STS), Land Parcel Classification (LPC), Flow Inference (FI), and Mobility Inference (MI). These tasks are widely studied in location-based services, traffic prediction, and spatiotemporal data mining, making them representative of domain-specific MapRL applications.

Among these, POIC, ASI, and LPC do not yet have specifically designed models. Below, we elaborate on the task definitions, datasets, and existing models for the remaining tasks, illustrating how MapRL techniques are applied in various domains.

\paratitle{Next POI Prediction:} The Next POI Prediction (NPP) task aims to recommend the most relevant points of interest (POIs) to users based on their historical behavior, interests, and current location. Common datasets for this task include those from social platforms like Foursquare \citeNew{fours1}, Instagram \citeNew{CAPE}, and Yelp\citeNew{yelp}. The Foursquare dataset, which includes global user check-in trajectory data, is the most widely used, while Instagram and Yelp offer smaller datasets but include valuable user review text that has recently been leveraged to enhance model accuracy. Traditional models often rely on Recurrent Neural Networks (RNNs) or Transformers to model sequential user behavior. DeepMove \citeNew{deepmove}, for instance, employs a GRU with an attention mechanism to predict the next POI a user might visit. Recent advancements integrate temporal and contextual factors (e.g., weather, time of day) to further improve recommendation accuracy.

\paratitle{Trajectory User Link:} The Trajectory User Link task aims to match anonymous trajectories with the users who generated them. This task is critical for various spatial-temporal applications, including location-based services and urban anomaly detection. Traditional methods typically train models using known user trajectory data, mapping trajectories into a vector space using RNNs or Transformers, followed by Multiple-layer preception with softmax to compute the probability of matching a trajectory to a user. A notable example, DeepTUL\citeNew{deeptul}, encodes trajectory data using GRUs, leveraging user history for embedding similarity computation. A key challenge in this task is sparse trajectory data, requiring robust generalization techniques to improve matching performance.

\paratitle{Travel Time Estimation:} The Travel Time Estimation (TTE) task aims to predict the travel time between the start and end of a given trajectory. Accurate TTE helps individuals optimize travel plans, avoid congested routes, and save time while also aiding traffic management in road planning and traffic control. Traditional TTE methods, such as using speed detectors (e.g., loop sensors), suffer from high installation costs and limited applicability. Moreover, simply summing the travel times for each road segment fails to account for intersection delays. With the rise of Didi Chuxing and other ride-hailing trajectory datasets, data-driven methods have gained popularity. Some approaches estimate travel time by averaging historical travel durations, but these often fail to handle real-time variations. DeepTTE \citeNew{deeptte} addresses these issues by using an LSTM to model temporal dependencies and incorporating external factors (e.g., weather, road conditions, driver behavior) to enhance prediction accuracy.

\paratitle{Similarity Trajectory Search:} The Similarity Trajectory Search task aims to find the most similar trajectory to a query trajectory from a trajectory database. The core of this task is to calculate the similarity between trajectories. Trajectory similarity measures can be classified into two categories: non-learned and learned measures. Non-learned measures, such as the Hausdorff distance \citeNew{hausdorff}, calculate similarity by matching points between trajectories but are computationally expensive, with a time complexity of $O(n^2)$, making them unsuitable for large datasets. In recent years, learned measures based on deep learning have gained popularity. These methods encode trajectories as vectors (trajectory embeddings) and compute the distance between embedding vectors using methods such as RNNs and self-attention models (like Transformers). Learned measures not only improve computational efficiency but also enhance similarity measurement accuracy, especially in cases with low-quality trajectories. Methods like NEUTRAJ\citeNew{neutraj} and T3S\citeNew{T3S} learn to approximate non-learned measures, further optimizing efficiency, while t2vec\citeNew{t2vec} and TrajCL\citeNew{TrajCL} employ self-supervised learning to directly learn from unlabeled trajectories.

\paratitle{Flow Inference \& Mobility Inference :} Mobility Inference predicts the flow of people or OD flow between land parcel over specific time periods. Flow Inference is a subtask of Mobility Inference, focusing on predicting the inflow or outflow of people in a parcel. These tasks are widely used for predicting passenger demand, especially in ride-hailing platforms like Didi and Uber. Graph-based models, such as ZEMob \citeNew{ZEMob}, construct spatial graphs where nodes represent land parcels and edges denote travel demand, using graph representation learning for prediction. However, these models often overlook temporal fluctuations. ODMP \citeNew{ODMP} introduces spatiotemporal graphs, leveraging GNNs, RNNs, and Transformers to capture both spatial relationships and temporal trends for more accurate forecasting.

\vspace{0.3cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 3
\newpage

\section{Response to Reviewer \#3}

%%%%%%%%%%%%% Comment 3.1
\subsection{Comment 3.1 and Response 3.1} \label{com:31}

\commenttitle{Comment 3.1 (W1)}

{\em (W1).} Taxonomy does not seem to be that novel as it is based on well-known concepts. A discussion on what are the main advantages and novelty of proposing the taxonomy is welcome.

\vspace{0.1cm}
\noindent
\commenttitle{Response}
 
We appreciate your insightful feedback regarding the novelty and advantages of our proposed taxonomy in Map Entity Representation Learning (MapRL). As suggested, we added a clearer discussion on what the main advantages and novelty of our taxonomy in the paper's Related Work section. Specific revisions are provided as follows:
\begin{cmt}[Revision of "Novelty" in paper's Introduction.]
To address the first challenge, we propose a novel taxonomy for \rl models, namely \tax, which organizes the essential components of an \rl model into four key elements: {\em Map Data}, {\em Encoder Models}, {\em Pre-training Tasks}, and {\em Downstream Tasks}. Unlike traditional taxonomies that categorize models by map entity types, \tax takes a functional approach, grouping encoder models into three paradigms—{\em Token-based}, {\em Graph-based}, and {\em Sequence-based}—each supporting specialized pre-training tasks. Only downstream tasks depend on the nature of the map entity. The key insight of our taxonomy is that the two core elements—Encoder Models and Pre-training Tasks—are not tightly coupled with specific map entity types. This decoupling of core components from entity-specific constraints fosters a more unified and transferable framework for MapRL, facilitating cross-domain integration and knowledge sharing.
\end{cmt}

\textbf{More Details:} In the following section, we provide a detailed discussion on the main advantages and novelty of our taxonomy.

\paratitle{Novelty of our Taxonomy.} While our taxonomy builds upon well-established principles, it is uniquely designed to address the distinct challenges of MapRL - the fragment challenge. Our taxonomy categorizes MapRL models based on their functional components—encoders and pretraining tasks—rather than entity type, allowing for a more generalizable and modular perspective. This method-centric classification introduces a novel way to organize MapRL approaches, promoting knowledge transfer between different subfields and enabling researchers to systematically explore model design choices.

\paratitle{Practical Advantages of Our Taxonomy.} Our taxonomy offers several practical benefits to researchers and practitioners:
\begin{itemize}[leftmargin=*]
    \item Guidance in Model Selection: By classifying MapRL models based on their underlying methodologies and corresponding pretraining tasks, our taxonomy helps researchers identify the most effective function modules for specific map entities and downstream tasks.
    \item Identification of Research Gaps: The structured framework reveals unexplored combinations of pretraining tasks and model architectures, providing insights into potential areas for future research and innovation.
    \item General Insights: Integrated with the VecCity library, our taxonomy provides a unified framework for understanding MapRL models across different entity types. 
\end{itemize}

% Thank you once again for your thoughtful feedback. We hope this clarifies the distinct contributions and importance of our work. Thank you again for your thoughtful feedback.

\vspace{0.3cm}

\newpage

%%%%%%%%%%%%% Comment 3.2
\subsection{Comment 3.2 and Response 3.2} \label{com:32}

\commenttitle{Comment 3.2 (W2)}

{\em (W2).} Scalability and efficiency of benchmarked algorithms are briefly discussed in section 4.2.1 and 4.2.2. It would be a great plus to extend the discussion in this sense.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

We sincerely appreciate your valuable feedback on the scalability analysis of MapRL models. As suggested, we have expanded our evaluation of the benchmarked models to focus on three core dimensions: effectiveness, efficiency, and the trade-offs between model size and inference time. The specific revisions in our paper are available in \underline{\updateo{\hyperref[sec:t43]{Section 4.3}}}. % outlined below, with detailed discussions

% \begin{cmt} [Revision of "Effectiveness" in paper's Section 4.3.1.]
% 1) {\em Performance Scalability.} Token-based MapRL models (represented by dashed lines) exhibit weaker performance scalability, showing limited improvement as the fine-tuning dataset size increases from 10\% to 50\%, with performance gains plateauing around the 30\% mark. In contrast, graph-based and sequence-based models maintain steady gains up to 50\%, demonstrating stronger scalability. Notably, methods incorporating contrastive learning techniques—such as CACSR, START, JCLRNT, and HREP—show particularly strong improvements, suggesting that contrastive learning further enhances performance as more data becomes available. However, due to the inherent instability of contrastive learning, increasing the number of negative samples may be necessary to ensure more stable results.

% Overall, token-based models show weaker performance scalability, with diminishing returns as dataset size increases, particularly beyond 30\%. In contrast, graph-based and sequence-based models, especially those employing contrastive learning methods (e.g., CACSR, START, JCLRNT, HREP), exhibit more significant performance improvements as the amount of labeled data increases, demonstrating stronger scalability in data-intensive scenarios. Moreover, existing \rl models exhibit varying sensitivity to the size of labeled data across different tasks. For tasks less influenced by temporal information, such as attribute inference (ASI, POIC, LPC) and Similarity Trajectory Search (STS), models maintain stable performance even with limited training data. However, for tasks with time-dependent labels, such as trajectory-related tasks (NPP, TUL, TTE) and Flow/Mobility Inference tasks (FI, MI), larger amounts of labeled data are necessary to effectively capture temporal dynamics.
% \end{cmt}


% \begin{cmt} [Revision of "Efficiency" in paper's Section 4.3.2]
% To fully investigate the efficiency scalability of MapRL models, we evaluate them across three key aspects: (1) Parameter count, representing the space complexity of the models; (2) Training time per epoch, indicating the time cost of training; and (3) Inference time, reflecting the time required for downstream task evaluation. These measurements are collected from all five datasets used in the main experiments, each with different entity counts. Figure.~\ref{fig:efficiency} presents the evaluation results: \fig~\ref{fig:efficiency} (a) to (c) show results for POI-oriented models, \fig~\ref{fig:efficiency} (d) to (f) display results for road segment-oriented models, and \fig~\ref{fig:efficiency} (g) to (i) provide results for land parcel-oriented models. The horizontal axis of all figures represents the number of entities on a $10^3$ scale, while the vertical axis represents the parameter count in millions, training time per epoch in seconds, and total inference time in seconds, respectively. Based on these figures, we have several key findings:

%  1) {\em Model Size:} Token-based models (dashed lines) generally achieve better scalability in parameter size, while sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) often have higher parameter counts. In contrast, graph-based models such as SARN, GMEL, MVURE, and HREP show relatively stable parameter counts as the number of entities increases, demonstrating better scalability in scenarios with large numbers of map entities.

% 2) {\em Training Time:} Token-based models (dashed lines) demonstrate better training time scalability in POI-oriented models but perform less efficiently in land parcel-oriented models. This difference is influenced by entity count variations, with POI datasets containing between $1 \times 10^4$ and $8 \times 10^4$ entities, while land parcel datasets range from $2 \times 10^2$ to $1 \times 10^4$ entities. The results suggest that token-based models may have a greater competitive advantage in large-scale datasets. Sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) generally incur longer training times. Graph-based models employing GAu pretraining tasks (HRNR, HRoad, GMEL, MGFN) show more-than-linear growth in training time, posing scalability challenges for large datasets, whereas HREP, despite using GAu pretraining, maintains relatively stable training time due to its lower space complexity.

% 3) {\em Inference Time:} All models show an increasing trend in inference time. However, the rise is more pronounced in POI- and land parcel-oriented models compared to road segment-oriented models, indicating that inference time is more heavily influenced by the number of entities in downstream tasks for POIs and parcels. Sequence-based models (e.g., CTLE, Toast, START, JCLRNT) generally require longer inference times, while HRNR stands out among road segment-oriented models with significantly higher inference times due to its dynamic graph construction during inference.
% \end{cmt}

% \begin{cmt} [Revision of "Trade-offs" in paper's Section 4.3.3.]
% In Section \ref{sec:experiment}, we conclude that more complex models often achieve higher accuracy. However, increased model complexity can lead to efficiency challenges, particularly in inference time, which may limit their practicality in real-world applications. The efficiency analysis in the previous section does not provide a direct view of the relationship between model complexity and inference time. To explore this trade-off, we conducted an experiment evaluating the relationship between parameter count and inference time. This experiment uses the same dataset as in Section 4.3.1 on effectiveness: POI-oriented models are evaluated on the Tokyo dataset, while road segment- and land parcel-oriented models are tested on the Xi’an dataset. To enable a unified comparison across the three entity types, the horizontal axis represents the parameter count (in millions), and the vertical axis represents the single-sample inference time (in milliseconds).

% Figure.\ref{fig:tradeoff} presents the results, showing that land-parcel-oriented models maintain relatively stable inference times despite increases in parameter size, likely due to lower downstream task complexity. In contrast, POI and road segment-oriented models exhibit a more linear or steeper increase in inference time as model complexity grows. Sequence-based models (e.g., Hier, CACSR, CTLE, JCLRNT, START, Toast) generally show higher inference times due to the integration of multiple encoders. Attention mechanisms, such as those employed by Transformers (Toast, JCLRNT, START) and the GAT(MGFN), contribute to increased parameter counts and inference times. Meanwhile, graph-based models (e.g., HyperRoad, SARN, GMEL, MGFN, HDGE, HREP) tend to maintain lower inference times, with the exception of HRNR, which uses dynamic graph construct during inference, leading to significantly higher inference times.
% \end{cmt}
% \textbf{More Detail:} In the following section, we provide a more detail disscution for the scalability issue from multiple perspectives, including effectiveness, efficiency and Trade-offs.


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/rebuttal/dive_all.pdf}
%     \caption{Results from varying fine-tuning data size.}
%     \label{fig:diveall}
% \end{figure}

% \paratitle{Effectiveness.}
% \noindent Effectiveness scalability assesses whether a model’s performance continues to improve as more data becomes available. In Section 4.4, we specifically investigate how reducing the fine-tuning dataset to 10\%, 20\%, 30\%, 40\%, and 50\% of its full-size impacts:
% \begin{itemize}[leftmargin=*]
%     \item Model Robustness Under Limited Data: By reducing the fine-tuning dataset size, we can identify which models remain reliable and maintain performance when data are scarce.
%     \item Performance Growth with Additional Data: Starting from 10\% of the fine-tuning dataset and scaling up to 50\% (a fivefold increase), we can evaluate which MapRL models most effectively leverage additional data to significantly boost performance.
% \end{itemize}
% The results were included in the initial draft and are shown in \fig~\ref{fig:diveall}. Based on these results, we analyzed model robustness under limited Data. However, our initial analysis lacked insights into performance scalability, i.e., how model performance improves as more labeled data becomes available. To address this, we have added a discussion on performance scalability in paper's Section 4.3. Specifically:

% 1) {\em Performance Scalability.} Token-based MapRL models (represented by dashed lines) exhibit weaker performance scalability, showing limited improvement as the fine-tuning dataset size increases from 10\% to 50\%, with performance gains plateauing around the 30\% mark. In contrast, graph-based and sequence-based models maintain steady gains up to 50\%, demonstrating stronger scalability. Notably, methods incorporating contrastive learning techniques—such as CACSR, START, JCLRNT, and HREP—show particularly strong improvements, suggesting that contrastive learning further enhances performance as more data becomes available. However, due to the inherent instability of contrastive learning, increasing the number of negative samples may be necessary to ensure more stable results.

% % 1) {\em Stability in Attribute Inference Tasks}: \rl models show stable performance across varying training data sizes in attribute inference tasks, such as POI Classification (POIC) in \fig~\ref{fig:dive}~(a), Average Speed Inference (ASI) in \fig~\ref{fig:dive}~(d), and Land Parcel Classification (LPC) in \fig~\ref{fig:dive}~(g). This stability arises because these tasks focus on inferring entity attributes, which are effectively captured during pre-training. As a result, the fine-tuning phase requires only a small amount of labeled data to maintain good performance.

% % 2) {\em Fluctuations in Trajectory-Related and Graph-Related Tasks}: Models exhibit notable performance fluctuations in trajectory-related tasks (e.g., NPP, TUL, TTE) and graph-related tasks (e.g., FI, MI). Trajectory-related tasks require sequence-level predictions, whereas most encoders and pre-training tasks generate single-entity embeddings, making these tasks especially sensitive to smaller fine-tuning datasets. By contrast, Similarity Trajectory Search (STS) relies on similarity comparisons rather than prediction, making it less effective. Additionally, Flow Inference (FI) and Mobility Inference (MI), although not strictly trajectory-based, capture human mobility flows that vary greatly over time. This temporal heterogeneity demands more labeled data to accurately model these patterns, leading to further performance variability when data are limited.




% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/rebuttal/efficient.pdf}
%     \caption{Model efficiency on model size, training time, and inference time.}
%     \label{fig:efficient}
% \end{figure}

% \paratitle{Efficiency.}
% \noindent We evaluate the efficiency of MapRL models across the following three aspects: (1) parameter count which represent the space complexity of MapRL models; (2) time cost per epoch, which identifies the time cost of training the models. We collect the time cost for 100 training epochs and take the mean of 100 epochs as the result; And (3) inference time, which identifies the time cost for the evaluation of the downstream task. These measurements are collected across all five datasets used in the main experiments. These datasets, which have different entity counts, help us investigate the scalability of model efficiency.

% 1)\emph{Paramter Count.} We measure the parameter count of all models, as shown in Figure 1 (a), (d), and (g). Figure 1 (a) presents the parameter count for POI-oriented models, (d) for road segment-oriented models, and (g) for land-parcel-oriented models. The horizontal axis represents the number of entities on a $10^3$ scale, while the vertical axis represents the parameter count in millions. Several key findings emerge:
% \begin{itemize}[leftmargin=*]
%     \item Token-based models (dashed lines) generally achieve better scalability in parameter size.
%     \item Sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) often exhibit higher parameter counts.
%     \item Graph-based models like SARN, GMEL, MVURE, and HREP, show slow changes in parameter count with increasing entity numbers, demonstrating better scalability in scenarios with a large number of map entities.
% \end{itemize}

% 2)\emph{Training Time.} We measure the per-epoch training time for all MapRL models, with results shown in Figure 1 (b), (e), and (h) for POI, road segment, and land-parcel-oriented models, respectively. The horizontal axis represents the number of entities (scaled to $10^3$), and the vertical axis shows the average training time per epoch (in seconds) over 100 epochs. Key findings include:
% \begin{itemize}[leftmargin=*]
%     \item Token-based models exhibit better scalability in POI-oriented models but perform worse in land-parcel-oriented models due to differences in entity counts: $1 \times 10^4 - 8 \times 10^4$ for POI and $2 \times 10^2 - 1 \times 10^4$ for land parcels. Therefore, token-based models may have a greater competitive advantage in large-scale datasets.
%     \item Sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) tend to incur higher training times.
%     \item Graph-based models using GAu (e.g., HRNR, HRoad, GMEL, MGFN) exhibit more-than-linear growth in training time, presenting challenges for large-scale datasets. HREP, which also uses GAu, does not show significant growth in training time, likely due to its lower space complexity.
% \end{itemize}

% 3)\emph{Inference Time.} We measure the inference time for all MapRL models, with results shown in Figure 1 (c), (f), and (i) for POI, road segment, and land-parcel-oriented models, respectively. The horizontal axis represents the number of entities on a $10^3$ scale, and the vertical axis shows inference time (in seconds). Key findings include:
% \begin{itemize}[leftmargin=*]
%     \item All MapRL models exhibit the same increasing trend. However, the rise in inference time is more pronounced for POI and land-parcel-oriented models compared to road segment-oriented models. This suggests that inference time is more strongly influenced by the number of entities in the downstream tasks for POI and parcel models.
%     \item Sequence-based models (e.g., CACSR, CTLE, Toast, START, JCLRNT) tend to incur higher inference times.
%     \item HRNR exhibits much higher inference times than other road segment-oriented models, largely due to the dynamic graph construction during inference.
% \end{itemize}



% \paratitle{Trade-offs.} Beyond the individual aspects of effectiveness and efficiency, we further analyze the trade-offs between model size and inference time through Figure \ref{fig:comtradeoff}, which visualizes the relationship between parameter count and inference time across all benchmarked models. To present the inference time for all models in one figure, we report the inference time per sample rather than the total inference time. As shown in Figure \ref{fig:comtradeoff}, the horizontal axis represents parameter count in millions, and the vertical axis represents single-sample inference time in milliseconds. Key observations include:
% \begin{itemize}[leftmargin=*]
%     \item land-parcel-oriented models maintain relatively stable inference times despite an increase in parameter size, possibly due to lower downstream task complexity. POI and road segment-oriented models show a more linear or sometimes steeper increase.
%     \item Models using sequence encoders (e.g., Hier, CACSR, CTLE, JCLRNT, START, Toast) generally increase inference times due to the integration of multiple encoders and heterogeneous pretraining tasks. 
%     \item Attention mechanisms (e.g., Transformers in Toast, JCLRNT, START, and GAT-based MGFN) increase both parameter counts and inference times.
%     \item Graph encoder-based models  (e.g., HyperRoad, SARN, GMEL, MGFN, HDGE, HREP) do not necessarily incur high inference times, except for HRNR, which uses multiple GNN layers during inference.
% \end{itemize}
% \noindent These results underscore the trade-offs between model size and inference time, providing insights into how to balance computational costs with performance requirements.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/rebuttal/time_tradeoff.pdf}
%     \caption{Trade-offs between model size and inference time.}
%     \label{fig:comtradeoff}
% \end{figure}

% \paratitle{Conclusion}
% \noindent We thank the reviewer for emphasizing the importance of scalability analysis. Our revised manuscript now provides a more structured discussion, encompassing effectiveness, efficiency, and their inherent trade-offs. We believe these findings will benefit both researchers and practitioners, helping to inform model selection based on computational constraints and performance needs.



\vspace{0.3cm}

%%%%%%%%%%%%% Comment 3.3
\subsection{Comment 3.3 and Response 3.3} \label{com:33}

\commenttitle{Comment 3.3 (W3)}

{\em (W3).} The link to download data is not working in the Github repo.

\vspace{0.1cm}
\noindent
\commenttitle{Response}

We apologize for the inconvenience caused by the non-functional data download link in our GitHub repository. This issue may be due to restrictions associated with Beihang University's hosting services. To ensure more reliable access, we have provided an alternative download link via \underline{\updateo{\href{https://drive.google.com/file/d/1JqnGsprG2zpJ4tisf0o3liOLy3GR7t0i/view?usp=drive_link}{Google Drive}}}.

We are committed to maintaining the availability and functionality of our tools and resources. If you encounter any further issues or have additional questions, please do not hesitate to contact us.
\vspace{0.3cm}

\bibliographystyleNew{ieeetr}
\bibliographyNew{sample1}


==> 4-experiment-backup.tex <==
% Table generated by Excel2LaTeX from sheet 'POI3'
\update1{
\begin{table*}[t]
  \centering
  \vspace{-0.3cm}
  \caption{Performance comparison of POI \rl methods on various datasets. The bold/underlined font means the best/the second-best
result. "↑" means bigger is better and "↓" means smaller is better.}
\vspace{-0.3cm}
  \resizebox{\textwidth}{!}{
  \setlength{\tabcolsep}{0.5mm}
    \begin{tabular}{c|cccc|cccc|cccc|cccc|cccc|cc}
    \toprule
    Dataset & \multicolumn{4}{c|}{New York} & \multicolumn{4}{c|}{Tokyo}    & \multicolumn{4}{c|}{Chicago}  & \multicolumn{4}{c|}{Singapore} & \multicolumn{4}{c|}{San Francisco} & \multicolumn{2}{c}{Overall} \\
    \midrule
    Task  & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c|}{NPP} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c|}{NPP} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c|}{NPP} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c|}{NPP} & \multicolumn{2}{c}{POIC} & \multicolumn{2}{c|}{NPP} & \multirow{2}{*}{\makecell{Pre Ave\\Rank}} & \multirow{2}{*}{\makecell{Pre\\Rank}} \\
    Metric & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ & ACC@1↑ & F1↑   & ACC@1↑ & ACC@5↑ &       &  \\
    \midrule
    SkipG & 0.071 & 0.012 & 0.126 & 0.309 & \underline{0.334} & \underline{0.042} & \underline{0.164} & 0.333 & 0.077 & 0.007 & 0.050 & 0.161 & 0.027 & 0.003 & 0.030 & 0.074 & 0.011 & 0.003 & 0.014 & 0.053 & 5.3   & 7 \\
    Tale  & 0.057 & 0.009 & \underline{0.152} & \textbf{0.341} & 0.212 & 0.037 & 0.145 & 0.297 & 0.096 & 0.009 & 0.094 & 0.230 & 0.029 & 0.005 & 0.043 & 0.101 & 0.009 & 0.001 & 0.007 & 0.046 & 4.8   & 6 \\
    Teaser & \textbf{0.079} & \textbf{0.014} & 0.131 & 0.329 & \textbf{0.354} & \textbf{0.048} & 0.137 & 0.241 & 0.077 & 0.005 & 0.029 & 0.137 & 0.065 & \textbf{0.018} & 0.033 & 0.078 & \underline{0.037} & \textbf{0.012} & 0.014 & 0.058 & 4.4   & 5 \\
    Hier  & 0.052 & 0.008 & 0.121 & 0.285 & 0.278 & 0.032 & 0.162 & \underline{0.335} & 0.086 & 0.011 & 0.036 & 0.161 & 0.041 & 0.006 & 0.079 & 0.163 & \textbf{0.039} & 0.007 & 0.012 & 0.108 & 4.2   & 4 \\
    P2Vec & \underline{0.074} & \underline{0.013} & 0.116 & 0.154 & 0.313 & 0.037 & 0.154 & 0.319 & \underline{0.111} & 0.012 & 0.143 & 0.393 & \underline{0.068} & \underline{0.014} & 0.075 & \underline{0.168} & 0.033 & \underline{0.011} & 0.019 & 0.046 & 3.7   & 3 \\
    CACSR & 0.028 & 0.004 & 0.135 & 0.331 & 0.232 & 0.010 & 0.159 & 0.325 & 0.104 & \underline{0.017} & \underline{0.146} & \underline{0.394} & 0.030 & 0.005 & \underline{0.103} & 0.126 & 0.018 & 0.004 & \textbf{0.077} & \textbf{0.158} & \underline{3.5} & 2 \\
    CTLE  & 0.048 & 0.006 & \textbf{0.154} & \underline{0.336} & 0.235 & 0.014 & \textbf{0.168} & \textbf{0.338} & \textbf{0.119} & \textbf{0.019} & \textbf{0.187} & \textbf{0.398} & \textbf{0.083} & 0.008 & \textbf{0.107} & \textbf{0.224} & 0.036 & 0.006 & \underline{0.060} & \underline{0.123} & \textbf{2.0} & 1 \\
    \midrule
    Task  & \multicolumn{2}{c}{TUL} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{TUL} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{TUL} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{TUL} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{TUL} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{Eff Ave\\Rank}}} & \multirow{2}{*}{\makecell{Eff\\Rank}} \\
    Metric & ACC@1↑ & F1↑ & Param↓ & Speed↓ & ACC@1↑ & F1↑ & Param↓ & Speed↓ & ACC@1↑ & F1↑ & Param↓ & Speed↓ & ACC@1↑ & F1↑ & Param↓ & Speed↓ & ACC@1↑ & F1↑ & Param↓ & Speed↓ &       &  \\
    \midrule
    SkipG & 0.625 & 0.317 & \textbf{2.632} & \textbf{2} & 0.452 & 0.243 & \textbf{2.013} & \textbf{3} & 0.314 & 0.085 & \textbf{0.937} & \textbf{1} & 0.158 & 0.047 & \textbf{2.513} & \textbf{3} & 0.123 & 0.138 & \textbf{0.414} & \textbf{1} & \textbf{1.0} & 1 \\
    Tale  & \textbf{0.699} & 0.429 & 8.611 & 5     & 0.395 & 0.219 & 8.111 & 12    & 0.609 & 0.360 & 2.910 & 2     & 0.300 & 0.164 & 9.919 & 13    & 0.329 & 0.151 & 1.107 & \textbf{1} & 4.4   & 6 \\
    Teaser & 0.608 & 0.307 & \underline{3.012} & \underline{3} & 0.464 & \underline{0.255} & \underline{2.318} & \underline{5} & 0.312 & 0.193 & \underline{1.064} & \textbf{1} & 0.173 & 0.152 & \underline{2.986} & \underline{5} & 0.556 & 0.184 & \underline{0.464} & \textbf{1} & \underline{1.8} & 2 \\
    Hier  & 0.635 & 0.347 & 8.253 & 5     & 0.493 & 0.251 & 7.631 & 8     & 0.521 & 0.289 & 6.550 & 2     & 0.136 & 0.142 & 8.133 & 9     & 0.557 & 0.242 & 6.025 & \textbf{1} & 4.2   & 4 \\
    P2Vec & 0.629 & 0.323 & 7.142 & 7     & 0.451 & 0.243 & 2.735 & 12    & 0.647 & 0.413 & 1.410 & 2     & \underline{0.386} & \underline{0.169} & 3.346 & 11    & 0.517 & 0.256 & 1.496 & \textbf{1} & 3.6   & 3 \\
    CACSR & 0.645 & \underline{0.431} & 9.921 & 43    & \underline{0.502} & 0.249 & 8.301 & 114   & \underline{0.659} & \underline{0.462} & 5.439 & 21    & 0.361 & 0.156 & 9.715 & 68    & \underline{0.611} & \underline{0.295} & 4.059 & 7     & 6.7   & 7 \\
    CTLE  & \underline{0.698} & \textbf{0.444} & 3.436 & 8     & \textbf{0.507} & \textbf{0.294} & 2.814 & 13    & \textbf{0.772} & \textbf{0.628} & 1.734 & 4     & \textbf{0.485} & \textbf{0.243} & 3.316 & 12    & \textbf{0.628} & \textbf{0.323} & 1.209 & \textbf{1} & 4.2   & 4 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:poi}%
\end{table*}%
}


\subsection{Evaluation \& Config Modules}

The evaluation module provides an {\em evaluation()} interface to measure the performance of \rl models on downstream tasks. \fullname offers a range of metrics tailored to different tasks. Specifically, it includes MAE, MSE, RMSE, R$^2$, and MAPE for regression tasks; Accuracy, Precision@k, Recall@k, F1@k, and Mean Rank (MR) for classification tasks; and Accuracy@k and MR for trajectory similarity search tasks.

The config module provides a configuration file as an interface for users to arrange the ``pre-training $\rightarrow$ fine-tuning $\rightarrow$ evaluation'' pipeline. To train and test a model using \name, users simply specify the required pre-built or custom models and functions for each step in the pipeline within the configuration file. The library then automatically generates the necessary script to run experiments based on this configuration. Users only need to execute the script, and \name will invoke the interface functions of each module to complete the experiment.


\section{Performance Benchmark}\label{sec:experiment}


In this section, we present performance comparison experiments for the pre-built \rl models in \name. These experiments serve three purposes: $i$) Demonstrating Usability and Power: To show that \name is a user-friendly and powerful toolkit for \rl model development and evaluation. $ii$) Establishing Performance Benchmarks: To provide standard performance benchmarks for mainstream \rl models using the datasets pre-loaded in \name. $iii$) Analyzing Component Contributions: To explore the contributions of different components in existing \rl models, offering insights for designing more effective and robust models.



\subsection{Datasets and Experimental Setups}

\subsubsection{Datasets} The dataset selection for our experiments follows these guiding principles: for each type of \rl model, we incorporate all datasets that meet the task requirements. Specifically, for POI-oriented \rl models, we use datasets from New York City, Chicago, Tokyo, Singapore, and San Francisco. For road-segment-oriented models, the datasets include Beijing, Xi'an, Chengdu, Porto, and San Francisco. For land-parcel-oriented models, we use datasets from Beijing, Xi'an, Chengdu, Porto, and San Francisco. Each dataset is divided into training, validation, and test sets following a 6:2:2 ratio, ensuring a balanced and reliable performance evaluation. For each downstream task, we apply end-to-end fine-tuning to achieve optimal performance.  


\subsubsection{Experimental Settings} In our experiments, the dimension of map entity representation vectors across all models is set to 128. For other model configurations, such as the number of layers and the dimensions of intermediate variables, we adopt the default settings from the original papers as initial values. We then use a trial-and-error approach to tune the parameters on each dataset, searching for the best performance configurations. All experiments are executed on an Ubuntu 20.04 system equipped with NVIDIA GeForce 3090 GPUs. The default batch size during model training is set to 64. In cases of out-of-memory (OOM) issues, the batch size is halved iteratively, with a minimum batch size of 8.




% Table generated by Excel2LaTeX from sheet 'Road3'
\begin{table*}[htbp]
  \centering
  \vspace{-0.3cm}
  \caption{Performance comparison of road segment \rl methods on various datasets.}
  \vspace{-0.3cm}
  \resizebox{0.98\textwidth}{!}{
  \setlength{\tabcolsep}{0.5mm}
    \begin{tabular}{c|cccc|cccc|cccc|cccc|cccc|cc}
    \toprule
    Dataset & \multicolumn{4}{c|}{Beijing}  & \multicolumn{4}{c|}{Chengdu}   & \multicolumn{4}{c|}{Xi'an}    & \multicolumn{4}{c|}{Porto}    & \multicolumn{4}{c|}{San Francisco} & \multicolumn{2}{c}{Overall} \\
    \midrule
    Task  & \multicolumn{2}{c}{ASI} & \multicolumn{2}{c|}{TTE} & \multicolumn{2}{c}{ASI} & \multicolumn{2}{c|}{TTE} & \multicolumn{2}{c}{ASI} & \multicolumn{2}{c|}{TTE} & \multicolumn{2}{c}{ASI} & \multicolumn{2}{c|}{TTE} & \multicolumn{2}{c}{ASI} & \multicolumn{2}{c|}{TTE} & \multirow{2}{*}{\makecell{Per Ave\\Rank}} & \multirow{2}{*}{\makecell{Per\\Rank}} \\
    Metric & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ & MAE↓  & RMSE↓ &       &  \\
    \midrule
    RN2Vec & 3.566 & 5.744 & 656.6 & 3050  & 6.490 & 13.90 & 105.9 & 154.8 & 6.237 & 12.72 & 130.38 & 190.5 & 4.380 & 7.896 & 97.8  & 144.5 & 2.978 & 5.797 & 289.0 & 1479  & 6.0   & 7 \\
    HRNR  & 3.157 & 5.508 & 625.1 & 3066  & 6.364 & 13.66 & 100.26 & 149.78 & 5.672 & 11.11 & 129.24 & 191.1 & 4.357 & 7.867 & 104.5 & 150.2 & 2.510 & 5.374 & 287.8 & 1445  & 5.8   & 6 \\
    SARN  & 2.798 & 5.479 & 566.8 & 2578  & \underline{6.025} & 13.41 & 95.64 & 148.3 & \textbf{5.315} & \textbf{10.60} & 117.0 & \textbf{178.7} & 4.286 & 7.779 & 99.5  & 145.8 & 2.481 & 5.303 & 279.0 & 1502  & 4.1   & 5 \\
    Toast & 2.837 & 5.512 & 513.0 & 2499  & 6.377 & 13.62 & \underline{90.7} & \underline{145.4} & 5.619 & 10.96 & \underline{116.3} & 184.9 & 4.354 & 7.883 & 96.4  & 144.6 & 2.553 & \underline{5.295} & \textbf{246.4} & \textbf{1270} & 3.6   & 4 \\
    HRoad & \textbf{2.726} & \textbf{5.411} & 610.3 & 2527  & \textbf{5.970} & \textbf{13.22} & 96.24 & 146.6 & 5.537 & \underline{10.81} & 116.6 & 187.4 & \underline{4.212} & \textbf{7.693} & 97.2  & \underline{144.3} & \underline{2.476} & \textbf{5.250} & 287.6 & 1546  & 3.5   & 3 \\
    START & \underline{2.738} & \underline{5.445} & \underline{509.4} & \underline{2489} & 6.066 & 13.47 & 92.3  & 145.9 & \underline{5.503} & 10.92 & 116.4 & \underline{183.4} & \textbf{4.210} & 7.792 & \underline{95.8} & 145.7 & \textbf{2.450} & 5.333 & \underline{261.8} & 1431  & \textbf{2.6} & 2 \\
    JCLRNT & 2.771 & 5.466 & \textbf{475.9} & \textbf{2442} & 6.354 & \underline{13.27} & \textbf{90.2} & \textbf{142.7} & 5.660 & 11.02 & \textbf{115.9} & 183.5 & 4.267 & \underline{7.699} & \textbf{94.6} & \textbf{143.4} & 2.534 & 5.368 & 264.5 & \underline{1416} & \underline{2.4} & 1 \\
    \midrule
    \midrule
    Task  & \multicolumn{2}{c}{STS} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{STS} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{STS} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{STS} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{STS} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{Eff Ave\\Rank}}} & \multirow{2}{*}{\makecell{Eff\\Rank}} \\
    Metric & ACC@3↑ & MR↓   & Param↓ & Speed↓ & ACC@3↑ & MR↓   & Param↓ & Speed↓ & ACC@3↑ & MR↓   & Param↓ & Speed↓ & ACC@3↑ & MR↓   & Param↓ & Speed↓ & ACC@3↑ & MR↓   & Param↓ & Speed↓ &       &  \\
    \midrule
    RN2Vec & 0.789 & 10.53 & 5.192 & 331   & 0.631 & 45.32 & \underline{0.708} & 19    & 0.695 & 11.208 & \underline{0.826} & 16    & 0.893 & 8.296 & \underline{1.453} & \textbf{3} & \underline{0.976} & \underline{6.179} & \underline{3.524} & 35    & \textbf{2.7} & 2 \\
    HRNR  & 0.809 & 9.915 & 5.699 & 281   & 0.698 & 37.12 & 1.188 & \textbf{5} & 0.709 & 10.580 & 1.321 & \textbf{4} & 0.807 & 11.170 & 1.948 & 80    & 0.915 & 6.988 & 4.066 & \underline{23} & 3.6   & 4 \\
    SARN  & 0.892 & 9.176 & \textbf{0.570} & \textbf{30} & 0.563 & 40.31 & \textbf{0.549} & \textbf{5}     & 0.686 & 7.384 & \textbf{0.551} & \underline{5} & 0.883 & 8.753 & \textbf{0.551} & \underline{10} & 0.963 & 6.879 & \textbf{0.563} & \textbf{19} & \underline{1.2} & 1 \\
    Toast & 0.828 & 9.755 & 10.01 & 495   & 0.678 & 18.64 & 1.840 & 192   & 0.749 & 5.874 & 1.566 & 132   & 0.895 & 9.031 & 3.045 & 252   & \textbf{0.978} & \textbf{5.934} & 7.021 & 253   & 6.0   & 6 \\
    HRoad & \underline{0.947} & \underline{8.491} & 5.398 & \underline{66} & 0.583 & 32.05 & 0.913 & 6     & 0.736 & 7.122 & 1.031 & 5     & 0.895 & 10.152 & 1.660 & 11    & 0.947 & 8.491 & 3.728 & 44    & 3.3   & 3 \\
    START & \textbf{0.948} & \textbf{7.867} & 6.238 & 1719  & \underline{0.713} & \underline{15.59} & 2.139 & 582   & \underline{0.755} & \underline{5.411} & 2.002 & 312   & \underline{0.905} & \underline{6.702} & 2.745 & 735   & 0.934 & 6.828 & 4.743 & 783   & 6.7   & 7 \\
    JCLRNT & 0.879 & 9.034 & \underline{5.114} & 434   & \textbf{0.724} & \textbf{14.34} & 1.049 & 287   & \textbf{0.797} & \textbf{4.746} & 0.912 & 150   & \textbf{0.927} & \textbf{4.778} & 1.649 & 345   & 0.957 & 6.284 & 3.630 & 198   & 4.3   & 5 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:road}%
\end{table*}%

\subsection{Overall Experimental Results}\label{sec:result}

\subsubsection{Experimental Results for POI \rl} Table~\ref{tab:poi} presents the performance of \rl models on downstream tasks, including POI Classification (POIC), Next POI Prediction (NPP), and Trajectory User Link (TUL). Each task is evaluated using two types of metrics. Additionally, model efficiency is assessed with two indicators: the number of parameters (Param) in millions and the time cost per epoch during pre-training (Speed) in seconds. The table also reports average performance rankings across tasks (\textit{Pre Ave Rank}) and the ranking based on the models' average performance (\textit{Pre Rank}). Similarly, efficiency rankings are given by \textit{Eff Ave Rank} and \textit{Eff Rank}. From Tab.~\ref{tab:poi}, we have the following observations.

1) {\em Importance of Sequence-based Encoders}: Models combining token-based and sequence-based encoders -- such as CTLE, CACSR, and Hier -- consistently outperform those relying solely on token-based encoders, highlighting the value of trajectory auxiliary data. Among these, models using Augmented Trajectory Contrastive Learning (ATrCL) and Masked Trajectory Recovery (MTR) tasks (\eg, CTLE and CACSR) achieve better performance than those focused on Trajectory Prediction (TrajP) tasks (\eg, Hier). This is likely because ATrCL and MTR capture long-range temporal dependencies across entire trajectories, while TrajP focuses only on consecutive POI dependencies.

2) {\em Impact of Relation Networks}: For token-based models, those incorporating relation networks -- such as Teaser and P2Vec -- outperform models without them, such as SkipGram and Tale, underscoring the value of relation network auxiliary data. However, for models with both token-based and sequence-based encoders, the inclusion of relation networks offers little additional benefit. This is likely due to the sparsity of POI trajectories, where the number of trajectories between two POIs is often dictated by geographical proximity. As a result, the information provided by relation networks overlaps significantly with that from trajectory data. Once the dependency within the trajectory data has been fully exploited, the relational network contributes limited additional information.

3) {\em TokRI vs. TRCL Tasks}: Token-based models using the Token Relation Inference (TokRI) task, such as Tale and P2Vec, relatively outperform those employing the Token Relation Contrastive Learning (TRCL) task, such as SkipGram and Teaser. With sufficient data, supervised learning via TokRI effectively leverages labeled data to generate more discriminative feature representations. In contrast, the indirect nature of contrastive learning in TRCL offers less direct utilization of labeled information, resulting in comparatively lower model performance.

4) {\em Efficiency of Token-based Models}: Token-based models exhibit lower computational complexity, making them more efficient. This makes them especially suitable for application scenarios where computational resources are limited, and performance requirements can be moderately compromised.

%\vspace{-0.2cm}
\subsubsection{Experimental Results for Road Segment \rl}

Table~\ref{tab:road} shows a performance comparison of road segment \rl models across three downstream tasks: Average Speed Inference (ASI), Travel Time Estimation (TTE), and Similarity Trajectory Search (STS). The following key observations can be drawn from the results:

1) {\em Full Pipeline Models Perform Best}: Models utilizing the complete token-graph-sequence pipeline, such as JCLRNT and START, achieve the highest performance compared to models with partial pipelines. Additionally, token-based + graph-based and token-based + sequence-based models -- such as HRNR, SARN, Toast, and HRoad -- outperform purely token-based models like RN2Vec, highlighting the value of integrating trajectory and relation network information. Graph-based and sequence-based encoders capture essential patterns that improve road segment representations.

2) {\em Multiple Pre-training Tasks Improve Performance}: Models with multiple types of pre-training tasks, \ie Toast, HRoad, START, and JCLRNT, outperform those with single-task pre-training, \ie HRNR and SARN. Notably, among token-based + graph-based models, HRoad, which integrates both NFI and GAu tasks, surpasses HRNR (GAu only) and SARN (AGCL only). Using diverse pre-training tasks enables the model to extract information from multiple perspectives, enhancing its ability to learn more comprehensive feature representations. Moreover, in the full-pipeline models, JCLRNT combines a sequence-oriented task (Augmented Trajectory Contrastive Learning) with a graph-oriented task (Augmented Graph Contrastive Learning) and outperforms START, which uses two sequence-oriented tasks (MTR and ATrCL). This suggests that even in models with multiple tasks, greater task heterogeneity can further enhance performance.


3) {\em Efficiency Trade-offs}: Simpler models with fewer modules, such as SARN and RN2Vec, are significantly more efficient. Models without sequence encoders, such as HRNR and HRoad, also exhibit better efficiency since incorporating trajectory data demands considerable memory and time. Improving the efficiency of trajectory-based models remains a key challenge for future research.




% Table generated by Excel2LaTeX from sheet 'Region3'
\begin{table*}[htbp]
  \centering
  \vspace{-0.3cm}
  \caption{Performance comparison of land parcel \rl methods on various datasets.}
  \vspace{-0.3cm}
  \resizebox{0.95\textwidth}{!}{
  \setlength{\tabcolsep}{0.5mm}
    \begin{tabular}{c|cccc|cccc|cccc|cccc|cccc|cc}
    \toprule
    Dataset & \multicolumn{4}{c|}{Beijing}  & \multicolumn{4}{c|}{Chengdu}   & \multicolumn{4}{c|}{Xi'an}    & \multicolumn{4}{c|}{Porto}    & \multicolumn{4}{c|}{San Francisco} & \multicolumn{2}{c}{Overall} \\
    \midrule
    Task  & \multicolumn{2}{c}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c}{LPC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c}{LPC} & \multicolumn{2}{c|}{FI} & \multirow{2}{*}{\makecell{Per Ave\\Rank}} & \multirow{2}{*}{\makecell{Per\\Rank}} \\
    Metric & ACC@1↑ & F1↑ & MAE↓  & RMSE↓ & ACC@1↑ & F1↑ & MAE↓  & RMSE↓ & ACC@1↑ & F1↑ & MAE↓  & RMSE↓ & ACC@1↑ & F1↑ & MAE↓  & RMSE↓ & ACC@1↑ & F1↑ & MAE↓  & RMSE↓ &       &  \\
    \midrule
    ZEMob & 0.380 & 0.110 & 30.90 & 55.19 & 0.339 & 0.115 & 154.9 & 441.2 & 0.316 & 0.138 & 133.7 & 326.2 & 0.298 & 0.204 & {527.5} & {595.1} & 0.820 & 0.477 & 509.1 & 910.5 & 5.2  & 7 \\
    GMEL  & 0.412 & 0.571 & \underline{27.68} & 58.91 & 0.338 & 0.109 & 154.8 & 441.1 & 0.330 & 0.359 & 133.1 & \underline{324.4} & 0.267 & 0.335 & {525.1} & {591.9} & 0.620 & \textbf{0.550} & 514.0 & 916.7 & 4.5  & 6 \\
    MGFN  & \underline{0.567} & \underline{0.601} & 30.09 & 54.45 & 0.345 & 0.135 & 154.6 & 448.2 & 0.330 & 0.162 & 132.7 & 324.9 & 0.304 & 0.246 & {531.3} & {596.9} & \underline{0.835} & 0.533 & 605.3 & 1011  & 4.4  & 5 \\
    HDGE  & 0.409 & 0.229 & 29.26 & 54.82 & 0.365 & 0.157 & 159.6 & 402.1 & 0.473 & 0.242 & 134.1 & 334.5 & 0.327 & 0.263 & {525.2} & {\underline{576.9}} & 0.820 & 0.450 & 511.8 & 926.4 & 4.3  & 4 \\
    MVURE & 0.479 & 0.267 & 28.13 & \underline{51.37}& 0.485 & 0.279 & 161.5 & 450.2 & 0.545 & 0.235 & 133.7 & 326.0 & 0.316 & 0.294 & {\underline{524.8}} & {592.4} & 0.820 & 0.450 & 511.2 & 913.1 & 4.1  & 3 \\
    ReMVC & \textbf{0.722} & \textbf{0.686} & 27.81 & 52.66 & \textbf{0.610} & \textbf{0.542} & \underline{147.7} & \underline{430.9} & \underline{0.567} & \underline{0.412} & \underline{131.5} & 324.6 & \textbf{0.404} & \underline{0.357} & {527.3} & {594.8} & 0.820 & 0.450 & \underline{444.7} & \underline{852.3} & \underline{3.0} & 2 \\
    HREP  & 0.524 & 0.405 & \textbf{22.91} & \textbf{45.85} & \underline{0.528} & \underline{0.445} & \textbf{124.0} & \textbf{309.6} & \textbf{0.611} & \textbf{0.494} & \textbf{127.9} & \textbf{312.3} & \underline{0.386} & \textbf{0.358} & {\textbf{498.0}} & {\textbf{574.5}} & \textbf{0.836} & \underline{0.538} & \textbf{438.4} & \textbf{799.3} & \textbf{2.2} & 1 \\
    \midrule
    \midrule
    Task  & \multicolumn{2}{c}{MI} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{MI} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{MI} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{MI} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{2}{c}{MI} & \multicolumn{2}{c|}{Efficiency} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{Eff Ave\\Rank}}} & \multirow{2}{*}{\makecell{Eff\\Rank}} \\
    Metric & MAE↓  & RMSE↓ & \multicolumn{1}{l}{Param↓} & \multicolumn{1}{l|}{Speed↓} & MAE↓  & RMSE↓ & \multicolumn{1}{l}{Param↓} & \multicolumn{1}{l|}{Speed↓} & MAE↓  & RMSE↓ & \multicolumn{1}{l}{Param↓} & \multicolumn{1}{l|}{Speed↓} & MAE↓  & RMSE↓ & \multicolumn{1}{l}{Param↓} & \multicolumn{1}{l|}{Speed↓} & MAE↓  & RMSE↓ & \multicolumn{1}{l}{Param↓} & \multicolumn{1}{l|}{Speed↓} &       &  \\
    \midrule
    ZEMob & 0.379 & 0.771 & 45.10 & 40 & \textbf{3.599} & 29.66 & 7.699 & 19  & \underline{3.776} & 17.63 & 5.670 & \textbf{1} & {44.85} & {72.30} & 1.047 & \textbf{1} & \textbf{5.837} & 23.48 & 2.335 & \textbf{1} & 4.0  & 3 \\
    GMEL  & 0.418 & 0.712 & \underline{0.118} & 713   & \underline{4.599} & 29.66 & \underline{0.118} & 193   & \textbf{3.668} & 17.60 & \underline{0.118} & 189   & {41.08} & {57.41} & 0.118 & 161   & 7.377 & 22.29 & 0.118 & 2  & 4.0 & 3 \\
    MGFN  & 0.283 & 0.694 & 1156  & 839  & 5.176 & 29.23 & 485.7 & \textbf{6} & 3.889 & 17.23 & 318   & 2  & {39.37} & {\underline{56.16}} & 53.67 & 2  & 6.846 & 22.22 & 42.19 & \textbf{1}  & 5.4  & 7 \\
    HDGE  & 0.389 & 0.759 & 12.91 & 1799  & 5.189 & \underline{29.00} & 1.505 & 601 & 3.863 & \textbf{16.85} & 1.217 & 75    & {38.69} & {\textbf{54.20}} & 0.440 & 117   & 7.397 & \underline{21.94} & 0.223 & 3  & 5.1  & 6 \\
    MVURE & \underline{0.281} & 0.685 & \textbf{0.097} & \underline{12} & 5.200 & 29.37 & \textbf{0.097} & 8   & 3.941 & 17.41 & \textbf{0.097} & \textbf{1} & {\underline{38.63}} & {62.21} & \underline{0.097} & \textbf{1} & 7.196 & 22.73 & \underline{0.097} & \textbf{1} & \textbf{2.1} & 1 \\
    ReMVC & \textbf{0.276} & \textbf{0.667} & 1.450 & 873   & 5.230 & 29.42 & 0.181 & 582   & 3.986 & 17.40 & 0.149 & 39    & {40.34} & {56.66} & \textbf{0.069} & 47  & 7.007 & 22.60 & \textbf{0.050} & 7  & 4.1  & 5 \\
    HREP  & 0.318 & \underline{0.677} & 0.182 & \textbf{9} & 5.270 & \textbf{28.33} & 0.182 & \underline{7}  & 3.949 & \underline{17.05} & 0.182 & \textbf{1} & {\textbf{37.42}} & {57.62} & 0.182 & 2  & \underline{6.754} & \textbf{21.71} & 0.182 & \textbf{1}  & \underline{3.3} & 2 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:region}%
  \vspace{-0.3cm}
\end{table*}%


\subsubsection{Experimental Results for Land Parcel \rl}

Table~\ref{tab:region} presents the performance comparison of land parcel \rl models on the downstream tasks of Land Parcel Classification (LPC), Flow Inference (FI), and Mobility Inference (MI). The following observations can be made:

1) {\em Incorporating POI Data Enhances Performance}: Models that utilize POI data, such as MVURE, ReMVC, and HREP (see the ``Map Entities'' column in Table~\ref{tab:models}), outperform those that do not. These models treat POI categories within a land parcel as features, enriching the representation of the parcel's functional characteristics. This approach provides valuable contextual information, improving the overall performance of the models.

2) {\em Limitations of Current Encoder Structures}: Most existing land parcel \rl models adopt a token-based + graph-based encoder structure, focusing on extracting information from relation networks. However, these models overlook the sequential dependencies within trajectories, limiting their effectiveness. Future research should explore advanced methods to capture trajectory sequence information relevant to land parcels for further improvements.

3) {\em Need for More Diverse Pre-training Tasks}: Current models mainly rely on the Graph Autoencoder (GAu) task for pre-training. However, experimental results show that tasks such as Augmented Token Contrastive Learning (AToCL) and Neighborhood Contrastive Learning (NCL) also yield good performance. Developing models that incorporate a broader range of pre-training tasks is a promising direction for enhancing land parcel \rl models.


\subsubsection{Summary for Overall Experiments} The overall experimental results highlight the following key findings across POI, road segment, and land parcel \rl models.

1) {\em Importance of Combined Encoders}:  Models employing a combination of token-based, graph-based, and sequence-based encoders consistently outperform those relying on single-type encoders. This demonstrates the value of integrating multiple data sources -- such as trajectories and relation networks -- to capture complex spatial, temporal, and relational patterns.

2) {\em Effectiveness of Diverse Pre-training Tasks}: Models that leverage multiple pre-training tasks usually perform better than those limited to a single task. This suggests that diverse pre-training strategies enhance the model's ability to learn comprehensive feature representations from different perspectives.

3) {\em Role of Auxiliary Data}: Incorporating POI, trajectory, and relation network data improves model performance across tasks. However, models that fully exploit trajectory dependencies achieve diminishing gains from relation networks, indicating some redundancy between these data sources.

4) {\em Trade-offs Between Performance and Efficiency}: While complex models with multiple encoders and tasks offer higher accuracy, they require more computational resources. Simpler token-based models remain attractive for applications where efficiency is critical, despite offering slightly lower performance.





\subsection{Performance over Small Datasets}\label{sec:smalldataset}

In the overall experiments, both the pre-training and fine-tuning steps are executed on the full training dataset. However, in practical applications, \rl models are often trained on abundant data while fine-tuned using limited labeled samples for downstream tasks. To assess the robustness of mainstream models under such conditions, we conduct a small dataset experiment.

In this experiment, we reduce the fine-tuning data size from 50\% to 10\% of the original training set and compare the result of pre-built models in \name. POI-oriented models are evaluated on the Tokyo dataset, while road-segment and land-parcel-oriented models are tested on the Xi'an dataset. Figure~\ref{fig:dive} presents the evaluation result: \fig~\ref{fig:dive}~(a) to (c) show results for POI-oriented models. \fig~\ref{fig:dive}~(d) to (f) display results for road-segment-oriented models. \fig~\ref{fig:dive}~(g) to (i) provide results for land-parcel-oriented models. From these figures, we make following observations:

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/dive_all.pdf}
    \caption{Results from varying fine-tuning data size.}
    \vspace{-0.2cm}
    \label{fig:dive}
    \vspace{-0.4cm}
\end{figure}

1) {\em Stability in Attribute Inference Tasks}: \rl models show stable performance across varying training data sizes in attribute inference tasks, such as POI Classification (POIC) in \fig~\ref{fig:dive}~(a), Average Speed Inference (ASI) in \fig~\ref{fig:dive}~(d), and Land Parcel Classification (LPC) in \fig~\ref{fig:dive}~(g). This stability arises because these tasks focus on inferring entity attributes, which are effectively captured during pre-training. As a result, the fine-tuning phase requires only a small amount of labeled data to maintain good performance.

2) {\em Fluctuations in Trajectory-Related Tasks}: Models show notable performance fluctuations in trajectory-related tasks, such as Next POI Prediction (NPP) in \fig~\ref{fig:dive}~(b), Trajectory User Link (TUL) in \fig~\ref{fig:dive}~(c), and Travel Time Estimation (TTE) in \fig~\ref{fig:dive}~(e). These tasks rely on sequence-level predictions, while encoders and pre-training tasks mostly focus on generating single-vector representations for individual entities. This mismatch makes trajectory-related tasks more sensitive to the size of the fine-tuning dataset, as limited labels reduce the model's ability to learn sequential dependencies effectively. For Similarity Trajectory Search (STS) in \fig~\ref{fig:dive}~(f), although it is a trajectory-related task, it involves similarity comparison rather than prediction so it is less affected by this mismatch.

3) {\em Fluctuations in Flow and Mobility Inference Tasks}: Models also show significant performance fluctuations in Flow Inference (FI) in \fig~\ref{fig:dive}~(h) and Mobility Inference (MI) in \fig~\ref{fig:dive}~(i), even though these tasks are not directly related to trajectory data. This is because the labels for these tasks reflect statistical data on human mobility flows over specific periods, which are highly time-heterogeneous, with label distributions varying significantly across periods. As a result, more labeled data is required to capture these complex temporal patterns accurately. 

Overall, existing \rl models exhibit varying sensitivity to the size of labeled data across different tasks. For tasks less influenced by temporal information, such as attribute inference (ASI, POIC, LPC) and Similarity Trajectory Search (STS), models maintain stable performance even with limited training data. However, for tasks with time-dependent labels, such as trajectory-related tasks (NPP, TUL, TTE) and flow/mobility inference tasks (FI, MI), larger amounts of labeled data are necessary to effectively capture temporal dynamics.


%\subsection{Comparing Different Model Architectures.}\label{sec:pretraintask}
%However, whether there is a direct relationship between the number of pretraining tasks and performance improvement remains unclear. In Section~\ref{sec:pretraintask}, we explore the impact of pretraining task selection and combinations on model performance.
%This aims to avoid the computational overhead of excessive tasks while maximizing performance improvements.


% Table generated by Excel2LaTeX from sheet 'Ablation2'
% \begin{table}[t]
%   \centering
%     \vspace{-0.3cm}
%   \caption{Results for CTLE variants on the Tokyo dataset.}
%     \vspace{-0.3cm}
%   \resizebox{0.95\columnwidth}{!}{
%   \setlength{\tabcolsep}{1.6mm}
%     \begin{tabular}{cc|ccccc}
%         \toprule
%     \multicolumn{2}{c|}{Methods} & \multicolumn{1}{c}{CTLE} & CTLE\% & CTLE\& & \multicolumn{1}{c}{CTLE*} & CTLE\$ \\
%     \midrule
%     \multicolumn{2}{c|}{\multirow{1}{*}{Encoder Core Arc}}  & \multicolumn{1}{c}{TE} & \multicolumn{1}{c}{TE} & \multicolumn{1}{c}{TE} & \multicolumn{1}{c}{TE} & \textcolor[rgb]{ 1,  0,  0}{LSTM} \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{3}[1]{*}{\makecell{Pretraining \\ Task}}} & \multicolumn{1}{c|}{TrajP} & \multicolumn{1}{c}{\ding{51}} & \ding{51}     & \textcolor[rgb]{ 1,  0,  0}{\ding{55}} & \ding{51}     & \multicolumn{1}{c}{\ding{51}} \\
%           & \multicolumn{1}{c|}{MTR} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\textcolor[rgb]{ 1,  0,  0}{\ding{55}}} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\ding{51}} \\
%           & \multicolumn{1}{c|}{ATrCL} & \multicolumn{1}{c}{\ding{55}} & \ding{55} & \ding{55} & \textcolor[rgb]{ 1,  0,  0}{\ding{51}} & \ding{55} \\
%     \midrule
%     \multirow{2}[1]{*}{POIC} & ACC@1↑ & \underline{0.048} & 0.032 & 0.041 & \textbf{0.050} & 0.043 \\
%           & F1↑ & \underline{0.006} & 0.002 & 0.005 & \textbf{0.007} & 0.006 \\
%     \multirow{2}[0]{*}{NPP} & ACC@1 & \underline{0.154} & 0.089 & 0.153 & \textbf{0.165} & 0.058 \\
%           & ACC@5↑ & \underline{0.336} & 0.193 & 0.332 & \textbf{0.352} & 0.147 \\
%     \multirow{2}[1]{*}{TUL} & ACC@1 & \underline{0.698} & 0.401 & 0.687 & \textbf{0.699} & 0.388 \\
%           & F1↑ & \underline{0.444} & 0.160 & 0.437 & \textbf{0.448} & 0.104 \\
%     \midrule
%     \multicolumn{2}{c|}{Per Rank} & 2     & 5     & 3     & 1 & 4 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:abl_poi}%
%     \vspace{-0.6cm}
% \end{table}%
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/rebuttal/top5_rank_poi.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/rebuttal/top5_rank_road.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/rebuttal/top5_rank_region.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

\begin{figure*}
    \centering
    \subfigure[Top 3 combinations for POI map entity.]{\includegraphics[width=0.33\textwidth]{figures/rebuttal/top5_rank_poi.pdf}}
    \subfigure[Top 3 combinations for segment map entity.]{\includegraphics[width=0.33\textwidth]{figures/rebuttal/top5_rank_road.pdf}}
    \subfigure[Top 3 combinations for parcel map entity.]{\includegraphics[width=0.33\textwidth]{figures/rebuttal/top5_rank_region.pdf}}
    \vspace{-4mm}
    \caption{Top 3 pretraining task combinations' preformance.}
    \vspace{-4mm}
    \label{fig:merged_images}
\end{figure*}


\vspace{-0.2cm}
\subsection{Comparing of Modified Models}\label{sec:pretraintask}

In this section, we conduct experiments to evaluate the influence of pre-training tasks and encoder structures on the performance of downstream tasks. We modify three representative \rl models -- CLTE, JCLRNT, and HREP -- which achieve the highest average performance in POI, road segment, and land parcel representation learning, respectively. Owing to \name's modular design, specific pre-training tasks can be easily removed from models, and new pre-training tasks can be seamlessly integrated.

The experimental results are shown in \tab\ref{tab:abl_poi} -- \ref{tab:abl_region}. In the figures, the black ``\ding{51}'' and ``\ding{55}'' indicate whether the corresponding pre-training tasks were originally included or excluded when the model was first proposed. In contrast, the red ``\textcolor[rgb]{1,0,0}{\ding{51}}'' and ``\textcolor[rgb]{1,0,0}{\ding{55}}'' indicate newly added or removed pre-training tasks. Additionally, we evaluate the impact of different backbone models by modifying the core architecture of encoders (highlighted in red in the ``Encoder Core Arc'' row). In the last row, we present the performance ranking of each variant for easier comparison and conclusion.


\paratitle{Comparison of CTLE Variants.} Among POI \rl models, CTLE achieves the best performance. In \tab\ref{tab:abl_poi}, we experiment with the following model variants for CTLE. 
(a) {\em CTLE}: Maintains the original model architecture.
(b) {\em CTLE\%}: Removes the Masked Trajectory Recovery (MTR) pre-training task.
(c) {\em CTLE\&}: Removes the Trajectory Prediction (TrajP) pre-training task.
(d) {\em CTLE*}: Integrates a new Augmented Trajectory Contrastive Learning (ATrCL) pre-training task, using the ATrCL task proposed by CACSR, which achieved the second-best performance in the overall POI experiments.
(e) {\em CTLE\$}: Replaces the core architecture of CTLE (a Transformer encoder) with an LSTM layer.

The downstream task results are presented in \tab\ref{tab:abl_poi}. From these experiments, we draw the following observations: $i$) {\em New Task Enhances Performance:} The CTLE* variant achieves the best performance across all downstream tasks, indicating that integrating the new ATrCL task significantly improves the model's capability. $ii$) {\em MTR Provides Richer Representations}: The CTLE\& variant outperforms CTLE\%, suggesting that the MTR task offers richer representation capabilities than the TrajP task. $iii$) {\em Transformer Encoder is Essential for Trajectory Tasks:} The performance of CTLE\$ drops by 59\% in the Next POI Prediction (NPP) task and 60\% in the 
Trajectory User Link (TUL) task, showing that the Transformer Encoder (TE) plays a crucial role in trajectory-related tasks. % by enhancing the model's sequence encoding abilities.


% % Table generated by Excel2LaTeX from sheet 'Ablation2'
% \begin{table}[t]
%   \centering
%     \vspace{-0.3cm}
%   \caption{Results for JCLRNT variants on the Xi'an dataset.}
%     \vspace{-0.3cm}
%   \resizebox{0.95\columnwidth}{!}{
%   \setlength{\tabcolsep}{1mm}
%     \begin{tabular}{cc|cccccc}
%     \toprule
%     \multicolumn{2}{c|}{Methods} & \multicolumn{1}{c}{JCLRNT} & JCLRNT\% & JCLRNT\& & \multicolumn{1}{c}{JCLRNT*} & JCLRNT\$ \\
%     \midrule
%     \multicolumn{2}{c|}{\multirow{2}{*}{Encoder Core Arc}} & TE    & TE    & TE    & TE    & \textcolor[rgb]{ 1,  0,  0}{LSTM} \\
%     \multicolumn{1}{c}{} &       & \multicolumn{1}{c}{GAT} & \multicolumn{1}{c}{GAT} & \multicolumn{1}{c}{GAT} & \multicolumn{1}{c}{GAT} & \multicolumn{1}{c}{GAT} \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{3}[1]{*}{\makecell{Pretraining \\ Task}}} & \multicolumn{1}{c|}{TokRI} & \multicolumn{1}{c}{\ding{55}} & \multicolumn{1}{c}{\ding{55}} & \ding{55} & \textcolor[rgb]{ 1,  0,  0}{\ding{51}} & \multicolumn{1}{c}{\ding{55}} \\
%           & \multicolumn{1}{c|}{AGCL} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\textcolor[rgb]{ 1,  0,  0}{\ding{55}}} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\ding{51}} \\
%           & \multicolumn{1}{c|}{ATrCL} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\textcolor[rgb]{ 1,  0,  0}{\ding{55}}} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\ding{51}} \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{2}[1]{*}{ASI}} & MAE↓   & \underline{5.660} & 5.708 & 5.744 & \textbf{5.601} & 5.702 \\
%     \multicolumn{1}{c}{} & RMSE↓  & \underline{11.02} & 11.06 & 11.11 & \textbf{10.90} & 11.00 \\
%     \multicolumn{1}{c}{\multirow{2}[0]{*}{TTE}} & MAE↓   & \underline{115.9} & 118.3 & 116.5 & \textbf{115.3} & 124.5 \\
%     \multicolumn{1}{c}{} & RMSE↓  & \underline{183.5} & 185.5 & 183.8 & \textbf{182.3} & 189.8 \\
%     \multicolumn{1}{c}{\multirow{2}[1]{*}{STS}} & ACC@3↑ & \underline{0.797} & 0.673 & 0.702 & \textbf{0.809} & 0.782 \\
%     \multicolumn{1}{c}{} & MR↓    & \underline{4.746} & 12.30 & 5.828 & \textbf{3.176} & 5.325 \\
%     \midrule
%     \multicolumn{2}{c|}{Per Rank} & 2 & 5 & 4 & 1 & 3 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:abl_road}%
%     \vspace{-0.5cm}
% \end{table}%

\paratitle{Comparison of JCLRNT Variants.}
Among road segment \rl models, JCLRNT achieves the best performance. As shown in \tab\ref{tab:abl_road}, we experiment with the following JCLRNT variants. (a) {\em JCLRNT:} Maintains the original model architecture.
(b) {\em JCLRNT\%:} Removes the ATrCL pre-training task.
(c) {\em JCLRNT\&:} Removes the Augmented Graph Contrastive Learning (AGCL) pre-training task.
(d) {\em JCLRNT*:} Adds a new Token Relation Inference (TokRI) pre-training task, using road type classification, as implemented in HRoad.
(e) {\em JCLRNT\$:} Replaces the Transformer with an LSTM as the sequence encoder.

The performance results on downstream tasks are presented in \tab\ref{tab:abl_road}. From the experimental results, we draw the following observations: $i$) {\em Comprehensive Pre-training Boosts Performance}:    JCLRNT* achieves the best performance across all downstream tasks by incorporating three pre-training tasks—TokRI, AGCL, and ATrCL—each aligned with the token-based, graph-based, and sequence-based encoders, respectively. This suggests that each encoder type benefits from having a tailored pre-training task. $ii$) {\em ATrCL Provides Richer Representations}: JCLRNT\% underperforms compared to JCLRNT\& in trajectory-related tasks like Travel Time Estimation (TTE) and Similarity Trajectory Search (STS). This indicates that ATrCL, a sequence-based pre-training task, offers richer representation capabilities than AGCL for these tasks. Even with a sequence encoder, the absence of ATrCL limits the model's ability to capture dependency effectively, impacting performance. $iii$) {\em Minor Impact of Replacing the Transformer Encoder:}    JCLRNT\$ shows relatively minor performance degradation when the Transformer Encoder is replaced by an LSTM. This suggests that the introduction of the graph encoder in JCLRNT helps extract relational information from network data, reducing the model's reliance on the Transformer.



% % Table generated by Excel2LaTeX from sheet 'Ablation2'
% \begin{table}[t]
%   \centering
%   \vspace{-0.3cm}
%   \caption{Results from HREP variants on the Xi'an dataset.}
%   \vspace{-0.3cm}
%   \resizebox{0.95\columnwidth}{!}{
%   \setlength{\tabcolsep}{1.2mm}
%     \begin{tabular}{cc|cccccc}
%     \toprule
%     \multicolumn{2}{c|}{Methods} & \multicolumn{1}{c}{HREP} & HREP\% & \multicolumn{1}{c}{HREP\&} & HREP* & HREP\$ \\
%     \midrule
%     \multicolumn{2}{c|}{\multirow{1}{*}{Encoder Core Arc}}  & \multicolumn{1}{c}{HeteGCN} & \multicolumn{1}{c}{HeteGCN} & HeteGCN & \multicolumn{1}{c}{HeteGCN} & \textcolor[rgb]{ 1,  0,  0}{GCN} \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{3}[1]{*}{\makecell{Pretraining \\ Task}}} & \multicolumn{1}{c|}{NFI} & \multicolumn{1}{c}{\ding{55}} & \multicolumn{1}{c}{\ding{55}} & \ding{55}     & \textcolor[rgb]{ 1,  0,  0}{\ding{51}} & \multicolumn{1}{c}{\ding{55}} \\
%           & \multicolumn{1}{c|}{GAu} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\textcolor[rgb]{ 1,  0,  0}{\ding{55}}} & \multicolumn{1}{c}{\ding{51}} & \multicolumn{1}{c}{\ding{51}} \\
%           & \multicolumn{1}{c|}{NCL} & \multicolumn{1}{c}{\ding{51}} & \textcolor[rgb]{ 1,  0,  0}{\ding{55}} & \ding{51} & \ding{51} & \multicolumn{1}{c}{\ding{51}} \\
%     \midrule
%     \multirow{2}[1]{*}{LPC} & ACC@1↑ & \underline{0.611} & 0.566 & 0.413 & \textbf{0.663} & 0.505 \\
%           & F1↑ & \underline{0.494} & 0.436 & 0.273 & \textbf{0.495} & 0.340 \\
%     \multirow{2}[0]{*}{FI} & MAE↓   & \underline{127.9} & 128.1 & 133.4 & \textbf{119.7} & 146.6 \\
%           & RMSE↓  & \underline{312.3} & 320.8 & 323.7 & \textbf{269.8} & 325.3 \\
%     \multirow{2}[1]{*}{MI} & MAE↓   & \underline{3.949} & 3.993 & 4.371 & \textbf{3.914} & 4.294 \\
%           & RMSE↓  & 17.05 & 18.58 & 17.69 & \textbf{15.62} & \underline{16.55} \\
%     \midrule
%     \multicolumn{2}{c|}{Per Rank} & 2     & 3     & 5     & 1 & 4 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:abl_region}%
%   \vspace{-0.6cm}
% \end{table}%

\paratitle{Comparison of HREP Variants.} Among land parcel \rl models, HREP achieves the best performance. As shown in \tab\ref{tab:abl_region}, we experiment with the following HREP variants.
(a) {\em HREP:} Maintains the original model architecture.
(b) {\em HREP\%:} Removes the Graph Autoencoder (GAu) pre-training task.
(c) {\em HREP\&:} Removes the Neighborhood Contrastive Learning (NCL) pre-training task.
(d) {\em HREP*:} Adds a new Node Feature Inference (NFI) pre-training task, incorporating human mobility inference, as implemented in MGFN.
(e) {\em HREP\$:} Replaces the heterogeneous GCN (HeteGCN) with a standard GCN as the graph encoder.

The performance results on downstream tasks are presented in \tab\ref{tab:abl_region}. From the experiments, we draw the following observations. $i$) {\em NFI Enhances Flow Inference Performance:} HREP* achieves the best results across all downstream tasks, including a 10\% improvement in the Flow Inference (FI) task, indicating that the NFI pre-training task significantly enhances the model's ability to predict flow-related information.
$ii$) {\em GAu Provides Richer Representations:} HREP\% outperforms HREP\&, suggesting that the GAu pre-training task is crucial for capturing relationships between entities and improving downstream task performance. $iii$) {\em HeteGCN Captures Diverse Entity Relationships:} HREP\$ experiences a significant performance drop, especially in the Land Parcel Classification (LPC) task, when the HeteGCN is replaced with a GCN. This indicates that HeteGCN better captures the diverse relationships between different types of entities, making it essential for land parcel representation learning.



\paratitle{Summary for Variant Experiments.} From the above experiments, we derive the following conclusions.

1) {\em More Types of Pre-training Tasks Lead to Better Performance:} Across all experiments, the best-performing models consistently incorporate the most diverse types of encoders and pre-training tasks. %For example, CTLE*, JCLRNT*, and HREP* achieve the highest performance by combining multiple pre-training tasks. 
This demonstrates that integrating a wider range of pre-training tasks enhances the model's ability.  %to learn comprehensive and robust representations.

2) {\em Suitable Pre-training Tasks Provide Greater Benefits:} Pre-training tasks tailored to specific downstream tasks significantly enhance performance. For instance, the Augmented Trajectory Contrastive Learning (ATrCL) task improves performance in trajectory-related tasks, such as Travel Time Estimation (TTE) and Similarity Trajectory Search (STS), while the Node Feature Inference (NFI) task greatly benefits Flow Inference (FI) tasks. This highlights the importance of aligning pre-training tasks with the specific requirements of downstream tasks to maximize model effectiveness.

3) {\em Encoder Architecture Matters for Task Performance:} The choice of encoder architecture has a significant effect. For instance, replacing the Transformer Encoder with an LSTM in CTLE and JCLRNT led to performance drops, especially in trajectory-related tasks. Similarly, HeteGCN outperforms a standard GCN in HREP by capturing more diverse entity relationships. 


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/rebuttal/time_tradeoff.pdf}
    \vspace{-8mm}
    \caption{Tradeoff between Model Paramters and Time Efficiency on average, across all avaliable dataset.}
    \label{fig:two_one_layout}
\end{figure}


==> backup2.tex <==
\section{Notations and Definitions}
%我们提供了地图实体的定义，并介绍了城市时空数据，包括GPS轨迹数据、POI 轨迹数据和OD数据。
In this section, we provide the definition of map entities and introduce urban spatial temporal data.
%一般来说，电子地图使用专门的时空数据文件格式进行组织，如 Shapefile 和 GeoJSON [main5] 文件，这些文件将地理坐标信息作为地图实体的专门属性。从几何角度看，地图实体可分为三类：点、线和区域

% \begin{figure}
%     \centering
%     \subfigure[Points]{
%     \includegraphics[width=0.3\linewidth]{figures/poi_cd.pdf}
%     }
%     \subfigure[Lines]{
%     \includegraphics[width=0.3\linewidth]{figures/road_cd.pdf}
%     }
%     \subfigure[Regions]{
%     \includegraphics[width=0.3\linewidth]{figures/region_cd.pdf}
%     }
%     \vspace{-2mm}
%     \caption{Comparison of performance across different training data size.}
%     \vspace{-2mm}
%     \label{fig:dive}
% \end{figure}



\subsection{Map Entities} In general, electronic maps are organized using specialized spatial-temporal data file formats, such as Shapefile and GeoJSON\cite{geojson} files, which incorporate geographic coordinate information as specialized attributes for map entities. From a geometry perspective, map entities can be classified into three categories: points, lines, and regions. \fig\ref{fig:entity} presents the urban map of Chengdu along with its associated entities.
% 点实体与一对几何坐标 $（纬度，经度）$ 相关联，通常用来表示地图上的兴趣点（POI）或 GPS 位置。线实体与一系列有序的点相关联，通常代表地图上的路段。区域实体与由点和封闭区域组成的边界相关联，通常代表地图上的行政区或人口普查区。每类实体都包括几个属性，如名称和类别。为方便起见，我们在下文中用 $v$ 表示地图实体，用 $\mathcal{V}$ 表示所有地图实体的集合。
% 一个点实体都对应着地图上的一个GPS location，由一对经纬度唯一标识，经常被用来表示POI。
A point entity corresponds to a pair of GPS coordinates $(latitude, longitude)$ and is commonly used to represent Points of Interest (POIs) or locations on the map. A line entity is associated with a series of ordered points, typically representing road segments. A region entity corresponds to a specific area on the map, typically representing administrative districts or census tracts. Each category of entity includes several auxiliary attributes, such as name and category. For convenience, we use $v$ to denote a map entity and $\mathcal{V}$ to represent the set of all map entities in the following.
%“A region entity corresponds to a functional area defined by a specific function or purpose, such as a living or residential area, or to statistical regions used for data collection and analysis, such as census tracts.”

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/entity.pdf}
    \caption{Urban Map with Corresponding map entities in Chengdu, China.}
    \label{fig:entity}
\end{figure}

% \subsection{Relations between Map Entitis} 
% %地图实体之间的关系有助于更好地学习实体表示。在以往的工作中，Road2Road 是一种常用的关系，表示路段是否相邻。研究人员通常通过构建一个道路网络，并采用图表示学习方法来增强路段表示，从而使用图结构来表示这种关系。另一个常用的关系是 POI2 区域，表示 POI 是否包含在某个区域内。这种关系通常用于区域表示学习。除了这两种关系外，还可以根据地理距离构建其他类型的关系，如 POI2POI 和 POI2Road。
% %不如用graph的形式描述这一段话
% %图结构是MERL中重要的数据。
% Relationships between map entities are crucial in MERL. Many models incorporate relational information between entities to obtain better representations. In previous work, Line2Line is a commonly used relationship which indicates whether road segments are adjacent. Researchers typically represent this relationship using a graph structure by constructing a road network and employing graph representation learning methods to enhance entity's representations. Another commonly used relationship is Point2Region, which indicates whether a point is contained within a certain region. This relationship is often used in region entity representation learning. 

\subsection{Urban Spatial Temporal Data} Urban spatial temporal data (USTD) refers to data generated by human movements in urban areas, typically consisting of a series of data samples with time and geographical location. Popular USTD used in MERL includes trajectory data and origin-destination flow (OD Flow) data. Trajectory data can be divided into two types based on the data source: GPS trajectory data and POI trajectory data. GPS trajectory data is collected from devices such as smartphones or GPS trackers, capturing precise movements of individuals over time. It is often used for line entity representation learning (LERL). POI trajectory data, collected from social platforms, logs the sequence of points visited by humans, providing insights into human movement patterns and preferences. This type of data is used for point entity representation learning (PERL). OD Flow data records the origin and destination of trajectories, summarizing the movement between different regions. This type of data is used for region entity representation learning (RERL), helping to understand the human mobility between regions.
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/pretraintask.png}
    \vspace{-8mm}
    \caption{Pretrain task for MERL.}
    \label{fig:pretrain}
\end{figure*}

%MERL框架示意图
\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{figures/RepresentLearning.pdf}
    \caption{The generic framework MERL.}
    \vspace{-4mm}
    \label{fig:generic}
\end{figure}



\section{A brief review of MERL}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/PretrainTask.pdf}
%     \caption{Pretrain task for MERL.}
%     \label{fig:pretrain}
% \end{figure*}


%正如 Bengio 等人[Representation Learning 2013]所指出的，一个好的表征应该能够表达一般知识，这些知识不针对任何特定任务，但对解决机器学习过程中的各种任务非常有用。在 MERL 领域，一个好的表示应该既能捕捉地图实体的内在语义属性，又能捕捉它们之间的时空依赖关系。
Representation learning aims to learn a data representation that can capture the general purpose priors for the input data and make it easier for the downstream task predictor to obtain useful information\cite{RepresentationLearning}. When it come to MERL, a good representation should capture the spatial and temporal correlations between the map entities.

Existing research typically employs the pretrain-finetune paradigm to learn representations for map entities. \fig\ref{fig:generic} illustrates a generic framework of MERL. In the pretrain phase, we use upstream data which is regradless of downstream task to train the representation model also known as upstream model. In the finetuning phase, the pretrained upstream model is fine-tuned to different downstream tasks in a supervised manner. This section focuses on the pretrain phase of MERL, aiming to provide a clear understanding of the existing MERL methods. The pretrain phase of MERL consists of two key components: the encoder model and the pretrain task. The role of the encoder model is to encode the raw data of entities into representation vectors, while the pretrain task provides optimization objectives for the model. The combination of these two key components enables MERL to learn more general representations.


\subsection{Encoder Model}
Based on the form of input, basic encoder model for MERL can be categorized into four types: Token Encoder, Sequence Encoder, Graph Encoder, and Hybrid Encoder. As the names suggest, the first three encoders take tokens, sequences, and graphs as inputs, respectively. The Hybrid encoder is composed of combinations of the aforementioned encoders, which can be either parallel or sequential. Formally, all encoders first convert the entity $v$ in the map entity set $\mathcal{V}$ to a vector $e_v \in \mathbb{R}^{d_e}$ through a lookup table $\mathcal{E} \in \mathbb{R}^{d_e \times |\mathcal{V}|}$, where $d_e$ is a hyperparameter representing the dimension of token embeddings.

After obtaining the token embeddings, token encoders typically apply simple transformations to these embeddings, such as concatenating position embeddings. Classic models such as skip-gram\cite{Word2Vec} and CBOW\cite{Word2Vec} belong to this category. The representations obtain through token encoder are fixed and ignore the useful information hidden within the context, which can lead to poor performance in downstream tasks.

In MERL, context includes sequence context and graph context. To model these contexts, sequence encoders often utilize sequence models such as LSTM\cite{CACSR}, GRU\cite{Hier}, and Transformer Encoder\cite{Toast,CTLE,JCLRNT} as their core architecture. In contrast, graph encoders often use graph neural networks to encode graph context information, such networks include GCN \cite{HREP}, Message Passing Networks \cite{HyperRoad,MGFN}, and GAT \cite{HRNR,START,SARN,GMEL,MVURE}.

In recent years, many hybrid encoder models have been applicated to MERL. Since some USTD data naturally has both temporal sequence context and spatial graph context, using both graph encoder and sequence encoder has become a common approach. For instance, START \cite{START} employs both a transformer encoder and a GAT as its core architecture. 



% \begin{figure}
%     \centering
%     \subfigure[Inference task]{
%     \includegraphics[width=0.8\linewidth]{figures/Inference.pdf}
%     }
%     \subfigure[Reconstruction task]{
%     \includegraphics[width=0.8\linewidth]{figures/recon.pdf}
%     }
%     \subfigure[Contrastive task]{
%     \includegraphics[width=0.8\linewidth]{figures/contrastive.pdf}
%     }
%     \vspace{-2mm}
%     \caption{Pretrain task for MERL.}
%     \vspace{-2mm}
%     \label{fig:pretrain}
% \end{figure}


\subsection{Pretrain Task}
%忽略编码器模型的差异，MERL 预训练任务可分为三类：推理型、对比型和重构型。基于推理的任务通过预测特定标签并不断完善预测结果来优化表征。对比型任务使用对比学习方法，通过提高正面示例之间的相似性和降低反面示例之间的相似性来优化表征。重构任务试图从表征空间中重构原始数据，确保在编码过程中不会丢失信息。
Pretraining tasks help the model learn meaningful and informative representations of the entities by optimizing them based on specific objectives[add cite]. This sets a solid foundation for more effective performance in downstream tasks. MERL pretraining tasks can be broadly classified into three types: inference, contrastive, and reconstructive.% Inference tasks enhance representations by predicting specific labels. Contrastive tasks aims to learn representations by increasing the similarity between positive examples and decreasing the similarity between negative examples[add cite]. Reconstructive tasks try to reconstruct the raw data from the latent representation space, ensuring no information loss during the encoding process[add cite]. 

\subsubsection{Inference tasks} This type of pretrain tasks convert input representations into expected output labels. MERL methods typically use the auxiliary attributes of entities as output labels. This type of task often combines multiple tasks to optimize representations. The illustration of inference tasks is shown in \fig\ref{fig:pretrain}(a).
%TODO list这里可以加一句，使用到的标签属于auxiliary label

\begin{table*}[htbp]
  \centering
  \caption{Reproduced Models in VecCity. "Core Arch" stands for Core Architecture. The "Input Entity" column shows the type of entity used as input for the models. The "USTD" column indicates which USTD data is required as input for the models. The "Network" column displays whether the models utilize graph structure data. TE: short for Transformer Encoder, Contr: short for Contrastive, Reconst: short for Reconstruct, Infer: short for Inference, S: short for Sampling, A: short for Augment, CV: short for Cross-view, MR: short for Masked Reconstruct, GR: short for General Reconstruction, R: short for Regression, C: short for Classification, PT: short for POI Trajectory, GT: short for GPS Trajectory, SPATIAL: short for SIGSPATIAL.}
  \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|cc|cc|ccc|ccc|ccc|c|c|c}
        \toprule
    \multirow{2}[2]{*}{} & \multirow{2}{*}{Method} & \multirow{2}{*}{Category} & \multicolumn{2}{c|}{Encoder Model} & \multicolumn{3}{c|}{Pretrain Task} & \multicolumn{3}{c|}{Input Entity} & \multicolumn{3}{c|}{USTD} & \multirow{2}{*}{Network} & \multirow{2}{*}{Venue} & \multicolumn{1}{c}{\multirow{2}{*}{Year}} \\
          & &\multicolumn{1}{c|}{} & Type  & Core Arc & Constr & Reconst & \multicolumn{1}{c|}{Infer} & Point & \multicolumn{1}{c}{Line} & Region & \multicolumn{1}{c}{PT} & \multicolumn{1}{c}{GT} & OD    & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\
    \midrule
    \multicolumn{1}{c|}{\multirow{7}[2]{*}{Point}} & SkipGram\cite{Word2Vec} & Token & Token & Skip-gram & \checkmark     & \multicolumn{1}{c}{} &       & \checkmark     &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\checkmark} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & ICLR  & 13 \\
          & POI2Vec\cite{POI2VEC} & Token & Token & CBOW  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & \checkmark     &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\checkmark} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & AAAI  & 17 \\
          & Teaser\cite{Teaser} & Token & Token & Skip-gram & \checkmark     & \multicolumn{1}{c}{} &       & \checkmark     &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\checkmark} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & WWW   & 17 \\
          & Tale\cite{TALE} & Token & Token & CBOW  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & \checkmark     &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\checkmark} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & TKDE  & 21 \\
          & Hier\cite{Hier} & Sequence & Sequential & LSTM  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & \checkmark     &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\checkmark} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & SPATIAL & 20 \\
          & CTLE\cite{CTLE} & Sequence & Sequential & TE    & \multicolumn{1}{c}{} & \checkmark    & \multicolumn{1}{c|}{\checkmark} & \checkmark     &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\checkmark} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & AAAI  & 21 \\
          & CACSR\cite{CACSR} & Sequence & Sequential & Bi-LSTM & \checkmark     & \multicolumn{1}{c}{} &       & \checkmark     &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\checkmark} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & AAAI  & 23 \\
    \midrule
    \multicolumn{1}{c|}{\multirow{7}[2]{*}{Line}} & RN2Vec\cite{RN2Vec} & Non Traj & Token & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{c|}{} & \checkmark     & TIST  & 20 \\
          & HRNR\cite{HRNR} & Non Traj & Graph & GAT   & \multicolumn{1}{c}{} & \checkmark    &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{c|}{} & \checkmark     & KDD   & 20 \\
          & SARN\cite{SARN} & Non Traj & Graph & GAT   & \checkmark     & \multicolumn{1}{c}{} &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{c|}{} & \checkmark     & EBDT  & 23 \\
          & HyperRoad\cite{HyperRoad} & Non Traj & Graph & GNN   & \checkmark & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \checkmark     & TKDD  & 23 \\
          & Toast\cite{Toast} & Traj enhance & Hybrid & CBOW \& TE & \checkmark & \checkmark    &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} & \checkmark     & CIKM  & 21 \\
          & JCLRNT\cite{JCLRNT} & Traj enhance & Hybrid & TE \& GAT & \checkmark & \multicolumn{1}{c}{} &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} & \checkmark     & CIKM  & 22 \\
          & START\cite{START} & Traj enhance & Hybrid & TE \& GAT & \checkmark     & \checkmark    &       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} & \checkmark     & ICDE  & 23 \\
    \midrule
    \multicolumn{1}{c|}{\multirow{7}[2]{*}{Region}} & HDGE\cite{HDGE} & Single-View & Token & Skip-gram & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c}{} &       & \checkmark     &       &       & \checkmark     & \multicolumn{1}{c|}{} & CIKM & 17 \\
          & ZEMob\cite{ZEMob} & Single-View & Token & Skip-gram & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c}{} &       & \checkmark     &       &       & \checkmark     & \multicolumn{1}{c|}{} & IJCAI & 18 \\
          & GMEL\cite{GMEL} & Single-View & Graph & GAT   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c}{} &       & \checkmark     &       &       & \checkmark     & \checkmark     & AAAI  & 20 \\
          & ReMVC\cite{REMVC} & Multi-View & Token & \multicolumn{1}{c|}{} & \checkmark & \multicolumn{1}{c}{} &       & \checkmark     &       & \checkmark     &       &       & \checkmark     & \multicolumn{1}{c|}{} & TKDE  & 22 \\
          & MVURE\cite{MVURE} & Multi-View & Graph & GAT   & \multicolumn{1}{c}{} & \checkmark    & \multicolumn{1}{c|}{\checkmark} & \checkmark     &       & \checkmark     & \multicolumn{1}{c}{\checkmark} &       & \checkmark     & \checkmark     & IJCAI & 20 \\
          & MGFN\cite{MGFN} & Multi-View & Graph & GNN   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c}{} &       & \checkmark     &       &       & \checkmark     & \checkmark     & IJCAI & 22 \\
          & HREP\cite{HREP} & Multi-View & Graph & GCN & \checkmark   & \checkmark   &       &      &       & \checkmark     &       &       & \checkmark     & \checkmark     & AAAI  & 23 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:models}%
\end{table*}%


%对比预训练任务通常可分为三种类型：基于采样的、基于数据增强的和基于交叉视图的。采样对比任务基于这样一种理念，即锚点样本与其相邻节点之间的相似性大于样本与非相邻节点之间的相似性。这些相邻节点可以通过轨迹共现、图邻接或共享辅助属性来构建。数据增强的基础是样本与其增强样本之间的相似性大于样本与其他样本之间的相似性。基于跨视图的任务假定，从同一实体的不同视图中学习到的表征应该是相似的。
\subsubsection{Contrastive tasks} In this category, pretrain tasks aim to learn representations by comparing positive and negative samples [add cite]. Specifically, the representation of anchor samples should be similar to positive samples and different from negative samples.  The core of contrastive tasks lies in constructing pairs of positive and negative samples. In the domain of MERL, contrastive tasks are generally classified into three types based on their construction approach: sampling based methods, data augmentation based methods, and cross-view based methods. Sampling-based methods operate on the principle that anchor samples should be similar to their neighboring samples, which can be identified through co-occurrence, adjacency, or shared auxiliary attributes. Data augmentation-based methods generate similar samples by adding noise to the anchor sample. Cross-view-based methods assume that representations learned from different views of the same entity should be similar. The illustration of contrastive tasks is shown in \fig\ref{fig:pretrain}(b).

\subsubsection{Reconstructive Tasks} In this category, pretrain tasks aim to reconstruct the original input from the representations and minimize the distance between the restored input and the original input. Mask and recover is a common used pretrain task, it masks a part of the input and try to recover the mask part using the entity representations. Another methods is autoencoder based methods. Different from the mask and recover, autoencoder based methods take unmasked input and try to reconstruct the whole input completely.
The illustration of reconstructive tasks is shown in \fig\ref{fig:pretrain}(c).

% Table generated by Excel2LaTeX from sheet "reproduced model"
% "Input Entity"列展示模型的输入实体类型，‘USTD’列则表示了模型需要哪些USTD数据作为输入，‘Network’列展示了模型是否使用到了图结构数据。


\subsection{Previous MERL Methods}
We categorized the previous studies published over the past decade based on the aforementioned taxonomy, and \tab\ref{tab:models} provides detailed information.

%这段话开头的意思是说，POI 轨迹数据之间的采样间隔比较大，距离远，我们不需要关注他的具体轨迹，只需要关注他到达的地图实体本身。所以，POI 表示学习更关注human 在时间空间和顺序方面的偏好，不需要考虑路网的限制。
\subsubsection{Previous Work on PERL} Due to the relatively long sampling intervals of USTD data for point entities, people can move significant distances between two sampling points. Consequently, PERL focuses more on the human preference, which encompass both temporal and spatial dimensions. Early models are based on word2Vec \cite{Word2Vec} models in neural language processing. The core idea is to model the co-occurrence of target points and their contexts in trajectories. We refer to these models as Token Models. However, the original Word2Vec methods, CBOW and Skip-gram, cannot capture the influence of temporal and spatial dimensions. To tackle this challenge, POI2Vec\cite{POI2VEC} and TALE\cite{TALE} extend the CBOW model by designing a novel huffman tree that incorporates the geographic influence and temporal influence. Teaser extends the skip-gram model by using hierarchical negative samples, ensuring that the similarity between the anchor sample and geographically closer negative samples is greater than that with farther negative samples. This design injects spatial information into the representations. In recent years, with the development of deep learning technology, sequence models have gained increasing attention due to their powerful ability to encode sequential information. We refer to these models, which use sequence encoders, as Sequence Models. HIER \cite{Hier} employ an RNN-based model as the encoder model and combines hierarchical spatial information by multi-block entity embedding. CTLE\cite{CTLE} uses the Transformer Encoder to encode POI trajectories and optimizes the entity embedding with the Masked Language Model pretrain task. CACSR\cite{CACSR} chooses the Bi-LSTM as the encoder model and design a novel trajectory augment algorithm to build positive samples, and then use the contrastive pretrain task to optimize entity embedding.

\subsubsection{Previous Work on LERL} USTD data for line is generated by human movement between road segments, with sampling intervals typically ranging from 15 to 30 seconds. This indicates that human movement usually involves relatively short geographic distances, leading to USTD for lines being constrained by the road network. Consequently, both human preferences and road network constraints should be considered in line representation learning. The initial models focused on capturing network information using graph representation learning methods without using trajectories to enhance entity representations. We refer to these models as Non-Trajectory Models. RN2Vec first collects paths through shortest path sampling, then employ the skip-gram model to learn line representations. HRNR\cite{HRNR} designs a hierarchical entity graph and learns entity representations by optimizing the graph reconstruction task. SARN\cite{SARN} constructs multiple graphs by considering both the adjacency and topological structure of the road network and designs a graph augmentation algorithm to build positive samples. It then uses contrastive learning to optimize entity embeddings. HyperRoad\cite{HyperRoad} captures high-order and long-range relationships in road networks by adding hyper node into the graph. And then HyperRoad employ multiple pretrain task to learn the entity embedding. In recent years, using trajectories to enhance line representation has become a research hotspot. We refer to these types of models as Trajectory-Enhanced Models. Toast\cite{Toast} adopts a two-stage method. In the first stage, Toast employs the skip-gram model with random walks to learn the initial entity representation vectors. In the second stage, Toast uses trajectory data to enhance the entity representations with two pretraining tasks: a masked reconstruction task and an augmentation-based contrastive task. JCLRNT\cite{JCLRNT} designs a Cross-View contrastive pretrain task, utilizing contrastive learning techniques to integrate the network view representation and trajectory view representation. START designs multiple types of trajectory self-supervised tasks to enhance trajectory representations and simultaneously improve line representations.

\subsubsection{Previous Work on RERL} RERL aims to learn region representations using graph representation learning methods. In previous works, the feature extract based on the relationships between region entities are termed inter-view feature. Additionally, each region may contain other types of entities such as point entities. The feature extract based on contain entities referred to the intra-view feature. Single-view models only utilize the inter-view to learn region representations, HDGE\cite{HDGE}, ZEMob\cite{ZEMob}, GMEL\cite{GMEL}, and MGFN\cite{MGFN} are classic single-view models. HDGE\cite{HDGE} extends DeepWalk\cite{Deepwalk} by using OD Flow transition matrix as graph. It performs random walks to gather node sequences and then learns region embeddings using the Skip-Gram model. ZEMob\cite{ZEMob} uses OD Flow data to calculate co-occurrence probabilities between entities and creates a pairwise mutual information (PMI) matrix. It then learns region embeddings with a PMI-extended Skip-Gram model. GMEL\cite{GMEL} and MGFN\cite{MGFN} employ graph neural networks as encoder model. GMEL uses multi-task learning to learn region representations by separately predicting incoming flow, outgoing flow, and OD flow based on entity representations extracted by GNN. MGFN uses clustering methods to create different movement patterns from human mobility data. Each pattern is a subgraph of the human mobility graph. It then learns region embeddings by predicting the PMI matrix based on the multiple subgraphs. The latest region representation learning methods are based on multi-view representation learning, such as MVURE\cite{MVURE}, ReMVC\cite{REMVC}, and HREP\cite{HREP}, which focus on integrating multi-view features to learn region representations. MVURE builds multi-view graphs using POI trajectories and OD Flow. MVURE\cite{MVURE} uses GAT to separately encode these graphs, then fuses the graph representations with attention mechanisms. It employs multi-graph reconstruction tasks to learn region embeddings. ReMVC\cite{REMVC} uses cross-view contrastive learning methods to align the inter-view and intra-view region representations. HREP\cite{HREP} uses heterogeneous graphs to combine multiple views into one graph. It then leverages graph reconstruction tasks and prompt learning techniques to learn multi-view region representations.

% 这里虽然写完了对方法的综述，但是并没有突出我们要实现库的必要性，我们可以通过一个开源与否的一列来表达实现库的必要性。
% \paratitle{Limitations:}Despite the significant progress these models have made in the field of MERL, there are several limitations that need to be addressed:
% \begin{itemize}
%     \item Lack of Implementation Details: Some models, such as Teaser, have not disclosed their hyperparameters. Additionally, models like Hier, RN2Vec, HDGE, and ZEMob have not provided open-source code, making it difficult for other researchers to replicate and build upon their work.
%     \item Limited Dataset Evaluation: The CTLE model, for example, has only been tested on two unpublished datasets, limiting the ability to evaluate its performance comprehensively. Most models have only been evaluated on datasets from two cities, which does not allow for a thorough assessment of their performance across different urban environments and contexts.
% \end{itemize}
% To ensure a more comprehensive and reliable comparison of MERL methods, it is crucial to conduct evaluations on a broader range of datasets, open-source all implementation details, and adopt standardized benchmarks and protocols.



 



==> backup4.tex <==

% Benchmark：如上文中我们所分析的一样，由于研究人员对于数据、应用和微调策略等部分的选择不同，导致了当前表示学习领域缺少一个标准，公平，全面的测评。VecCity的出现解决了上述问题的挑战。我们基于VecCity对其所复现的20多个模型进行了评估，为研究人员提供一个清楚，准确的模型效果认知。
% experimental Setting:预训练策略要讲清楚，训练集、评估和测试集的划分讲清楚。

%CityVector：我们将在9个城市上预训练的表征和模型参数进行公开，由于所有的实体数据取自osm，所以在城市时空表示学习领域具有一定的普遍适用，可以帮助研究人员省去从头训练的成本，并可直接获得在下游任务表现更佳的表征。
%这里可以测试一下，基于我们的预训练表征，可以对那些端到端的模型有多大的增强。

\section{Experimental and Analysis}
%在本章中，我们在第4.1节所述的数据集上，对第3.3节中提到的21种MERL方法进行了实验。实验过程遵循第4节中描述的管道。为了确保结果的可靠性和公平性，我们对每种方法进行了全面的超参数优化，使其性能达到或超过原始论文中报告的水平。我们的目标是展示VecCiity作为一个易于使用且强大的资源，为MERL方法提供了一个便捷和公平的评估平台。
In this section, we conducted experiments on the datasets described in Section 4.1, using the 21 MERL methods mentioned in Section 3.3. The experimental process followed the pipeline outlined in Section 4. To ensure the reliability and fairness of the results, we performed comprehensive hyperparameter optimization for each method, achieving performance that matches or exceeds the levels reported in the original papers. Our objective is to demonstrate VecCiity as a user-friendly and powerful resource, providing a convenient and fair evaluation platform for MERL methods.

\subsection{Experimental Setup}

\subsubsection{Datasets}
To conduct comprehensive and thorough experiments on the models, we utilized all datasets that meet the data requirements, and tested them on the downstream tasks introduced in \tab\ref{tab:tasks}. For the PERL algorithms, Point Trajectory data is essential for the LC and TUL downstream task, thus we selected datasets from New York, Chicago, Porto, Tokyo, Singapore, and San Francisco for testing. For the LERL algorithms, both TTE and STS rely on GPS Trajectory data, so we chose datasets from Beijing, Xi'an, Chengdu, Porto, Tokyo, Singapore, and San Francisco. Due to the sparsity of the Tokyo dataset, most models showed unacceptable performance on this dataset, hence Tokyo was excluded from the line entity test data. For the Region MERL algorithms, OD Flow data and the label information required for Region Classification are indispensable, so we selected datasets from Beijing, Xi'an, Chengdu, Porto, and San Francisco as the Region datasets. All datasets were split into training, validation, and test sets in a 6:2:2 ratio. All data preprocessing procedures and intermediate results can be found in the github repository.

\subsubsection{Implementation details}To ensure the fairness of the experiments, we set the embedding size of all models to 128. The settings for other hyperparameters were based on those reported in the original papers. The batch size was set to 64; in the case of out-of-memory (OOM) issues, it was halved (to a minimum of 8). For parameters such as learning rate, dropout, and temperature, we adjusted them on each dataset to ensure the performance was at least as good as reported in the original papers, where possible. All experiments were conducted on an Ubuntu 20.04 system with NVIDIA GeForce 3090 GPUs.

In addition, we preprocessed the trajectory data. Following previous work, for POI trajectory data, we removed POI trajectories shorter than 3 points and users with fewer than 3 trajectories, and truncated trajectories longer than 128 points. For GPS trajectory data, we removed trajectories shorter than 10 points and truncated those longer than 128 points.

\subsection{Experimental Result}
\begin{figure}
    \centering
    \subfigure[Point]{
        \includegraphics[width=0.4\textwidth]{figures/poi_nemenyi.pdf}
    }
    \subfigure[Line]{
        \includegraphics[width=0.4\textwidth]{figures/road_nemenyi.pdf}
    }
    \subfigure[Region]{
        \includegraphics[width=0.4\textwidth]{figures/region_nemenyi.pdf}
    }
    \vspace{-5mm}
    \caption{Nemenyi test: this heatmap displays the average rankings of models across all datasets for specific tasks. "SG" stands for SkipGram, "P2V" represents the POI2Vec model, and "HRoad" denotes the HyperRoad model.}
    \label{fig:rank}
\end{figure}

\subsubsection{Point entity representation learning, PERL} \tab\ref{tab:poires} reports the performance of PERL methods on three downstream tasks. To provide a more intuitive observation of the model performance rankings, we present the average rankings of the models on various tasks in Figure 6. From \fig\ref{fig:rank}, we observe that recently proposed sequential models, including Hier, CTLE, and CACSR, perform exceptionally well on the LC task, achieving the best average results across all city datasets. This indicates that they have learned higher quality entity representations. The Teaser model performed poorly on the LC task because it introduced time embedding during pre-training to enhance representations, whereas in the LC task, we only used entity embedding without time embedding, leading to its failure in the LC task. Point2Vec and Tale are CBOW-based models that rely on hierarchical classification methods for context node recognition during pre-training. In downstream tasks, the absence of intermediate node participation resulted in these models' poorer performance on the LC task.

\begin{table}[t]\small
  \centering
  \caption{Performance comparison of PERL methods on various datasets.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc}
    \toprule
    \multirow{2}[1]{*}{Dataset} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{Method}} & \multicolumn{2}{c|}{LC} & \multicolumn{2}{c|}{LP} & \multicolumn{2}{c|}{TUL} & \multicolumn{2}{c}{Efficient} \\
\cmidrule{3-10}          & \multicolumn{1}{c|}{} & ACC@1 & F1-Ma & ACC@1 & ACC@5 & ACC@1 & F1-Ma & Param & Speed \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{New York City}}} & SkipGram & 0.341 & 0.303 & \underline{0.097} & \textbf{0.242} & \textbf{0.383} & \underline{0.191} & \textbf{2.6} & \textbf{2} \\
          & POI2Vec & 0.415 & 0.467 & \textbf{0.099} & \underline{0.234} & 0.336 & 0.158 & 27.1  & 7 \\
          & Teaser & 0.160 & 0.113 & 0.087 & 0.227 & 0.303 & 0.127 & \underline{3.0}   & \underline{3} \\
          & Tale & 0.478 & 0.487 & 0.095 & 0.222 & 0.319 & 0.152 & 8.6   & 5 \\
          & Hier & 0.425 & 0.432 & 0.086 & 0.197 & 0.259 & 0.116 & 8.3   & 5 \\
          & CTLE & \textbf{0.712} & \textbf{0.717} & 0.095 & 0.219 & \underline{0.357} & \textbf{0.202} & 3.4   & 8 \\
          & CACSR & \underline{0.595} & \underline{0.602} & 0.095 & 0.221 & 0.338 & 0.177 & 9.9   & 73 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Tokyo}}} & SkipGram & 0.482 & 0.374 & \textbf{0.174} & \textbf{0.388} & \textbf{0.457} & \textbf{0.339} & \textbf{2.0} & \textbf{3} \\
          & POI2Vec & 0.513 & 0.471 & 0.146 & 0.324 & 0.345 & 0.259 & 2.7   & 12 \\
          & Teaser & 0.370 & 0.242 & \underline{0.168} & \underline{0.378} & 0.409 & 0.294 & \underline{2.3}   & \underline{5} \\
          & Tale & 0.608 & 0.553 & 0.163 & 0.364 & 0.380 & 0.269 & 8.1   & 12 \\
          & Hier & 0.560 & 0.534 & 0.159 & 0.348 & 0.345 & 0.245 & 7.6   & 8 \\
          & CTLE & \textbf{0.742} & \textbf{0.727} & 0.165 & 0.359 & \underline{0.418} & \underline{0.320} & 2.8   & 13 \\
          & CACSR & \underline{0.675} & \underline{0.640} & 0.164 & 0.361 & 0.399 & 0.295 & 8.3   & 114 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Chicago}}} & SkipGram & 0.327 & 0.308 & \underline{0.104} & \textbf{0.264} & \textbf{0.459} & 0.253 & \textbf{0.9} & \textbf{1} \\
          & POI2Vec & 0.365 & 0.362 & 0.076 & 0.183 & 0.343 & 0.213 & 1.4   & 2 \\
          & Teaser & 0.154 & 0.077 & 0.088 & 0.229 & 0.367 & 0.173 & \underline{1.1}   & \underline{1} \\
          & Tale & 0.527 & 0.580 & 0.099 & 0.240 & 0.438 & 0.245 & 2.9   & 2 \\
          & Hier & 0.355 & 0.350 & 0.085 & 0.198 & 0.300 & 0.151 & 6.6   & 2 \\
          & CTLE & \textbf{0.766} & \textbf{0.778} & \textbf{0.108} & \underline{0.244} & 0.440 & \textbf{0.289} & 1.7   & 4 \\
          & CACSR & \underline{0.647} & \underline{0.679} & 0.103 & 0.242 & 0.439 & \underline{0.267} & 5.4   & 43 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Porto}}} & SkipGram & 0.208 & 0.158 & \textbf{0.135} & \textbf{0.329} & 0.518 & 0.354 & \textbf{0.3} & \textbf{1} \\
          & POI2Vec & 0.078 & 0.014 & 0.024 & 0.072 & 0.068 & 0.020 & 53.7  & 4 \\
          & Teaser & 0.094 & 0.017 & 0.075 & 0.207 & 0.266 & 0.110 & \underline{0.3}   & 1 \\
          & Tale & 0.459 & 0.443 & 0.129 & 0.299 & 0.511 & 0.344 & 0.5   & 1 \\
          & Hier & 0.086 & 0.036 & 0.098 & 0.219 & 0.245 & 0.141 & 5.9   & 1 \\
          & CTLE & \textbf{0.798} & \textbf{0.800} & \underline{0.133} & \underline{0.308} & \textbf{0.552} & \textbf{0.407} & 1.1   & 1 \\
          & CACSR & 0.632 & 0.628 & 0.130 & 0.303 & \underline{0.518} & \underline{0.375} & 3.8   & 7 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Singapore}}} & SkipGram & 0.544 & 0.525 & \textbf{0.106} & \textbf{0.266} & \textbf{0.301} & \textbf{0.182} & \textbf{2.5} & \textbf{3} \\
          & POI2Vec & 0.607 & 0.609 & 0.091 & 0.216 & 0.239 & 0.155 & 3.3   & 11 \\
          & Teaser & 0.378 & 0.353 & \underline{0.102} & \underline{0.261} & 0.248 & 0.134 & \underline{3.0}   & \underline{5} \\
          & Tale & 0.659 & 0.648 & 0.098 & 0.241 & 0.236 & 0.131 & 9.9   & 13 \\
          & Hier & 0.652 & 0.638 & 0.100 & 0.237 & 0.240 & 0.137 & 8.1   & 9 \\
          & CTLE & \textbf{0.781} & \textbf{0.770} & 0.102 & 0.241 & \underline{0.277} & \underline{0.178} & 3.3   & \textbf{12} \\
          & CACSR & \underline{0.720} & \underline{0.709} & 0.100 & 0.241 & 0.256 & 0.154 & 9.7   & 119 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Sanfransico}}} & SkipGram & 0.313 & 0.320 & 0.104 & \textbf{0.252} & \textbf{0.444} & 0.237 & \textbf{0.4} & \textbf{1} \\
          & POI2Vec & 0.095 & 0.037 & 0.036 & 0.092 & 0.144 & 0.058 & 1.5   & 1 \\
          & Teaser & 0.117 & 0.050 & 0.080 & \underline{0.212} & 0.330 & 0.129 & \underline{0.5}   & 1 \\
          & Tale & 0.559 & 0.609 & 0.101 & 0.230 & \underline{0.442} & 0.239 & 1.1   & 1 \\
          & Hier & 0.230 & 0.204 & 0.077 & 0.181 & 0.231 & 0.102 & 6.0   & 1 \\
          & CTLE & \textbf{0.789} & \textbf{0.794} & \textbf{0.111} & 0.239 & 0.437 & \textbf{0.274} & 1.2   & 1 \\
          & CACSR & \underline{0.674} & \underline{0.701} & \underline{0.106} & 0.235 & 0.440 & \underline{0.257} & 4.1   & 7 \\
    \bottomrule
    \end{tabular}%
 }
 \vspace{-2mm}
\label{tab:poires}
\end{table}

We observed that in the LP and TUL tasks, the results among all models showed minimal differences. The most basic SkipGram model achieved better average rankings than all competitors across all datasets. Both LP and TUL tasks are trajectory based tasks that require sequence encoding layers such as LSTM and Transformer to encode sequence information. Although sequential based models train their encoding models during pretrain phase, intuitively, these models should perform better on sequence tasks compared to token based models. However, the experimental results contradict this intuition.

From the data frequency shown in \tab\ref{tab:datasets}, we can see that the original data of POI Trajectory is very sparse, with an low average visit frequency. In this case, simple token based models can achieve good data fitting through fine-tuning, with faster speed and lower memory consumption. We believe that as the visit frequency increases, the performance of sequential models will surpass that of token based models.

To validate the above hypothesis, we adjusted the data filtering conditions to remove sparse nodes and conducted further tests on dense nodes in the datasets for the two sequence tasks. Due to space limitations, we only present the experimental results on the New York City (NYC) dataset, as shown in \fig\ref{fig:dpoi}. We preprocessed the NYC dataset with minimum visit frequencies of 50, 100, 150, and 200. In the processed datasets, we observed that as the visit density of data points increased, the performance of the sequential models CTLE and CACSR in both sequence tasks surpassed that of the SkipGram model, which performed better in the original dataset. Although the performance of the Hier model did not surpass the SkipGram model in the tested scenarios, it showed the same upward trend. This also confirms our previous hypothesis that "as data density increases, sequential models perform better in trajectory based tasks."

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/dive_poi.pdf}
    \vspace{-5mm}
    \caption{Performance of methods with varying minimum visit frequency in the New York City dataset. The horizontal axis shows the minimum visit frequency.}
    \label{fig:dpoi}
    \vspace{-5mm}
\end{figure}

\subsubsection{Line entity representation learning, LERL}
\tab\ref{tab:road} reports the performance of LERL on downstream tasks. From the results, we can observe that for the TSI task, the non-trajectory-enhanced methods HyperRoad and SARN achieved the best classification results. Both of these methods primarily utilize graph neural networks, demonstrating the effectiveness of graph neural networks in LERL applications. In the two trajectory-based tasks, TTE and STS, the trajectory-enhanced methods Toast, JCLRNT, and START outperformed other methods that did not use trajectory enhancement. This indicates that utilizing trajectory data for pre-training in upstream tasks can effectively capture trajectory features and enhance trajectory-based downstream tasks. However, in the SG dataset, we observed that the HyperRoad model's performance on the TTE task was almost 80\% better than that of the trajectory-based representation learning methods. As shown in the data statistics in \tab\ref{tab:datasets}, the SG dataset has relatively sparse trajectory data, leading to a decrease in the accuracy of the trajectory-enhanced representation learning methods on this dataset.

% Table generated by Excel2LaTeX from sheet 'Road'
\begin{table}[htbp]\small
  \centering
  \caption{Performance comparison of line entity representation learning methods on various datasets.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc}
    \toprule
    \multirow{2}[1]{*}{Dataset} & \multirow{2}[1]{*}{Method} & \multicolumn{2}{c|}{TSI} & \multicolumn{2}{c|}{TTE} & \multicolumn{2}{c|}{STS} & \multicolumn{2}{c}{Efficient} \\
\cmidrule{3-10}          &       & MAE   & RMSE  & MAE   & RMSE  & HR@3  & MR    & Param & Speed \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Beijing}}} & RN2Vec & 4.81  & 9.28  & 339.90 & 601.30 & 0.948 & 18.92 & \underline{5.2}   & 331 \\
          & HRNR & 5.30  & 12.39 & 348.40 & 782.58 & \underline{0.977} & 22.77 & 5.7   & 281 \\
          & SARN & 4.70  & \underline{8.98}  & 324.1 & 563.5 & 0.955 & 12.812 & \textbf{0.6} & \textbf{30} \\
          & HyperRoad & \textbf{4.62} & \textbf{8.97} & \underline{311.1} & 562.6 & 0.953 & 25.148 & 5.4   & \underline{66} \\
          & Toast & \underline{4.66}  & 9.01  & 318.3 & 567.1 & \textbf{0.978} & 13.543 & 10.6  & 495 \\
          & JCLRNT & 4.77  & 9.05  & \textbf{297.7} & \textbf{529.0} & \underline{0.974} & \textbf{7.952} & 5.4   & 434 \\
          & START & 4.77  & 9.06  & \underline{312.6} & \underline{553.8} & 0.969 & \underline{9.360} & 6.3   & 1719 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Chendu}}} & RN2Vec & 14.32 & \underline{27.20} & 148.6 & 212.6 & 0.696 & 10.513 & \underline{0.7}   & 19 \\
          & HRNR & 16.74 & 31.69 & 164.6 & 248.3 & 0.699 & 8.730 & 1.2   & \underline{5} \\
          & SARN & \underline{14.48} & 27.53 & 150.6 & 204.5 & 0.698 & 12.334 & \textbf{0.5} & \textbf{5} \\
          & HyperRoad & \textbf{14.17} & \textbf{26.94} & 138.7 & 193.9 & \underline{0.713} & \underline{8.518} & 0.9   & 6 \\
          & Toast & 14.73 & 27.36 & \textbf{124.1} & \textbf{185.7} & 0.703 & 9.782 & 1.6   & 193 \\
          & JCLRNT & 14.83 & 27.61 & \underline{133.2} & \underline{191.8} & \textbf{0.732} & \textbf{8.440} & 0.9   & 287 \\
          & START & 14.54 & 27.80 & 147.6 & 204.9 & 0.703 & 10.897 & 2.0   & 582 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Xi'an}}} & RN2Vec & 13.24 & 22.36 & 180.5 & 273.5 & 0.731 & \underline{7.706} & \underline{0.8}   & 16 \\
          & HRNR & 13.68 & 23.28 & 297.3 & 529.4 & 0.725 & 8.485 & 1.3   & 4 \\
          & SARN & \textbf{12.73} & \textbf{22.23} & 174.2 & 276.7 & 0.609 & 28.289 & \textbf{0.6} & \textbf{5} \\
          & HyperRoad & \underline{13.05} & 22.38 & 173.5 & 265.7 & 0.702 & 10.199 & 1.0   & \underline{5} \\
          & Toast & 13.58 & 23.03 & \underline{164.7} & \textbf{227.1} & 0.721 & 8.266 & 1.9   & 132 \\
          & JCLRNT & 13.45 & \underline{22.94} & \textbf{154.8} & \underline{227.4} & \textbf{0.750} & \textbf{6.875} & 1.1   & 150 \\
          & START & 13.38 & 22.89 & 171.7 & 237.3 & \underline{0.732} & 7.960 & 2.1   & 312 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Porto}}} & RN2Vec & 7.07  & 12.38 & 140.9 & 206.1 & 0.866 & 14.726 & \underline{1.5}   & \textbf{3} \\
          & HRNR & 7.15  & 12.43 & 171.8 & 215.4 & 0.847 & 16.031 & 1.9   & 80 \\
          & SARN & 7.05  & \underline{12.25} & 130.7 & 188.5 & 0.873 & 9.259 & \textbf{0.6} & \underline{10} \\
          & HyperRoad & \underline{6.97}  & \textbf{12.21} & \underline{119.8} & \textbf{168.6} & \underline{0.882} & 8.805 & 1.7   & 11 \\
          & Toast & 7.11  & 12.29 & 123.2 & 180.1 & 0.879 & \underline{7.862} & 3.1   & 252 \\
          & JCLRNT & 7.07  & 12.35 & \textbf{116.7} & \underline{171.0} & \textbf{0.894} & \textbf{2.556} & 1.7   & 345 \\
          & START & \textbf{6.96} & 12.38 & 146.3 & 269.1 & 0.861 & 10.721 & 2.8   & 735 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Singapore}}} & RN2Vec & 38.58  & 81.02  & 1350.2  & 1384.6  & 0.653  & \underline{44.33}  & 4.6   & 98 \\
          & HRNR & 39.60  & 82.31  & 807.1  & 987.2  & 0.639  & 51.23  & 5.2   & 21 \\
          & SARN & \underline{38.12}  & \underline{80.16}  & 706.9  & 778.2  & 0.646  & 42.58  & \textbf{0.6} & 27 \\
          & HyperRoad & \textbf{37.94} & \textbf{79.68} & \textbf{247.1} & \textbf{348.8} & 0.633  & 52.42  & 4.8   & 32 \\
          & Toast & 38.42  & 80.85  & 1042  & 1064  & 0.658  & 60.20  & 9.5   & \underline{12} \\
          & JCLRNT & 38.31  & 80.93  & \underline{650.5}  & \underline{684.9}  & \underline{0.671}  & 56.10  & 4.8   & \textbf{5} \\
          & START & 38.28  & 80.72  & 1063.0  & 1084  & \textbf{0.676} & \textbf{42.47} & \underline{3.7}   & 29 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Sanfransico}}} & RN2Vec & 4.14  & 9.71  & 259.3  & \underline{698.2}  & 0.876  & 111.93  & \underline{3.5}   & 35 \\
          & HRNR & 4.17  & 10.09  & 312.4  & 732.1  & \underline{0.889}  & 121.73  & 4.1   & \underline{23} \\
          & SARN & 4.13  & 9.61  & 263.6  & \textbf{691.1} & 0.862  & 101.67  & \textbf{0.6} & \textbf{19} \\
          & HyperRoad & \underline{4.08}  & \textbf{9.36} & \underline{228.1}  & 707.1  & 0.884  & \underline{83.33}  & 3.7   & 44 \\
          & Toast & 4.23  & \underline{9.59}  & \textbf{227.8} & 698.6  & 0.871  & 108.55  & 7.3   & 237 \\
          & JCLRNT & 4.09  & 9.70  & 231.8  & 706.5  & \textbf{0.900} & \textbf{81.73} & 3.8   & 198 \\
          & START & \textbf{4.06} & 9.82  & 230.7  & 714.6  & 0.871  & 83.51  & 4.8   & 783 \\
    \bottomrule
    \end{tabular}%
  }
  \vspace{-2mm}
  \label{tab:road}%
\end{table}%


\subsubsection{Region entity representation learning, RERL}
%由于region的下游任务中需要crime数据，因此我们只能使用NYC和chicago这两个数据集对区域表示学习方法在3个下游任务上进行了实验。模型在下游任务上的性能表现如表5所示。
\tab\ref{tab:region} reports the performance of RERL models on downstream tasks. By comparing the performance of different models, we can draw several important conclusions.
Firstly, multi-view models such as MVURE, MGFN, ReMVC, and HREP significantly outperform other single-view models across all tasks. This demonstrates that incorporating internal views is an effective method for region representation learning. Specifically, multi-view approaches can integrate information from multiple perspectives, resulting in richer and more comprehensive feature representations. This is particularly important in complex tasks that require the integration of diverse information sources for accurate predictions.
% Table generated by Excel2LaTeX from sheet 'Regoin'
\begin{table}[htbp]
  \centering
  \caption{Performance comparison of region entity representation learning methods on various datasets.}
  \resizebox{0.97\linewidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc}
    \toprule
    \multirow{2}[1]{*}{Dataset} & \multirow{2}[1]{*}{Method} & \multicolumn{2}{c|}{RC} & \multicolumn{2}{c|}{FI} & \multicolumn{2}{c|}{MFI} & \multicolumn{2}{c}{Efficient} \\
    \cmidrule{3-10}          &       & ACC@1   & F1-ma & MAE   & RMSE  & MAE   & RMSE  & Param & Speed \\
    \midrule
        \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Beijing}}} & ZEMob & 0.111 & 0.380 & 30.88 & 55.14 & \textbf{0.279} & 0.663 & 45.1  & 40 \\
          & HDGE & 0.222 & 0.409 & 19.26 & \underline{42.82} & 0.329 & 0.659 & 12.9  & 1799 \\
          & GMEL & 0.412 & 0.571 & \textbf{17.68} & 48.91 & 0.418 & 0.712 & \underline{0.12}  & 713 \\
          & MVURE & 0.232 & 0.472 & 29.45 & 54.15 & \underline{0.280} & 0.667 & \textbf{0.10} & \underline{1.2} \\
          & MGFN & \underline{0.667} & \underline{0.701} & 20.13 & 41.37 & 0.283 & \underline{0.649} & 5156 & 2839 \\
          & ReMVC & \textbf{0.762} & \textbf{0.790} & 27.01 & 51.94 & 0.281 & 0.657 & 1.5   & 872.5 \\
          & HREP & 0.557 & 0.585 & \underline{17.75} & \textbf{38.39} & 0.285 & \textbf{0.626} & 0.2   & \textbf{1.1} \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Chendu}}} & ZEMob & 0.210 & 0.371 & 141.9 & 572.2 & \underline{1.792} & 6.604 & 7.7   & 19 \\
          & HDGE & 0.188 & 0.359 & 159.6 & 402.1 & 2.238 & 6.333 & 1.5   & \underline{5.2} \\
          & GMEL & 0.338 & 0.301 & 154.8 & 441.1 & 3.122 & 9.442 & \underline{0.12}  & 193 \\
          & MVURE & 0.285 & 0.477 & 155.8 & 436.8 & 1.997 & 6.949 & \textbf{0.10} & 287 \\
          & MGFN & 0.322 & 0.476 & \textbf{104.6} & \textbf{278.2} & \textbf{1.753} & \textbf{4.974} & 486   & \textbf{5.1} \\
          & ReMVC & \textbf{0.641} & \textbf{0.687} & 147.7 & 430.9 & 2.029 & 6.800 & 0.18  & 582 \\
          & HREP & \underline{0.403} & \underline{0.502} & \underline{114.0} & \underline{315.1} & 1.847 & \underline{5.093} & 0.18  & 6 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Xi'an}}} & ZEMob & 0.200 & 0.387 & 123.2 & 292.8 & 1.648 & 5.024 & 5.7   & \textbf{0.2} \\
          & HDGE & 0.243 & 0.376 & 120.0 & 271.2 & 1.899 & 4.653 & 1.2   & 75 \\
          & GMEL & 0.330 & 0.359 & 133.1 & 324.4 & 2.997 & 10.363 & \underline{0.12}  & 189 \\
          & MVURE & 0.300 & 0.543 & 130.8 & 309.8 & 1.758 & 5.068 & \textbf{0.10} & \underline{0.9} \\
          & MGFN & 0.282 & 0.515 & 86.3  & \textbf{190.7} & \textbf{1.469} & \textbf{3.368} & 318   & 1.2 \\
          & ReMVC & \textbf{0.591} & \textbf{0.672} & 126.9 & 317.0 & 1.801 & 5.116 & 0.15  & 39 \\
          & HREP & \underline{0.482} & \underline{0.606} & \textbf{84.31} & \underline{209.3} & \underline{1.511} & \underline{3.484} & 0.2   & 1.0 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Porto}}} & ZEMob & 0.213 & 0.304 & 3270  & 5805  & 120.74 & 405.82 & 1.0   & \textbf{0.4} \\
          & HDGE & \textbf{0.493} & \textbf{0.495} & 2514  & 4200  & 125.42 & 285.88 & 0.4   & 117 \\
          & GMEL & 0.267 & 0.335 & 3305  & 5824  & 127.50 & 391.64 & 0.12  & 261 \\
          & MVURE & 0.274 & 0.287 & 2282  & 3899  & 106.95 & 278.08 & \underline{0.10}  & \underline{0.9} \\
          & MGFN & \underline{0.480} & \underline{0.474} & \underline{1489}  & \textbf{3336} & \textbf{90.76} & \textbf{229.02} & 53.7  & 2 \\
          & ReMVC & 0.385 & 0.398 & \textbf{1488} & \underline{3702}  & 119.43 & 316.26 & \textbf{0.07} & 47 \\
          & HREP & 0.370 & 0.409 & 2134  & 4110  & \underline{105.48} & \underline{246.70} & 0.2   & 1.0 \\
    \midrule
    \multirow{7}[2]{*}{\rotatebox[origin=c]{90}{\textbf{Sanfransico}}} & ZEMob & 0.450 & 0.820 & 489.0 & 884.2 & 6.805 & 20.88 & 2.3   & \textbf{0.1} \\
          & HDGE & 0.526 & 0.825 & 396.8 & 668.9 & 6.057 & 18.14 & 0.2   & 3 \\
          & GMEL & 0.620 & 0.850 & 514.0 & 916.7 & 7.377 & 22.29 & 0.12  & 1.2 \\
          & MVURE & 0.550 & 0.830 & 300.0 & 626.7 & 5.464 & 17.43 & \underline{0.10}  & \underline{0.9} \\
          & MGFN & \underline{0.643} & \underline{0.851} & \underline{295.1} & \textbf{474.8} & \textbf{4.639} & \textbf{13.43} & 42.2  & 0.9 \\
          & ReMVC & 0.450 & 0.820 & 367.6 & 795.6 & 6.628 & 21.53 & \textbf{0.05} & 7 \\
          & HREP & \textbf{0.673} & \textbf{0.861} & \textbf{256.0} & \underline{519.2} & \underline{5.095} & \underline{14.62} & 0.2   & 1.0 \\
    \bottomrule
    \end{tabular}%
  }
  \vspace{-5mm}
  \label{tab:region}%
\end{table}%

Second, we observe that while the MGFN model achieves the best performance in many scenarios, it uses a large number of model parameters and has longer time consumption. This indicates that although high-complexity models can bring performance improvements, their high computational cost and resource consumption may become limiting factors in practical applications. In particular, on the BJ dataset, the MGFN model encountered an OOM (out of memory) issue in the default environment. We used three times the default GPU memory setting to execute it properly.

Considering both accuracy and efficiency, the HREP model, being a recent model, achieved state-of-the-art performance. The HREP model optimizes parameter usage and computation time while maintaining high performance, making it more feasible for practical applications. This also highlights the importance of considering both performance and resource efficiency when designing models.

\subsection{Dive into Sequnce Encoder}
Although we discussed in Sections 6.1 and 6.2 that sequence-based methods can effectively enhance entity representation when the data volume is sufficient, we must not overlook the impact of high-quality representations from upstream training models on downstream results. To further explore when pre-trained sequence encoders should be applied, we tested three different approaches to executing downstream tasks: Static, No Finetune, and Finetune.

\begin{figure*}
    \centering
    \subfigure[Point]{
    \includegraphics[width=0.45\textwidth]{figures/bar_poi.pdf}
    }
    \subfigure[Line]{
    \includegraphics[width=0.44\textwidth]{figures/bar_road.pdf}
    }
    \vspace{-2mm}
    \caption{Comparison of sequential models' performance across different downstream execution methods}
    \vspace{-2mm}
    \label{fig:bar}
\end{figure*}

Static refers to using only the representations learned from upstream tasks and fine-tuning them with LSTM as the downstream model in the downstream tasks. No Finetune (NFT) means not fine-tuning the representation model in the downstream tasks but only training the task-specific header, typically an MLP network layer. Finetune (FT), as described in Sections 6.1 and 6.2, involves fine-tuning the sequence encoder in the downstream tasks. We conducted further tests on three sequential models from PERL (Hier, CTLE, and CACSR) and three from LERL (Toast, JCLRNT, and START) in trajectory based tasks, with results shown in \fig\ref{fig:bar}.

We found that in the downstream tasks for PERL, the Static approach outperformed the FT approach, indicating that in cases of sparse data, discarding the sequence encoder used in the upstream tasks can achieve better results in downstream tasks. This finding emphasizes that using simple models and direct representation methods may be more effective in handling tasks with sparse data.

In the downstream tasks for LERL, the FT approach outperformed the Static approach, which proves that for denser datasets, using pre-trained sequence encoders can achieve better results. This suggests that in data-rich scenarios, complex pretrain models can better capture and utilize the information within the data, thereby enhancing the performance of downstream tasks. The poorer performance of the FT approach compared to the Static approach in SG dataset further supports this view. This may be due to the SG dataset having less trajectory data, preventing the pre-trained sequence encoder from fully leveraging its advantages.

Additionally, in the downstream tasks for PERL, the NFT approach performed very poorly in the TUL task, which is significantly different from the upstream task. This indicates that the current methods still have room for improvement in terms of generalization. Particularly when the nature of the downstream task differs greatly from that of the upstream task, relying solely on pretrain representations from the upstream task may not suffice to meet new task's demands. Therefore, choosing the appropriate training and fine-tuning strategy is crucial in practical applications.

Overall, these experimental results suggest that when choosing pretrain and fine-tuning strategies, the characteristics of the dataset and the specific requirements of the tasks must be considered. Simple models and static fine-tuning strategy may be more effective for sparse data, while complex pretrain models can better improve performance in data-rich scenarios. Moreover, for downstream tasks that differ significantly from upstream tasks, special attention should be paid to the model's generalization ability, and targeted adjustments to training and fine-tuning strategies may be necessary.




==> others.tex <==

%2) {\em Suitable Pre-training Tasks Provide Greater Benefits:} Suitable pre-training tasks can significant enhance performance of the well-matched downstream tasks. For example, relevant examples are the augmented graph contrastive learning pre-training task for the travel time estimation and similarity trajectory search downstream tasks, and the node feature inference pre-training task for flow inference downstream tasks.


%The Augmented Graph Contrastive Learning (AGCL) can offer richer   This indicates that AGCL, a graph-based pre-training task, offers richer representation capabilities than ATrCL for these tasks. AGCL (TTE) and Similarity Trajectory Search (STS) Node Feature Inference (NFI) pre-training task significantly enhances the model's ability to predict flow-related information. the   downstream tasks

%well-matched pre-training tasks (e.g., ATrCL for CTLE, TokRI for JCLRNT, and NFI for HREP) enhances model generalization and improves downstream task performance.

%aligned with core model architectures have a more significant impact on performance. For example, AGCL improves JCLRNT more than ATrCL in trajectory-related tasks, while GAu plays a crucial role in HREP by effectively capturing relational information between entities.



%\paratitle{Comparison for CTLE Variants.} In the POIs \rl models, CTLE achieves the best performance. In the \tab\ref{tab:abl_poi}, we carry out experiments on the following model variations:
%(a) {\em CTLE} maintains the original model architecture.
%(b) {\em CTLE\%} removes the Masked Trajectory Recovery (MTR) pretraining task;
%(c) {\em CTLE\&} removes the Trajectory Predcition (TrajP) pretraining task;
%(d) {\em CTLE*} integrates a new Augmented Trajectory Contrastive Learning (ATrCL) pre-training task into CTLE. In particular, we use the ATrCL pre-training task proposed by CACSR~\cite{??}, which achieve the second best performance in POIs overall experiments;
%(e) {\em CTLE\$} replaces the core architecture of CTLE, \ie a Transformer encoder, with a bidirectional LSTM layer.
%
%The results of the downstream tasks are shown in \tab\ref{tab:abl_poi}. Based on these experiments, we draw the following conclusions:
%First, the CTLE* variant performs the best across all downstream tasks, indicating that the new added ATrCL task significantly improves the model's generalization performance; Second, The CTLE\& variant outperforms CTLE\%, suggesting that the MTR task provides richer representation capabilities for the model compared to the TrajP task; Finally, the performance of CTLE\* drops by 59\% in the NPP task and 60\% in the TUL task, showing that the Transformer Encoder (TE) plays a crucial role in handling trajectory-related tasks, particularly in enhancing sequence encoding capabilities.


In this section, we construct experiments to evaluation the influence of pre-training tasks, structure of encoders to the performance of downstream tasks. In the experiments, we add or remove pre-training tasks from three representative \rl model, CLTE, JCLRNT, and HREP, which achieve the best average performance in POI, road segment, and land parcel representation learning, respectively.  Owing to \name's modular design, specific pre-training tasks can be easily removed from models, and new pre-training tasks can be seamlessly integrated.

The experiment results are given in \tab\ref{tab:abl_poi} - \ref{tab:abl_region}. In the figures, the black ``\ding{51}'' and ``\ding{55}'' indicates the corresponding pre-training tasks are natively equipped or not equipped when a \rl model was proposed, while the red ``\textcolor[rgb]{1,0,0}{\ding{55}}'' and ``\textcolor[rgb]{1,0,0}{\ding{51}}'' indicates the corresponding pre-training tasks are newly added or removed from a \rl model. Moreover, we also evaluate the impact of different backbone model for encoders through modified core architecture of encoders (see the red words in the ``Encoder Core Arc'' row). In the last row, we present the ranking of performance for each variant for convenient to get a conclusion.


%the backbone model of the encoder modified \multicolumn{2}{c|}{\multirow{2}{*}{Encoder Core Arc}} As illustrated in \tab\ref{tab:abl_poi}, \tab\ref{tab:abl_road}, and \tab\ref{tab:abl_region}, we use "\ding{51}" and "\ding{55}" to represent the relationship between pretraining tasks and the original model: "\ding{51}" indicates that the original model integrates the corresponding pretraining task, while "\ding{55}" means the task is not integrated. Additionally, "\textcolor[rgb]{1,0,0}{\ding{55}}" denotes the removal of a specific pretraining task, while "\textcolor[rgb]{1,0,0}{\ding{51}}" represents the addition of a new one. We also test the importance of the sequence encoder and graph encoder to further analyze their impact on model performance. Finally, in the last row, we present the ranking of performance for each variant as its {\em Pre Rank}.


%explore the relationship between pretraining tasks, model structure, and the model's performance on downstream tasks. As shown in Section~\ref{sec:result}, we find that CLTE, JCLRNT, and HREP achieve the best average performance in their respective map entities, so we select these three models for our experiments. Owing to VecCity's modular design, we can not only remove specific pretraining tasks from the models but also easily integrate new pretraining tasks.

%Besides, for these tasks, we also find that models with multiple encoders, such as , usually perform better than those only utilizing a single encoder in this scenario. These tasks require encoders to transform multiple map entities into a representation sequence. The object of downstream tasks is using the representation sequence to give the prediction. There is a big different between the encoder pre-training and the down To achieve accurate sequence prediction, the model must capture the complex dynamic dependencies between entities in the trajectory data. However, due to the substantial differences between these downstream tasks and the pretraining tasks and, the significant temporal variations in these dependencies, the model requires a large amount of labeled data to accurately capture these changes. Specifically, we find that models leveraging multiple encoders usually perform better than those only utilizing a single encoder in this scenario.



%sequence-based pretraining tasks (such as JCLRNT, START, and Toast) demonstrate greater stability in the STS task. Although the STS task also focuses on trajectories, its goal is not to predict additional trajectory labels but to compare the similarity between different trajectories. Since trajectories consist of map entities, their similarity essentially reflects the similarity of the entities they contain. As a result, models that utilize sequence-based pretraining tasks perform relatively well on this task.

%This is evident in the POI Classification (POIC) task shown in \fig~\ref{fig}(a), the Average Speed Inference (ASI) task in \fig\ref{fig}(d), and the Land Parcel Classification (LPC) task in \fig\ref{fig}~(g).

%First, \rl models demonstrate stability concerning changes in training data size when applied to attribute inference downstream tasks, like the POI Classification (POIC) task shown in \fig~\ref{fig:dive}~(a), the Average Speed Inference (ASI) task shown in \fig~\ref{fig:dive}~(d), and the Land Parcel Classification (LPC) task shown in the \fig~\ref{fig:dive}~(g). The stability in these tasks is since they directly infer entity attributes, which have already been thoroughly learned during the pretraining phase. As a result, the fine-tuning phase requires only a small amount of labeled data to achieve good performance.

%We use the commonly employed Tokyo and Xi'an datasets as the datasets for this scenario, with Tokyo for POI \rl and Xi'an for both road segment \rl and land parcel-oriented \rl. %One of the main benefits of pretraining is that it allows the model to perform well on downstream tasks with less labeled data. To test the generalization performance of existing \rl models, we reduce the training data size in the fine-tuning phase and compare the models' performance. We use the commonly employed Tokyo and Xi'an datasets as the datasets for this scenario, with Tokyo for POI \rl and Xi'an for both road segment \rl and land parcel \rl. Specifically, we vary the training data size from 10\% to 50\% of the original size. Apart from data size, all other configurations remain consistent with the mainstream experiments. As shown in \fig~\ref{fig:dive}, the performance of POI \rl is presented in \fig~\ref{fig:dive}~(a) to (c), with each figure corresponding to a different downstream task. Additionally, the performance of road segment and land parcel \rl is shown in \fig~\ref{fig:dive}~(d) to (f) and \fig~\ref{fig:dive}~(g) to (i), respectively. From the table, we have the following observations.

%However, most current experiments have been conducted on abundant training data, and the model's ability to generalize on smaller datasets requires further investigation. In Section~\ref{sec:smalldataset}, we conduct a comprehensive analysis of the model’s performance on smaller datasets to assess its robustness under limited data conditions, providing deeper insights into its generalization capacity.

%These findings provide valuable insights for developing more effective and scalable \rl models, balancing performance and resource efficiency based on specific use cases.

%Based on the experimental results from three types of map entities, we summarize the following two key insights about \rl.

%\paratitle{Advantages of Incorporating Multiple Encoders.} Introducing multiple encoders allows the models to explore and analyze data more effectively, leading to superior performance. This suggests that fully utilizing multi-dimensional information can greatly enhance the model's representational power and generalization ability.


%\paratitle{Complementarity of Multiple Pretraining Tasks.} Combining multiple pretraining tasks effectively enhances the model’s ability to capture complex features, demonstrating that task complementarity supports better feature extraction. However, whether there is a direct relationship between the number of pretraining tasks and performance improvement remains unclear. In Section~\ref{sec:pretraintask}, we explore the impact of pretraining task selection and combinations on model performance.
%This aims to avoid the computational overhead of excessive tasks while maximizing performance improvements.

existing land parcel \rl models primarily focus on extracting information from network relationships, while paying insufficient attention to the sequential dependencies in trajectory data.

Second, most land parcel \rl models rely on the Graph Autoencoder (GAu) as the core pretraining task for self-supervised learning. However, experimental results show that models, such as ReMVC and HREP, using contrastive learning tasks, such as Token Relation Contrastive Learning (TRCL) or Neighborhood Contrastive Learning (NCL), generally outperform those based on GAu. This suggests that contrastive learning strategies may be more effective at capturing relationships between land parcel entities.

Third, existing land parcel \rl models primarily focus on extracting information from network relationships, while paying insufficient attention to the sequential dependencies in trajectory data. This is a limitation of current land parcel \rl models. Future research could explore more effective methods for mining trajectory sequence information related to land parcels to enhance model performance.

%incorporating POI features as an additional feature in land parcel \rl models enhances overall performance. This suggests that land parcel \rl relies not only on geographic information but also on the influence of the POIs it contains. It highlights the importance of incorporating POI entities to improve the parcel \rl models.

Table~\ref{tab:road} gives the performance comparison for road segment \rl models on the downstream tasks of Average Speed Inference (ASI), Travel Time Estimation (TTE), and Similarity Trajectory Search (STS). From the table, we have the following observations.

First, the models adopted the complete token-graph-sequence pipeline, such as JCLRNT and START, achieve the best performance compared the model only adopted partial modules. Moreover, the token-based+graph-based and token-based+sequence-based models, such as HRNR, SARN, Toast, and HRoad, outperform the only token-based model, \ie RN2Vec. These phenomenons highlights that the rich information provided by trajectories and relation networks play critical roles in road segment representation learning. Intergrading graph-based and sequence-based encoders into the \rl models can effectively capture the information.


Second, the model with multiple types of pre-training tasks, \ie Toast, HRoad, START, and JCLRNT, have better performance than with signal types of pre-training tasks, \ie HRNR and SARN. Particularly, in the token-based + graph-based models, the performance HRoad, which adopts both the NFI and GAu pre-training tasks, is better than HRNR (only the GAu task) and SARN (only the AGCL task). Using different types of pre-training tasks enables the model to extract information from the data from multiple perspectives, enhancing its ability to learn comprehensive feature representations. This multi-faceted approach allows the model to achieve better overall performance. Moreover, in the full pipeline models, JCLRNT adopts a sequence-oriented task (Augmented Trajectory Contrastive Learning) and a graph-oriented task (Augmented Graph Contrastive Learning). Its outperforms the START, which adopts two graph-oriented tasks. Stronger task heterogeneity can further improve the performance of the model.

Third, in terms of efficiency, models with fewer modules, such as SARN and RN2Vec, demonstrate significantly better performance. Additionally, models without sequence encoders are far more efficient than those with them. Incorporating trajectory data into road segment \rl models is a resource-intensive process, consuming substantial memory and time. Improving the efficiency of this process remains an open challenge.

%we find that incorporating trajectory data into road segment \rl models consistently improves model performance, highlighting the rich information provided by trajectory data and its critical role in road segment representation learning. Furthermore, models that integrate graph encoders to capture network relationships (such as JCLRNT and START) significantly outperform those that do not consider network relationships (such as Toast). This demonstrates that combining sequence encoders to model trajectory data with graph encoders to capture network relationships between entities can substantially enhance overall model performance.


%Second, designing specific pre-training tasks for each encoder in multi-encoder algorithms can effectively enhance model performance. For example, Toast assigns the TRCL task to the token encoder and introduces the MTR and ATrCL tasks for the sequence encoder, while JCLRNT assigns the ATrCL task to the sequence encoder and the Augmented Graph Contrastive Learning (AGCL) task to the graph encoder. Models with such targeted pre-training tasks generally perform better than those without these strategies.

%Second, token models, which only use token encoders, perform better when they incorporate the network relationship data, like in Teaser and P2Vec. In contrast, models that don't use network relationship data, such as SkipGram and Tale, show weaker performance in downstream tasks. As shown in Table~\ref{tab:models}, token models usually employ the Token Relation Inference (TokRI) task and Token Relation Contrastive Learning (TRCL) task to extract the relationships between map entities. However, these pretraining tasks struggle to capture long-term dependencies in trajectory data, which limits the model's ability to extract relationship information from trajectories effectively. In this situation, token models need to directly incorporate network relationship data to enhance their performance.

%Additionally, we observe that the token models employing the TokRI task gain a better result than those employing TRCL. This is mainly because, with sufficient data, the supervised learning method (i.e., TokRI) can fully leverage the information in the labeled data to learn more discriminative feature representations, thereby significantly improving model performance.

%Based on the \tax of map entity representation learning models, we propose an easy-to-use toolkit for \rl model development, named \name. Figure~\ref{fig:framework} shows the framework of the \fullname, which consists of three functional modules corresponding to the four elements of \rl models as outlined in the taxonomy in Section~\ref{sec:taxonomy}. A {\em Data Module} corresponds to the map data element of \rl given in Section~\ref{sec:taxonomy_data}, which is responsible for preparing and processing data. An {\em Upstream Module} corresponds to the encoder and pre-training elements given in Section~\ref{sec:taxonomy_pretraining}, which is responsible for representation vector encoding and model pre-training. A {\em Downstream Module} corresponds to the downstream task element given in Section~\ref{sec:taxonomy_downstream}, which is responsible for model fine-tuning and model performance evaluation on downstream tasks.


%\begin{itemize}[leftmargin=*]
%\item {\em Data Module.} This module corresponds to the data element of \rl given in Sec.~\ref{sec:taxonomy_data}, which is responsible for preparing and processing data for the subsequent modules.
%\item {\em Upstream Module.} This module corresponds to the pre-training element of \rl given in Sec.~\ref{sec:taxonomy_pretraining}, which is responsible for representation vector encoding and model pre-training.
%\item {\em Downstream Module.} This module corresponds to the downstream task element of \rl given in Sec.~\ref{sec:taxonomy_downstream}, which is responsible for model fine-tuning and model performance evaluation on downstream tasks.
%\end{itemize}
%In this section, we provide a detailed information about the three modules.

%In the following sections, we will provide detailed information about the core modules within VecCity: Data, Upstream, and Downstream. Additionally, we will explain how these modules work together to create a unified and standardized process for MERL.

%\textcolor{red}{\tab~\ref{tab:models} provides a summary of existing \rl methods. We first group these methods based on the entities they focus on. We then further list the model details about model encoders and pretraining tasks according to the taxonomy introduced in the above section. We find that most models use an architecture that combines multiple encoders, following a ``token $\rightarrow$ graph $\rightarrow$ sequence'' encoding order. Additionally, during the pretraining phase, the models are equipped with tailored pretraining tasks for each encoder, which helps to enhance their learning capabilities on specific types of data. The effectiveness of this design is thoroughly explored and validated in the experiments presented in Section~\ref{sec:experiment}. The table also outlines the data used by each method, including map entities, features, and auxiliary data.

%In terms of features, we present the valuable features used by the token encoder, such as semantic features (Sem), spatial features (Spa), and temporal features (Temp). For auxiliary data, trajectory data (Traj) is categorized into check-in trajectory (CIT) and coordinates trajectory (CDT), while network relationships (Rel) are divided into geographical relationship (GR) and social relationship (SR).}

%The downstream tasks consist of two components: {\em Downstream Models} and {\em Fine-tuning Loss}. The downstream model the representation vectors generated by the encoders to complete a given prediction or classification task. The fine-tuning loss is used to finetune the encoders to enhance the adaptability of representation vectors for specific downstream tasks. The first is the downstream model, which uses the representation vectors generated by the encoders as inputs to complete a given prediction or classification task. The second is the fine-tuning loss function, which is used to finetune the encoders to enhance the adaptability of representation vectors for specific downstream tasks.


%In the TrajP tasks, the labels to be predicted can be various. For example, Hier~\cite{Hier1} directly adopts entity IDs as prediction labels. CTLE~\cite{CTLE} uses the visiting time as a label to incorporate the temporal information. In the MTR tasks, the difference among various approaches is shown in how masking positions are selected. A basic approach is to randomly select positions in trajectories for masking~\cite{CTLE}. However, this method fails to consider the sequential dependence among samples along the trajectory. To overcome this issue, START~\cite{START} and Toast~\cite{Toast} select continuous sub-sequence of a trajectory for masking. In the ATrCL tasks, various methods also utilize distinct augmentation techniques. For example, JCLRNT~\cite{JCLRNT} generates augmented trajectories by randomly deleting or replacing trajectory samples. Considering the context information, START~\cite{START} selects a continuous sub-sequence to delete or replaces it with a new sub-sequence. CACSR~\cite{CACSR} augments trajectories by adding white noise to the representations.

%\textcolor{red}{JGRM~\cite{JGRM} claims that trajectories processed through map matching lose the rich information inherent in the original GPS sequences. For example, attributes like angular speed and acceleration in GPS data can indicate the congestion state of road segments. Therefore, JGRM incorporates the original GPS sequences as augmented trajectories to train the encoder model.} road segment representation learning like

%In existing studies on sequence-based models, most approaches utilize multiple types of the aforementioned tasks in their pre-training process.

%Similar to the augmented token contrastive learning,

{\em Masked Trajectory Recovery (MTR).} This task is inspired by the
     masked language model (MLM) in pre-trained language model~\cite{bert,roberta}. The task randomly masks a part of the samples in a trajectory and adopts an autoencoder method to recover the masked samples. Specifically, given a trajectory $tr$ and its masked version $\tilde{tr}$, the task adopts an autoencoder to recover the masked trajectory as $\hat{tr}= Dec(\tilde{\bm{S}}),~ \tilde{\bm{S}}=Enc(\tilde{tr})$, where $Enc(\cdot)$ is the encoder, $Dec(\cdot)$ is a decoder, which is implemented by a sequential deep model, and $\hat{tr}$ is the recovered trajectory. The objective function is to minimize the distance between ${tr}$ and $\hat{tr}$.

\begin{equation}\small
           \hat{tr}= Dec\left(\bm{S}\right),~ \bm{S}=Enc\left(\tilde{tr}\right),
     \end{equation}


          we randomly replace a certain proportion of samples as the $MASK$ placeholder. The masked trajectory is denoted as $\tilde{tr}$. Then,

      The objective function of this task is to minimize the distance between the predicted trajectory fragment {\small $\hat{tr}_{[k+1:K]}$} and its ground truth.

%      uses the first $k$ samples as inputs to predict the rest samples as
      \begin{equation}\label{}\small
        \hat{tr}_{[k+1:K]} = Pre\left(\bm{S}_{[1:t]}\right), ~\bm{S}_{[1:k]} = Enc\left(tr_{[1:k]}\right),
      \end{equation}

%Similarly, START~\cite{START} integrates the travel time through road segments into the attention mechanism of Transformers to capture temporal patterns and travel semantics.

%In trajectory data, each location sample usually includes a timestamp. Integrating time information from the timestamp into the representation of entities has become a key focus of sequence-based encoders. Early methods divide time into slots and use the indexes of the slots, such as the hour of a day or the day of a week, as input features of token-based encoders~\cite{JCLRNT,POI2VEC,Teaser}. Moreover, some models incorporate temporal information into components of the backbone sequential models. For example, JCLRNT~\cite{JCLRNT}, Toast~\cite{Toast} and CTLE~\cite{CTLE} integrate the temporal information of entities within trajectories into the positional encoding of Transformers. START~\cite{START} incorporates the travel time of the road segment into the attention mechanism of Transformers to model temporal regularities and travel semantics of trajectories.

%In existing studies on graph-based models, most approaches utilize multiple types of the aforementioned tasks in their pre-training. the encoder of %HREP~\cite{HREP}, MGFN~\cite{MGFN}, and MVURE~\cite{MVURE} use OD flows to calculate the adjacency matrix between entities.% while \textcolor{red}{Region2Vec~\cite{Region2Vec} also uses the spatial distance between entities to calculate the adjacency matrix. Since both OD flows and spatial distances are continuous values, their pre-training tasks not only determine the existence of connections between map entities but also estimate the weights of these connections.}

%  {\em Graph Autoencoder \textit{(GAu)}.} This task adopts an autoencoder to reconstruct the adjacency matrix of relation networks from the representations of map entities. Specifically, given the representation vectors of all map entities, denoted as $\bm{H}$, the graph autoencoder adopts a function to reconstruct the adjacency matrix $\bm{E}$ as $\hat{\bm{E}} = \phi\left(\bm{H} \bm{H}^\top\right)$,      where $\hat{\bm{E}}$ is the reconstructed adjacency matrix, and $\phi(\cdot)$ is a neural network. Here, the graph-based encoder is the encoder of the autoencoder, and $\phi(\cdot)$ is the decoder. The learning objective is to minimize the difference between $\hat{\bm{E}}$ and $\bm{E}$.     {\em Augmented Graph Contrastive Learning \textit{(AGCL)}.} This task applies data augmentation contrastive learning on map entity relation networks. Given a relation network $G$ and its augmented version $\tilde{G}$, the task considers the representations for the same node with different versions as positive samples while for the different nodes as negative samples.

a graph-based model first employs a token-based encoder to generate embeddings for each entity. These embeddings are denoted as $\bm{R} = \{\bm{c}_1, \ldots, \bm{c}_I\}$. The graph-based encoder then takes $\bm{R}$ and the relation network $G$ as inputs to a graph neural network (GNN), generating representation vectors for the map entities (nodes) as
\begin{equation}\label{}
  \bm{H} = \left\{\bm{h}_1, \ldots, \bm{h}_i, \ldots, \bm{h}_I\right\} = \mathrm{GNN}\left(\bm{R}, G\right),
\end{equation}
where $\bm{h}_i$ is the representation vector for the $i$-th map entity, and $\mathrm{GNN}(\cdot)$ denotes the encoder.
%In many \rl models, the graph-based encoders are used as inputs for the following encoding steps, such as sequence-based encoders~\cite{START,JCLRNT}.

The novelty of the TokRI and TRCL tasks lies in the methods of token relations construction, which include two ways. $i$) The first is directly using geographical distance between entities to construct token relations. For example, in the TokRI tasks, RN2Vec~\cite{RN2Vec} establishes relationships between entities based on their spatial proximity. If the geographical distance between a pair of entities is below a preset threshold, RN2Vec sets ${y}_{i,j}=1$. In the TRCL tasks, Teaser~\cite{Teaser} considers the $K$ nearest entities as positive entities in its token relation contrastive learning. $ii$) The second way to establish the entity relations is using auxiliary data. A commonly approach is to consider entities along the same trajectory as being related. In the TokRI tasks, POI2Vec~\cite{POI2VEC} and Tale~\cite{TALE} treat a trajectory as a sentence and the entities within it as words, where entities along the same trajectory serve as the context for each other. Both models utilize the Continuous Bag of Words (CBOW) model~\cite{Word2Vec}, a variant of the word2vec model, to learn representation vectors. In the TRCL tasks, Teaser~\cite{Teaser} uses SkipGram~\cite{Word2Vec} with negative sampling to exploit the context relations of entities along the same trajectory. When trajectory data is missing, the relations can be generated by performing a random walk on the relation network~\cite{HDGE}. Besides using trajectories, ZEMob~\cite{ZEMob} and DeepMove~\cite{DeepMove2} utilize OD flows between entities to identify relationships.

For augmented token contrastive learning tasks, the novelty lies in augmented samples generation. For example, ReMVC~\cite{REMVC} and RegionDCL~\cite{RegionDCL} augment data by replacing or dropping a portion of the anchor entity's features.


% For example, the Hier model employs spatial hierarchical embeddings to extend the features of locations~\cite{hier}. Given a city map divided into grid-based land parcels, Hier aggregates multiple basic grids into an area and further groups multiple areas into a region. For each grid-based land parcel, Hier assigns an embedding vector at each level (region, area, and grid) and combines these embedding vectors to generate the final token representation for the grid entity. The embedding vectors for the region and area to which a grid belongs can be viewed as extended features for the grid. Moreover, one type of map entity can also be used to generate features for another type of entity. For example, the token encoders in ReMVC~\cite{REMVC}, ReCP\cite{ReCP}, Region2Vec\cite{Region2Vec}, and MVURE~\cite{MVURE} use the categories of POIs within or near a land parcel or road segment to generate features for them.



%XXX~\cite{???} and XXX~\cite{???} utilize the categories of surrounding POIs to extract features of land parcels or road segments.
%extract features of land parcels and road segments from
%utilize the categories of surrounding POIs of land parcels or road segments in their token encoders.


%Spatial features are represented by the location coordinates of map entities. A common approach divides the city map into grid-based land parcels, with each grid corresponding to a unique embedding vector that is shared by entities within the same grid. This preserves spatial proximity between map entities. Hier~\cite{Hier1} enhances this by aggregating multiple grids into areas, and multiple areas into regions, assigning an embedding vector at each level (region, area, and grid). These vectors are combined to generate the final representation for entities, with the region and area embeddings serving as extended features for the grid.
%{\em Spatial Features (Spa)}, and {\em Temporal Features (Temp)}.  {\em Semantic Features (Sem)},
%Temporal features are derived from recorded times in trajectory or social relationship data. These features help capture co-occurrence relationships between events happening at the same or similar times. A common approach divides the day into multiple time segments (e.g., hourly or half-hourly intervals), with each segment assigned a unique embedding as the temporal feature for the entities.

Semantic features are primarily determined by the intrinsic characteristics of map entities. Common approaches use the category of map entities, such as the functional types of POI entities and the road types of road segment entities, as their semantic features. Additionally, some land parcel \rl methods use the quantity of POI categories within a parcel as its semantic features~\cite{REMVC}.

%, existing studies primarily focus on identifying valuable features from raw map entities and auxiliary data. Based on current research, we categorize the valuable features into three main types: {\em Semantic Features (Sem)}, {\em Spatial Features (Spa)}, and {\em Temporal Features (Temp)}.

\begin{itemize}[leftmargin=*]
    \item {\em Semantic Features.} \textcolor[rgb]{1,0,0}{Semantic features are primarily determined by the intrinsic characteristics of map entities. Common approaches use the category of map entities, such as the functional types of POI entities and the road types of road segment entities, as their semantic features. Additionally, some land parcel \rl methods use the quantity of POI categories within a parcel as its semantic features~\cite{REMVC}.}
    \item  {\em Spatial Features.} \textcolor[rgb]{1,0,0}{Spatial features are represented by the location coordinates of map entities. A common approach divides the city map into grid-based land parcels, with each grid corresponding to a unique embedding vector that is shared by entities within the same grid. This preserves spatial proximity between map entities. Hier~\cite{Hier1} enhances this by aggregating multiple grids into areas, and multiple areas into regions, assigning an embedding vector at each level (region, area, and grid). These vectors are combined to generate the final representation for entities, with the region and area embeddings serving as extended features for the grid.}
    \item {\em Temporal Features.} \textcolor[rgb]{1,0,0}{Temporal features are derived from recorded times in trajectory or social relationship data. These features help capture co-occurrence relationships between events happening at the same or similar times. A common approach divides the day into multiple time segments (e.g., hourly or half-hourly intervals), with each segment assigned a unique embedding as the temporal feature for the entities.}
\end{itemize}

%In this two-step pipeline, {\em Encoder Models}, {\em Pre-training Tasks}, and {\em Downstream Tasks} are the three basic components for a \rl model. In this section, we give a brief review of the three components. a typical \rl model and its application can be divided into two steps: {\it pre-training} and {\it fine-tuning}. In the pre-training step, a \rl model uses raw map entities and auxiliary data as inputs and uses an encoder model to convert the inputs as a representation vector. Moreover, the \rl model uses pre-training tasks to train the parameters of the encoder model. In the fine-tuning step, the encoder model is used to encode raw map entities and auxiliary data as representation vectors for downstream tasks. We use the objective functions of the downstream tasks to fine-tune the encoder parameters. In this two-step pipeline, {\em Encoder Models}, {\em Pre-training Tasks}, and {\em Downstream Tasks} are the three basic components for a \rl model. In this section, we give a brief review of the three components.

%hinders the progress of \rl research.

impedes the progress of the field.

%not only impedes the progress of the field but also makes it difficult to establish guiding design principles through fair and consistent model performance comparisons.

This issue hinders the field’s progress as well as makes it challenging to establish guiding design principles through fair model performance comparison.


%Our taxonomy begins by outlining the essential components of a mapRL model and providing a review of its structure. In our view, a mapRL model comprises four key elements: input data, encoder models, pre-training tasks, and downstream tasks. The input data can be further categorized into **Map Entity Data** and **Auxiliary Data**. Encoder models are classified into three types: **Token-based**, **Sequence-based**, and **Graph-based** models.

%The pre-training tasks vary according to the type of encoder model used.

%Notably, the characteristics of the three core modules—input data, encoder models, and pre-training tasks—are not tightly coupled with the type of Map Entity involved. Only the pre-training tasks exhibit dependency on the Map Entity type. This taxonomic approach differs fundamentally from the traditional classification of mapRL models based solely on Map Entity types, offering a unified framework for the representation modeling of diverse Map Entities.

%\item
%\end{itemize}

%These achievements have led researchers to place increasing emphasis on pre-training, driving the continuous evolution of related technologies. However, applying pre-trained representation learning to map entities, which is also named {\em Map Entity Representation Learning (\rl)}, still presents numerous challenges.
%\begin{itemize}[leftmargin=*] \item




%{\bf Issuse 1. Complex spatiotemporal characteristics.} Unlike image and text data, where data representation derives from clear structures or intuitive patterns, the data representation of map entities primarily stems from their spatial-temporal dependencies. This uniqueness complicates the understanding of data related to map entities. For instance, capturing spatial dependencies involves recognizing relationships between adjacent entities, while complex topological structures require models that can capture hierarchical and multi-view relationships. Additionally, temporal dependencies necessitate models that can adapt to changing environments and identify trends within the data. Therefore, developing advanced methods capable of modeling these complex spatial and temporal relationships is essential for efficiently representing map entities.

%{\bf Issuse 2. Lack of standardized benchmark.} Standardized and user-friendly pipelines form the foundation for the rapid development of pre-trained representation learning in natural language processing~\cite{squad} and computer vision\cite{mmdetection}. An effective pipeline provides a consistent framework for model training and evaluation, ensuring the reproducibility and comparability of research findings.
%As illustrated in \fig\ref{fig:arxiv}, the field of map entity representation learning (\rl) is garnering increasing attention.
%The need for standardized benchmarks and flexible pipelines in \rl is growing with an increasing number of methods being developed for diverse datasets and scenarios. 
